Gamma counterparts for robust nonlinear combinatorial and discrete optimization

Gamma uncertainty sets have been introduced for adjusting the degree of conservatism of robust counterparts of (discrete) linear programs. The contribution of this paper is a generalization of this approach to (mixed integer) nonlinear optimization programs. We focus on the cases in which the uncertainty is linear or concave but also derive formulations for the general case. By applying reformulation techniques that have been established for nonlinear inequalities under uncertainty, we derive equivalent formulations of the robust counterpart that are not subject to uncertainty. The computational tractability depends on the structure of the functions under uncertainty and the geometry of its uncertainty set. We present cases where the robust counterpart of a nonlinear combinatorial program is solvable with a polynomial number of oracle calls for the underlying nominal program. Furthermore, we present robust counterparts for practical examples, namely for (discrete) linear, quadratic and piecewise linear settings. Keywords: Budget Uncertainty, Discrete Optimization, Combinatorial Optimization,

==> Applications_preprint.tex <==
\section{Appendix} \label{A}
\subsection{Numerical study} \label{Sec:App}
The programs were implemented in Python 3.7. To solve the optimization programs, we used Gurobi 9.0.1. \cite{Gurobi} running on machines with Xeon E3-1240 v5 CPUs (4 cores, 3.5 GHz each).
\subsubsection{Vehicle routing problem with soft time windows under uncertainty}
We elaborate on Example~\ref{Ex:UncertainBounds} based on \cite{Dummies} and \cite{VRPSTW}. We consider a complete digraph $D=(N,A)$ with nodes $N:=[n]$, a start depot $0$ and a copy of the start depot $n+1$, and the digraph $\bar{D} = (V, \bar{A})$ with nodes $V:= [n+1]_0$ and arcs 
\begin{gather*}
\bar{A} = A \cup \{(0,j): \ j \in N\} \cup \{(i,n+1): \ i \in N \cup \{0\}\}.
\end{gather*}
The following data are given: For every arc $a \in \bar{A}$, the travel time is $t_a$ and for every node $i \in N$, a service time $s_i$ and a soft due time $b_i$ is given. Given a homogeneous fleet of $K$ vehicles, all nodes $i \in N$ have to be 'visited' by exactly one vehicle exactly once and with as little delay as possible. The vehicles start and end at the depot. In the following, the binary variables $x_{i,j}^k \in \{0,1\}$ for $(i,j) \in \bar{A}$ and $k \in [K]$ denote whether vehicle $k$ 'uses' arc $(i,j)$ and the real variables $T_i \in \R_{\geq 0}$ for  $i \in V$ denote the arrival time of a vehicle at node $i$. With this notation, we obtain the following optimization program (with $\delta^{\mathrm{out}}(v)$ and $\delta^{\mathrm{in}}(v)$, we denote the outgoing and the incoming arcs of $v \in V$ in the graph $\bar{D}$):
\begin{subequations}
\begin{align}\label{Prob:VRPTSW}
\min_{x,T} & \ \sum_{i \in N} \max \{0, T_i - b_i\}, \\
\text{s.t.} & \ \sum_{k\in[K]} \sum_{(i,j)\in\delta^{\mathrm{out}}(i)}x_{i,j}^{k}=1\ \forall{i}\in{N},  \label{Const:VehR1} \\
	& \sum_{(0,j)\in\delta^{\mathrm{out}}(0)}x_{0,j}^{k}=1 \ \forall{k}\in[K],  \label{Const:VehR2} \\
	& \sum_{(i,j)\in\delta^{\mathrm{in}}(j)}x_{i,j}^{k} - \sum_{(j,i)\in\delta^{\mathrm{out}}(j)}x_{j,i}^{k}=0 \ \forall k\in [K] ,  j\in N,  \label{Const:VehR3} \\
	&\sum_{(i,n+1)\in \delta^{\mathrm{in}}(0)} x_{i,0}^{k} = 1 \ \forall k \in [K],  \label{Const:VehR4} \\
	&x_{i,j}^{k}(T_{i} + s_i + t_{i,j} - T_j)\leq 0 \ \forall k \in [K], \ (i,j)\in A,  \label{Const:VehR5} \\
    &x_{i,j}^{k} \in \{0,1\} \ \forall k \in [K], \ (i,j)\in A, \label{Const:Binary}\\
    &T_i \geq 0 \ \forall i \in V. \label{Const:Time_Non_Negative}
\end{align}
\end{subequations}

%\todo{es sollte gesagt werden dass es verschiedene modelle fuer VRP gibt, und
%wir uns hier lediglich eines davon rausgreifen.}
%\todo{An Frauke: Ist schon dadurch geschehen, dass wir die Spezifizierung nach einer Quelle gemacht haben. Habe noch hinzugefügt, dass Subtour Elimination Constraints durch (59f) redundnt gemacht werden.}

Constraint~\eqref{Const:VehR1} ensures that each $i \in N$ is served exactly once by exactly one vehicle. Constraints~\eqref{Const:VehR2} and \eqref{Const:VehR4} ensure that each vehicle leaves and enters the depot or stays at the depot. In combination with constraints \eqref{Const:VehR1}, \eqref{Const:VehR2} and \eqref{Const:VehR4}, constraint~\eqref{Const:VehR3} ensures that each node is served exactly once and by exactly one vehicle. Constraint~\eqref{Const:VehR5} ensures that, if vehicle $k$ serves node $j$ after node $i$, the arrival time $T_j$ is at least as large as the arrival time $T_i$ added to the time it requires for serving $i$ and going from $i$ to $j$. Finally, \eqref{Const:Binary} and \eqref{Const:Time_Non_Negative} ensure that $x$ is binary and $T$ is non--negative. Note that this formulation is only one of many possibilities to formulate vehicle routing problems -- for an overview, we refer the reader to \cite{SurveyVRP}. We attempt to be robust against scenarios of the set $\bigtimes_{i \in N} [\overline{b}_i - \Delta b_i, \overline{b}_i]$. Solving the $\Gamma$--counterpart for all $\Gamma \in [m]$ would show how many shifts of the due times are possible without any (or only little) delay. \\
For our experiments we use the Solomon instances r101, r102, c101, c102, rc101 and rc102. If these names begin with r, the nodes are generated randomly, if they begin with c, they are clustered, and otherwise some nodes are generated randomly and some are clustered -- for a detailed description of the construction, see \cite{Solomon}. As due time $b_i$ we chose the start time specified in the original instance for the customer, i.e., node $i$. The uncertainty set was constructed randomly, i.e., $\Delta b_i$ is a uniformly distributed random variable in $[0,\overline{b}_i]$. Since we were ultimately aiming to find optimal solutions for the $\Gamma$--counterpart, we tested $N=[8]$ and $N=[10]$, $K \in [3]$ and all $\Gamma \in N$, and calculated the optimal solutions for the respective nominal program. We selected the first $|N|$ customers of the list of customers given in the resp. instance.

\begin{figure}[H]
\centering
\scalebox{0.68}{\input{8_Patients_4_diagramms.tex}}
\caption{Optimal values for the respective $\Gamma$--counterparts for instances rc101 (upper left), rc102 (upper right), c101 (lower left) and r102 (lower right), with $N = [8]$ and $K \in [3]$. If a yellow point for a value of $\Gamma$ is 'missing', its value coincides with the green point of the same $\Gamma$.\label{Fig:OptValues8}}
\end{figure}
In Figure~\ref{Fig:OptValues8} we have the robust optimal values
for $N = [8]$, $K \in [3]$ and the instances rc101, rc102, c101 and
r102 (we have neglected the other two cases and the results for $N=[10]$ because the graphs are similar). As expected, the optimum value, i.e., the waiting time, increases with an
increasing number of vehicles $K$. In addition, at $K = 1$ the optimal value for increasing $\Gamma$ strongly rises, while at $K = 2,3$ the change in the optimal value is not so marked. This is also to be expected: If there is exactly one vehicle, the changes in the due times are supposed to be met by this one vehicle, which is clearly not really possible, especially in clustered settings. However, the total delays are more robust for $K = 2,3$ -- while the robust values differ between $K = 1,2,3$, the difference
between $K=1$ and $K=2$ is much higher than in $K=2$ and $K=3$. So if more vehicles are available, this can lead to more robust solutions. The difference  in the price of robustness is evident, e.g. in c101: For $K = 1$ the nominal optimal value is less than $200$ and for $K = 2,3$ it is $0$. For $\Gamma = 1$ and $K = 1$ we obtain a delay of at least $400$, while for $K = 2,3$ we remain around the optimal nominal value for $K = 1$. For $\Gamma = 2$ the delay increases only slightly and does not change afterwards. However, for $K = 1$, the optimum value increases up to $\Gamma = 6$ and is above $1200$, while for $K = 2,3$ the optimum value is below $200$. We note that for other cases, the difference between the nominal optimal values and the optimal values for $\Gamma \geq 1$ is not as large as can be seen in r102. In this particular case, the increase in nominal optimal values for $\Gamma$ stopped at $\Gamma = 2$ for all $K = 1,2,3$. \\
Table~\ref{Table:8_Patients} and Table~\ref{Table:10_Patients} show the running time to solve
the $\Gamma$--counterpart for $\Gamma \in [2]$, the nominal program for all instances with $N = [8], [10]$ and $K \in [3]$. As the number of
constraints increases with more customers and more vehicles, i.e., rising $|N|$ and $K$, the running time increases in most cases. Note that when reformulating the
$\Gamma$--counterpart, only the objective of the subproblems~\eqref{Prob:SubProbVRPRec} will be affected, while the
optimal solutions of the other subproblems can be reused. Thus, of the
$2|N| + 1$ programs, only $|N|$ programs need to be solved to obtain an optimal solution of the $\Gamma$ counterpart when different values of $\Gamma$ are considered. This explains the fact that the running time for $\Gamma = 2$ is usually at most half as large as that for $\Gamma =1$. We note that the value of $\Gamma$ does not have any other significant influence on the running time and that the running times are relatively high, especially for $|N| = 10$. 


\begin{table}[H]
\centering
\caption{Running time of various instances in seconds for $\Gamma= 1,2$, the nominal case, $N = [8]$ and $K = 1,2,3$. \label{Table:8_Patients}}
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
Instances: & \multicolumn{3}{|c|}{Nominal case}& \multicolumn{3}{|c|}{$\Gamma = 1$} & \multicolumn{3}{|c|}{$\Gamma = 2$} \\
  \cline{2-10}
$N = [8]$ & $K = 1$ & $K = 2$ & $K = 3$ & $K = 1$ & $K = 2$ & $K = 3$ & $K = 1$ & $K = 2$ & $K = 3$\\ \hline
r101 & 17 & 1 & 2 & 79 & 43 & 26& 40 & 15 & 14 \\ \hline
r102 & 11& 22 & 15 & 105 & 356 &246 & 49 & 136 & 123 \\ \hline 
c101 & 1 & 1 & 1 & 28 & 7 & 8 & 19 & 4 & 5 \\ \hline
c102 & 10 & 21 & 24 & 124 & 394 & 434 & 62 & 183 & 298 \\ \hline
rc101 & 5 & 1 & 2 & 107 & 156 & 224& 30& 19& 22 \\ \hline
rc102 & 7 & 69 & 291 & 101 & 823 & 2965 & 49 & 284& 1282 \\ \hline
\end{tabular}
\end{table}


\begin{table}[H]
\centering
\caption{Running time of various instances in seconds for $\Gamma= 1,2$, the nominal case, $N = [10]$ and $K = 1,2,3$. If no optimal solution has been obtained after 24 hours, the resp. fields are marked with --. \label{Table:10_Patients}}
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}

\hline
Instances: & \multicolumn{3}{|c|}{Nominal case}& \multicolumn{3}{|c|}{$\Gamma = 1$} & \multicolumn{3}{|c|}{$\Gamma = 2$} \\
  \cline{2-10}
$N = [10]$ & $K = 1$ & $K = 2$ & $K = 3$ & $K = 1$ & $K = 2$ & $K = 3$ & $K = 1$ & $K = 2$ & $K = 3$ \\ \hline
r101 & 551 & 6 & 3 & 9080 & 5178 & 2316 & 5612 & 1525 & 376 \\ \hline
r102 & 1175 & 1066 & 119 & 15358 & 54885 & 15637 & 9433 & 18285 & 5875 \\ \hline 
c101 & 15 & 2 & 5 & 8026 & 2444 & 168 & 4161 & 65 & 28 \\ \hline
c102 & 1566 & 431 & 111 & 22081 & 32098 & 21335 & 15285 & 12692 & 12703  \\ \hline
rc101 & 681 &14 &  7& 8279 & 11024 & 9364 & 2949 & 1253& 350 \\ \hline
rc102 & 902 & 2505 & 8425 & 13327 & 70041 & -- & 6804 & 37788 &--  \\ \hline

\end{tabular}
\end{table}
%\todo{Für die leeren Felder hat der HPC den Job beendet, ohne dass die Walltime gesprengt wurde (aus Speicherplatzgründen. Ich versuchs heut nochmal, ansonsten könnte man unter Umständen auch versuchen, mit einer Gap zu arbeiten. Oder die Laufzeiten wegzulassen - dass ein VRPSTW auf Optimalität zu lösen praktisch ein Ding der Unmöglichkeit ist, ist an sich ja kein Staatsgehemnis... :)}


This concludes our numerical study of the VRPGTW under uncertainty. As already mentioned, we used an optimization oracle to solve the programs given in Example~\ref{Ex:UncertainBounds} as a MINLP instead of using any VRPTGW solvers to demonstrate that our reformulation can be solved to optimality. In the future, it might be interesting to conduct experiments including instances with more customers but rather than solving them to global optimality, they could be solved only to a certain gap, i.e., to find solutions which are 'sufficiently robust' or to apply a VRPTGW oracle.
%Thus, for each $k \in [m]$, by applying Equations~\eqref{Eq:Case1} and ~\eqref{Eq:Case2}, we have to solve the optimization problems
%\begin{alignat*}{2}
%\min_{x,T} & \ \sum_{i \in [m]} \max\{0, T_i - \overline{b}_i, x_i - \overline{b}_i + \Delta b_i - \Delta b_k \} + \Gamma \Delta b_k &\\
%\text{s.t.} & (x,T) \in \mathcal{X}, \\
%& x_k \geq \overline{b}_k
%\end{alignat*}
%and
%\begin{alignat*}{2}
%\min_{x} & \ \sum_{i \in [m]} \max\{0, x_i - \overline{b}_i, x_i - \overline{b}_i + \Delta b_i - x_k + \overline{b}_k -\Delta b_k \} + \Gamma (x_k - \overline{b}_k + \Delta b_k) &\\
%\text{s.t.} & x \in \mathcal{X}, \\
%& x_k \in [\overline{b}_k - \Delta b_k, \overline{b}_k].
%\end{alignat*}
%For $k = 0$, we have to solve
%\begin{align*}
%\min_{x} & \ \sum_{i \in [m]} \max \{0,x_i - \overline{b}_i + \Delta b_i\} \\
%&\text{s.t.} x \in \mathcal{X}.. 
%In the following, we test this for various $\Gamma$:

%
%\begin{figure}[h]
%\centering
%\begin{tikzpicture}
%
%\definecolor{color0}{rgb}{0.75,0.75,0}
%
%\begin{axis}[
%legend cell align={left},
%legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
%tick align=outside,
%tick pos=left,
%x grid style={white!69.0196078431373!black},
%xlabel={$\Gamma$},
%xmin=-0.5, xmax=10.5,
%xtick style={color=black},
%xtick={0,1,2,3,4,5,6,7,8,9,10},
%xtick={0,1,2,3,4,5,6,7,8,9,10},
%xtick={0,1,2,3,4,5,6,7,8,9,10},
%xtick={0,1,2,3,4,5,6,7,8,9,10},
%xticklabels={0,1,2,3,4,5,6,7,8,9,10},
%xticklabels={0,1,2,3,4,5,6,7,8,9,10},
%xticklabels={0,1,2,3,4,5,6,7,8,9,10},
%xticklabels={0,1,2,3,4,5,6,7,8,9,10},
%y grid style={white!69.0196078431373!black},
%ylabel={Robust opt. value},
%ymin=27.475199110678, ymax=2347.3957947711,
%ytick style={color=black}
%]
%\addplot [semithick, green!50!black, mark=*, mark size=3, mark options={solid}, only marks]
%table {%
%0 357.731090451871
%1 500.079036757012
%2 612.332759419592
%3 674.726666758932
%4 720.856079833044
%5 759.331676610509
%6 797.807273387974
%7 828.969607392891
%8 858.352387385337
%9 871.465746128311
%10 871.465746128311
%};
%\addlegendentry{r101}
%\addplot [semithick, blue, mark=*, mark size=3, mark options={solid}, only marks]
%table {%
%0 132.926135277061
%1 874.685428441234
%2 1398.84671392549
%3 1662.96729123004
%4 1882.54803409491
%5 2038.4926308289
%6 2181.04648378273
%7 2222.74981474695
%8 2230.23883141975
%9 2237.72786075047
%10 2241.94485860472
%};
%\addlegendentry{c101}
%\addplot [semithick, red, mark=*, mark size=3, mark options={solid}, only marks]
%table {%
%0 220.23377348622
%1 311.771143458983
%2 380.453596009687
%3 449.134541909007
%4 500.127152726736
%5 521.407687719259
%6 542.688222711782
%7 559.220927357124
%8 559.220927357124
%9 559.220927357124
%10 559.220927357124
%};
%\addlegendentry{rc101}
%\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}, only marks]
%table {%
%0 540.362825670662
%1 614.039932565699
%2 664.658832760788
%3 710.380468916
%4 724.924544846314
%5 724.924544846314
%6 724.924544846314
%7 724.924544846314
%8 724.924544846314
%9 724.924544846314
%10 724.924544846314
%};
%\addlegendentry{rc102}
%\end{axis}
%\end{tikzpicture}
%\caption{Optimal value for $\Gamma$--counterparts of different Solomon-Instances with $|N| = 10$ and $|K| = 1$}
%\end{figure}
%
%\begin{table}[H]
%\centering
%\caption{running time for solving $\Gamma$--counterparts of different Solomon-Instances in seconds for $\Gamma = 1, \dots, 5$ for $|N| = 10$ and $|K| = 1$} 
%\begin{tabular}{|l|r|r|r|r|r|r|}
%\hline
%{} &                $\Gamma = 1$ &            $\Gamma = 2$ &            $\Gamma = 3$ &            $\Gamma = 4$ &            $\Gamma = 5$ \\
%\hline
%r101 &     9545.489140 &  5042.905104 &  4324.250047 &  4212.468293 &  4110.318647 \\ \hline
%c101 &     12503.402265 &  6638.992851 &  6677.901501 &  7045.367498 &  5866.937606 \\ \hline
%rc101 &     7891.869775 &  4397.152880 &  4585.326988 &  4824.234331 &  4297.296250 \\ \hline
%rc102 &    10676.436401 &  7463.172886 &  6771.126355 &  6529.340730 &  5886.227531 \\ 
%\hline
%\end{tabular}
%\end{table}
%
%\begin{table}[H]
%\centering
%\caption{running time for solving $\Gamma$--counterparts of different Solomon-Instances in seconds for $\Gamma = 6, \dots, 10$ for $|N| = 10$ and $|K| = 1$} 
%\begin{tabular}{|l|r|r|r|r|r|r|}
%\hline
%{} &         $\Gamma=  6$  &     $\Gamma =  7$  &           $\Gamma = 8$  &  $ \Gamma = 9$  &  $\Gamma =  10$  \\
%\hline
%r101 &  3772.634931 &  3835.745150 &  3698.588385 &  3381.610417 &  3322.267367 \\ \hline
%c101 &  6531.435335 &  5992.171862 &  5847.719429 &  5491.516783 &  5122.379986 \\ \hline
%rc101 &  4511.206877 &  4020.620868 &  3876.803881 &  3246.952558 &  4098.225415 \\ \hline
%rc102 &  5821.010860 &  4701.883650 &  5228.163494 &  4738.204280 &  4804.154813 \\
%\hline
%\end{tabular}
%\end{table}



%\begin{tabular}{lr}
%\toprule
%{} &  robust\_optimal\_value \\
%\midrule
%0 &              0.132746 \\
%1 &             93.250696 \\
%2 &            141.581281 \\
%3 &            178.945579 \\
%4 &            184.394430 \\
%5 &            188.321483 \\
%6 &            188.321483 \\
%7 &            188.321483 \\
%8 &            188.321483 \\
%\bottomrule
%\end{tabular}



\subsubsection{Quadratic assignment problem under uncertainty}
Here, we solve and compare different reformulations of the $\Gamma$--counterpart of the QAP. We have chosen instances from \cite{QAP2015} and from the QAPLIB \cite{QAPlib}. The goal of this section is to prototypically evaluate whether the new reformulations can be solved within a similar order of
magnitude when compared to that of the nominal versions. As we do not have an efficient problem--specific QAP oracle at hand, we chose small instances where the $\Gamma$--counterpart could be solved with Gurobi within 24 hours. As expected, instances with less uncertain coefficients are computationally easier to handle. Therefore, by choosing scr12, we included an instance with $c_{i,j} = 0$ for some $(i,j) \in [12]^2$. We also chose fei9, an instance that was examined in \cite{QAP2015}. For fei9, the number of facilities is $n = 9$, while for scr12, it is %(from \cite{QAPlib})
$n =12$ (both taken from \cite{QAP2015}). Finally, we also chose nug12 from \cite{QAPlib}. 
%% and omitted the last
%six facilities and locations, since no other instance with $n<12$ is available
%in QAPLIB. %\todo{Kann man hier nicht sagen, dass man die letzten $6$
          %Facilities und locations weglässt? Käme mir einfacher
%vor}.
%The modified instance with $n=6$ is denoted as nug6. 
%\todo{Matrizen? $u^k$ waren bisher maximal Vektoren, wieso sind das hier Matrizen?} Each instance describes a QAP, i.e., the distances between the locations and the amount of transferred goods between the facilities are given. For every instance we chose three matrices $u^k$ with $k \in [3]$ which define the maximum deviation for the flow $\Delta c_{ij}$ for $(i,j) \in [n]$.
For each instance, we generated three different uncertainty sets. For fei9, the uncertainty set $\mathcal{U}_1$ is taken from \cite{QAP2015}. Other uncertainty sets, denoted by $\mathcal{U}_2$ and
$\mathcal{U}_3$, are generated randomly: for all $(i,j) \in [n]^2$, $\Delta c_{ij} \in [0,\bar{c}_{ij}]$ is randomly chosen. %each tuple $(i,j)\in [n]^2$. %\todo{Hier gibt es einen Notationsclash: die uncertainty sets waren immer $\mathcal{U}$, aber es haben sich $\mathcal{U}^i$ immer auf einzelne Funktionen $f^i$ bezogen - ich weiß nicht, ob das hier genauso ist... Was ich später verwirrend finde, ist der Begriff uncertainty setting, den gabs im Paper vorher gar nicht und ich kann mich auch nicht entsinnen, den schon mal gelesen zu haben. Kann man nicht in Formeln beschreiben, wie das geht? Also an den Instanznamen irgendwie einen Index dran hängen, der das Setting klar macht und sagen, wie im jeweiligen Setting verfahren wird..?}
%matrices with entries $u^k_{ij} = \Delta c_{ij} \in [0,\bar{c}_{ij}],
%(i,j)\in [n]^2$ and $k \in \{2,3\}$.
%\todo{ich wollte hier gerade Formeln vermeiden, eben weil die Notation
%nicht ganz klar ist, und ich dachte es ist leicht genug dass wir es
%einfach in Text schreiben. ansonsten muss man als leser nochmal
%zurueckblaettern... $u^1$ ist nicht die unsicherheitsmenge,
%sondern die Instanz, die dann so heisst (so ist es ja im Plot, die
%Kurven haben das Label).}
For scr12 and nug6, $\mathcal{U}_1$ is generated by setting $\Delta c_{ij} =
0.1  \bar{c}_{ij}$ for all $(i,j) \in [n]^2$. Furthermore, $\mathcal{U}_2$ and $\mathcal{U}_3$ are generated randomly analogously to fei9. 
%, equals the number of $\bar{c}_{ij} \neq 0$.

%Starting with the first experiment we have to compute the robust optimal solution for different $\Gamma$.
In Figure~\ref{Fig:obj} the change in the objective value for different $\Gamma$ can be observed for two of our instances are shown. As expected, the optimal objective value is increasing in $\Gamma$. As can be seen for scr12, only a mild increase in cost of
robust protection can be seen for increasing values of $\Gamma$. %is
%almost negligible, even for large $\Gamma$ values it gets
%remarkable for larger uncertainties. %\todo{Dennis: Den letzten Satz
                                %hat die Lektorin nicht
%verstanden. Und ich auch nicht...}

\begin{figure}[H]
\begin{center}
\centering
\begin{subfigure}[c]{0.43\textwidth}
\begin{tikzpicture}[y=.008cm, x=.1cm,font=\sffamily, only marks]
 	%axis
	\draw (0,0) -- coordinate (x axis mid) (40,0);
	\draw (0,600) -- coordinate (x axis mid) (40,600);
	\draw (40,0) -- coordinate (y axis mid) (40,600);
    	\draw (0,0) -- coordinate (y axis mid) (0,600);
    	
    	%ticks
    	\foreach \x in {0,10,...,40}
     		\draw (\x,0pt) -- (\x,-3pt)
     		node[anchor=north] {\x};
     	\foreach \x in {0,10,...,40}
     		\draw (\x,615) -- (\x,600);
    	\foreach \y in {0,100,...,600}
     		\draw (0pt,\y) -- (-3pt,\y) 
     			node[anchor=east] {\y }; 
     	\foreach \y in {0,100,...,600}
     		\draw (40,\y) -- (41.5,\y);
	%labels      
	\node[below=0.8cm] at (20,-10) {$\Gamma$};
	\node [rotate=90] at(-10,300) {objective value};

	%plots
	\draw[blue] plot[mark=*, style={mark size=0.8pt}, mark options={fill=blue}] 
	    file {neuobjpap9u2.data};
	\draw[violet] plot[ mark=*, style={mark size=0.8pt}, mark options={fill=violet}] 
	    file {objpap9.data};
	 \draw[red] plot[ mark=*, style={mark size=0.8pt}, mark options={fill=red}] 
	    file {neuobjpap9u1.data};
	%\draw[black] plot[ mark=none, mark options={fill=white}] 
	%   file {objscr15.data};	    
	 \matrix [draw,left] at (39,150) {
  \node [shape=circle, draw=violet,label=right:fei9 with $\mathcal{U}_1$ ] {}; \\
   \node [shape=circle, draw=red,label=right:fei9 with $\mathcal{U}_2$ ] {}; \\  	 
  \node [shape=circle, draw=blue,label=right: fei9 with $\mathcal{U}_3$ ] {}; \\
  %\node [shape=circle, draw=black, label=right: scr15 in $10^2$] {}; \\
};
\end{tikzpicture}
\subcaption{Optimal objective value $\times 10^{-4}$ for different values of $\Gamma$  for fei9.  \label{fig:objpap9}}
\end{subfigure}%
\hspace{0.1cm}
\begin{subfigure}[c]{0.55\textwidth}
\begin{tikzpicture}[y=.008cm, x=.11cm,font=\sffamily, only marks]
 	%axis
	\draw (0,0) -- coordinate (x axis mid) (60,0);
		\draw (0,600) -- coordinate (x axis mid) (60,600);
    	\draw (60,0) -- coordinate (y axis mid) (60,600);
    	\draw (0,0) -- coordinate (y axis mid) (0,600);
    	%ticks
    	\foreach \x in {0,10,...,60}
     		\draw (\x,0pt) -- (\x,-3pt)
			node[anchor=north] {\x};
		\foreach \x in {0,10,...,60}
     		\draw (\x,615) -- (\x,600);
    	\foreach \y in {0,100,...,600}
     		\draw (0pt,\y) -- (-3pt,\y) 
     			node[anchor=east] {\y }; 
     	\foreach \y in {0,100,...,600}
     		\draw (60,\y) -- (61.5,\y);
	%labels      
	\node[below=0.8cm] at (30,-10) {$\Gamma$};

	%plots
	\draw[blue] plot[ mark=*, style={mark size=0.8pt}, mark options={fill=blue}] 
	    file {neuobjscr12u2.data};
	\draw[violet] plot[ mark=*, style={mark size=0.8pt}, mark options={fill=violet}] 
	    file {objscr12.data};
	 \draw[red] plot[ mark=*, style={mark size=0.8pt}, mark options={fill=red}] 
	    file {neuobjscr12u1.data};
	%\draw[black] plot[ mark=none, mark options={fill=white}] 
	%   file {objscr15.data};	    
	 \matrix [draw,left] at (59,150) {
  \node [shape=circle, draw=violet,label=right:scr12 with $\mathcal{U}_1$] {}; \\ 
   \node [shape=circle, draw=red,label=right:scr12 with $\mathcal{U}_2$] {}; \\
  \node [shape=circle, draw=blue,label=right: scr12 with $\mathcal{U}_3$] {}; \\ 
  %\node [shape=circle, draw=black, label=right: scr15 in $10^2$] {}; \\
};
\end{tikzpicture}
\subcaption{Optimal objective value $\times 10^{-2}$ for different values of $\Gamma$ for scr12. \label{fig:objscr12}}
\end{subfigure}
\caption{Optimal solution for different instances.}\label{Fig:obj}
\end{center}
\end{figure}
%\begin{subfigure}[c]{0.55\textwidth}
%\begin{tikzpicture}[y=.008cm, x=.11cm,font=\sffamily, only marks]
% 	%axis
%	\draw (0,0) -- coordinate (x axis mid) (30,0);
%		\draw (0,200) -- coordinate (x axis mid) (30,200);
%    	\draw (30,0) -- coordinate (y axis mid) (30,200);
%    	\draw (0,0) -- coordinate (y axis mid) (0,200);
%    	%ticks
%    	\foreach \x in {0,10,...,30}
%     		\draw (\x,0pt) -- (\x,-3pt)
%			node[anchor=north] {\x};
%		\foreach \x in {0,10,...,30}
%     		\draw (\x,215) -- (\x,200);
%    	\foreach \y in {0,100,...,200}
%     		\draw (0pt,\y) -- (-3pt,\y) 
%     			node[anchor=east] {\y }; 
%     	\foreach \y in {0,100,...,200}
%     		\draw (30,\y) -- (31.5,\y);
%	%labels      
%	\node[below=0.8cm] at (15,-10) {$\Gamma$};
%    \node [rotate=90] at(-9.3,100) {objective value};
%	%plots
%	\draw[blue] plot[ mark=*, style={mark size=0.8pt}, mark options={fill=blue}] 
%	    file {objnug6u2.data};
%	\draw[violet] plot[ mark=*, style={mark size=0.8pt}, mark options={fill=violet}] 
%	    file {objnug6.data};
%	 \draw[red] plot[ mark=*, style={mark size=0.8pt}, mark options={fill=red}] 
%	    file {objnug6u1.data};
%	%\draw[black] plot[ mark=none, mark options={fill=white}] 
%	%   file {objscr15.data};	    
%	 \matrix [draw,left] at (59,150) {
%  \node [shape=circle, draw=violet,label=right:nug6 with $u_1$] {}; \\ 
%   \node [shape=circle, draw=red,label=right:nug6 with $u_2$] {}; \\
%  \node [shape=circle, draw=blue,label=right: nug6 with $u_3$] {}; \\ 
%  %\node [shape=circle, draw=black, label=right: scr15 in $10^2$] {}; \\
%};
%\end{tikzpicture}
%\subcaption{Optimal objective value for different $\Gamma$ for nug6 \label{fig:objnnug6}}
%\end{subfigure}


Now we compare the running time of different equivalent formulation of the $\Gamma$--counterpart. In particular, we test following formulations: 
\begin{itemize}
\item \texttt{QAP}: Formulation~\eqref{Prob:QAP_Reform_Two}.
\item $\texttt{QAP}_\texttt{red}$: Formulation~\eqref{Prob:QAP_Reform_Two} after reducing the number of subproblems with Theorem~\ref{Theo:RedNumber}.
\item \texttt{MIP}: A linearized QAP under uncertainty after applying Theorem~1 of \cite{IntroGamma}.
\item \texttt{BP}: A linearized QAP under uncertainty after applying Proposition~\ref{Prop:Tractable_Gamma_Comb}.
\item $\texttt{BP}_\texttt{red}:$ A linearized QAP under uncertainty after applying Proposition~\ref{Prop:Tractable_Gamma_Comb} and Theorem 1 of \cite{Lee2014}. 
\end{itemize} 
In particular, we apply a standard linearization: the product of two binary variables $x$ and $y$ can be replaced by a binary variable $z$ and the set of inequalities
\begin{gather*}
z \leq x, \ z \leq y, \ z \geq x + y - 1.
\end{gather*}
%We denote the formulation as given in the following:
%use the reformulation derived in Example~\ref{ex:QAP_genau}, 
%denoted as $QAP$, to obtain robust optimal solutions for different $\Gamma$. In the following, we denote the reformulation $\mathrm{QAP}$ with $n^4+1$ subproblems as $\mathrm{QAP}$ and the reduction with . Furthermore,we linearize problem by. The $\Gamma$--counterpart of the reformulations are equivalent to reformulations in \ref{Prop:Gamma_MIP} and \ref{Prop:Tractable_Gamma_Comb}, denoted by $\mathrm{QAP}_{\text{MIP}}$ and $\mathrm{QAP}_{\text{BP}}$. %and different instances.


%\begin{subfigure}[l]{\textwidth}
%\begin{tikzpicture}[y=.008cm, x=.13cm,font=\sffamily, only marks]
% 	%axis
%	\draw (0,300) -- coordinate (x axis mid) (90,300);
%		\draw (0,900) -- coordinate (x axis mid) (90,900);
%    	\draw (0,300) -- coordinate (y axis mid) (0,900);
%        \draw (90,300) -- coordinate (y axis mid) (90,900);
%    	%ticks
%    	\foreach \x in {0,10,...,90}
%     		\draw (\x,300) -- (\x,285)
%			node[anchor=north] {\x};
%		\foreach \x in {0,10,...,90}
%     		\draw (\x,915) -- (\x,900);
%    	\foreach \y in {300,400,...,900}
%     		\draw (0pt,\y) -- (-3pt,\y) 
%     			node[anchor=east] {\y  }; 
%     	\foreach \y in {300,400,...,900}
%     		\draw (90,\y) -- (91.5,\y);
%	%labels      
%	\node[below=0.8cm] at (45,290) {$\Gamma$};
%	\node [rotate=90] at(-9.3,550) {objective value};
%
%	%plots
%	\draw[blue] plot[ mark=*, style={mark size=0.8pt}, mark options={fill=blue}] 
%	    file {neuobjnug12u2.data};
%	\draw[violet] plot[ mark=*, style={mark size=0.8pt}, mark options={fill=violet}] 
%	    file {objnug12.data};
%	 \draw[red] plot[ mark=*, style={mark size=0.8pt}, mark options={fill=red}] 
%	    file {neuobjnug12u1.data};
%	%\draw[black] plot[ mark=none, mark options={fill=white}] 
%	%   file {objscr15.data};	    
%	 \matrix [draw,left] at (89,450) {
%	   \node [shape=circle, draw=violet,label=right:nug12 with $u_1$ ] {}; \\
%   \node [shape=circle, draw=red,label=right:nug12 with $u_2$ ] {}; \\
%  \node [shape=circle, draw=blue,label=right: nug12 with $u_3$  ] {}; \\
%  %\node [shape=circle, draw=black, label=right: scr15 in $10^2$] {}; \\
%};
%\end{tikzpicture}
%\subcaption{ Optimal objective value for different $\Gamma$ for nug12 \label{fig:objngy12}}
%\end{subfigure}
%\caption{Optimal solution for different instances}\label{Fig:obj}
%\end{center}
%\end{figure}
%
%
%
%We now compare the running times to solve the new reformulation $QAP$
%with those from \citep{IntroGamma}, see
%Remark~\ref{Rem:QAPLinearizations}. As all reformulations are exact,
%the solution values are the same. Using the original reformulation by
%Bertsimas and Sim, there are two
%possible settings. The first, denoted as $QAP_\mathrm{MIP}$,
%rewrites a nominal QAP instance as an MIP problem, using
%standard linearization. This MIP is then reformulated as one
%(enlarged) MIP using Proposition~\ref{Prop:Gamma_MIP} (see
%\cite{IntroGamma}, Theorem 1). In this second setting, the QAP is solved in oracle-polynomial time as a
%binary problem (BP) using Proposition~\ref{Prop:Tractable_Gamma_Comb}
%(see \cite{IntroGamma}, Theorem 3) and is denoted as $QAP_\mathrm{BP}$. As an oracle, we use Gurobi to solve the standard-linearized
%QAPs.
%
%To solve problem~\eqref{Prob:QAP_RobCP}, denoted by $QAP$, we determine solutions for
%\eqref{Prob:thetanichtnull} and \eqref{Prob:thetanull} and take the
%minimum of the objective values. %In the oracle calls, we do not need to
%%consider tuples $(i,j,r,s)\in [n]^4$ with $i=j$ and $r=s$. %, which amounts to %P for every $\theta_{ijrs}(x)=\Delta c_{ij}d_{rs}$ with $(i,j,r,s )\in [n]^4$ and $\theta_0(x)=0$ like shown in Example~\ref{ex:QAP_genau}. \todo{Hier kann man glaube ich schon viel mehr auf die Examples und auf Remarks eingehen und muss nicht mehr mit $\theta(x)$ um sich schlagen, wenn das schon alles in der Reformuling entknotet ist - vor allem, wenn $x$ schon gar keinen Einfluss mehr hat.}
%%This implies, we have
%%solving $n^4+1$ QAPs. % to determine the robust optimal solution.
%%However, $\theta_{ijrr}(x)=\Delta c_{ij} d_{rr} = 0 = \theta_0(x)$ since we know $d_{rr} = 0 $ for all $r \in  [n]$. Therefore, we do not have to consider any $\theta_{ijrs}(x)$ with $r=s$ in the outer optimization problem. 
%Since the obtained solution %$x$
%does not depend on $\Gamma$, we do not have to solve QAPs again when changing $\Gamma$ to
%$\Gamma_\mathrm{new}$, and we reuse all determined solutions.
%Reformulation $QAP_\textrm{adv}$ slightly improves over $QAP$ in the
%sense that it avoids additional unnecessary computations. 
%% Indeed,
%%we note that we can also omit the oracle call for all tuples $(i,j,r,s)\in[n]^4$
%%with $i=j$ and $r \neq s$ as then, either $x_{ir}=1=x_{is}$ which
%%leads to an infeasible assignment, or $\theta_{ijrs}(x)=0$. 
%
%
%%for $x$ and compare the objective values adding $\theta_{ijrs}(x)(\Gamma_\text{new}-\Gamma  )$.
%%To find the optimal solution for another $\bar{\Gamma}$ we only have to determine \[\min_{\theta} y^*_{\theta \Gamma} + \theta (\bar{\Gamma}-\Gamma). \]
%%Since the QAP is no linear problem we have to linearize the objective first.
%%For all $i,j,r,s \in [n]$, we apply a standard linearization of $x_{ir}x_{js}$ and introduce auxiliary variables $z_{ijrs}$, such that
%%\begin{align*}
%%& z_{irjs} \ge x_{ir} +x_{js} -1, \quad \forall (i,j,r,s) \in [n]^4,\\
%%&z_{irjs} \le x_{ir} , \quad \forall (i,j,r,s) \in [n]^4,\\
%% & z_{irjs} \le  x_{js}, \quad \forall (i,j,r,s) \in [n]^4,\\
%%& z_{irjs} \in [0,1], \quad \forall (i,j,r,s) \in [n]^4.
%%\end{align*}
%%The variables $z_{ijrs}$ are subject to the uncertain 'coefficients' $c_{ij}d_{rs} \in [d_{rs}\overline{c}_{ij}, d_{rs}(\overline{c}_{ij} + \Delta c_{ij})]$.
%%With that we have a MIP and can use the standard $\Gamma$-approach of Proposition~\ref{Prop:Gamma_MIP} (see \cite{IntroGamma} Theorem 1). We denote the resulting MIP as $QAP_\text{MIP}$. Because of the linearization we get $n^4$ more variables but we have to solve only one MIP.
%%If we further define $z_{ijrs} \in \{0,1\}$ we can apply Proposition~\ref{Prop:Tractable_Gamma_Comb} (see \cite{IntroGamma} Theorem 3). 
%%The resulting binary problem is denoted as $QAP_\text{BP}$. In that case we also have $n^4$ more variables like with $QAP_\text{MIP}$ but we also have to solve the same amount of single BPs like with problem $QAP$ and compare them.
%%Being exact reformulations the solutions of the $\Gamma$--counterpart determined in Example~\ref{ex:QAP_genau}, and the solutions of $QAP_\text{MIP}$ and $QAP_\text{BP}$ are the same. 
%%The running time in our approach depends on the time needed to
%%solve a QAP. Therefore, this method is useful if an oracle for solving QAP is
%%available. As we do not have such an oracle available, we used \texttt{Gurobi} to solve the QAPs.
%%To reduce the time needed to solve $QAP$, we omit redundant
%%$\theta$. The optimal objective value of
%%problem~\eqref{Prob:thetanull} is equivalent to the minimal objective
%%value of the inner optimization problem of
%%problem~\eqref{Prob:thetanichtnull} for any $\theta_{ijrs}(x)=0$ and
%%$(i,j,r,s)\in [n]^4$. We therefore omit all $\theta = 0$ except for
%%$\theta_0$.
%%\todo{Ich
%%  glaube, hier durfte man nicht alles streichen, denn $QAP_{adv}$
% % sollte glaube ich eine Form sein, bei der man von den $n^4 + 1$
%  %Problemen nochmal ein paar weglassen kann. - ok, das muss ich mit
%  %Jana dann nochmal besprechen} %\todo{Ich weiß nicht, wie verständnlcih das mit den $\theta$ ist.... Sollte man nicht über redundante Indizes sprchen? Und wurde das nicht weiter oben schon erklärt?}
The nominal programs can be solved  within a few seconds.
A comparison of running times for fei9, scr12 and nug12 and $\Gamma = 1$ can be found in
Tables \ref{Table_U1}, \ref{Table_U2} and \ref{Table_U3}. If no optimal solution could be computed after 24 hours, we stopped the process. Running times are measured in seconds. 
%For a QAPLIB topology, results do not differ much for different
%uncertainty sets. Results are reported for instance $\mathcal{U}_1$.
%\todo{Aktualisieren}
%
%%Table \ref{Table_solve} reports the running times for solving the
%%different reformulations. %Although the results are for $\Gamma=0$, the
%%running times differ as the (nominal) problem is written and solved
%%differently in each case, as described above.
%It turns out that for
%different values of $\Gamma$, the running times for solving $QAP$,
%$QAP_\mathrm{adv}$ and $QAP_\mathrm{BP}$ almost do not differ. Only solving the enlarged
%MIP, namely $QAP_\mathrm{MIP}$ gets more difficult for larger values of
%$\Gamma$. 
%For $QAP_\mathrm{MIP}$, one MIP with $n^4$ additional variables and $3\times n^4$ additional constraints has to be solved.
%For $QAP$, the single QAPs are smaller than the MIP but $\mathcal{O}(n^4)$ of them have to be solved. Therefore, it is not clear which method is
%faster. %even if the time needed to solve one QAP is smaller than the time needed to solve the MIP the running time of $QAP$ can exceed the running time of $QAP_\mathrm{MIP}$. 
%For $QAP_\mathrm{adv}$, less QAPs have to be solved than in $QAP$, but
%the reformulation is still slower than
%$QAP_\mathrm{MIP}$. $QAP_\mathrm{BP}$ has additional variables and constraints, like the MIP reformulation, but also $\mathcal{O}(n^4)$ BPs have to be solved. Consequently, this reformulation is the slowest to solve.
%
%%Since the constraints do not change for the different QAP and BP we can recycle our model for $QAP$, $QAP_\mathrm{adv}$ and $QAP_\mathrm{BP}$.\\
%%We note at this point that for $QAP$ some additional constraints are possible to speed up the process. In Example~\ref{ex:QAP_genau} we derived $\theta_{k_1k_2k_3k_4}=c_{k_1k_2}d_{k_3k_4}x_{k_1k_3}x_{k_2k_4}$. If $\theta_{k_1k_2k_3k_4}=0$ the inner optimization problem of Problem~\eqref{Prob:thetanichtnull} is equivalent to Problem~\eqref{Prob:thetanull} and the optimal objective value will not be better. Therefore, the objective value of Problem~\eqref{Prob:thetanichtnull} can only be smaller than the solution of Problem~\eqref{Prob:thetanull} if $\theta_{k_1k_2k_3k_4}>0$. Hence, $x_{k_1k_3}=x_{k_2k_4}=1$ has to hold. We therefore compute a solution for every $\theta_{k_1k_2k_3k_4}$ and demand that $x_{k_1k_3}=x_{k_2k_4}=1$. In this way, some variables are already defined at the beginning of the process and thus the running time is accelerated. However, the QAP structure will be lost and a QAP solver might not be able to compute a solution. Therefore, this reformulation is no part of that experiment.
%
%%\todo{Frauke: Was sind die korrekten Laufzeiten fuer Gamma
%%  Null? Hier gibt es ja noch gar keine Reformulierungen? Oder handelt
%%  es sich hier um einmal das standard-linearisierte MIP (QAP-MIP)
%%  vs. das QAP mit Gurobi zu loesen, ohne Linearisierung (QAP)? dann
%%  muessten die beiden anderen Zeilen adv / BP weg... Dann ist aber
%%  immer noch seltsam dass sich die laufzeiten zwischen gamma null und
%%  gamma = 1 kaum unterscheiden...}
%%\begin{table}[H]
%%\centering
%%\caption{Comparison of running times for different instances for $\Gamma = 0$,  - if not solvable within 24 hours \label{Table_solve}} 
%%\begin{tabular}{|l|r|r|r|}
%%\hline 
%%CPU (s) & nug6 & fei9 & scr12 \\ 
%%\hline 
%%$QAP$& 79 & 4684 & 51221  
%% \\ 
%%\hline 
%%$QAP_\mathrm{adv}$  &50 & 2217
%% & 23711  \\ 
%%\hline 
%%$QAP_\mathrm{MIP}$  &1 & 14 & 714  \\ 
%%\hline 
%%$QAP_\mathrm{BP}$ &  418 & - & - \\ 
%%\hline 
%%\end{tabular}
%%\end{table}
%%\todo{Dennis: Ich habe jetzt mal selber den nominellen Teil programmiert, hatte recherchiert und die Laufzeiten wirken astronomisch. Tatsächlich bekamm ich beim reinen QAP, wenn man es nominell löst, für scr12 eine Laufzeit von $2,5$ Sekunden statt 51221.... ich hab mir dann erschlossen, dass hier tatsächlich mit dem Gamma-Counterpart gearbeitet wurde, verstehe aber nicht warum, anstatt einfach das nominelle Problem zu lösen. Wenn man die $n^4 + 1$ mit 2.5 multipliziert, kommt man ungefähr auf die 51000, so hatte ihc mir das dann erschlossen... aber sollte man nicht außer $QAP_MIP$ (ist da eigentlich auch der Gamma-Counterpart genommen worden oder die Linearisierung des nominellen?) und QAP alle rauswerfen und lediglich mit dem nominellen arbeiten? Es gibt ja im nominellen genau gar keinen grund, den Counterpart zu benutzen, oder sehe ich da was falsch...? V.a. bei 50000 vs 2.5....}
%%\todo{Dennis: Wie sehen die Modelle im nominellen Falla $\Gamma = 0$
%%  aus? Warum betrachtet man verschiedene Modelle? Kann man nicht
%%  einfach nur das UrsprungsQAP lösen? Wie wirkt sich das adv in
%%  nominellan aus, wenn ich doch nur ein QAP lösen muss?}
%%\todo{Dennis: max im Index bitte mit mathrm oder text so getsalten wir MIP oder BP im text.}
\begin{table}[H]
\centering
\caption{Comparison of running times for different instances for $\Gamma = 1$ and the deterministically constructed uncertainty set $\mathcal{U}_1$. -- if not solvable within 24 hours. \label{Table_U1}} 
\begin{tabular}{|l|r|r|r|}
\hline 
 CPU (s)& nug12 & fei9 & scr12  \\ 
\hline 
$\texttt{QAP}$& -- & 3420 & 36579
 \\ 
\hline 
$\texttt{QAP}_\texttt{red}$ & 1054  & 174 & 221  \\ 
\hline 
$\texttt{MIP}$ & 31417 & 25 &  1718 \\ 
\hline 
$\texttt{BP}$ & -- & 86243 & -- \\ 
\hline 
$\texttt{BP}_\texttt{red}$ & 34318 & 4096 & 49126 \\ 
\hline
\end{tabular}
\end{table}
\begin{table}[H]
\centering
\caption{Comparison of running times for different instances for $\Gamma = 1$ and the deterministically constructed uncertainty set $\mathcal{U}_2$. -- if not solvable within 24 hours. \label{Table_U2}} 
\begin{tabular}{|l|r|r|r|}
\hline 
 CPU (s)& nug12 & fei9 & scr12  \\ 
\hline 
$\texttt{QAP}$& -- & 3542 & 74641
 \\ 
\hline 
$\texttt{QAP}_\texttt{red}$ & 591  & 178 & 298  \\ 
\hline 
$\texttt{MIP}$ & 24655 & 25 &  819 \\ 
\hline 
$\texttt{BP}$ & -- & -- & -- \\ 
\hline 
$\texttt{BP}_\texttt{red}$ & -- & 4538 & 73847 \\ 
\hline
\end{tabular}
\end{table}
\begin{table}[H]
\centering
\caption{Comparison of running times for different instances for $\Gamma = 1$ and the randomly constructed uncertainty set $\mathcal{U}_3$. - if not solvable within 24 hours. \label{Table_U3}} 
\begin{tabular}{|l|r|r|r|}
\hline 
 CPU (s)& nug12 & fei9 & scr12  \\ 
\hline 
$\texttt{QAP}$ & -- & 3503 & 45851
 \\ 
\hline 
$\texttt{QAP}_\texttt{red}$ & 9507  & 178 & 275  \\ 
\hline 
$\texttt{MIP}$ & 19550 & 30 &  1860 \\ 
\hline 
$\texttt{BP}$ & -- & -- & -- \\ 
\hline 
$\texttt{BP}_\texttt{red}$ & -- & 4384 & 56979 \\ 
\hline
\end{tabular}
\end{table}
It is evident that the instances with $n=12$ can be solved more
efficiently than the linearizations after reducing the number of
subproblems by excluding all redundant scenarios (applying
Theorem~\ref{Theo:RedNumber}, neglecting identical subproblems and
taking symmetry of coefficients into account), for all regarded
uncertainty sets. Only for the smaller instance, \texttt{MIP} is
faster. This demonstrates the benefit of the reformulations
proposed here. Without using them, the corresponding robust
counterparts are algorithmically very challenging. All instances have in common that without reducing
the number of programs, i.e., avoiding a repetition of scenarios or
applying Theorem~\ref{Theo:RedNumber}, these instances cannot be
solved within the time limit, even for smaller instances.

Finally, we would like to point out two things: Firstly, if one would
like to solve $\Gamma$--counterpart for different values of $\Gamma$,
it is preferable to apply $\texttt{QAP}_\texttt{red}$ since one only
has to calculate the optimal solutions of the subproblems for $\Gamma
= 1, 2$, since the value of $\Gamma$ does not influence the
subproblems. Secondly, this computational study 
demonstrates that our formulations are applicable in
practice. Naturally, instead of using Gurobi, one can also use
algorithms that solve QAPs more efficiently. However, for
our purposes, our method proved to be highly beneficial, when compared to the standard
linearization approach.
%%%%%
%%%%%In our tests, solving $QAP_\mathrm{MIP}$ was faster than the other reformulations if a solution for only a single $\Gamma$ is required. However, we would like to point out that this situation can easily change when considering at a robust optimization problem for which a problem-specific efficient oracle is at hand. Many combinatorial optimization problems have been addressed by intensive research efforts, resulting in efficient implementations that can serve as oracles. In this case, it may be reasonable to assume that solving the new reformulation is beneficial as efficient oracles can be used, rather than solving a (usually considerably increased) MIP. This situation is comparable to the original reformulation by Bertsimas and Sim. %\todo{Kann man hier nicht Bezug nehmen auf Section 4, genau wi eam Anfang von diesem Abschnitt, in dem genau auf Reformulierungen, die verwenden werden, hingewiesen werden?}
%%%%%Let us consider a situation where even without an oracle, solving our reformulation is beneficial. Assuming we need to
%%%%%determine a solution for more than one $\Gamma$, the MIP has to be solved again for $QAP_\mathrm{MIP}$ whereas this is not the case for $QAP_\mathrm{BP}$ and for $QAP$. For each of the inner optimization problems of \eqref{Prob:thetanichtnull}, the optimal solution for \eqref{Prob:thetanull} can be reused. Thus, we only have to compare the objective values with the weighting of the new $\Gamma$, which can quickly be done.
%%%%%% \todo{was ist hier das outer optimization problem? worauf beziehst du dich, welche formel?}. 
%%%%%%This is possible within seconds.
%%%%%The sum of the running times for different values of $\Gamma$ are compared in Tables \ref{Table0.25}-\ref{Table1}. We note that  $\Gamma_\mathrm{\max}=20$ for nug6, $\Gamma_\mathrm{\max}= 34$ for fei9 and $\Gamma_\mathrm{\max}=56$ for scr12. 
%%%%%%Considering in addition the nominal case, at most $\Gamma_{max} +1$
%%%%%%many problems need to be solved.
%%%%%We now compare
%%%%%running times for determining solutions for
%%%%%$\left\lceil\frac{\Gamma_\mathrm{\max} +1}{4}\right\rceil$ (Table~\ref{Table0.25}), $\left\lceil\frac{\Gamma_\mathrm{\max}
%%%%%  +1}{2}\right\rceil$(Table~\ref{Table0.5}), $\left\lceil\frac{3(\Gamma_\mathrm{max} +1)}{4}\right\rceil$ (Table~\ref{Table0.75}) or
%%%%%$\Gamma_\mathrm{\max}$ (Table~\ref{Table1}) different $\Gamma$.
%%%%%As discussed previously, the running times for $QAP$, $QAP_\mathrm{adv}$ and $QAP_\mathrm{BP}$ for several $\Gamma$ do not markedly differ from the running times for a single $\Gamma$.
%%%%%However, the running times for $QAP_\mathrm{MIP}$ rise dramatically for increasing $\Gamma$ values.
%%%%%For scr12, solving $QAP_\mathrm{adv}$ is faster than $QAP_\mathrm{MIP}$ if
%%%%%half of all possible $\Gamma$ must be computed, as shown in Table~\ref{Table0.5}. %For fei9 and nug6, our reformulations are slower than $QAP_\mathrm{MIP}$. 
%%%%%It can therefore be concluded even without an efficient
%%%%%oracle, solving the new reformulation is
%%%%%beneficial provided solutions for several $\Gamma$ values need to be determined simultaneously. 
%%%%%
%%%%%\begin{table}[H]
%%%%%\centering
%%%%%\caption{Comparison of the sum of the running times for solving $\left\lceil\frac{\Gamma_\mathrm{\max} +1}{4}\right\rceil$ different $\Gamma$ in seconds, - if not solvable in 24 hours \label{Table0.25}} 
%%%%%\begin{tabular}{|l|r|r|r|}
%%%%%\hline 
%%%%%CPU (s)& nug6 $\Gamma = [5]$ & fei9 $\Gamma = [8]$ & scr12 $\Gamma =[14]$   \\ 
%%%%%\hline 
%%%%%$QAP$ &79 & 4684 & 51221 
%%%%% \\ 
%%%%%\hline 
%%%%%$QAP_\mathrm{adv}$ &50 &2217 & 23711  \\ 
%%%%%\hline 
%%%%%$QAP_\mathrm{MIP}$ & 4 & 326 & 11106 \\ 
%%%%%\hline 
%%%%%$QAP_\mathrm{BP}$ & 418 & - & - \\ 
%%%%%\hline 
%%%%%\end{tabular}
%%%%%\end{table}
%%%%%
%%%%%%\todo{Und auch hier sieht es wieder komisch aus, dass QAP, QAPadv und QAPBP sich nicht mal um eine Sekunde unterscheiden.}
%%%%%\begin{table}[H]
%%%%%\centering
%%%%%\caption{Comparison of the sum of the running times for solving $\left\lceil\frac{\Gamma_\mathrm{\max} +1}{2}\right\rceil$ different $\Gamma$ in seconds, - if not solvable in 24 hours \label{Table0.5}}
%%%%%\begin{tabular}{|l|r|r|r|}
%%%%%\hline 
%%%%%CPU (s) &  nug6 $\Gamma = [10]$  & fei9 $\Gamma = [17]$ & scr12 $\Gamma = [28]$\\ 
%%%%%\hline 
%%%%%$QAP$&79 & 4684 & 51222 
%%%%% \\ 
%%%%%\hline
%%%%%$QAP_\mathrm{adv}$ &50 & 2217 & 23712  \\ 
%%%%%\hline  
%%%%%$QAP_\mathrm{MIP}$ & 9 & 766 & 18117 \\ 
%%%%%\hline 
%%%%%$QAP_\mathrm{BP}$ & 418 & - & -\\ 
%%%%%\hline
%%%%%\end{tabular} 
%%%%%\end{table}
%%%%%
%%%%%\begin{table}[H]
%%%%%\centering
%%%%%\caption{Comparison of the sum of the running times for solving $\left\lceil\frac{3(\Gamma_\mathrm{\max} +1)}{4}\right\rceil$ different $\Gamma$ in seconds, - if not solvable in 24 hours \label{Table0.75}} 
%%%%%\begin{tabular}{|l|r|r|r|}
%%%%%\hline 
%%%%%CPU (s)&nug6 $\Gamma=[15]$ & fei9 $\Gamma = [26]$ & scr12 $\Gamma = [42]$  \\  
%%%%%\hline 
%%%%%$QAP$ & 79 & 4684 & 51223 
%%%%% \\ 
%%%%%\hline
%%%%%$QAP_\mathrm{adv}$ & 50  & 2217 & 23712 \\ 
%%%%%\hline  
%%%%%$QAP_\mathrm{MIP}$ &13  & 1224 & 37714 \\ 
%%%%%\hline 
%%%%%$QAP_\mathrm{BP}$ & 418 & - & -  \\ 
%%%%%\hline 
%%%%%\end{tabular}
%%%%%\end{table}
%%%%%
%%%%%
%%%%%\begin{table}[H]
%%%%%\centering
%%%%%\caption{Comparison of the sum of the running times for solving $\Gamma_\mathrm{\max}$ different $\Gamma$ in seconds, - if not solvable in 24 hours \label{Table1}} 
%%%%%\begin{tabular}{|l|r|r|r|}
%%%%%\hline 
%%%%% CPU (s) & nug6 $\Gamma =[20]$ & fei9 $\Gamma = [34]$ & scr12 $\Gamma = [56] $\\ 
%%%%%\hline 
%%%%%$QAP$ &79 & 4685 & 51223 
%%%%% \\ 
%%%%%\hline 
%%%%%$QAP_\mathrm{adv}$ &50 & 2217 & 23712 \\ 
%%%%%\hline 
%%%%%$QAP_\mathrm{MIP}$ &17  & 1669 & 56516   \\ 
%%%%%\hline 
%%%%%$QAP_\mathrm{BP}$ & 418 & - & -  \\ 
%%%%%\hline 
%%%%%\end{tabular}
%%%%%\end{table}
%%%%%%\todo{Dennis: Warum mal mit nominell und mal ohne? Ist das nominelle in dieser Betrachtung relevant?}


%\todo[inline]{Wir werden noch versuchen das als kombinatorisches Problem umzuschreiben und dann mit der Supportfunktion etwas hanhabbares herauszubekommen. Im paper wurde linearisiert, damit werden wir uns dann vergleichen}
%In \cite{QAP2012} it is assumed that the locations of the facilities are uncertain.
%This is the case if, for example, it is not yet certain where exactly construction is to take place. 
%Formally two uncertain $\bar{u}^1_r$ and $\bar{u}^2_r$ coordinates are therefore assigned to each facility $r$ with $\bar{u}^1_r=[u^1_r,u^1_r+\Delta u^1_r]$ and $\bar{u}^2_r=[u^2_r,u^2_r + \Delta u^2_r]$.
%This leads to the fact that the distance between two facilities is uncertain and is labeled $d(\xi)$. 
%The uncertainty set can now be modeled as 
%%box uncertainty $\mathcal{U}_b^{\xi}=\{(\xi^1,\xi^2):\xi^1,\xi^2\in \mathbb{R}^n, 0 \le \xi^1,\xi^2 \le 1 \forall r \in N\}$ which is very conservative and covers all possibilities within an interval or
%$\Gamma$ uncertainty $\mathcal{U}^{\xi}_{\Gamma}=\{\xi \in U_b^{\xi}: \sum_{r=1}^n (\xi_r^1+\xi_r^2)\le \Gamma\}$. 
% With this the uncertain distance is determined as: 
%\begin{align*}
%& d_{rs}(\xi)=|u^1_r-u^1_s+\xi \Delta u^1_r-\xi \Delta u^1_s|+|u^2_r-u^2_s+\xi_r^x \Delta u^2_r-\xi_r^y \Delta u^2_s|\\
%&\xi \in \mathcal{U}^{\xi}_{\Gamma}
%\end{align*}
%The following optimization problem has to be solved for the robust counterpart
%\todo{Frauke: Was ist q?}
%\begin{align}
%\min_{x\in \mathcal{X}} \max_{\xi \in \mathcal{U}_{\Gamma}^{\xi}} q_{d}(x,\xi) 
%\tag*{\llap{RQAP(d)}}
%\end{align}
%Since the maximum requires solving a nonconvex optimization problem, some transformations has to be made to make it tractable.
%First it can be shown that $q_{d}(x,\xi)$ is piecewise linear and convex in the uncertainty \cite{QAP2012}. 
%Furthermore, it is assumed that $\Gamma$ is integer.
%Since an extreme point is assumed where all $\xi$ are 0 or 1, all possible combinations are calculated for all distances of two facilities. 
%Then the robust counterpart can be determined, via calculating the objective function at the extreme points.
%By introducing further variables and transformations a MILP can be obtained. As a convention, the extreme distances are defined as $d_{\bar{rs}}^x$ for $\xi =1 $ and as $d_{\underline{rs}}^1$ for $\xi=0$ on the location variables $r$ and $s$ in $d_{rs}^1$.
%Some variables are defined in advance for the sake of readability.
%\todo[inline]{Deren Linearisierung sollte vielleicht nicht so genau aufgeführt sein. Das wird vermutlich noch auskommentiert, wir würden aber gerne schaun, ob wir etwas handhabbares mit Fenchel herausbekommen und dann damit vergleichen}
%\begin{align*}
%& C_{rs}^1 = 0.5 (d_{\overline{r}\underline{s}}^1+d_{\underline{rs}}^1+d_{\underline{r}\bar{s}}^1-d_{\overline{rs}}^1),\\
%& C_{rs}^2 = 0.5 (d_{\overline{r}\underline{s}}^2+d_{\underline{rs}}^2+d_{\underline{r}\bar{s}}^2-d_{\overline{rs}}^2)\\
%& B_{rs}^1 = 0.5 (d_{\overline{r}\underline{s}}^1-d_{\underline{rs}}^1-d_{\underline{r}\bar{s}}^1+d_{\overline{rs}}^1),\\
%& B_{rs}^2 = 0.5 (d_{\overline{r}\underline{s}}^2-d_{\underline{rs}}^2-d_{\underline{r}\bar{s}}^2+d_{\overline{rs}}^2)\\
%&D_{rs}^1 = 0.5 (d_{\overline{r}\underline{s}}^1-d_{\underline{rs}}^1+d_{\underline{r}\bar{s}}^1-d_{\overline{rs}}^1),\\
%& D_{rs}^2 = 0.5 (d_{\overline{r}\underline{s}}^2-d_{\underline{rs}}^2+d_{\underline{r}\bar{s}}^2-d_{\overline{rs}}^2)\\
%& c_{rs}(x)= \sum_{i=1}^n\sum_{j=1}^n c_{ij}d_{rs}x_{ir}x{js}, 
%\end{align*}
%\begin{align}
%\begin{split}
%\min_{x\in \mathcal{X}} & \sum_{r=1}^{n}\sum_{s=1}^n [(C^1_{rs}+C^2_{rs})c_{rs}(x)+u_{rs}^1+u_{rs}^2]+\Gamma \theta + \sum_{r=1}^n (p_r^1+p_r^2) \\
%s.t. & \sum_{s=1}^n u_{rs}^1 + p_r^1 +\theta \ge \sum_{s=1}^{n} B_{rs}^1 (c_{rs}(x)+c_{sr}(x)), \forall r \in [n]\\
%& \sum_{s=1}^n u_{rs}^2 + p_r^2 + \theta \ge \sum_{s=1}^{n} B_{rs}^2 (c_{rs}(x)+c_{sr}(x)), \forall r \in [n]\\
%& -D_{rs}^1 c_{rs}(x) \le u_{rs}^1\le D_{rs}^1 c_{rs}(x), \forall i,r,s \in [n]\\
%&-D_{rs}^2 c_{rs}(x) \le u_{rs}^2\le D_{rs}^2 c_{rs}(x), \forall i,r,s > r \in [n]\\
%&z,p_r^1,p_r^2 \ge 0 ,  \forall r,s \in [n]
%\end{split}
%\end{align}
%Now we want to compare (RQAP) with QAP robustified by the methods in this chapter.
%In order to apply Theorem~\ref{Theo:FenchelGammaCounterpart}, the objective function has to be concave in  the uncertainty. 
%This is obviously not the case with $q_{d}(x,\xi)$, instead convexity in the uncertainty can be verified. 
%%\begin{align*}
%%& f_i(\lambda \xi + (1- \lambda)\bar{\xi}) = \\
%%&c_{ij}x_{ir}x_{js}( |u^1_r-u^1_s + (\lambda \xi_r u^1 + (1- \lambda)\bar{\xi_r^1})\bar{u}^1_r-(\lambda \xi_s^1 + (1- \lambda)\bar{\xi_s^1})\bar{u^1_s}|+
%%\\ & |u^2_r-u^2_s + (\lambda \xi_r^2 + (1- \lambda)\bar{\xi_r^2})\bar{u}^2_r-(\lambda \xi_s^2 + (1- \lambda)\bar{\xi_s^2})\bar{u}^2_s|)= \\
%%&c_{ij}x_{ir}x_{js}( |(\lambda+1-\lambda)(u^1_r-u^1_s) + (\lambda \xi_r^1 + (1- \lambda)\bar{\xi_r^1})\bar{u}^1_r-(\lambda \xi_s^1 + (1- \lambda)\bar{\xi_s^1})\bar{u}^1_s|+\\
%%& |(\lambda+1-\lambda)(u^1_r-u^1_s) + (\lambda \xi_r^2 + (1- \lambda)\bar{\xi_r^2})\bar{u}^2_r-(\lambda \xi_s^2 + (1- \lambda\bar{\xi_s^2})\bar{u}^2_s|)\le\\
%%&c_{ij}x_{ir}x_{js}( \lambda|| u^1_r- u^1_s + \xi_r^1\bar{u^1_r}- \xi_s^1 \bar{u}^1_s|+ |u^2_r-u^2_s +  \xi_r^2 \bar{u}^2_r + - \xi_s^1 \bar{u}^2_s||) +\\
%%&(1-\lambda)|| u^1_r- u^1_s + \bar{\xi_r^1}\bar{u}^1_r- \bar{\xi}^1_s \bar{u}^1_s|+ |u^2_r-u^2_s +  \bar{\xi}_r^2\bar{u}^2_r  - \bar{\xi}_s^2 \bar{u}^2_s||=\\
%%& \lambda c_{ij}x_{ir}x_{js}(| u^1_r- u^1_s + \xi_r^1\bar{u}^1_r- \xi_s^1 \bar{u}^1_s|)+ |u^2_r-u^2_s +  \xi_r^2\bar{u}^2_r  - \xi_s^2 \bar{u}^2_s|) + \\
%%&(1-\lambda)c_{ij}x_{ir}x_{js}(| u^1_r- u^1_s + \bar{\xi}_r^1\bar{u}^1_r)- \bar{\xi}_s^1 \bar{u}^1_s|)+ |u^2_r-u^2_s +  \bar{\xi}_r^2\bar{u}^2_r  - \bar{\xi}_s^2 \bar{u}^2_s|)=\\
%%& \lambda f(\xi)+(1-\lambda) f(\bar{\xi})
%%\end{align*}
%\todo[inline]{Ab hier ist noch ein Fehler, weil die Unsicherheiten nicht unabhängig sin. Daher kann man das nicht ohne weiteres anwenden}
%In order to get an optimization problem that is tractable, we reparametrize.
%For this, the objective function $f(\xi)^Tg(x)$ is rewritten as $b^Tg(x)$ with 
%$\mathcal{U}=\{(\xi,b): u\in \mathcal{U}=\bar{\mathcal{U}}, b= f(\xi)\}$. Thus, the function is linear in uncertainty. 
%With the convex envelope of $\bar{\mathcal{U}}$ RC can be determined.
%Since the uncertainties are independent of each other,  for the objective function follows $f_i(\xi)=f_i(\xi_i)$.
%Other changes have been applied so that $f_i(\xi)=c_{ij}x_{ir}x_{js}(| u^1_r- u^1_s + \xi_r^1\bar{u}^1_r - \xi_s^1 \bar{u}^1_s|+ |u^2_r-u^2_s +  \xi_r^2\bar{u}^2_r  - \xi_s^2 \bar{u}^2_s|)$. 
%In this case the uncertainty set can be expanded to $\mathcal{U}=\{-1 \le \xi \le 1\}$, because the $\xi$ are moving the spots apart. For negative $\xi$ improve the optimisation problem those will never be part of the worst case and so the uncertainty set can be expanded to $\xi \ge -1$. 
%This makes it easy to calculate the convex hull.
%The objective function can be linearized to
%\begin{align*}
%&b^Tg(x)\\
%& (u,b) \in \mathcal{U}=\{(\xi,b): \xi \in \mathcal{U}, b= f(\xi)\}
%\end{align*}
%For the fenchel duality we need $conv(\mathcal{U})$.
%The uncertainty sets are equivalent due to the linearity.
%\[conv(\mathcal{U})= \{(\xi_i,b_i)| -1 \le \xi_i \le 1, b_i \ge f_i(\xi_i), 2b_i \le f_i(1)(a_i+1) - f_i(-1)(a_i-1), \forall i\}\]
%The last inequality follows from the convexity inequality$f(\lambda x + (1-\lambda) y)\le \lambda f(x) +(1-\lambda) f(y)$ with $x=1, y=-1$ and $\lambda = \frac{\xi_i-1}{2}$.
%With this the robust counterpart is
%\[b^Tg(x) \qquad (\xi_i,b_i) \in conv(\mathcal{U}).\]
%Because of the following equality
%\[\delta^*(y|\mathcal{U}_1 \times \dots \times \mathcal{U}_n)= \sum_{i=1}^n \delta^*(y|\mathcal{U}_i)\]
%we divide our uncertainty set into three and get for the QAP
%\[ \delta^*(y^i|\mathcal{U}_i) = \min_{y^{i1}, y^{i2}, y^{i3}} \{ \delta^*(y^{i1}|\mathcal{U}_{i1})+\delta^*(y^{i2}|\mathcal{U}_{i2})+\delta^*(y^{i3}|\mathcal{U}_{i3})|y_{i1}+y^{i2}+y^{i3} = y^i\}.\]
%For those uncertainty sets we can derive the support function.
%\begin{align*}
%&\delta^*(y^{i1}|\mathcal{U}_{i1}) = \max_{\xi_i,b_i}\{y_1^{i1}\xi_i+y_2^{i1}b_i | |\xi_i|\le 1 \} = \begin{cases}|y_1|&\text{if } y_2^{i1}=0\\\infty&\text{else}\end{cases}\\
%&\delta^*(y^{i2}|\mathcal{U}_{i2})= \max_{\xi_i,b_i}\{y_1^{i2}\xi_2+y_2^{i2}b_i|f_i(\xi_i)-b_i \le 0\} =\min_{a_i\ge 0}\{a_if_i^*(\frac{y_1^{i2}}{a_i})|y_2^{i2} = -a_i\}\\
%&\delta^*(y^{i3}|\mathcal{U}_{i3})= \max_{\xi_i,b_i}\{y_1^{i3}\xi_i+y_2^{i3}b_i | \alpha_i^T(\left(\begin{array}{c} \xi_i \\ b_i \end{array}\right) )\le \gamma\} = \min_{z_i \ge 0}\{\gamma z_i | z_i \alpha_i =y^{i3}\}\\
%&\text{where}\\
%& \alpha_i = \left(\begin{array}{c} f_i(-1)-f_i(1) \\ 2 \end{array}\right)\\
%&\gamma_i = f_i(1)+f_i(-1)
%\end{align*}
%With that the robust counterpart can be written as 
%\begin{align}
%\begin{split}
%&(u_0)^Tx + \sum_i |y_1^{i1}|+ \sum_i a_i f^*_i(\frac{y_1^{i2}}{a_i})+\frac{1}{2}\sum_i \gamma_ia_i \le 0\\
%&y_1^{i1}+y_1^{i2}+\frac{1}{2}a_i(f_i(-1)-f_i(1))= v_i\\
%&a \ge 0 \end{split}
%\tag*{\llap{FRC(QAP)}}
%\end{align}
%Because of the linearity of the uncertainty the conjugate function equals $0$ and also $u_0=0$. With that:
%\begin{align}
%\begin{split}
%& \sum_i |y_1^{i1}|+\frac{1}{2}\sum_i \gamma_ia_i \le 0\\
%&y_1^{i1}+y_1^{i2}+\frac{1}{2}a_i(f_i(-1)-f_i(1))= v_i\\
%&a \ge 0 \end{split}
%\tag*{\llap{FRC(QAP)}}
%\end{align}


%$\rightarrow$ application for SFB \cite{QAM}\\
%\todo[inline]{Jana: Paper reinstellen, welche relevant sind}
%\todo[inline]{Jana: Paper zusammenfassen (Achtung Notation!)}
%\todo[inline]{Jana: Bisherige Ergebnisse auf das QAP anwenden -> sieht man vergleichbares? Modelle sind äquivalent?!}
%\todo[inline]{Dennis: Für die MA relevant?} 

%\subsection{Robust scheduling}

%\cite{RobustScheduling}

%\subsection{Lagrangian Relaxation under uncertainty}


==> Conclusion_OR.tex <==
\section{Conclusion} \label{Sec:Conclus}
In this paper, we studied $\Gamma$--counterparts of discrete nonlinear
optimization problems under uncertainty in the objective. We established reformulations of $\Gamma$--counterparts by applying reformulations techniques developed in \cite{Fenchel}. Similar to $\Gamma$--uncertainties in \cite{IntroGamma} and \cite{PriceRobust}, our reformulations work for general MINLPs and for combinatorial optimization problems with linear uncertainty when attempting to optimize over the original feasible set $\mathcal{X}$. While those reformulations are not necessarily computationally tractable, we have provided examples where this is indeed the case, namely for linear uncertainties involving $0/1$--functions, programs involving some kind of assignment structure.
Furthermore, we discussed the general case with an application in logistics. %Finally, for our computational study, we showed that our reformulations are applicable in practice and can outperform linearized $\Gamma$--counterparts.
Possible further research for this topic include extensive numerical studies for the derived reformulations that could be based on our prototypical study in the electronic companion. Furthermore, one could also investigate whether the generalizations of \cite{Poss12}, \cite{Poss14} and \cite{POSS2018} to the nonlinear $\Gamma$--counterpart are possible and tractable as well. Finally, one could attempt to investigate cases where one could extend the optimization oracle from $\mathcal{X}$ to $\mathcal{X}_\mathcal{Q}$ as in the setting of Theorem~\ref{Cor:LinInt} or to perform, under further assumptions, more reformulations that reduce the number of the problems from exponential to polynomial im $m$, similar to Theorem~\ref{Theo:CorrDoNotCare}. %Furthermore, the price of robustness was not investigated in this publication as it was in \cite{PriceRobust} which could also be subject to future research.
%Our theoretical results predominantly center on reformulations and generalizations that raise further questions: Furthermore, one could further analyze the effect of coefficients correlated by uncertainty in a linear setting, not only for the $\Gamma$--approach but in general. In \cite{PriceRobust}, MIPs with constraints subject to uncertainty have been discussed. In this case, the authors proposed probabilistic guarantees for a solution $x$ staying feasible when the number of coefficients realizing an uncertainty bigger than the anticipated $\Gamma$. It would be interesting to obtain similar probabilistic guaranteed for MINLPs. %Finally, from a practical point of view, one could conduct numerical studies that compare our counterparts with other models and concepts of robust optimization. %While we outlined possibilities for the QAP already in Section~\ref{Sec:App}, one could use other approaches in the sense of different concepts for robust optimization, e.g. the adversarial approach \cite{ApplDec2} or an adjustable setting that applies decision rules, e.g. \cite{ApplDec1}.


==> Generalization_OR.tex <==
\subsection{Introduction of our model and applications} \label{Sec:General}
In this subsection, we extend  program~\eqref{Prob:Gamma_Comb} to MINLPs that are subject to uncertainty in the
objective. %We note that the case of constraints subject to uncertainty can be handled analogously and can be found in Appendix A.
%In addition, by including several examples from a range of areas, we show that the new robust counterpart is beneficial in various situations, as it leads to new formulations and less conservative solutions, when compared to the standard counterpart from Proposition~\ref{Prop:Tractable_Gamma_Comb}. Finally, we apply the counterpart to nonlinear discrete optimization problems. Since the case of uncertainty in the constraints can be
%tackled analogously, we refer, for the rest of this paper, to Appendix
%A for this case.\\
We consider the program
\begin{align}\label{Prob:GeneralNomOpt}
\begin{split}
\inf_{x \in \mathcal{X}} & \sum_{i \in [m]} \ \overline{f}_i(x),
\end{split} 
\end{align}
where $\overline{f}_i \colon \R^n \to \R$ is an arbitrary but fixed function for every $i \in [m]$ and $\mathcal{X} \subseteq \Z^p \times \R^{n-p}$ where $p \in [n]_0$. We assume that every function $\overline{f}_i$ is 'contaminated' by an uncertainty set $\mathcal{U}_i \subseteq \R^{L_i}$, i.e., we define %extend $\overline{f}_i$ to 
%\begin{gather*}
$f_i \colon \R^n \times \mathcal{U}_i \to \R$
%\end{gather*} 
with $f_i(x,\overline{u}^i):= \overline{f}_i(x)$ for a nominal scenario $\overline{u}^i \in \mathcal{U}_i$ and $L_i$ is the dimension of the uncertain parameter $u^i \in \mathcal{U}_i$. We focus on the uncorrelated case, i.e., we assume that uncertainties of different functions $f_i$ are uncorrelated, i.e., the uncertainty set of $\sum_{i \in [m]} f_i(x, u^i)$ is $\mathcal{U} := \bigtimes_{i \in [m]} \mathcal{U}_i$. This ensures that the different uncertainty sets $\mathcal{U}_i$ have no influence on each other. Hence the robust counterpart of program~\eqref{Prob:GeneralNomOpt} without 'restricting' $\mathcal{U}$ further is
\begin{align}\label{Prob:GeneralStrictOpt}
\begin{split}
\inf_{x \in \mathcal{X}} & \sum_{i \in [m]} \ \sup_{u^i \in \mathcal{U}_i} f_i(x,u^i).
\end{split} 
\end{align} 
We say that, if $\mathcal{U}^i$ is convex and $f_i(x,\cdot): \mathcal{U}^i \to \R$ is concave for every $x \in \mathcal{X}$, then the uncertainty is concave. Furthermore, if there exists a function $l_i\colon \mathcal{X} \to \R^{L_i}$ with $f_i(x,u^i) = (u^i)^Tl_i(x)$ for every $x \in \mathcal{X}, u^i \in \mathcal{U}^i$, we call the uncertainty linear.
%An overview of methods for tackling
%problem~\eqref{Prob:GeneralStrictOpt} can be found e.g. in
%\cite{NonlinearRO}.  \todo[inline]{Hier nochmal erwähnen?}
%Future research could consider generalizations of problem~\eqref{Prob:GeneralStrictOpt}
%by taking correlated uncertainties into
%account %of each
%%function $f_i$
%%are correlated, i.e.,
%so that the objective under uncertainty reads $\max_{u \in
% \mathcal{U}} \sum_{i \in [m]} f_i(x,u^i)$.\\ %Here, we aim at
%generalizing the flexible $\Gamma$-approach for uncorrelated
%interval uncertainties and leave the correlated case
%subject to future research. \\
%In the linear case in Section 2, one attempted to be robust against
%$\Gamma$ changing coefficients.
\\
To reduce over--conservatism, we aim to be robust against at most $\Gamma$ functions deviating from their nominal scenario and obtain the following:
\begin{alignat}{2}\label{Prob:GeneralGammaCounterpart}
\inf_{x \in \mathcal{X}} & \left\{ \sup_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} \sup_{u^i \in \mathcal{U}_i} f_i(x,u^i) + \sum_{i \in [m] \setminus \mathcal{S}} f_i(x, \overline{u}^i) \right\} \right\}.
\end{alignat}
Program~\eqref{Prob:GeneralGammaCounterpart} is henceforth referred to as the $\Gamma$-counterpart of program~\eqref{Prob:GeneralNomOpt}. Naturally, it is more general than~\eqref{Prob:Gamma_Comb}. To demonstrate that this generalization is natural, we consider linear uncertainties: Assume that $f_i$ is subject to linear uncertainty for every $i \in [m]$ and that $\mathcal{U}^i$ is convex and compact. Then there exists $w^i \in \mathcal{U}^i$, such that $\sup_{u^i \in \mathcal{U}^i} f_i(x,u^i) = f_i(x,w^i) \in \R$. Then we obtain
\begin{alignat*}{2}
%\inf_{x \in \mathcal{X}} & \left\{ \sup_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} \sup_{u^i \in \mathcal{U}_i} f_i(x,u^i) + \sum_{i \in [m] \setminus \mathcal{S}} f_i(x,\overline{u}^i) \right\} \right\} \\
\eqref{Prob:GeneralGammaCounterpart}
&= \inf_{x \in \mathcal{X}}  \left\{ \sup_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} f_i(x,w^i) + \sum_{i \in [m] \setminus \mathcal{S}} f_i(x, \overline{u}^i) \right\} \right\} \\
&= \inf_{x \in \mathcal{X}}  \left\{ \sup_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} f_i(x,w^i) - f_i(x,\overline{u}^i) + \sum_{i \in [m]} f_i(x, \overline{u}^i) \right\} \right\} \\
&= \inf_{x \in \mathcal{X}}  \left\{ \sum_{i \in [m]} f_i(x, \overline{u}^i) + \sup_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} f_i(x,w^i - \overline{u}^i)\right\} \right\} \\
&= \inf_{x \in \mathcal{X}}  \left\{ \sum_{i \in [m]} f_i(x, \overline{u}^i) + \sup_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} \sup_{z^i \in \mathcal{U}_i - \overline{u}^i} f_i(x,z^i)\right\} \right\}.
\end{alignat*}
In particular, if $\mathcal{U}_i = [\overline{u}_i, \overline{u}_i + \Delta u_i] \subseteq \R_{\geq 0}$ and $f_i(x,u_i) = u_ix_i \geq 0$ for all $u_i \in \mathcal{U}_i$, then
\begin{gather*}
\sup_{z_i \in \mathcal{U}_i - \overline{u}_i} f_i(x,z_i) = \Delta u_i x_i
\end{gather*}
and one obtains program~\eqref{Prob:Gamma_Comb}. \\
Before we continue with our discussion for handling the $\Gamma$--counterpart in Section~\ref{sec:Non_Linear_Objective_Functions}, we present some application examples.
%\begin{example}\label{Rem:GeneralizeComb}
%For functions $f(x,c) = c^Tx$ with interval uncertainty for every coefficient $c_i$, problem~\eqref{Prob:GeneralGammaCounterpart} is equivalent to problem~\eqref{Prob:Gamma_Comb}:  By inserting $
%n = m, \ \mathcal{U}_i := [\overline{c}_i, \overline{c}_i + \Delta c_i] \ \forall i \in [n], \ f_i(x,c_i) := c_i \cdot x_i \ \forall i \in [n]$ into \eqref{Prob:GeneralGammaCounterpart},  
%we obtain 
%\begin{alignat*}{2}
%\min_{x \in \mathcal{X}} & \left\{ \max_{\mathcal{S} \subseteq [n]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} \max_{c_i \in [\overline{c}_i, \overline{c}_i + \Delta c_i]} c_ix_i + \sum_{i \in [n] \setminus \mathcal{S}} \overline{c}_ix_i \right\} \right\}.
%\end{alignat*}
%If $\mathcal{X} \subseteq \{0,1\}^n$, then
%$\max_{c_i \in [\overline{c}_i, \overline{c}_i + \Delta c_i]} c_ix_i = \overline{c}_i x_i + \Delta c_i x_i$  
%and formulation~\eqref{Prob:Gamma_Comb} is obtained.
%\end{example}

%\subsection{Applications}
%The next example demonstrates that the new counterpart can be applied in a broader context in comparison to the original counterpart of Bertsimas and Sim. It can deal with higher-dimensional uncertainty sets, e.g. ellipsoids or polyhedra, and is not restricted to one-dimensional intervals.
%
%\begin{example}\label{Ex:cx}
%\todo[inline]{Umschreiben zu einem BP, Spannbaum rausschmeißen. Vielleicht auch ein allgemeines BP und da zeigen, warum dies nicht so ist?} 
%We consider the calculation of a minimum spanning tree in a connected
%graph with four edges under uncertainty. Let the nominal problem be
%given by
%\begin{align}\label{Prob:Ex3.2.Nom}
%\begin{split}
%\min_x & \ \overline{c}_1 x_1 + \overline{c}_2 x_2 + \overline{c}_3 x_3 + \overline{c}_4 x_4, \\
%\mathrm{s.t.} & \ x \in \mathcal{X} := \{(1,1,1,0)^T, (1,1,0,1)^T, (1,0,1,1)^T, (0,1,1,1)^T\},
%\end{split}
%\end{align}
%with $\overline{c}_i := 1$ for $i \in [4]$. For $\varepsilon > 0$, the correlated
%uncertainty of $c_1$ and $c_2$ is given by $
%\mathcal{U}^{(1,2)}:= \begin{pmatrix} 1 - \varepsilon,  1-\varepsilon \end{pmatrix}^T + \{c \in \R^2: \ c_1^2 + c_2^2 \leq 1\},$
%the uncertainty of $c_3$ and $c_4$ is $\mathcal{U}^3 := \mathcal{U}^4:=[1,1.5]$.% \\
%%The next example covers a case for which the objective is linear but the uncertainty is not only contained in intervals. Consider Let $G = (V,E)$ be an undirected graph with $4$ nodes, i.e., $V = (1,2,3,4)$, and $E=(e, f, g, h)$ with 
%%\begin{gather*}
%%e := \{1,2\}, \ f := \{2,3\}, \ g:= \{3,4\} \text{ and } h:= \{4,1\}.
%%\end{gather*} 
%%We aim to obtain a minimal spanning tree of $G$. The nominal cost of the edges is given by $\overline{c}_e = 1- \varepsilon,  \overline{c}_h = 1$, $ \overline{c}_f = 1 - \varepsilon$, $\overline{c}_g = 1$ for a sufficiently small $\varepsilon > 0$ and the nominal problem is $\min_{x \in \mathcal{X}} \overline{c}^Tx$.
%%with $x$ denoting the incidence vectors of the resp. spanning tree and $\mathcal{X}:=\{(1,1,1,0)^T, (1,0,1,1)^T, (1,1,0,1)^T, (0,1,1,1)^T\}$ denoting the set of spanning trees of $G$. %It is easy to see that $x^*=(1,1,0,1)$ is the nominal optimum. \\
%%The coefficients are assumed to be subject to uncertainty: The costs of $e$ and $f$ are correlated within the ellipsoidal uncertainty set% While the costs for $g$ are $\mathcal{U}_g := [1,1.5]$, the costs for $e$ and $f$ are correlated:
%%\begin{gather*}
%%\mathcal{U}^{e,f}:= \begin{pmatrix} 1 - \varepsilon,  1-\varepsilon \end{pmatrix}^T + \{c \in \R^2: \ c_e^2 + c_f^2 \leq 1\}.
%%\end{gather*}
%%The costs of $g$ and $h$ are uncorrelated and within the interval uncertainty set $\mathcal{U}^{g} = \mathcal{U}^h:= [1,2]$.
%We set $f_{1,2}(x_1,x_2,c_1,c_2):= c_1x_1 + c_2x_2$ for $(c_1,c_2) \in \mathcal{U}^{(1,2)}$, $f_3(x_3,c_3) := c_3x_3$ and $f_4(x_4,c_4):=c_4x_4$ for $c_3 \in \mathcal{U}^3$ and $c_4 \in \mathcal{U}^4$. 
%The $\Gamma$-counterpart~\eqref{Prob:GeneralGammaCounterpart} is  given by
%\begin{gather}\label{Prob:GammaSpanningTree}
%\min_{x \in \mathcal{X}} \left\{ \max_{\mathcal{S} \subseteq \{(1,2), 3,4\}, |\mathcal{S}| \leq \Gamma} \left\{ \sum_{I \in \mathcal{S}} \max_{c_I \in \mathcal{U}^I} f_I(x_I,c_I)  + \sum_{I \in \{(1,2),3,4\} \setminus \mathcal{S}} f_I(x_I, \overline{c}_I)  \right\} \right\}.
%\end{gather}
%%Application of Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} results in $x^* = (1,1,0,1)$ being the robust optimal solution for $\Gamma = 1,2$ in the unique optimal solution $(e,g)$ for both $\Gamma = 1$ and $\Gamma = 2$. \\
%For $\Gamma = 1$, the objective values of the feasible solutions of ~\eqref{Prob:GammaSpanningTree} are displayed in Table~\ref{TableSpanningTree}. The optimal solutions are thus  $(1,1,1,0)$ and $(0,1,1,1)$.
%\begin{table}[H]
%\centering
%\caption{Objective values for the feasible solutions of problem~\eqref{Prob:GammaSpanningTree} for $\Gamma = 1.$\label{TableSpanningTree}}
%\begin{tabular}[c]{|l|l|}
%\hline
%Feasible solution & Objective Value \\ \hline
%$(1,1,1,0)^T$ & $3 - 2 \varepsilon + \sqrt{2}$\\ \hline
%$(1,1,0,1)^T$ & $3 - 2 \varepsilon + \sqrt{2}$\\ \hline
%$(1,0,1,1)^T$ & $4 - \varepsilon$ \\ \hline
%$(0,1,1,1)^T$ & $4 - \varepsilon$ \\ \hline
%\end{tabular}
%\end{table}
%Since the uncertainty set is not an interval uncertainty set, Proposition~\ref{Prop:Tractable_Gamma_Comb} cannot be applied directly. However, we obtain the setting of problem~\eqref{Prob:Gamma_Comb} by replacing $\mathcal{U}^{(1,2)}$ with the uncertainty intervals
%$\mathcal{U}^1 = \mathcal{U}^2 := [-\varepsilon,2 - \varepsilon]$ for
%$c_1$ and $c_2$, respectively. By doing this, we technically ignore the correlation of $c_1$ and
%$c_2$, since $\mathcal{U}^{(1,2)} \subseteq \mathcal{U}^1 \times \mathcal{U}^2$. Using the reformulation obtained by an application of Proposition 2.1 may
%thus lead to more conservative solutions. 
%Indeed, in this case, the optimal solution of
%problem~\eqref{Prob:Gamma_Comb} is $(1,1,1,0)$ and $(1,1,0,1)$ for all
%$\Gamma = 1,2,3,4$. However, these are exactly the solutions which are
%\emph{not} optimal for problem~\eqref{Prob:GammaSpanningTree} for
%$\Gamma = 1$. Consequently, in general, Proposition 2.1. is not applicable to general uncertainty sets by 'ignoring'
%correlations.%, i.e., additional constraints on the uncertainties.
%\end{example}
%While Example~\ref{Ex:cx} focused on $\min_{x \in \mathcal{X}} c^Tx$
%under non-interval uncertainty, the next example focuses on problems
%of the form $\min_{x \in \mathcal{X}} u^TBx$ for a real matrix $B \in \R^{m \times n}$ with $u$ being subject to interval uncertainty. %\in \R^{m}$.
\paragraph{Single--machine scheduling under uncertainty.}
This application was firstly discussed under uncertainty in \cite{RobustScheduling} and \cite{Tadayon2015}. A set of $m$ jobs $\mathcal{J}$ must be scheduled on a single machine. The machine requires a processing time $\overline{p}_j \in \R_{\geq 0}$ to finish job $j \in \mathcal{J}$ without preemption. The completion time of job $j$ that depends on the schedule $x$ and on the processing time $\overline{p}:=(\overline{p}_j)_{j \in \mathcal{J}}$ is denoted by $C_j(x,\overline{p})$. With $\mathcal{X}$, we denote the set of feasible schedules (the binary variable $x_{i,j}$ indicates whether job $j$ is scheduled at position $i$):
\begin{gather*}
\mathcal{X} := \left\{x \in \{0,1\}^{[m] \times |\mathcal{J}|}: \sum_{i \in [m]} x_{i,j} = 1 \ \forall j \in \mathcal{J}, \ \sum_{j \in \mathcal{J}} x_{i,j} = 1 \ \forall i \in [m] \right\}.
\end{gather*}
Assuming that every job $j$ contributes weight $w_j \in \R_{\geq 0}$
to the objective, we aim to minimize the total completion time:
\begin{gather}\label{Prob:WeightedScheduling}
\min_{x \in \mathcal{X}} \sum_{j \in \mathcal{J}} C_j(x,\overline{p}).
\end{gather} 
Program~\eqref{Prob:WeightedScheduling} is equivalent to
\begin{gather}\label{Prob:UnWeightedScheduling}
\min_{x \in \mathcal{X}} \sum_{j \in \mathcal{J}} \overline{p}_j \sum_{i \in [m]} (m+1-i)x_{i,j}.
\end{gather}
%where
%\begin{gather*}
%x_{i,j} = \begin{cases} 1, & \text{job $j$ is scheduled at position $i$},\\
%0, & \text{otherwise}. \end{cases}
%\end{gather*}
If the processing time $p_j$ is subject to
uncertainty $\mathcal{U}_j=[\overline{p}_j,
 \overline{p}_j + \Delta p_j]$ for each job $j \in \mathcal{J}$, then the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} of program~\eqref{Prob:UnWeightedScheduling} is
% \begin{alignat*}{2}
%\min_{x \in \mathcal{X}} & \left\{ \max_{\mathcal{S} \subseteq \mathcal{J}: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{j \in \mathcal{S}} \max_{p_j \in \mathcal{U}_j} p_j \sum_{i \in [m]} (m+1-j)x_{i,j} + \sum_{j \in \mathcal{J} \setminus \mathcal{S}} \overline{p}_j \sum_{i \in [m]} (m+1-j)x_{i,j} \right\} \right\},
%\end{alignat*}
%which is equivalent to  %due to $\max_{p_j \in \mathcal{U}_j} p_j \sum_{i \in [m]} (m+1-j)x_{i,j} = (\overline{p}_j + \Delta p_j)\sum_{i \in [m]} (m+1-j)x_{i,j}$,  
\begin{gather}\label{Prob:GammaScheduling}
\min_{x \in \mathcal{X}} \left\{ \sum_{j \in \mathcal{J}} \overline{p}_j \sum_{i \in [m]} (m+1-i)x_{i,j} + \max_{\mathcal{S} \subseteq \mathcal{J}: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{j \in \mathcal{S}} \Delta p_j \sum_{i \in [m]} (m+1-i)x_{i,j} \right\} \right\}
\end{gather}
since the uncertainty is linear. \\
%\end{example}
While program~\eqref{Prob:GammaScheduling} looks very similar to
\eqref{Prob:Gamma_Comb}, there is an important difference: The variables $x_{i,j}$ are not multiplied with exactly one coefficient but each uncertain parameter $p_j$ is multiplied with a linear combination of the variables $x_{i,j}$ for fixed $j \in \mathcal{J}$. Thus, the objective of the nominal program~\eqref{Prob:UnWeightedScheduling} is linear in $p$ and
in $x$ but has the form $\min_{x \in \mathcal{X}} u^TBx$ for a real
matrix $B$ instead of $\min_{x \in \mathcal{X}} u^Tx$. Thus, Proposition 2.1 and the original results of \cite{IntroGamma} cannot be applied.
%The next application we present is the quadratic assignment problem (QAP) which was first discussed under uncertainty in \cite{QAP2012} and \cite{QAP2015} \todo{regret robustness?}  
%\begin{example}\label{Ex:QAP}
\paragraph{Quadratic assignment problem under uncertainty.}
The QAP %, see for example \cite{QAP2015},
models the process of assigning $n \in \mathbb{N}$ facilities to $n$ locations such that the cost of transporting goods is minimized. %, resulting of the
%amount of material between facilities multiplied with the distance of
%the locations. 
  %The material handling costs between the facilities, given the flow i.e., the amount of goods transported between two facilities and the distance between two locations should be minimized.
%$c_{ij}$ is the flow between the facilities $i$ and $j$, $(i,j) \in [n]^2$ and $d_{rs}$ is the distance between the locations $r$ and $s$, $(r,s) \in [n]^2$.
%The task is to minimize the cost resulting of the transport of the goods:  TO DO!!!!!
%%which is defined as the product of the amount of material which is transported between two facilities and the distance between the corresponding locations.
%A facility is to assigned to exactly one location and each location is supposed to be used exactly once. 
With binary variables $x_{i,r}$, $i,r \in [n],$ that indicate whether facility $i$ is assigned to location $r$,
%\begin{align*}
%x_{i,r} = \begin{cases}
%1, & \text{if facility } i \text{ is located at }r, \\
%0, & \text{otherwise} \\
%\end{cases}, 
%\end{align*}
the feasible set can be modeled as 
\begin{gather*}
\mathcal{X} = \left\{x \in \{0,1\}^{[n]^2}: \sum_{i\in [n]} x_{i,r}= 1 \ \forall r \in [n], \sum_{r \in [n]} x_{i,r}=1 \ \forall i \in [n]\right\}.
\end{gather*}
For each pair of facilities $(i,j) \in [n]^2$, $c_{i,j} \geq 0$  denotes the flow between $i$ and $j$ and  for all pair of locations $(r,s) \in [n]^2$, $d_{r,s} \geq 0$ denotes the distance between $r$ and $s$. Thus, the QAP can be modeled with
\begin{gather*}
\min_{x\in \mathcal{X}} \sum_{(i,j,r,s) \in [n]^4} c_{i,j} d_{r,s}x_{i,r}x_{j,s}.
\end{gather*}  
In \cite{QAP2015}, the authors have assumed that the flow is subject to interval uncertainty. Their goal was to obtain solutions that are robust against at most $\Gamma$ deviations from the nominal scenario: We seek protection against uncertainties in $c_{i,j}$ that are modeled by a perturbation of at most $\Delta c_{i,j} \geq 0$ for all $(i,j)\in [n]^2$, i.e., $c_{i,j} \in \mathcal{U}_{i,j} = [\overline{c}_{i,j}, \overline{c}_{i,j}+ \Delta c_{i,j}]$. The $\Gamma$-counterpart~\eqref{Prob:GeneralGammaCounterpart} is, since the uncertainty is linear, given by:
\begin{align}\label{Prob:QAP_RobCP}
\begin{split}
&\min_{x\in \mathcal{X}} \left\{ \sum_{(i,j,r,s) \in [n]^4} \overline{c}_{i,j}d_{r,s}x_{i,r}x_{j,s} + \max_{\mathcal{S} \subseteq [n]^2:|\mathcal{S}|\le \Gamma} \left\{  \sum_{(i,j)\in \mathcal{S}}  \sum_{r,s\in [n]} \Delta \overline{c}_{i,j} d_{r,s}x_{i,r}x_{j,s} \right\} \right\} .
\end{split}
\end{align} 
%\end{example}
%The next application is a, to the best of our knowledge, new variant under uncertainty for piecewise linear functions.
%\begin{example}\label{Ex:VRP}
\paragraph{Logistics with deadline uncertainties.}
Problems occuring in the application of logistics involving deliveries within given due times can often be modeled as combinatorial programs with (non--)linear objective functions, e.g. taxi routing, delivery of goods or patient transport. For all three of these cases, being on time is important for customer satisfaction. At the same time, it is usually not problematic when vehicle arrives too early for a pick--up. \\
For tasks $i \in [m]$, we denote the due time with $b_i \in \R$.
If a job is finished after $b_i$, then penalty costs occur. A
program for (unweighted) penalty costs is 
\begin{align}\label{Prob:BoundNom}
\begin{split}
\inf_{x \in \mathcal{X}} & \ \sum_{i \in [m]} \max\{0,x_i - b_i\}.
\end{split}
\end{align} 
Program~\eqref{Prob:BoundNom} may arise in transportation logistics, for example as a special case of vehicle
routing problems with general time windows, see \cite{VRPSTW}. 
In practice, the due time can be uncertain: We assume that $b_i \in \mathcal{U}_i := [\overline{b}_i - \Delta b_i, \overline{b}_i]$ for some nominal scenario $\overline{b}_i$ and a perturbation $\Delta b_i$. 
To reduce conservatism, the objective is to ensure robustness against $\Gamma$ deviations of the due times, resulting in the following program:
\begin{align}\label{Prob:UncertainBounds}
\begin{split}
\inf_{x \in \mathcal{X}} & \ \left\{ \sup_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} \max\{0,x_i - \overline{b}_i + \Delta b_i\} + \sum_{i \in [m] \setminus \mathcal{S}} \max\{0, x_i - \overline{b}_i\} \right\} \right\}. 
\end{split}
\end{align}
Problem~\eqref{Prob:UncertainBounds} is obtained from $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} by setting $f_i(x,b) := \max\{0, x_i - b_i\}$.
%\end{example}


%\todo[inline][inline]{hier brauchen wir noch einen kommentar, was wir aus dem
%  QAP-Beispiel lernen, und wenn es zB lediglich ein Verweis darauf
%  ist, dass wir spaeter darauf zurueckkommen werden und zeigen, dass
%  die reformulierung vorteile hat, oder sowas in der art}
%%In a final example, we consider a feasibility problem under uncertainty which we can tackle with our approach: 
%%Example~\ref{Rem:GeneralizeComb} shows that the $\Gamma$-counterpart
%is a possibility for generalizing model~\eqref{Prob:Gamma_Comb} to
%mixed-integer nonlinear optimization problems. We furthermore would like to point out that Proposition~\ref{Prop:Tractable_Gamma_Comb} is only applicable in the case of interval uncertainty and, in particular, uncorrelated uncertainty - for more details, see Appendix A.
%\todo{Gute Überleitung?}
%Having introduced several different applications that motivate the robust counterpart defined here, in the next section we present computationally tractable reformulations of \eqref{Prob:GeneralGammaCounterpart}. 
%\begin{remark}
%Our given $\Gamma$-counterpart~\eqref{Prob:GeneralGammaCounterpart} is
%only one possible extension of the approach of
%\citep{IntroGamma}. Alternatively, it could be assumed that, for
%each function $f_i(x,u^i)$ with $u^i \in \R^{L_i}$, the objective could be robust against at most $\Gamma_i$ coefficients deviating from their nominal scenario. In formulas, this corresponds to 
%\begin{gather}\label{Prob:GeneralizationII}
%\min_{x \in \mathcal{X}} \sum_{i \in [m]} \max_{\mathcal{S} \subseteq [L_i], |\mathcal{S}| \leq \Gamma_i} \max_{u^i \in {\mathcal{U}^i_{\mathcal{S}}}} f_i(x,u^i),
%\end{gather}
%where 
%$\mathcal{U}_\mathcal{S}^{i}:= \{u^i \in \mathcal{U}^i: \ u_j^i = \overline{u}_j^i \ \forall j \notin \mathcal{S}\}.$
%However, this formulation is only technically a generalization of the $\Gamma$-counterpart introduced in \cite{IntroGamma}, since in
%this case, it would be possible to set $f_i(x,u) = u^Tx$, i.e., $m = 1$ and $L_1 = n$, with only one $\Gamma$ and obtain problem~\eqref{Prob:Gamma_Comb}. 
%%Furthermore, for separable functions
%%$f_i(x,u^i) = g_i(u^i)h_i(x)$ for some functions $g_i\colon
%%\mathcal{U}_i \to \R$ and $h_i \colon \mathcal{X} \to \R$, it is
%%straightforward to solve the maximization problems, since 
%%\begin{gather*}
%%\max_{S \subseteq [L_i], |S| \leq \Gamma_i} \max_{u^i \in \mathcal{U}_S^{i}} f_i(x,u^i) = \max_{S \subseteq [L_i], |S| \leq \Gamma_i} h_i(x) \max_{u^i \in \mathcal{U}_S^{i}} g_i(u^i).
%%\end{gather*}
%%where the inner maximization problem can be solved
%%analytically\todo[inline][inline]{wer sagt dass das analytisch geloest werden kann,
%%  stimmt das fuer alle fkt g?}.
%Thus, we opt for the
%$\Gamma$-counterpart~\eqref{Prob:GeneralGammaCounterpart}. %Different 
%%discussion about ~\eqref{Prob:GeneralizationII}
%%is possible subject to future research.%only be applicable, when the $f_i(x,u^i)$ are not separable in $x$ and $u^i$, i.e., there are no real-valued functions $g_i$ and $h_i$, such that $f_i(x,u^i) =g_i(u^i)^Th_i(x)$, because in this case, one could assume that..
%%While this approach would still a generalization of the linear case %of Problem~\eqref{Prob:Gamma_Comb} we want to note that $\Gamma_i \in \{0,1\}$  However, if one assumes $f_i(x,u_i) = u_i \cdot x_i$, uneeds to set $m = 1$ and $\Gamma_1 = \Gamma$). However, our $\Gamma$-counterpart seems to be more natural, especially in terms of combinatorial optimization. 
%\end{remark} 


==> Non_Linear_Objective_Functions_OR.tex <==
%!TEX root = main.tex

\section{Reformulations for programs with uncertain objectives} \label{sec:Non_Linear_Objective_Functions} 
In this section, we present equivalent reformulations for the
$\Gamma$--counterpart introduced in Section~\ref{Sec:General}. Several of the proofs are inspired by those in \cite{IntroGamma}. It turns out that it is possible to obtain first reformulations of $\Gamma$-- counterpart~\eqref{Prob:GeneralGammaCounterpart} without any assumptions on the functions $f_i$ or the uncertainty sets $\mathcal{U}^i$.  % It also turns out that the bottleneck in solving the $\Gamma$--counterpart is solving $\max_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x,\overline{u}^i)$ for each $i \in [m]$: 
\begin{lemma}\label{Lem:ReModel}
Let $\Gamma \in [m]$. Then $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
\begin{align}\label{Prob:GeneralReModel}
\begin{split}
\inf_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
\mathrm{s.t.\;} & x \in \mathcal{X}, \\
& p_i + \theta \geq \sup_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i) \ \forall i \in [m], \\
& p \in \R^m_{\geq 0}, \theta \in \R_{\geq 0}.
\end{split}
\end{align}
\end{lemma}
\proof{Proof.}
The structure of the proof is similar to the proof of Theorem 3 in \cite{IntroGamma}. With the binary variables
\begin{gather*}
s_i := \begin{cases} 1, \text{ if $i \in \mathcal{S}$,}\\ 
0, \text{ otherwise,} \\
\end{cases} 
\end{gather*}
$i \in [m]$, the inner maximization program of $\Gamma$--counterpart \eqref{Prob:GeneralGammaCounterpart} is equivalent to
\begin{align}\label{Prob:LinearOrdering}
\begin{split}
\sup_{s} & \ \sum_{i \in [m]} f_i(x, \overline{u}^i) + s_i(\sup_{u^i \in \mathcal{U}_i} f_i(x, u^i) - f_i(x, \overline{u}^i)), \\
\text{s.t.} & \ \sum_{i \in [m]} s_i \leq \Gamma, \\
& \ s \in \{0,1\}^m.
\end{split}
\end{align}
%This is a binary program with $\sum_{i \in [m]} f_i(x,
%\overline{u}^i)$ being independent of the decision variable $s$ and a
%knapsack constraint with equal, unit weights and integral
%capacity. Thus,
%we can recycle the proof of
%Proposition~\ref{Prop:Tractable_Gamma_Comb}:
Clearly, program~\eqref{Prob:LinearOrdering} is equivalent to its LP
relaxation. Inserting its dual into $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} proves the claim.
%Its dual is
%\begin{alignat*}{2}
%\min_{p, \theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x, \overline{u}^i) + \sum_{i \in [m]} p_i, \\
%\text{s.t.} & \ p_i + \theta \geq \max_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i) \ \forall i \in [m], \\
%& p, \theta \geq 0.
%\end{alignat*} 
\endproof
In Lemma~\ref{Lem:ReModel}, to obtain a tractable formulation, it is necessary to reformulate the inequality
%obtain a tractable formula for $\sup_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i),$ i.e. to solve a maximization problem over the uncertainty set. In the following subsection, we assume that the uncertainty is concave to apply results of \cite{Fenchel}. In \cite{Fenchel}, the authors proposed various ways of reformulating inequality
\begin{gather}\label{Ineq:RobustNonCon}
p_i + \theta \geq \sup_{u^i \in \mathcal{U}_i} f(x,u^i) - f(x, \overline{u}^i)
\end{gather}
for all $i \in [m]$. In \cite{Fenchel}, the authors proposed various approaches, especially for linear/concave uncertainties which will be discussed in the subsequent subsections. We demonstrate one approach for the non--concave case that uses the notion of term--wise parallel vectors for a non--convex quadratic program in Section~\ref{Sec:Reformulations}. For other approaches, we refer to \cite{Fenchel} and \cite{NonlinearRO}. \\

%even if $f$ is \emph{not} concave in the uncertainty (we note that, since we concentrate on single inequalities, we neglect the indices of the inequalities in model~\eqref{Prob:GeneralReModel} for better readibility). We briefly discuss two of their stated approaches (for more details, see \cite{Fenchel}): \\
%On the one hand, if $f(x,u) = h(u)^Tg(x)$ for all $u \in \mathcal{U}$ and $x \in \mathcal{X}$, one can attempt to compute the uncertainty set's convex hull and reformulate inequality 
%%Set $b := h(u)$ and $\overline{\mathcal{U}} :=\mathcal{U} \times h(\mathcal{U})$. Clearly, inequality~\eqref{Ineq:RobustNonCon} is equivalent to $
%\begin{gather*}
%p + \theta \geq \max_{(u,b) \in \mathrm{conv}(\mathcal{U} \times h(\mathcal{U}))} {b}^Tg(x) - f(x, \overline{u}).
%\end{gather*}
%which is 'easier' since the uncertainty is linear instead of non-concave. On the other hand, 
%%Since $b^Tg(x)$ is linear in $b$ -- and thus concave -- $\overline{\mathcal{U}}$ can be replaced with its convex hull and the
%%reformulations of Subsection~\ref{subsec:Concave} can be applied. However, finding the convex hull of a
%%given set is generally NP-hard. 
%% In this case $f(u)$ does not have to be concave and $g(x)$ may attain negative values.
%%Through parameterization $b=f(u)$ we obtain as robust counterpart
%%\[b^Tg(x)\le 0 \qquad \forall (u,b) \in \bar{U},\]
%%with $\bar{U}=\{(u,b)| b=f(u), u \in \mathcal{U}\}$.
%%Now the lefthand side is linear in the uncertainty, so we can replace the uncertainty set with its convex hull. 
%%If we can determine $conv(\bar{U})$ Fenchel duality can be applied. \\
%%The second approach was introduced in \cite{TermWise} and was discussed for robust optimization in \cite{Fenchel}:
%under the assumption that inequality~\eqref{Ineq:RobustNonCon} can be formulated as
%\begin{align}\label{Ineq:SecondApproach}
%u^Tg_1(x)+h(u)^Tg_2(x)\le p + \theta + f(x,u) \qquad \forall u: \ \alpha_k^Tu+\beta_k^Th(u) \le \gamma_k, k \in [K],
%\end{align}
%% Another approach assumes it is possible tor write the robust counterpart as \[u^Tg_1(x)+f(u)^Tg_2(x)\le 0 \qquad \forall u \alpha_k^Tu+\beta_k^Tf(a) \le \gamma_k, k \in [K].\]
%one can attempt to apply the notion of \emph{term-wise parallel vectors} \cite{TermWise}: After setting $b:=h(u)$, inequality~\eqref{Ineq:SecondApproach} is equivalent to 
%\begin{align}\label{Ineq:Parametrizing}
%u^Tg_1(x)+b^Tg_2(x)\le 0 \qquad \forall (u,b): \ \alpha_k^Tu+\beta_k^Tb \le \gamma_k, k \in [K], b=h(u).
%\end{align}
%While the left-hand side of the inequalities are clearly linear -- and thus, concave -- in $u$, the lifted uncertainty set $
%\mathcal{V} := \{(u,b): \alpha_k^Tu+\beta_k^Tb \le \gamma_k, k \in [K], \ b = h(u)\}
%$
%is generally not convex and thus, the theory of Subsection~\ref{subsec:Concave} cannot be applied for reformulating \eqref{Ineq:Parametrizing}. However, if $\mathcal{V}$ is replaced with  
%$
%\mathcal{V}^{\mathrm{rel}} := \{(u,b): \alpha_k^Tu+\beta_k^Tb \le \gamma_k, k \in [K], \ b \leq h(u)\}
%$
%in \eqref{Ineq:Parametrizing}, one can apply said theory since $\mathcal{V}^{\mathrm{rel}}$ is convex. If $\alpha_k$ and $\beta_k$ are term-wise parallel and $\max_{(u,b) \in \mathcal{V}^{\mathrm{rel}}} u^Tg_1(x)+b^Tg_2(x)$ exists and is finite for every $x \in \mathcal{X}$,
%\eqref{Ineq:Parametrizing} and
%\begin{gather}\label{Ineq:Relax}
%u^Tg_1(x)+b^Tg_2(x)\le p + \theta + f(x,u) \qquad \forall (u,b) \in \mathcal{V}^{\mathrm{rel}}
%\end{gather} 
%are equivalent. 
%%However, this changes when $\alpha_k$ and $\beta_k$ are \emph{term-wise parallel} \cite{TermWise, Fenchel}:
%%\begin{definition}
%%Consider a family of $K$ inequalities, given by
%%\begin{gather*}
%%\alpha_k^T u + \beta_k^T b \leq \gamma_k \ \forall k \in [K],
%%\end{gather*}
%%where $\alpha_k, \beta_k \in \R^L, \gamma_k \in \R$ for all $k \in [K]$. The vectors $\alpha_k,\ \beta_k$ are called \emph{term-wise parallel} if 
%%\begin{gather*}
%%\mathrm{rank}\{(\alpha_{kl},\beta_{kl}), \ k \in [K]\} \leq 1 \ \forall l \in [L].
%%\end{gather*}
%%\end{definition}
%%With this notion, inequalities~\eqref{Ineq:Parametrizing} and \eqref{Ineq:Relax} are equivalent if $\alpha_k$ and $\beta_k$ are term-wise parallel and if $\max_{(u,b) \in \mathcal{V}^{\mathrm{rel}}} u^Tg_1(x)+b^Tg_2(x)$ exists and is finite for every $x \in \mathcal{X}$.
%Then $x$ satisfies inequality~\eqref{Ineq:RobustNonCon} if and only if for all $k \in [K]$ there exist vectors $v^k \in \R^n$, such that
%% If $b \ge f(\bar{u})$ it has been proven that there is another optimal solution for $u$ that satisfies $b=f(u)$. Because of that both robust counterparts are equivalent and we can use Fenchel duality for the latter. The final counterpart is then:
%\begin{align*}
%&\sum_{l\in[L]} \left(g_{2l}(x)+\sum_{k\in[K]} \beta_{kl}v_k\right)h^*\left(-\frac{g_{1l}(x)+\sum_{k\in[K]}\alpha_{ki}v_k}{g_{2l}(x)+\sum_{k\in[K]} \beta_{kl}v_k}\right)+\sum_{k\in[K]} \gamma_kv_k \le p + \theta + f(x,\overline{u}),\\
%&g_{2l}(x)+\sum_{k\in[K]} \beta_{kl}v_k \ge 0 \ \forall l \in [L],\\
%&v\ge 0,
%\end{align*}
%see \cite{Fenchel}, Subsection 4.3. We demonstrate an application in Section~\ref{Sec:Reformulations}. Otherwise, one can still attempt to obtain reformulations, although it is less straightforward. We show a 1--dimensional example where this is possible in Section~\ref{Sec:Reformulations}. 
Furthermore, one can reformulate program~\eqref{Prob:GeneralReModel} to obtain a program with feasible set $\mathcal{X}$ and without variables $p$ and $\theta$:
\begin{lemma}\label{Rem:NoFenchel}
If $\Gamma \in [m]$, then $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%Theorem~\ref{Theo:GeneralGammaCounterPartWithoutDual} also holds in a more general version: By Lemma~\ref{Lem:ReModel},
%the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to model~\eqref{Prob:GeneralReModel} and by applying the proof of Theorem~\ref{Theo:GeneralGammaCounterPartWithoutDual} to model~\eqref{Prob:GeneralReModel} we obtain
\begin{align}\label{Prob:GammaCombCounterpartWithoutFenchel}
\begin{split}
\inf_{k \in [m]_0} & \left\{ \inf_{x \in \mathcal{X}} \left\{ \Gamma \theta^k(x) + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \sup\{0, \theta^i(x) - \theta^k(x) \} \right\} \right\}, \\
\end{split}
\end{align}
where $\theta^k(x) := \sup_{u^k \in \mathcal{U}_k} f_k(x,u^k) - f_k(x,\overline{u}^k)$ and $\theta^0(x) := 0$. 
%Note that % The only difference between problems~\eqref{Prob:GammaCombCounterpartWithoutFenchel} and \eqref{Prob:GeneralGammaCounterpartWithoutDual} is that one can not apply Fenchel's Inequality. However, due to definition, $\theta^k(x) \geq 0$. In other words: 
%the only difference between \eqref{Prob:GeneralGammaCounterpartWithoutDual} and \eqref{Prob:GammaCombCounterpartWithoutFenchel} is that in the general case, Proposition~\ref{Prop:GeneralPrinciple} could not be applied (which results in the lack of variables $v^i$) and $\max_{u^k \in \mathcal{U}_k} f_k(x,u^k) - f_k(x, \overline{u}^k)$ still needs to be solved. We include an example of this case in Subsection~\ref{Subsec:Non-Concave}.
\end{lemma}
\proof{Proof.}
Since $\Gamma \in [m]$, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to \eqref{Prob:GeneralReModel}. Since for all $i \in [m]$, $p_i$ only occurs in exactly one inequality, we obtain
\begin{gather}\label{Eq:optimal_p}
p^*_i = \sup \{0, \sup_{u^i \in \mathcal{U}_i} f_i(x^*,u^i) - f_i(x^*, \overline{u}^i) )- \theta^* \} \ \forall i \in [m]
\end{gather}
for an optimal solution $(x^*,p^*,\theta^*)$ of~\eqref{Prob:GeneralReModel}. Inserting equation~\eqref{Eq:optimal_p} into the objective function of \eqref{Prob:GeneralReModel} results in 
\begin{align}\label{Eq:piecewiselinearlem}
 \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \sup \{0, \sup_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i) ) - \theta \}.
\end{align}
Since $\eqref{Eq:piecewiselinearlem}$ is convex and piecewise linear in $\theta$, either $\theta^*=0$ or %Next, we prove that either $\theta^* = 0$ or there exists $k \in [m]$ such that
%\begin{gather}\label{Eq:OptimalTheta}
$\theta^* = \theta^k(x)$ %\max_{u^k \in \mathcal{U}_k} f_k(x^*,u^k) - f_k(x^*,\overline{u}^k)$
%\end{gather}
for one $k \in [m]$.  %Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, the minimum is furthermore obtained either at $0$ or 
%Assume that $(x,v^1, \dots, v^m, \theta)$ is feasible and that $\theta$ is equal to 0 nor does it fulfill equation~\eqref{Eq:OptimalTheta} for any $k \in [m]$. Thus, the sets
%\begin{align*}
%S^{<}&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k)  < \theta\} \text{ and } \\
%S^>&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) > \theta\}
%\end{align*}
%are a partition of $[m]$, i.e., $S^< \cup S^> = [m]$ and $S^< \cap S^> = \emptyset$. The objective can be rewritten as:
%\begin{alignat*}{2}
%&\Gamma\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} \left( -f_k(x,v^k) + \support{k} - \theta \right) \\
%&= (\Gamma - |S^>|)\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} -f_k(x,v^k) + \support{k}. 
%\end{alignat*}
%We consider different cases for $S^>$:
%\begin{itemize}
%\item[\underline{First case:}] $S^> = \emptyset$. \\
%In this case, $S^< = [m]$. The solution $(x,v^1, \dots, v^m, \overline{\theta})$ with
%\begin{gather*}
%\overline{\theta} := \max_{k \in [m]} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) 
%\end{gather*}
%has a better objective value than $(x,v^1, \dots, v^m, \theta)$, since $\overline{\theta} < \theta$.
%\item[\underline{Second case:}] $S^> = [m]$.\\
%In this case, 
%\begin{gather*}
%0 \leq \theta < f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) \ \forall k \in [m].
%\end{gather*}
%We set $
%\overline{\theta} := \min_{k \in [m]} (\overline{u}^k)^Tv^k + \delta^*({A^k}^Tv^k \mid \mathcal{Z}_k) - f_k(x,\overline{u}^k) - f_k(x,v^k) $
%
%and since $\Gamma \in [m]$, the objective value of $(x,v^1, \dots, v^m, \overline{\theta})$ is at most the objective value of $(x,v^1, \dots, v^m, \theta)$. 
%\item[\underline{Third case:}] $S^> \neq \emptyset, [m]$. \\
%In this case, there exist $k,l \in [m]$, such that \begin{align*}
%&f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k} < \theta \\
%&< f_l(x,\overline{u}^l) - f_l(x,\overline{u}^l) - f_l(x,v^l) + \support{l}.
%\end{align*}
%In particular, it can be assumed without loss of generality that 
%\begin{gather*}
%k= \mathrm{argmax}_{i \in S^<} \theta - f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i}, \\
%l= \mathrm{argmin}_{i \in S^>} f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i} - \theta.
%\end{gather*} 
%We set 
%\begin{gather*}
%\overline{\theta}:= \begin{cases} f_l(x,\overline{u}^l) + \support{l} - f_l(x,\overline{u}^l) - f_l(x,v^l), & \text{if $|S^>| > \Gamma$,} \\
%\max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}, & \text{otherwise.}
%\end{cases}
%\end{gather*} 
%%and otherwise, set
%%\begin{gather*}
%%\overline{\theta}:= \max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}.
%%\end{gather*}
%In both cases, we obtain a feasible solution with a better objective.
%\end{itemize} 
%We define
%\begin{gather*}
%\theta^k(x,v^k) := f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k - f_k(x,\overline{u}^k) - f_l(x,v^k) + \support{k}
%\end{gather*}
%for $k \in [m]$ and $\theta^0 := 0$. 
%Thus, the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%\begin{alignat*}{2}
%\min_{k \in \{0, \dots, m\}} & \min_{x \in \mathcal{X}} \Gamma \theta^k(x) + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, \theta^i(x)- \theta^k(x) \}. 
%%\text{s.t.} & x \in \mathcal{X}. \\
%\end{alignat*}
%Finally, by application of Fenchel's inequality (cf. \cite{ConvexAnalysis}, Chapter 12) and Assumption~\ref{Ass:General}, (iii) $\theta^k(x,v^k) \geq 0$ is redundant since 
%%$\theta^0(x,v^0) = 0$ by definition and for $k \in [m]$, 
%\begin{gather*}
%\support{k} \geq 0 \Leftrightarrow \exists \zeta \in \mathcal{Z}_k: \ \zeta^T({A^k})^Tv^k \geq 0.
%\end{gather*}
\endproof
%As an application, we demonstrate the formulation of Lemma~\ref{Rem:NoFenchel} for Example~\ref{Ex:VRP}. 
\subsection{Concave Uncertainties} \label{subsec:Concave}
%Until now, we have made no assumptions about $f_i$ or
%$\mathcal{U}_i$. 
In this subsection, we will focus on programs that fulfill the following assumptions:
\begin{assumption}\label{Ass:General}
For $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} and for all $i \in [m]$ we assume:
\begin{itemize}
\item[(i)] There is a nominal scenario $\overline{u}^i \in \R^{L_i}$, a matrix $A^i \in \R^{L_i \times m_i}$ and a convex set $\mathcal{Z}_i \subseteq \R^{m_i}$, such that $
\mathcal{U}_i = \{\overline{u}^i + A^i \zeta^i\mid \ \zeta^i \in
\mathcal{Z}_i\}$, i.e., $\mathcal{U}_i$ is an affine transformation of a convex set (and thus, convex).
\item[(ii)] The uncertainty of $f_i$ is concave (we recall that this definition implies that $f_i(x,\cdot): \mathcal{U}^i \to \R$ is concave for every $x \in \mathcal{X}$).
\item[(iii)] The nominal scenario $\overline{u}^i$ is contained in the relative interior of $\mathcal{U}_i$.
\end{itemize}
\end{assumption}
%Since convex sets stay convex under affine-linear transformations,
%(i) implies that $\mathcal{U}^i$ is convex.
Convexity of the uncertainty set (i) is a typical assumption in robust optimization, see \cite{RobustBook}. 
%Furthermore, we note that $0 \in \mathcal{Z}_i$ implies $\overline{u}^i \in \mathcal{U}^i$ which is, again, a straight-forward assumption. 
%We note that, iwf $f_i(x,u^i)$ is \emph{convex} in $x$, (i) can be assumed without loss of generality; for more details, see 
%\todo[inline][inline]{Dennis: Ben-Tal nachlesen}
Assumptions (ii) and (iii) are required to apply the techniques from \cite{Fenchel}. To this end, we need some tools of convex analysis:
\begin{definition}
Let $\mathcal{X} \subseteq \R^n$ and $\mathcal{A} \subseteq \R^m$ be a convex set. Let $f \colon \mathcal{X} \times \mathcal{A} \to \R, \ (x,a) \mapsto f(x,a)$ be a function that is concave in $a$ for every $x \in \mathcal{X}$. For an arbitrary, but fixed $x \in \mathcal{X}$, the function
\begin{alignat*}{4}
f_{*}(x, \cdot) \colon & \R^n & \to & \ \R \cup \{-\infty\}, \\
& a & \mapsto & \inf_{y \in \mathcal{A}} \{a^Ty - f(x,y)\}
\end{alignat*}
is called the (partial) concave conjugate with respect to $a$. For a non--empty set $\mathcal{S} \subseteq \R^n$, the function
\begin{alignat*}{4}
\delta^*(\cdot \mid \mathcal{S})  \colon & \R^n & \to & \ \R \cup \{\infty\}, \\
& x & \mapsto & \sup_{y \in \mathcal{S}} y^Tx
\end{alignat*}
is called the support function of $\mathcal{S}$.
\end{definition}
%\begin{remark}
%With our notation, we aim to stay close to the notation of \cite{Fenchel}. For example, $\delta^*(\cdot \mid \mathcal{S})$ is the \emph{convex conjugate} of the indicator function. Since we do not require the exact definition of convex conjugates or indicator functions, we neglect them in this paper. For more details, see \cite{Fenchel} or \cite{ConvexAnalysis}.
%\end{remark}
%\todo[inline][inline]{Dennis: Proper definitions...}
The main result of \cite{Fenchel} is the following reformulation:
\begin{prop}(\cite{Fenchel}, Theorem 2)\label{Prop:GeneralPrinciple}
Under Assumption~\ref{Ass:General}, inequality
\begin{gather*}
\sup_{u^i \in \mathcal{U}_i} f_i(x,u^i) \leq 0
\end{gather*}
is satisfied if and only if there is a vector $v^i \in \R^{L_i}$, such that
\begin{gather}\label{Ineq:GeneralPrinciple}
\left(\overline{u}^i\right)^T v^i + \delta^*((A^i)^Tv^i \mid \mathcal{Z}_i) - f_{i,*}(x,v^i) \leq 0.
\end{gather}
\end{prop}
%\proof{Proof.}
%See Theorem 2 in \cite{Fenchel}.
%\endproof
%Proposition~\ref{Prop:GeneralPrinciple} implies that we can verify
%whether a given $x$ satisfies a given inequality under uncertainty by
%solving a deterministic inequality without uncertainty. Furthermore,
We note that convexity of $f_i$ in $x$ implies that the left-hand side of inequality~\eqref{Ineq:GeneralPrinciple} is also convex, since $\delta^*$ is convex in $v^i$ and $f_{i,*}$ is concave in $(x,v^i)$, see \cite{Fenchel}.\\ By applying Proposition~\ref{Prop:GeneralPrinciple} to
program~\eqref{Prob:GeneralReModel}, we obtain an equivalent reformulation of $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart}: %which is deterministic: 
\begin{corollary}\label{Prop:FenchelGammaCounterpart}
Let $\Gamma \in [m]$. Under Assumption~\ref{Ass:General}, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to %Problem~\eqref{Prob:GeneralReModel} 
\begin{align}\label{Prob:FenchelGammaCounterpart}
\begin{split}
\inf_{x,p,\theta,v^1, \dots, v^m} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i \\
\mathrm{s.t.}\; & x \in \mathcal{X} \\
& p_i + \theta \geq (\overline{u}^i)^Tv^i + \support{i} - f_{i,*}(x,v^i) - f_i(x, \overline{u}^i) \ \forall i \in [m] \\
& p, \theta \geq 0.
\end{split}
\end{align}
%%Furthermore, if $f_i$ is linear in the uncertainty for some $i \in [m]$, i.e., $f_i(x,u^i)={(u^i)}^Tl_i(x)$ for a function $l_i \colon \R^n \to \R^{L_i}$, the inequality constraints of problem~\eqref{Prob:FenchelGammaCounterpart} are equivalent to 
%%\begin{align}\label{Prob:FenchelGammaCounterpartLinear}
%%\begin{split}
%%%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%%%\text{s.t.} & x \in \mathcal{X}, \\
%% p_i + \theta \geq  \supportx{i}\\
%%%& p, \theta \geq 0.
%%\end{split}
%%\end{align}
%%for each $i \in [m]$.
\end{corollary}
\proof{Proof.}
Since $\Gamma$ is integral, Lemma~\ref{Lem:ReModel} holds. Proposition~\ref{Prop:GeneralPrinciple} implies that for each $i
\in [m]$, 
\begin{gather*}
p_i + \theta \geq ({\overline{u}^i})^Tv^i + \support{i} - f_{i,*}(x,v^i) - f_i(x, \overline{u}^i)
\end{gather*}
is satisfied for $v \in \R^{L_i}$ if and only if 
%\begin{gather*}
$p_i + \theta \geq \sup_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i).$
%\end{gather*}
%which proves the first part of the claim. In the case where $f_i$ is linear in $u^i$, we have
%\begin{gather*}
%f_{i,*}(x,v^i) \neq -\infty \Leftrightarrow v^i = l_i(x),
%\end{gather*} 
%which implies $f_{i,*}(x,l_i(x)) = 0$ \cite{Fenchel}. Since inequality~\eqref{Ineq:GeneralPrinciple} is not fulfilled for $f_{i,*}(x,v^i) = - \infty$, $v^i = l_i(x)$ holds. Inserting this into the inequality constraints of problem~\eqref{Prob:FenchelGammaCounterpart} results in the claim, since $f_i(x, \overline{u}^i) = (\overline{u}^i)^Tl_i(x)$.
%\begin{align*}
%%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%%\text{s.t.} & x \in \mathcal{X}, \\
%p_i + \theta \geq (\overline{u}^i)^Tl_i(x) + \supportx{i} - f_i(x,\overline{u}^i) \ \forall i \in [m]. 
%%& p, \theta \geq 0.
%\end{align*} 
%Since $f_i(x, \overline{u}^i) = (\overline{u}^i)^Tl_i(x)$, the claim follows.
\endproof
%\todo{Remark einfädeln als Korollar.}
%\todo{Bemerkung machen, wie sich viele konkave Settings zu linear umformulieren lassen.}
In general, program~\eqref{Prob:FenchelGammaCounterpart} is not compuationally tractable. The support function and the concave conjugate with respect to $v^i$ are optimization programs themselves that depend on a new decision variable $v^i$. In \cite{Fenchel}, the authors derived finite reformulations for various uncertainty sets $\mathcal{U}_i$, including geometries like ellipsoids, polyhedra, cones, boxes, Minkowski sums or their intersections and uncertainty sets that are described by various functions, e.g. convex functions or separable functions and. Their findings can also be applied here. For details, we refer to Tables 1, 2 and 3 in \cite{Fenchel}. 
%In this section, we extend
%Propositions~\ref{Prop:Tractable_Gamma_Comb} and \ref{Prop:Gamma_MIP}
%to more general classes of optimization problems which are subject to
%uncertainty in the objective. For the case of uncertainty in the constraints, we refer to Appendix B. \\
%We first consider 
%\emph{nominal} optimization problems that are of the form
%\begin{align}\label{Prob:GeneralNomOpt}
%\begin{split}
%\min_x & \sum_{i \in [m]} \ \overline{f}_i(x),\\
%\text{s.t.} & \ x \in \mathcal{X}
%\end{split} 
%\end{align}
%where $\overline{f}_i \colon \R^n \to \R$ is an arbitrary, but fixed function for every $i \in [m]$. %In the following, we call problem~\eqref{Prob:GeneralNomOpt} the \emph{nominal problem}. \\
%We assume that every function $\overline{f}_i$ is subject to an
%uncertainty set $\mathcal{U}_i$, i.e., we set %extend $\overline{f}_i$ to 
%\begin{gather*}
%f_i \colon \R^n \times \mathcal{U}_i \to \R
%\end{gather*} 
%with $f_i(x,\overline{u}^i):= \overline{f}_i(x)$ for a nominal
%scenario $\overline{u}^i \in \mathcal{U}_i$. Like in Section 2, we focus on the
%uncorrelated case by assuming that uncertainties of different functions $f_i$ are uncorrelated, i.e., the uncertainty set of $f(x,u) := \sum_{i \in [m]} f_i(x, u^i)$ is $\mathcal{U} := \bigtimes_{i \in [m]} \mathcal{U}_i$.
%Hence the robust counterpart of problem~\eqref{Prob:GeneralNomOpt} reads
%\begin{align}\label{Prob:GeneralStrictOpt}
%\begin{split}
%\min_x & \sum_{i \in [m]} \ \max_{u^i \in \mathcal{U}_i} f_i(x,u^i),\\
%\text{s.t.} & \ x \in \mathcal{X}.
%\end{split} 
%\end{align} 
%An overview over methods for tackling
%problem~\eqref{Prob:GeneralStrictOpt} can be found e.g. in
%\cite{NonlinearRO}. 
%%Future research could consider generalizations of problem~\eqref{Prob:GeneralStrictOpt}
%%by taking correlated uncertainties into
%%account %of each
%%%function $f_i$
%%%are correlated, i.e.,
%%so that the objective under uncertainty reads $\max_{u \in
%% \mathcal{U}} \sum_{i \in [m]} f_i(x,u^i)$.\\ %Here, we aim at
%%generalizing the flexible $\Gamma$-approach for uncorrelated
%%interval uncertainties and leave the correlated case
%%subject to future research. \\
%%In the linear case in Section 2, one attempted to be robust against
%%$\Gamma$ changing coefficients.
%Generalizing the setting from the previous section, we aim to be protected against at most $\Gamma$ functions deviating from their nominal scenario:
%\begin{alignat}{2}\label{Prob:GeneralGammaCounterpart}
%\min_{x \in \mathcal{X}} & \left\{ \max_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} \max_{u^i \in \mathcal{U}_i} f_i(x,u^i) + \sum_{i \in [m] \setminus \mathcal{S}} f_i(x, \overline{u}^i) \right\} \right\}.
%\end{alignat}
%This problem is henceforth called \emph{$\Gamma$--counterpart}. To demonstrate that this generalization is natural, we start by showing that it
%generalizes the linear version \eqref{Prob:Gamma_Comb}.
%% state some applications for which this $\Gamma$--counterpart is a
%%natural robustification, and briefly discuss another possible
%%generalization. 
%\begin{example}\label{Rem:GeneralizeComb}
%For functions $f(x,c) = c^Tx$ with interval uncertainty for every coefficient $c_i$,
%problem~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
%problem~\eqref{Prob:Gamma_Comb}: inserting $ %\begin{gather*}
%n = m, \ \mathcal{U}_i := [\overline{c}_i, \overline{c}_i + \Delta c_i] \ \forall i \in [n], \ f_i(x,c_i) := c_i \cdot x_i \ \forall i \in [n]$ into \eqref{Prob:GeneralGammaCounterpart}, %\end{gather*} 
%one obtains 
%\begin{alignat*}{2}
%\min_{x \in \mathcal{X}} & \left\{ \max_{\mathcal{S} \subseteq [n]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} \max_{c_i \in [\overline{c}_i, \overline{c}_i + \Delta c_i]} c_ix_i + \sum_{i \in [n] \setminus \mathcal{S}} \overline{c}_ix_i \right\} \right\}.
%\end{alignat*}
%If $\mathcal{X} \subseteq \{0,1\}^n$, then
%$\max_{c_i \in [\overline{c}_i, \overline{c}_i + \Delta c_i]} c_ix_i = \overline{c}_i x_i + \Delta c_i x_i
%$  
%and one obtains formulation~\eqref{Prob:Gamma_Comb}.
%\end{example}
%\begin{example}
%The next example covers a case for which the objective is linear but the uncertainty is not only contained in intervals. Let $G = (V,E)$ be an undirected graph with $4$ nodes, i.e., $V = (1,2,3,4)$, and $E=(e, f, g, h)$ with 
%\begin{gather*}
%e := \{1,2\}, \ f := \{2,3\}, \ g:= \{3,4\} \text{ and } h:= \{4,1\}.
%\end{gather*} 
%We aim to obtain a minimal spanning tree of $G$. The nominal cost of the edges is given by $\overline{c}_e = 1- \varepsilon,  \overline{c}_h = 1$, $ \overline{c}_f = 1 - \varepsilon$, $\overline{c}_g = 1$ for a sufficiently small $\varepsilon > 0$ and the nominal problem is $\min_{x \in \mathcal{X}} \overline{c}^Tx$.
%with $x$ denoting the incidence vectors of the resp. spanning tree and $\mathcal{X}:=\{(1,1,1,0)^T, (1,0,1,1)^T, (1,1,0,1)^T, (0,1,1,1)^T\}$ denoting the set of spanning trees of $G$. %It is easy to see that $x^*=(1,1,0,1)$ is the nominal optimum. \\
%The coefficients are assumed to be subject to uncertainty: The costs of $e$ and $f$ are correlated within the ellipsoidal uncertainty set% While the costs for $g$ are $\mathcal{U}_g := [1,1.5]$, the costs for $e$ and $f$ are correlated:
%\begin{gather*}
%\mathcal{U}^{e,f}:= \begin{pmatrix} 1 - \varepsilon,  1-\varepsilon \end{pmatrix}^T + \{c \in \R^2: \ c_e^2 + c_f^2 \leq 1\}.
%\end{gather*}
%The costs of $g$ and $h$ are uncorrelated and within the interval uncertainty set $\mathcal{U}^{g} = \mathcal{U}^h:= [1,2]$.
%The $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is  given by
%\begin{gather}\label{Prob:GammaSpanningTree}
%\min_{x \in \mathcal{X}} \left\{ \max_{\mathcal{S} \subseteq \{\{e,f\}, g,h\}, |\mathcal{S}| \leq \Gamma} \left\{ \sum_{I \in \mathcal{S}} \max_{(c_{I_1}, c_{I_2}) \in \mathcal{U}^I} c_{I_1}x_{I_1} + c_{I_2}x_{I_2} + \sum_{I \in \{\{e,f\}, g,h\} \setminus \mathcal{S}} {\overline{c}_{I_1}}x_{I_1} + {\overline{c}_{I_2}}x_{I_2} \right\} \right\}.
%\end{gather}
%Application of Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} results in $x^* = (1,1,0,1)$ being the robust optimal solution for $\Gamma = 1,2$ in the unique optimal solution $(e,g)$ for both $\Gamma = 1$ and $\Gamma = 2$. \\
%For $\Gamma = 1$, the objective values of the incidence vectors are given in Table~\ref{TableSpanningTree}. The optimal solutions are thus given by $(1,1,1,0)$ and $(0,1,1,1)$.
%\begin{table}[H]
%\centering
%\caption{Objective values for the feasible solutions problem~\eqref{Prob:GammaSpanningTree} for $\Gamma = 1.$\label{TableSpanningTree}}
%\begin{tabular}[c]{|l|l|}
%\hline
%Incidence vector & Objective Value \\ \hline
%$(1,1,1,0)$ & $4 - \varepsilon$\\ \hline
%$(1,1,0,1)$ & $3 - 2 \varepsilon + \sqrt{2}$\\ \hline
%$(1,0,1,1)$ & $3 - 2 \varepsilon + \sqrt{2}$ \\ \hline
%$(0,1,1,1)$ & $4 - \varepsilon$ \\ \hline
%\end{tabular}
%\end{table}
%robust optimal solutions would be
%$(1,0,1,1)$ and $(0,1,1,1)$ with optimal value $4 - \varepsilon$. However, $(1,1,0,1)$ or $(1,1,1,0)$ would be strictly worse, because
%\begin{gather*}
%\max_{(c_e,c_f) \in \mathcal{U}^{e,f}} c_e + c_f = \sqrt{2}.
%\end{gather*}
%and thus, the objective value is $3 - 2 \varepsilon + \sqrt{2} > 4 - \varepsilon$ for $\varepsilon \in (\sqrt{2} - 1, 1)$. 
%Since the uncertainty set is not a pure interval uncertainty set, one can not apply Proposition~\ref{Prop:Tractable_Gamma_Comb}.  However, if we replace $\mathcal{U}^{e,f}$ with the uncertainty sets $\mathcal{U}^e = \mathcal{U}^f := [1-\varepsilon,2 - \varepsilon]$ for $c_e$ and $c_f$, one obtains that for each $\Gamma = 1,2,3,4$, the optimal solution of problem~\eqref{Prob:Gamma_Comb} would be $(1,1,1,0)$ and $(1,1,0,1)$. However, these are exactly the solutions which are \emph{not} optimal for problem~\eqref{Prob:GammaSpanningTree} for $\Gamma = 1$. Consequently, in general, ignoring correlations can lead to too conservative solutions.
%\todo[inline]{Die genauen Berechnungen könnte man in den Appendix stecken oder dem Lesen überlassen. Ich finde nicht, dass das hier einen Mehrwert darstellt. Man könnte hier noch graphisch den Baum und die Unsicherheitsmengen darstellen zum besseren verständnis.}
%\end{example}
%\begin{example}\label{Ex:Scheduling}
%We consider a single-machine scheduling problem: A set of $m$ jobs
%$\mathcal{J}$ has to be scheduled on a single machine. The machine
%requires a \emph{processing time} $\overline{p}_j \in \R_{\geq 0}$ for finishing job $j \in \mathcal{J}$ without preemption. With $C_j(x,\overline{p})$ we denote the completion time of job $j$ which depends on the actual schedule $x$ and on the processing time $\overline{p}:=(\overline{p}_j)_{j \in \mathcal{J}}$. With $\mathcal{X}$, we the
%set of feasible schedules:
%\begin{gather*}
%\mathcal{X} := \{x \in \{0,1\}^{[m] \times \mathcal{J}}: \sum_{i \in [m]} x_{i,j} = 1 \ \forall j \in \mathcal{J}, \ \sum_{j \in \mathcal{J}} x_{i,j} = 1 \ \forall i \in [m] \}.
%\end{gather*}
%Assuming that every job $j$ is weighted with a weight $w_j \in \R_{\geq 0}$, we aim to minimize the weighted total completion time:
%\begin{gather}\label{Prob:WeightedScheduling}
%\min_{x \in \mathcal{X}} \sum_{j \in \mathcal{J}} w_j C_j(x,\overline{p}).
%\end{gather} 
%If $w_j = 1 \ \forall j \in \mathcal{J}$, 
%problem~\eqref{Prob:WeightedScheduling} is equivalent to
%\begin{gather}\label{Prob:UnWeightedScheduling}
%\min_{x \in \mathcal{X}} \sum_{j \in \mathcal{J}} \overline{p}_j \sum_{i \in [m]} (m+1-i)x_{i,j},
%\end{gather}
%where
%\begin{gather*}
%x_{i,j} = \begin{cases} 1, & \text{job $j$ is scheduled at position $i$},\\
%0, & \text{otherwise}. \end{cases}
%\end{gather*}
%Now, we assume for each job $j$ that the processing time $p_j$ is subject to
%uncorrelated uncertainty $\mathcal{U}_j=[\overline{p}_j,
% \overline{p}_j + \Delta p_j]$. Although the objective of
%\eqref{Prob:UnWeightedScheduling} is linear in $p$ and in $x$, one
%cannot simply apply Proposition~\ref{Prop:Tractable_Gamma_Comb}: While the uncertainties are not correlated for the different jobs $j \in \mathcal{J}$, they are correlated for the schedules: If $\overline{p}_j$ is subject to uncertainty, the variables $x_{i,j}$ are influenced for all $i \in [m]$, while in the setting of
%Proposition~\ref{Prop:Tractable_Gamma_Comb}, an uncertainty influences exactly one variable. Applying Proposition~\ref{Prop:Tractable_Gamma_Comb} that assumes uncorrelated
%uncertainties, could therefore result in an overly conservative reformulation. 
%\\
%The $\Gamma$--counterpart introduced in this section can be applied,
%and reads 
%\begin{gather*}
%\min_{x \in \mathcal{X}} \sum_{j \in \mathcal{J}} \overline{p}_j \sum_{i \in [m]} (m+1-i)x_{i,j} + \max_{\mathcal{S} \subseteq \mathcal{J}: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{j \in \mathcal{S}} \Delta p_j \sum_{i \in [m]} (m+1-i)x_{i,j} \right\}.
%\end{gather*}
%\end{example}
%
%\begin{example}\label{Ex:VRP}
%Logistics problems involving deliveries within given time windows can be modeled as combinatorial optimization problems with non-linear objective functions. As an example, consider taxi routing, delivery of goods or patient transports. These three cases have in common that on the one
%hand, being on time is important for the satisfaction of the customers.
%On the other hand, it usually is not problematic if a
%vehicle arrives too early for a pick-up. \\
%Therefore, by ignoring earliest arrival times, a job $i$ shall be
%finished until a point in time $b_i \in \R$.
%If it is finished after $b_i$, penalty costs occur. A
%model for (unweighted) penalty cost that are linear in the distance
%from $b_i$ is given by
%\begin{align}\label{Prob:BoundNom}
%\begin{split}
%\min_{x \in \mathcal{X}} & \ \sum_{i \in [m]} \max\{0,x_i - b_i\}.
%\end{split}
%\end{align} 
%We note that such tasks may arise in transportation logistics, for
%example as a special case of Vehicle
%Routing Problems with Soft Time Windows, see \cite{VRPSTW}. They
%also occur in energy contexts, see e.g. Chapter 4 in
%\cite{Probust}. \\
%We now assume that the time windows are uncertain. %, i.e., $b$ is
%subject to uncertainty.
%Assuming that $b_i \in \mathcal{U}_i := [\overline{b}_i - \Delta b_i, \overline{b}_i + \Delta b_i]$ for some nominal scenario $\overline{b}_i$ and a perturbation $\Delta b_i$, the $\Gamma$--counterpart is given by
%\begin{align}\label{Prob:UncertainBounds}
%\begin{split}
%\min_{x \in \mathcal{X}} & \ \max_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \sum_{i \in \mathcal{S}} \max\{0,x_i - \overline{b}_i + \Delta b_i\} + \sum_{i \in [m] \setminus \mathcal{S}} \max\{0, x_i - \overline{b}_i\}. 
%\end{split}
%\end{align}
%\end{example}
%\begin{example}\label{Ex:QAP}
%The Quadratic Assignment Problem as considered in \cite{QAP2015}
%models the process of assigning $n \in \mathbb{N}$ facilities to $n$
%locations. For each pair of facilities $i$
%and $j$, $(i,j) \in [n]^2$, the amount $c_{ij}$ of exchanged goods
%between $i$ and $j$ is given. Furthermore, the distance $d_{rs}$ between
%two locations $r, s \in [n]$, is given as well. %The material handling costs between the facilities, given the flow i.e., the amount of goods transported between two facilities and the distance between two locations should be minimized.
%$c_{ij}$ is the flow between the facilities $i$ and $j$, $(i,j) \in [n]^2$ and $d_{rs}$ is the distance between the locations $r$ and $s$, $(r,s) \in [n]^2$.
%
%The task is to minimize the cost for transportation which is defined as the product of the amount of material which is transported between two facilities and the distance between the corresponding locations.
%We introduce binary variables $x_{ir}$ to indicate whether facility $i$ is positioned at location $r$:
%\begin{align*}
%x_{ir} = \left\{
%\begin{array}{ll}
%1, & \text{if facility } i \text{ is located at }r, \\
%0, & \, \text{otherwise.} \\
%\end{array}
%\right.
%\end{align*}
%To ensure that each facility is assigned to exactly one location and that for every location, exactly one facility is assigned, we define the feasible region $\mathcal{X}$ as:
% \[\mathcal{X} = \left\{x \in \{0,1\}^{[n]^2}: \sum_{i\in [n]} x_{ir}= 1 \quad \forall r \in [n], \sum_{r \in [n]} x_{ir}=1 \quad \forall i \in [n]\right\}.\]
%We seek protection against uncertainties in $c_{ij}$ for all $(i,j)\in [n]^2$ that is modeled by a perturbation of at most $\Delta c_{ij}$, e.g. $c_{ij} \in \mathcal{U}_{ij} = [\bar{c}_{ij}, \bar{c}_{ij}+ \Delta c_{ij}]$.
%With the uncertainty set $\mathcal{U} := \bigtimes_{(i,j)\in [n]^2} \mathcal{U}_{ij}$ the %resulting optimization problem can be modeled as
%\begin{align*}
%\min_{x\in \mathcal{X}} \max_{c \in \mathcal{U}}  \sum_{i=1}^n \sum_{j=1}^n \sum_{r=1}^n \sum_{s=1}^n c_{ij} d_{rs}x_{ir}x_{js}.
%\end{align*}
%Using the flexible $\Gamma$-approach as in the setting of Problem~\eqref{Prob:GeneralGammaCounterpart} the $\Gamma$--counterpart is given by:
%\begin{align}\label{Prob:QAP_RobCP}
%\begin{split}
%&\min_{x\in \mathcal{X}} \sum_{(i,j,r,s) \in [n]^4} \bar{c}_{ij}d_{rs}x_{ir}x_{js} + \max_{\mathcal{S} \subseteq [n]^2:|\mathcal{S}|\le \Gamma}  \sum_{(i,j)\in \mathcal{S}}  \sum_{(r,s)\in [n]^2} \Delta \bar{c}_{ij} d_{rs}x_{ir}x_{js} .
%\end{split}
%\end{align}
%We note, that since the objective is quadratic the reformulations from \cite{IntroGamma} can not be used.
%\end{example}
%
%\begin{example}\label{SFB}
%Assume that for a set of $m$ objects $O_1, \dots, O_m$, e.g., particles, each shall be characterized by an $n$-dimensional data set comprised of attributes $A_1,A_2,\dots,A_n, n \geq 2$, that are measured in
%practical experiments. 
%\begin{table}[H]
%    \centering
%    \begin{tabular}{l|c|c}
%         & Object $O_1$ & Object $O_2$  \\
%     $A_1$   &  & \\
%     $A_2$ (weight)     & & 
%    \end{tabular}
%    \caption{Values of attributes of objects}
%    \label{tab:my_label}
%\end{table}
%%Attributes may for example be weights or different diameters \todo[inline][inline]{Durchmesser von...?}. 
%\todo[inline][inline]{...Goal: TABELLE FÜLLEN!!! Problemaufzählung: Warum geht das nicht so einfach? Simultane Messung und nur k Attribute und Messungenauigkeiten. Was ist das nominalle Problem? [HYPERGRAPHEN] (Formulierung der Tabellenfüllung). Was ist das robuste Problem, also wo kommt die Unsicherheit mit rein?} 
%However, often one cannot measure all
%attributes simultaneously, but only a limited number $k < n$ of these. \todo[inline][inline]{Beispiel: Referenz?}
%The goal is the reconstruction of the values of $A_1, A_2, \dots, A_n$ for each object from these $k$-dimensional measurements. We assume that we conduct $N \in \mathbb{Z}_{\geq 0}$ measurements. %Through one measurement the values of $k$ attributes are determined. \todo[inline]{immer die gleichen?}
%The result of measurement $j \in [N]$ are $m$ $k$-tuples of values, one for each object $o$, denoted as $a^o_j \in \R^k$. We note that this is a slight abuse of notation, we note that due to the simultaneous measurement, we do not know which tuple $a^o_j$ belongs to which of the objects $O_1, \dots, O_m$. %w%hile $a^i_j$ has $m$ entries, after a measurement we do not know which value for attribute $i$ belongs to which object. But for one measurement $j \in [N]$  %$A_i$ For measurement $M_i$, the  We order the measurements so that $A_i, \ldots, A_{i+k}$ are determined at measurement $M_i$ for $i \in [n]$. \todo[inline]{Was ist denn Attribut $A_{n+k}$? Sollte man hier nicht vielleicht besser mit Subindizes arbeiten, also $A_{i_k}$?}
%%For each attribute $A_i$ we denote the vector that contains all
%%values of $A_i$ as $a^i$. 
%%\todo[inline]{koennen wir hier nicht
%%  noch in k Messungen arbeiten? Es muss auch noch erklaert werden dass wir hier der Einfachheit halber annehmen dass keine Messung doppelt vorkommt, oder? Warum werden hier die Hypergraphen genannt? Spielen spaeter keine Rolle mehr... ich faende es gut wenn es hier im Text noch in k-Tupeln erklaert waere, und bei den Formeln reduziert man es auf k=2. welches Optiierungsproblem steckt dahinter wenn man k Messungen hat, ist es ein Hypergraph Matching in einem Graphen der jeweils Hyperkanten aus k Knoten hat? das sollte auch so erklaert werden, finde ich. es sollte dann auch am Ende dazugesagt werden was bei k > 2 das Optimierungsproblem ist. Ich hatte schon gemutmasst dass
%%es sich um ein polynomiales Optimierungsproblem mit Monomen der Laenge k handelt - ist das korrekt? sollte auch mit gesagt werden, am schluss koenntest du wieder allgemeiner werden und sagen (im Text) dass im Allgemeinen bei k > 2 ein XYZ Optimierungsproblem entsteht.}
%If two measurements $j_1, j_2 \in [N]$ determine the same attribute $A_i$, $i  \in [n]$ and if two tuples $a^{(o_1,j_1)}$ and $a^{(o_2,j_2)}$ share the value of an attribute $A_i$, the tuples belong to the same particle. Thus, the values of the shared attribute are the same. Therefore, we aim to combine these tuples. % that contain the same or an equal value for the common attribute. 
%%Note that we need to conduct at least $N \geq \frac{n-1}{k-1}$ to ensure that there exists a relation through these tuples between all measurement. 
%%However, if a measurement determines attributes that in no other measurement are determined no relation can be found.% Therefore we need at least $\frac{n-1}{k-1}$ measurements to find a tuple of all $n$ attributes. 
%% For a better understanding, we want to model the problem as a matching on a
%%hypergraph. Each node of the graph represents a tuple of values that are determined in a measurement. An edge between those nodes only exists if both tuples 
%%belong to the same object. We aim to find edges that connect $\frac{n-1}{k-1}$
%%nodes. Two connected nodes cannot be output
%%of the same measurement.
%%If $n=2$ and $k=1$ the resulting optimization problem is an assignment problem. \todo[inline][inline]{Referenz auf die assignment Struktur des Schedulings und des Assignment Problems?}
%%For $n>2$ a multidimensional assignment problem has to be
%%solved. 
%\todo[inline][inline]{WAS IST DAS OPTIMIERUNGSPROBLEM??? NOMINELL????}
%For avoiding issues regarding notation, we formulate the resulting optimization problem for $m=5$ objects with $n=4$ attributes for which we conduct $N = 3$ measurements which measure $k = 2$ attributes. 
%From each measurement we obtain a binary vector, indicating if two values belong to the same particle. \todo[inline][inline]{aber gehören nicht Attribute zu einem Partikel....?} %Those vectors are given through the measurements and are no decision variables.  \todo[inline][inline]{Der Satz kann weg. Man muss den Text glaub ich nur verständlicher aufschreiben. Du schreibst an vielen Stellen etwas von Knoten/Kanten/Tupeln/Vektoren ohne die Strukturen notatiostechnisch wirklich zu benutzen. Das sollten wir mal diskutieren.}
%%\begin{align*}
%%&\nu^1_{ij} = \left\{
%%\begin{array}{ll}
%%1, & \text{if in }M_1\text{ a pair } \ a^1_{i} \in a^1 \text{ and }a^{2}_{j} \in a^{2}, (o_1,o_2)\in [m]^2 \text{ was determined}, \\
%%0, & \, \text{otherwise} \\
%%\end{array}
%%\right.
%%\end{align*} \todo[inline][inline]{Hier stimmt was nicht: oben sind die $a^i$ noch Vektoren und hier haben die Vektoren auf einmal elemente?}
%%\begin{align*}
%%&\nu^2_{jk} = \left\{
%%\begin{array}{ll}
%%1, & \text{if in }M_2\text{ a pair } \ a^2_{j} \in a^2 \text{ and }a^{3}_{k} \in a^{3}, (j,k)\in [m]^2 \text{ was determined}, \\
%%0, & \, \text{otherwise} \\
%%\end{array}
%%\right.
%%\end{align*}
%%\begin{align*}
%%nu^3_{kr} = \left\{
%%\begin{array}{ll}
%%1, & \text{if in }M_3\text{ a pair } \ a^3_{k} \in a^k \text{ and }a^{4}_{r} \in a^{4}, (k,r)\in [m]^2 \text{ was determined}, \\
%%0, & \, \text{otherwise} \\
%%\end{array}
%%\right.
%%\end{align*}
%%\todo[inline][inline]{Ich finde es unschön, wenn $k=4$ und dann $k$ auf einmal ein Laufindex ist...}
%%The aim is to find tuples of values $(a_i^1, a_j^2, a_k^3, a_r^4)$ that belong to one object. 
%Our decision variables are binary variables indicating which
%values belong to the same particle: 
%\todo[inline][inline]{$x_{(o_j, l_i),....} \in j \in [m] \times [N]$}
%\begin{align*}
%&x_{(o_1,j_1), \dots, (o_n,j_n)} = \left\{
%\begin{array}{ll}
%1, & \text{if there is an object with } (a^1_{i}, a^2_{j},a^3_k, a^4_{r}),(i,j,k,r)\in[m]^4 \\
%0, & \, \text{otherwise}. \\
%\end{array}
%\right.
%\end{align*}
%\todo[inline][inline]{Dann kann man die Variable schon direkt bei der Def. der Tupel definieren? Wenn dann schon klar ist, was wir eigentlich optimieren wollen...}
%%For ease of exposition, we assume that if for two particles the same value of an attribute is measured this value is listed two times in the vector. So no tuple has to be assigned to two particles.
% We thus determine $x \in
%\mathcal{X}$ with 
%\begin{align*}
%\mathcal{X}=\left\{x \in \{0,1\}^{4m}: \right. & \left. \sum_{(j,k,r) \in [m]^3} x_{ijkr} =1 \quad \forall i \in [m],
% \sum_{(i,k,r) \in [m]^3} x_{ijkr} =1 \quad \forall j \in [m],\right.\\
%&\left. \sum_{(i,j,r) \in [m]^3} x_{ijkr} =1 \quad \forall k \in [m], \sum_{(i,j,k) \in [m]^3} x_{ijkr} =1 \quad \forall r \in [m] \right\}.
%\end{align*} 
%\todo[inline][inline]{ab hier stiege ich leider komplett aus....}
%If we want to assign the values $(a_i^1, a_j^2, a_k^3, a_r^4)$ to one particles we have to make sure the pair $(a^1_i,a^2_j)$ was determined in $M_1$, $(a^2_j,a^3_k)$ was determined in $M_2$ and $(a^3_k,a^4_r)$ was determined in $M_3$.
%The deviation of $a_j^2$ and its measured values in $M_1$ and $M_2$ for one tuple $(a_i^1, a_j^2, a_k^3, a_r^4)$ can be determined through the binary vectors $y^1$ and $y^2$ as:
%\[ \left|a^{2}_{j}-\sum_{l \in [m]}a^{2}_{l}y^1_{il}\right|+\left|a^{2}_{j}-\sum_{l \in [m]}a^{2}_{l}y^{2}_{lk}\right|.\]
%Note that $\sum_{l \in [m]}y^{s}_{lk} = 1 \ \forall s \in [1,2,3], k \in [m]$.
%Since we have to consider this difference also for $a^3_k$ we define
%the sum of the differences of $a^2_j$ and $a^3_k$:
%\[c_{ijkr} = \left|a^{2}_{j}-\sum_{l \in [m]}a^{2}_{l}y^1_{il}\right|+\left|a^{2}_{j}-\sum_{l \in [m]}a^{2}_{l}y^{2}_{lk}\right|+ \left|a^{3}_{k}-\sum_{l \in [m]}a^{3}_{l}y^3_{jl}\right|+\left|a^{3}_{k}-\sum_{l \in [m]}a^{3}_{l}y^{4}_{lr}\right|. \]
%This difference should be minimized.
%We also assume that there might be inaccuracies in the measurement. So
%it is possible that the measured values of the attributes might
%vary. Therefore $c_{ijkr}$ is uncertain with $c_{ijkr} \in \mathcal{U}_{ijkr} = [\bar{c}_{ijkr}, \bar{c}_{ijkr} + \Delta c_{ijkr}]$. The resulting robust counterpart can be written as:
%% \todo[inline]{von was?hier steht ja noch gar nichts von robustheit...} problem is a multidimensional assignment problem: 
%\begin{align*}
%\min_{x\in \mathcal{X}} \sum_{(i,j,k,r) \in [m]^4} x_{ijkr} +
%\max_{\mathcal{S}\subseteq [m]^4: |\mathcal{S}|\le \Gamma} \left\{\sum_{(i,j,k,r) \in \mathcal{S}} \max_{c_{ijkr} \in\mathcal{U}_{ijkr}} c_{ijkr} + \sum_{(i,j,k,r) \in [m]^4 \setminus \mathcal{S}} \bar{c}_{ijkr} \right\}.
%\end{align*}
%\todo[inline][inline]{Das Optimierungsproblem, kann das so stimmen? 1. Ist das innerste Maximum klar und du hast das glaube ich bei der leztten Summe schon verwendet. Zweitens, wenn sich die Koeffizienten deterministich aus den $a_{blubb}$ zusammensetzen, 3. Warum minimieren wir über die $x$? Deine zulässige Menge heißt doch: Für jede Messung muss es ein Objekt geben, was diese Attrbute hat, oder nicht? 4. Das x und das c haben keinen Zusammenhang, man könnte das große Maximierungsproblem direkt rausziehen! Also müssten doch die $a_i$ unsicher sicher sein? Da ist irgendwo ein Wurm drin. Oder das Problem ist doch ne Spur zu konstruiert....}
%With that we can find correlations for different attributes, even if
%the measurements might be inaccurate.
%\end{example}
%
%%%Example~\ref{Rem:GeneralizeComb} shows that the $\Gamma$--counterpart
%%is a possibility for generalizing model~\eqref{Prob:Gamma_Comb} to
%%mixed-integer nonlinear optimization problems. We furthermore would like to point out that Proposition~\ref{Prop:Tractable_Gamma_Comb} is only applicable in the case of interval uncertainty and, in particular, uncorrelated uncertainty - for more details, see Appendix A.
%\begin{remark}
%Our application of the flexible $\Gamma$-approach is only one possible
%extension of the approach of \citep{IntroGamma}. One could also assume
%that, for each function $f_i(x,u^i)$ with $u^i \in \R^{L_i}$, we would
%like to be robust against at most $\Gamma_i$ many uncertain
%coefficients. In formulas, this corresponds to 
%\begin{gather}\label{Prob:GeneralizationII}
%\min_{x \in \mathcal{X}} \sum_{i \in [m]} \max_{\mathcal{S} \subseteq [L_i], |\mathcal{S}| \leq \Gamma_i} \max_{u^i \in \mathcal{U}_{\mathcal{S}^{i}}} f_i(x,u^i)
%\end{gather}
%where 
%\begin{gather*}
%\mathcal{U}_S^{i}:= \{u^i \in \mathcal{U}^i: \ u_j^i = \overline{u}_j^i \ \forall j \notin S\}.
%\end{gather*}
%This approach would only technically be a generalization of the
%$\Gamma$--counterpart introduced in \cite{IntroGamma} as well, since in
%this case, one could set for the special case $f_i(x,u) = u^Tx$, i.e., $m = 1$ and $L_1 = n$ with only one $\Gamma$. 
%%Furthermore, for separable functions
%%$f_i(x,u^i) = g_i(u^i)h_i(x)$ for some functions $g_i\colon
%%\mathcal{U}_i \to \R$ and $h_i \colon \mathcal{X} \to \R$, it is
%%straightforward to solve the maximization problems, since 
%%\begin{gather*}
%%\max_{S \subseteq [L_i], |S| \leq \Gamma_i} \max_{u^i \in \mathcal{U}_S^{i}} f_i(x,u^i) = \max_{S \subseteq [L_i], |S| \leq \Gamma_i} h_i(x) \max_{u^i \in \mathcal{U}_S^{i}} g_i(u^i).
%%\end{gather*}
%%where the inner maximization problem can be solved
%%analytically\todo[inline]{wer sagt dass das analytisch geloest werden kann,
%%  stimmt das fuer alle fkt g?}.
%Thus, we stay with the
%$\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart}, and a
%discussion about models generalized from~\eqref{Prob:GeneralizationII}
%is possible subject to future research.%only be applicable, when the $f_i(x,u^i)$ are not separable in $x$ and $u^i$, i.e., there are no real-valued functions $g_i$ and $h_i$, such that $f_i(x,u^i) =g_i(u^i)^Th_i(x)$, because in this case, one could assume that..
%%While this approach would still a generalization of the linear case %of Problem~\eqref{Prob:Gamma_Comb} we want to note that $\Gamma_i \in \{0,1\}$  However, if one assumes $f_i(x,u_i) = u_i \cdot x_i$, uneeds to set $m = 1$ and $\Gamma_1 = \Gamma$). However, our $\Gamma$--counterpart seems to be more natural, especially in terms of combinatorial optimization. 
%\end{remark} 
%After having introduced several different applications that motivate the robust counterpart defined here, we next present algorithmically
%tractable reformulations. It turns out that a bottleneck of
%solving~\eqref{Prob:GeneralGammaCounterpart} consists in solving
%\begin{gather*}
%\max_{u^i \in \mathcal{U}_i} f_i(x,u^i)
%\end{gather*} 
%for each $i \in [m]$.
%\begin{lemma}\label{Lem:ReModel}
%If $\Gamma$ is integral, the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%\begin{align}\label{Prob:GeneralReModel}
%\begin{split}
%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%\text{s.t.} & x \in \mathcal{X}, \\
%& p_i + \theta \geq \max_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i) \ \forall i \in [m], \\
%& p \in \R^m_+, \theta \in \R_+.
%\end{split}
%\end{align}
%\end{lemma}
%\proof{Proof.}
%With the binary variables
%\begin{gather*}
%s_i := \begin{cases} 1, \text{ if $i \in \mathcal{S}$,}\\ 
%0, \text{ otherwise,} \\
%\end{cases} 
%\end{gather*}
%for $i \in [m]$, the inner maximization problem of \eqref{Prob:GeneralGammaCounterpart} is equivalent to
%\begin{align}\label{Prob:LinearOrdering}
%\begin{split}
%\max_{s} & \ \sum_{i \in [m]} f_i(x, \overline{u}^i) + s_i(\max_{u^i \in \mathcal{U}_i} f_i(x, u^i) - f_i(x, \overline{u}^i)), \\
%\text{s.t.} & \ \sum_{i = 1}^m s_i \leq \Gamma, \\
%& s \in \{0,1\}^m.
%\end{split}
%\end{align}
%%This is a binary program with $\sum_{i \in [m]} f_i(x,
%%\overline{u}^i)$ being independent of the decision variable $s$ and a
%%knapsack constraint with equal, unit weights and integral
%%capacity. Thus,
%%we can recycle the proof of
%%Proposition~\ref{Prop:Tractable_Gamma_Comb}:
%Clearly, problem~\eqref{Prob:LinearOrdering} is equivalent to its LP
%relaxation. Its dual is
%\begin{alignat*}{2}
%\min_{p, \theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x, \overline{u}^i) + \sum_{i=1}^m p_i \\
%\text{s.t.} & p_i + \theta \geq \max_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i) \ \forall i \in [m] \\
%& p, \theta \geq 0.
%\end{alignat*} 
%Inserting this equivalent reformulation into problem~\eqref{Prob:GeneralGammaCounterpart} proves the claim.
%\endproof
%\todo[inline]{Reformulierung über die optimalen Werte, aber vielleicht nicht die gleichen optimalen Lösungen?} 

%We note that for the rest of this section, we assume that all minima or maxima are well-defined, which is the case in combinatorial settings since the feasible sets are usually compact or finite.

%\subsection{Reformulations of robust counterparts with assumptions}

\subsection{Linear Uncertainties} \label{subsec:Linear}
%Until now, we have made no assumptions about $f_i$ or
%$\mathcal{U}_i$. 
During the last decades, research has been focused on linear uncertainties and they are well--studied. Thus, in this subsection, we will show how one can deal with linear uncertainties in the context of MINLPs under uncertainty, noting that many combinatorial programs are dealing with linear uncertainty (as we will also demonstrate in Section~\ref{Sec:Reformulations}):
\begin{assumption}\label{Ass:GeneralLinear}
For $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} and for all $i \in [m]$, Assumption~\ref{Ass:General} holds with the following modification:
\begin{itemize}
%\item[(i)] There is a nominal scenario $\overline{u}^i \in \R^{L_i}$, a matrix $A^i \in \R^{L_i \times m_i}$ and a convex set $\mathcal{Z}_i \subseteq \R^{m_i}$, such that $
%\mathcal{U}_i = \{\overline{u}^i + A^i \zeta^i\mid \ \zeta^i \in
%\mathcal{Z}_i\}$, i.e., $\mathcal{U}_i$ is an affine transformation of a convex set (and thus, convex).
\item[$\text{(ii)}^*$] The uncertainty is linear, i.e., there exists a function $l_i \colon \mathcal{X} \to \R^{L_i}$ such that 
\begin{gather*}
f_i(x,u^i) = (u^i)^Tl_i(x)\  \forall u^i \in \mathcal{U}_i, \ x \in \mathcal{X}.
\end{gather*}
%\item[(iii)] The nominal scenario $\overline{u}^i$ is contained in the relative interior of $\mathcal{U}_i$.
\end{itemize}
\end{assumption}
%Since convex sets stay convex under affine-linear transformations,
%(i) implies that $\mathcal{U}^i$ is convex.
We start by formulating Corollary~\ref{Prop:FenchelGammaCounterpart} under Assumption~\ref{Ass:GeneralLinear}:
\begin{corollary}\label{Prop:FenchelGammaCounterpartLinear}
Let $\Gamma \in [m]$. Under Assumption~\ref{Ass:GeneralLinear}, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to %Problem~\eqref{Prob:GeneralReModel} 
\begin{align}\label{Prob:FenchelGammaCounterpartLin}
\begin{split}
\inf_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} (\overline{u}^i)^Tl_i(x) + p_i, \\
\mathrm{s.t.}\; & x \in \mathcal{X}, \\
& p_i + \theta \geq  \supportx{i} \ \forall i \in [m], \\
& p, \theta \geq 0.
\end{split}
\end{align}
\end{corollary}
\proof{Proof.}
Since $\Gamma$ is integral, Corollary~\ref{Prop:FenchelGammaCounterpart} holds. Since the uncertainty is linear, we have
\begin{gather*}
f_{i,*}(x,v^i) \neq -\infty \Leftrightarrow v^i = l_i(x),
\end{gather*} 
see \cite{Fenchel}. Since inequality~\eqref{Ineq:GeneralPrinciple} is naturally not fulfilled for $f_{i,*}(x,v^i) = - \infty$, $v^i = l_i(x)$ holds. Inserting this into program~\eqref{Prob:FenchelGammaCounterpart} proves the claim, since $f_i(x, \overline{u}^i) = (\overline{u}^i)^Tl_i(x)$.
%\begin{align*}
%%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%%\text{s.t.} & x \in \mathcal{X}, \\
%p_i + \theta \geq (\overline{u}^i)^Tl_i(x) + \supportx{i} - f_i(x,\overline{u}^i) \ \forall i \in [m]. 
%%& p, \theta \geq 0.
%\end{align*} 
%Since $f_i(x, \overline{u}^i) = (\overline{u}^i)^Tl_i(x)$, the claim follows.
\endproof
 
\begin{remark}
We note that naturally, similar to $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} being a generalization of program~\eqref{Prob:Gamma_Comb}, Corollary~\ref{Prop:FenchelGammaCounterpartLinear} is a generalization of Theorem~1 in \cite{IntroGamma}.
\end{remark}



%\begin{example} %For illustrative purposes, we study the case $\mathcal{Z}_i := \{\zeta^i \mid || \zeta_i ||_p \leq \rho\},$ where $f_i$ is linear in the uncertainty.
% We also show that the second part of Theorem~\ref{Theo:FenchelGammaCounterpart} is a generalization of Proposition~\ref{Prop:Gamma_MIP}. 
%In \cite{Fenchel}, several examples for the support function and the concave conjugate have been determined and given explicitly which is, of course, possible here as well. We will come back to that later in this section. In a first step, we show what happens when $f_i(x,\overline{u}^i)$ is not only concave but linear in $\overline{u}^i$:
%\begin{theorem}\label{Theo:GeneralLinearUncertainty}
%Let $\Gamma$ be integral and assume that Assumptions (i), (ii) and (iii) hold. Assume that for all $i \in [m]$, there is a function $l_i(x)\colon \R^n \to \R^n $, such that $f_i(x,u^i) = (u^i)^Tl_i(x)$, i.e., $f_i$ is linear in the uncertainty. Then Problem~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
%\begin{align}\label{Prob:FenchelGammaCounterpartLinear}
%\begin{split}
%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i \\
%\text{s.t.} & x \in \mathcal{X} \\
%& p_i + \theta \geq  \supportx{i} \ \forall i \in [m] \\
%& p, \theta \geq 0.
%\end{split}
%\end{align}
%\end{theorem}
%\proof{Proof.}
%Since Assumptions (i), (ii) and (iii) hold and since $\Gamma$ is integral, Theorem~\ref{Theo:FenchelGammaCounterpart} holds and Problem~\eqref{Prob:GeneralGammaCounterpart} is Problem~\eqref{Prob:FenchelGammaCounterpart}. In \cite{Fenchel}, the authors showed that in the case $f_i$ being linear in $u^i$, 
%\begin{gather*}
%f_{i,*}(x,v^i) \neq -\infty \Leftrightarrow v^i = l_i(x)
%\end{gather*} 
%and that $f_{i,*}(x,l_i(x)) = 0$. Since $f_{i,*}(x,v^i) = - \infty$ would lead to infeasibility of Problem~\eqref{Prob:FenchelGammaCounterpartLinear}, $v^i = l_i(x) \ \forall i \in [m]$. \\
%Inserting this into Problem~\eqref{Prob:FenchelGammaCounterpart} results in
%\begin{align*}
%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%\text{s.t.} & x \in \mathcal{X}, \\
%& p_i + \theta \geq (\overline{u}^i)^Tl_i(x) + \supportx{i} - f_i(x,\overline{u}^i) \ \forall i \in [m], \\
%& p, \theta \geq 0.
%\end{align*} 
%Since $f_i(x, \overline{u}^i) = (\overline{u}^i)^Tl_i(x)$, the claim follows.
%\endproof
%Theorem~\ref{Theo:GeneralLinearUncertainty} implies that in the case
%of linearity in the uncertainty, the problem of solving the robust
%counterpart mainly reduced to determining $\supportx{i}$ for all $i
%\in [m]$. In \cite{Fenchel}, the authors did that for various
%uncertainty sets $\mathcal{U}_i$, including explicit geometries like
%ellipsoids, polyhedra, cones, boxes, Miskowski sums or their
%intersections and uncertainty sets which are describes by various
%functions, e.g. convex functions or separable functions. For
%illustrative purposes, we show two examples: the cases of
%$\mathcal{Z}_i$ being a polyhedron for all $i \in [m]$ and
%$\mathcal{Z}_i$ being defined by the $p$-norm for all $i \in [m]$.
%\begin{example}\label{Ex:Polyhedra}
%As it was shown in \cite{Fenchel} and in \cite{RobustBook}, when $\mathcal{U}_i = \{\overline{u}^i + A^i \zeta^i \mid C^i \zeta^i \leq d^i\}$, i.e., $\mathcal{Z}^i = \{\zeta^i \mid C^i \zeta^i \leq d^i\}$ being a non-empty, full-dimensional polyhedron,
%\begin{gather*}
%\supportx{i} = \max_{\zeta^i: C^i \zeta^i \leq d^i } (\zeta^i)^T(A^i)^Tl_i(x) 
%\end{gather*}
%and thus by strong duality
%\begin{gather*}
%\supportx{i} = \min_{y^i: (C^i)^Ty^i = (A^i)^Tl_i(x), y \geq 0} (d^i)^T y^i
%\end{gather*}
%Hence problem~\eqref{Prob:FenchelGammaCounterpartLinear} is equivalent to
%\begin{align}\label{Prob:FenchelGammaCounterpartLinearPolyhedra}
%\begin{split}
%\min_{x,p,\theta,y^i} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%\text{s.t.} & x \in \mathcal{X}, \\
%& p_i + \theta \geq (d^i)^Ty^i \ \forall i \in [m], \\
%& (C^i)^Ty^i = (A^i)^Tl_i(x) \ \forall i \in [m], \\
%& p, \theta, y^1, \dots, y^m \geq 0.
%\end{split}
%\end{align}
%\end{example}
%\todo[inline][inline]{ich habe das Label vom ursprÃ¼nglichen Beispiel 3.14 Ã¼bernommen. Der Querverweis fuktioniert genauso}
%\begin{example}\label{Ex:Norm}
%Let $p \in [1, \infty]$. If we assume that $\mathcal{Z}_i := \{\zeta^i \mid || \zeta_i ||_p \leq \rho\}$ for an arbitrary $\rho \in \R_{\geq 0}$, then (we again refer to \cite{Fenchel} and \cite{RobustBook}) 
%\begin{gather*}
%\supportx{i} = \rho || (A^i)^Tl_i(x) ||_q,
%\end{gather*}
%where $q$ satisfies $\frac1p + \frac1q = 1$ for $p \neq \infty$ and $q = 1$ otherwise. Then problem~\eqref{Prob:FenchelGammaCounterpartLinear} is equivalent to problem~\eqref{Prob:GeneralReModel}: 
%\begin{align}\label{Prob:FenchelGammaCounterpartLinearPolyhedra}
%\begin{split}
%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%\mathrm{s.t.} &  \ x \in \mathcal{X}, \\
%& p_i + \theta \geq \rho || (A^i)^Tl_i(x) ||_q \ \forall i \in [m], \\
%& p, \theta \geq 0. 
%\end{split}
%\end{align}
%\end{example}
%We also show that the second part of Proposition~\ref{Prop:FenchelGammaCounterpart} is a generalization of Proposition~\ref{Prop:Gamma_MIP}.
%\begin{example}
%Consider an MIP with an uncertain objective under interval uncertainty.
%% Similar to Example~\ref{Rem:GeneralizeComb}, we set the various parameters and insert them into problem~\eqref{Prob:FenchelGammaCounterpartLinearPolyhedra}:
%%\begin{gather*}
%%\mathcal{U}_i := [\overline{c}_i - \Delta c_i, \overline{c}_i + \Delta c_i], \ \overline{u}^i := \overline{c}_i, \ f_i(x,u^i) := u^i \cdot x_i, \ \mathcal{X}:=\{x \in \Z^{r} \times \R^{n-r} \mid Ax \leq b\}.
%%\end{gather*}
%%Thus, the uncertainty set is as an affine
%The uncertainty set for each coefficient can be rewritten as an affine
%transformation of a (one-dimensional) box:
%\begin{gather*}
%\mathcal{U}_i := \{\overline{c}_i + \Delta c_i\zeta_i \mid |\zeta_i| \leq 1\}, 
%\end{gather*}
%i.e., $\mathcal{Z}_i := \{\zeta_i \in \R: \ |\zeta_i| \leq 1\}.$ With the notation
%from Example~\ref{Ex:Norm}, $p= \rho = 1$ and $A^i = \Delta
%c_i$. After linearizing constraints that contain absolute values, inserting this into model~\eqref{Prob:FenchelGammaCounterpartLinearPolyhedra} results in
%\begin{align*}
%\min_{x,p,\theta,z} & \ \Gamma \theta + \sum_{i \in [n]} \overline{c}_ix_i + p_i, \\
%\mathrm{s.t.} & \ x \in \mathcal{X}, \\
%& p_i + \theta \geq \Delta c_i z_i  \ \forall i \in [n], \\
%& x_i \in [-z_i, z_i] \ \forall i \in [n], \\
%& p, \theta \geq 0.
%\end{align*}
%%i.e., problem~\eqref{Prob:RobCounterpartMIP}. 
%\end{example}
%For more details on other uncertainty set geometries, we refer to Section 3 and
%to Table 1 in \cite{Fenchel}. \\
%While one can now give a reformulation for MINLPs without
%uncertainty,
For combinatorial optimization under interval uncertainty, it is usually essential to obtain a tractable reformulation for which the feasible set is not altered, as oracles for program~\eqref{Prob:GeneralNomOpt} can then be used to solve the resp. $\Gamma$--counterpart. In the case of linear uncertainty, this can be achieved by adding the additional assumption of $l_i$, $i \in [m]$, being non--negative on $\mathcal{X}$ and altering $\mathcal{X}$:
%%\todo[inline]{Thm 4.8 leistet
%%das aber noch nicht, weil da noch die v Werte dabeisind, oder? Das
%%muesste man dann noch dazusagen, dass das naechste thm a step towards
%%reaching this goal darstellt, oder sowas in der art.}
%%\todo[inline]{Dennis: da kommen wir auch nur im Linearen hin, ich hab das jetzt danach kommentiert. Man kann die PArameter $v^i$ aber eigentlich frei bestimmen, so dass es von der allgemeinen Struktur abhängt, was man mit dem Problem macht (zum Beispiel mehr Fallunterscheidungen, bei denen man $\theta^k$ bestimmen kann).}
%%\begin{theorem}\label{Theo:GeneralGammaCounterPartWithoutDual}
%%Let $\Gamma \in [m]$. Under Assumption~\ref{Ass:General}, the $\Gamma$--counterpart \eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%%\begin{align}\label{Prob:GeneralGammaCounterpartWithoutDual}
%%\begin{split}
%%\min_{k \in [m]_0} & \min_{\substack{x \in \mathcal{X}, v^1 \in \R^{L_1}, \\  \dots, v^m \in \R^{L_m}}} \Gamma \theta^k(x,v^k) + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, \theta^i(x,v^i) - \theta^k(x,v^k) \}, \\
%%%\text{s.t.} & \ x \in \mathcal{X} \\
%%%& \theta^k \geq 0. \\
%%%& \theta^k = \overline{u^k}^Tv^k - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k) + \support{k}).
%%\end{split}
%%\end{align}
%%with $\theta^0(x,v^0):=0 \text{ and }$
%%\begin{gather*}
%%\theta^k(x,v^k) := (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k)  \ \forall k \in [m].
%%\end{gather*}
%%If $f_i$ is linear in the uncertainty, i.e., $f_i(x,u^i) = (u^i)^Tl_i(x),$ for $l_i\colon \R^n \to \R^{L_i}, $ problem~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
%%\begin{align}\label{Prob:GeneralGammaCounterpartWithoutDualLinear}
%%\begin{split}
%%\min_{k \in [m]_0} & \min_{x \in \mathcal{X}} \Gamma \theta^k(x) + \sum_{i \in [m]} (\overline{u}^i)^Tl_i(x) + \max \{0, \theta^i(x) - \theta^k(x) \}, \\
%%%\text{s.t.} & x \in \mathcal{X} \\
%%%& \theta^k \geq 0. \\
%%%& \theta^k = \overline{u^k}^Tv^k - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k) + \support{k})
%%\end{split}
%%\end{align}
%%where $\theta^0(x) = 0$ and $\theta^k(x) = \supportx{k}$. 
%%\end{theorem}
%%\proof{Proof.}
%Since Assumption~\ref{Ass:General} holds and $\Gamma \in [m]$, the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
%\eqref{Prob:FenchelGammaCounterpart}. Analogously to the proof in Lemma~\ref{Rem:GeneralizeComb}, one can show that
%\begin{gather}\label{Eq:optimal_p}
%p^*_i = \max \{0, (\overline{u}^i)^Tv^{i,*} + \support{i} -f_{i,*}(x^*,v^{i,*}) - f_i(x^*, \overline{u}^i) - \theta^* \}
%\end{gather}
%%for an optimal solution $(x^*,p^*,\theta^*,v^{1,*}, \dots, v^{m,*})$ for all $i \in [m]$ and that of~\eqref{Prob:FenchelGammaCounterpart}. Inserting equation~\eqref{Eq:optimal_p} into the objective function of \eqref{Prob:FenchelGammaCounterpart} results in 
%%\begin{align}\label{Eq:piecewiselinear}
%% \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, (\overline{u}^i)^Tv^i + \support{i}-f_{i,*}(x,v) - f_i(x, \overline{u}^i) - \theta \}.
%%\end{align}
%%Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, 
%and that $\theta^*$ equals $0$ or there exists $k \in [m]$ such that
%\begin{gather}\label{Eq:OptimalTheta}
%\theta^* = (\overline{u}^k)^Tv^{k,*} + \support{k} - f_{k}(x^*
%,\overline{u}^k) - f_{k,*}(x^*,v^{k,*}).
%\end{gather}
%%for one $k \in [m]$. %Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, the minimum is furthermore obtained either at $0$ or 
%%Assume that $(x,v^1, \dots, v^m, \theta)$ is feasible and that $\theta$ is equal to 0 nor does it fulfill equation~\eqref{Eq:OptimalTheta} for any $k \in [m]$. Thus, the sets
%%\begin{align*}
%%S^{<}&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k)  < \theta\} \text{ and } \\
%%S^>&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) > \theta\}
%%\end{align*}
%%are a partition of $[m]$, i.e., $S^< \cup S^> = [m]$ and $S^< \cap S^> = \emptyset$. The objective can be rewritten as:
%%\begin{alignat*}{2}
%%&\Gamma\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} \left( -f_k(x,v^k) + \support{k} - \theta \right) \\
%%&= (\Gamma - |S^>|)\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} -f_k(x,v^k) + \support{k}. 
%%\end{alignat*}
%%We consider different cases for $S^>$:
%%\begin{itemize}
%%\item[\underline{First case:}] $S^> = \emptyset$. \\
%%In this case, $S^< = [m]$. The solution $(x,v^1, \dots, v^m, \overline{\theta})$ with
%%\begin{gather*}
%%\overline{\theta} := \max_{k \in [m]} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) 
%%\end{gather*}
%%has a better objective value than $(x,v^1, \dots, v^m, \theta)$, since $\overline{\theta} < \theta$.
%%\item[\underline{Second case:}] $S^> = [m]$.\\
%%In this case, 
%%\begin{gather*}
%%0 \leq \theta < f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) \ \forall k \in [m].
%%\end{gather*}
%%We set $
%%\overline{\theta} := \min_{k \in [m]} (\overline{u}^k)^Tv^k + \delta^*({A^k}^Tv^k \mid \mathcal{Z}_k) - f_k(x,\overline{u}^k) - f_k(x,v^k) $
%%
%%and since $\Gamma \in [m]$, the objective value of $(x,v^1, \dots, v^m, \overline{\theta})$ is at most the objective value of $(x,v^1, \dots, v^m, \theta)$. 
%%\item[\underline{Third case:}] $S^> \neq \emptyset, [m]$. \\
%%In this case, there exist $k,l \in [m]$, such that \begin{align*}
%%&f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k} < \theta \\
%%&< f_l(x,\overline{u}^l) - f_l(x,\overline{u}^l) - f_l(x,v^l) + \support{l}.
%%\end{align*}
%%In particular, it can be assumed without loss of generality that 
%%\begin{gather*}
%%k= \mathrm{argmax}_{i \in S^<} \theta - f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i}, \\
%%l= \mathrm{argmin}_{i \in S^>} f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i} - \theta.
%%\end{gather*} 
%%We set 
%%\begin{gather*}
%%\overline{\theta}:= \begin{cases} f_l(x,\overline{u}^l) + \support{l} - f_l(x,\overline{u}^l) - f_l(x,v^l), & \text{if $|S^>| > \Gamma$,} \\
%%\max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}, & \text{otherwise.}
%%\end{cases}
%%\end{gather*} 
%%%and otherwise, set
%%%\begin{gather*}
%%%\overline{\theta}:= \max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}.
%%%\end{gather*}
%%In both cases, we obtain a feasible solution with a better objective.
%%\end{itemize} 
%%We define
%%\begin{gather*}
%%\theta^k(x,v^k) := f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k - f_k(x,\overline{u}^k) - f_l(x,v^k) + \support{k}
%%\end{gather*}
%%for $k \in [m]$ and $\theta^0 := 0$. 
%Thus, the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%\begin{alignat*}{2}
%\min_{k \in [m]_0} & \min_{\substack{x \in \mathcal{X}, v^1 \in \R^{L_1}, \\  \dots, v^m \in \R^{L_m}}} \Gamma \theta^k(x,v^k) + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, \theta^i(x,v^i)- \theta^k(x,v^k) \}, \\
%& \ \ \mathrm{s.t.} \ \theta^i(x,v^i) \geq 0 \ \forall i \in [m]. \\
%\end{alignat*}
%Finally, by application of Fenchel's inequality (cf. \cite{ConvexAnalysis}, Chapter 12) and Assumption~\ref{Ass:General}, (iii) $\theta^i(x,v^i) \geq 0$ is redundant since 
%%$\theta^0(x,v^0) = 0$ by definition and for $k \in [m]$, 
%\begin{gather*}
%\support{i} \geq 0 \Leftrightarrow \exists \zeta \in \mathcal{Z}_i: \ \zeta^T({A^i})^Tv^i \geq 0
%\end{gather*}
%and the first statement follows. If $f_i$ is linear in the uncertainty, $f_{i,*}(x,v^k) \neq -\infty$ is equivalent to $v^i = l_i(x)$ and the equivalence of \eqref{Prob:GeneralGammaCounterpart} and \eqref{Prob:GeneralGammaCounterpartWithoutDualLinear} follows. %we obtain $\support{i} = \Delta u_i l_i(x)$ and the claim follows.
%\endproof
%Due to the fact that we also need to optimize over the variables $v^i$, the first part of  Theorem~\ref{Theo:GeneralGammaCounterPartWithoutDual} is not an exact analogon to Proposition~\ref{Prop:Tractable_Gamma_Comb}.\todo[inline]{Remark und Vergleich mit Lemma 4.2?} However, we have obtained a reformulation of non-linear (combinatorial) optimization problems under uncertainty for which the constraints of the decision variables $x$ does not change. In addition, in the case of linearity in the uncertainty, another step can be taken and the variables $v^i$ can be determined on the spot. 

\begin{theorem}\label{Cor:LinInt}
Let $\Gamma \in [m]$ and consider the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} under interval uncertainty $\mathcal{U}_k = [\overline{u}_k, \overline{u}_k + \Delta u_k]$ for some $\overline{u}_k, \Delta u_k \in \R_{\geq 0}^{L_k}$ for all $k \in [m]$. If the uncertainty is linear with $f(x,u_k) = u_k^Tl_k(x)$ and $l_k(x) \geq 0$ holds for all $x \in \mathcal{X}$ and all $k \in [m]$, then program~\eqref{Prob:GeneralGammaCounterpart} is equivalent to   %, $\theta^k(x) = \Delta u_k l_k(x)$, resulting in %%problem~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
\begin{align}\label{Prob:CombinatorialGammaCounterPartWithoutDualLinear}
\begin{split}
\inf_{k \in [m]_0} & \left\{ \inf_{\mathcal{Q} \subseteq [m]} \left\{ \inf_{x \in \mathcal{X_\mathcal{Q}}} \left\{ \Gamma \Delta u_k^T l_k(x) + \sum_{i \in [m]} \overline{u}_i^Tl_i(x) + \sum_{q \in \mathcal{Q}} \Delta u_q^T l_q(x) - \Delta u_k^T l_k(x) \right\} \right\} \right\},
\end{split}
\end{align}
with $\Delta u_0 := l_0(x) := 0$ and 
\begin{gather*}
\mathcal{X}_\mathcal{Q} := \{x \in \mathcal{X}: \Delta u_q^T l_q(x) - \Delta u_k^T l_k(x) \geq 0 \ \forall q \in \mathcal{Q}, \ \Delta u_q^T l_q(x) - \Delta u_k^T l_k(x) \leq 0 \ \forall q \in [m] \setminus \mathcal{Q}\}.
\end{gather*}
%  If the uncertainty is 1-dimensional and $l_k$ is binary for all $k \in [m]$, i.e., $u_k \in \R$ and $l_k(x) \in \{0,1\}$ for all $x \in \mathcal{X}$, \eqref{Prob:GeneralGammaCounterpart} is equivalent to
%\begin{align}\label{Prob:CombinatorialGammaCounterPartWithoutDualLinearBinary}
%\begin{split}
%\min_{k \in [m]_0} & \Gamma \Delta u_k + \min_{\substack{x \in \mathcal{X},\\ l_k(x) = 1}} \sum_{i \in [m]} (\overline{u}_i + \max \{0, \Delta u_i - \Delta u_k\})l_i(x),
%\end{split}
%\end{align}
%i.e., the $\Gamma$--counterpart is equivalent to the minimum of $m+1$ nominal problems and an additional constraint.
\end{theorem}
%\todo[inline]{Auch hier: Können wir nicht über exponentiell viele Probleme gehen?}
\proof{Proof.}
Let $e^j$ be the vector of only ones in $\R^j$. Since $l_k$ is non--negative, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} does not change when one replaces $\mathcal{U}_k$ with $\mathcal{U}^\varepsilon_k := [\overline{u}_k - \varepsilon e^{L_k}, \overline{u}_k + \Delta u_k]$ for any $\varepsilon > 0$ and Assumption~\ref{Ass:GeneralLinear} holds. Thus, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to \eqref{Prob:FenchelGammaCounterpart}. Analogously to the proof of Lemma~\ref{Rem:NoFenchel}, one can show that
\begin{gather}\label{Eq:lin_optimal_p}
p^*_i = \max \{0, \supportx{i} - \theta^* \}
\end{gather}
%for an optimal solution $(x^*,p^*,\theta^*,v^{1,*}, \dots, v^{m,*})$ for all $i \in [m]$ and that of~\eqref{Prob:FenchelGammaCounterpart}. Inserting equation~\eqref{Eq:optimal_p} into the objective function of \eqref{Prob:FenchelGammaCounterpart} results in 
%\begin{align}\label{Eq:piecewiselinear}
% \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, (\overline{u}^i)^Tv^i + \support{i}-f_{i,*}(x,v) - f_i(x, \overline{u}^i) - \theta \}.
%\end{align}
%Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, 
and that $\theta^*$ equals $0$ or there exists $k \in [m]$ such that
\begin{gather}\label{Eq:lin_OptimalTheta}
\theta^* = \supportx{k} = \Delta u_k^Tl_k(x)
\end{gather}
for optimal $p^*$ and $\theta^*$. Note that the last equation in \eqref{Eq:lin_OptimalTheta} holds since $l_k$ is non--negative.
%for one $k \in [m]$. %Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, the minimum is furthermore obtained either at $0$ or 
%Assume that $(x,v^1, \dots, v^m, \theta)$ is feasible and that $\theta$ is equal to 0 nor does it fulfill equation~\eqref{Eq:OptimalTheta} for any $k \in [m]$. Thus, the sets
%\begin{align*}
%S^{<}&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k)  < \theta\} \text{ and } \\
%S^>&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) > \theta\}
%\end{align*}
%are a partition of $[m]$, i.e., $S^< \cup S^> = [m]$ and $S^< \cap S^> = \emptyset$. The objective can be rewritten as:
%\begin{alignat*}{2}
%&\Gamma\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} \left( -f_k(x,v^k) + \support{k} - \theta \right) \\
%&= (\Gamma - |S^>|)\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} -f_k(x,v^k) + \support{k}. 
%\end{alignat*}
%We consider different cases for $S^>$:
%\begin{itemize}
%\item[\underline{First case:}] $S^> = \emptyset$. \\
%In this case, $S^< = [m]$. The solution $(x,v^1, \dots, v^m, \overline{\theta})$ with
%\begin{gather*}
%\overline{\theta} := \max_{k \in [m]} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) 
%\end{gather*}
%has a better objective value than $(x,v^1, \dots, v^m, \theta)$, since $\overline{\theta} < \theta$.
%\item[\underline{Second case:}] $S^> = [m]$.\\
%In this case, 
%\begin{gather*}
%0 \leq \theta < f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) \ \forall k \in [m].
%\end{gather*}
%We set $
%\overline{\theta} := \min_{k \in [m]} (\overline{u}^k)^Tv^k + \delta^*({A^k}^Tv^k \mid \mathcal{Z}_k) - f_k(x,\overline{u}^k) - f_k(x,v^k) $
%
%and since $\Gamma \in [m]$, the objective value of $(x,v^1, \dots, v^m, \overline{\theta})$ is at most the objective value of $(x,v^1, \dots, v^m, \theta)$. 
%\item[\underline{Third case:}] $S^> \neq \emptyset, [m]$. \\
%In this case, there exist $k,l \in [m]$, such that \begin{align*}
%&f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k} < \theta \\
%&< f_l(x,\overline{u}^l) - f_l(x,\overline{u}^l) - f_l(x,v^l) + \support{l}.
%\end{align*}
%In particular, it can be assumed without loss of generality that 
%\begin{gather*}
%k= \mathrm{argmax}_{i \in S^<} \theta - f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i}, \\
%l= \mathrm{argmin}_{i \in S^>} f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i} - \theta.
%\end{gather*} 
%We set 
%\begin{gather*}
%\overline{\theta}:= \begin{cases} f_l(x,\overline{u}^l) + \support{l} - f_l(x,\overline{u}^l) - f_l(x,v^l), & \text{if $|S^>| > \Gamma$,} \\
%\max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}, & \text{otherwise.}
%\end{cases}
%\end{gather*} 
%%and otherwise, set
%%\begin{gather*}
%%\overline{\theta}:= \max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}.
%%\end{gather*}
%In both cases, we obtain a feasible solution with a better objective.
%\end{itemize} 
%We define
%\begin{gather*}
%\theta^k(x,v^k) := f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k - f_k(x,\overline{u}^k) - f_l(x,v^k) + \support{k}
%\end{gather*}
%for $k \in [m]$ and $\theta^0 := 0$. 
 Thus, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
\begin{alignat*}{2}
\inf_{k \in [m]_0} & \left\{ \inf_{\substack{x \in \mathcal{X}}} \left\{ \Gamma u_k^Tl_k(x) + \sum_{i \in [m]} (\overline{u}^i)^Tl_i(x) + \max \{0, \Delta u_i^Tl_i(x) - \Delta u_k^Tl_k(x)\} \right\} \right\}.
%& \ \ \mathrm{s.t.} \ \theta^i(x) \geq 0 \ \forall i \in [m]. 
\end{alignat*}
This proves the claim since $\mathcal{Q}$ encodes which maximization terms are non--negative.
%By application of Fenchel's inequality (cf. \cite{ConvexAnalysis}, Chapter 12) and since Assumption~\ref{Ass:General}, (iii) holds, $\theta^i(x,v^i) \geq 0$ is redundant since 
%%$\theta^0(x,v^0) = 0$ by definition and for $k \in [m]$, 
%\begin{gather*}
%\support{i} \geq 0 \Leftrightarrow \exists \zeta \in \mathcal{Z}_i: \ \zeta^T({A^i})^Tv^i \geq 0
%\end{gather*}
%and the first statement follows.
%Since $f_i$ is linear in the uncertainty, $f_{i,*}(x,v^k) \neq -\infty$ is equivalent to $v^i = l_i(x)$ and since $l_k$ is non-negative, $\support{k} = \Delta u_k^T l_k(x)$ and the equivalence of \eqref{Prob:GeneralGammaCounterpart} and \eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear} follows. 

%Since $l_k$ is non-negative, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} does not change when one replaces $\mathcal{U}_k$ with $\mathcal{U}^\varepsilon_k := [\overline{u}_k - \varepsilon e^{L_k}, \overline{u}_k + \Delta u_k]$ for any $\varepsilon > 0$ that is sufficiently small and Assumption~\ref{Ass:General} is fulfilled. Thus, the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to \eqref{Prob:FenchelGammaCounterpart}. Analogously to the proof of Lemma~\ref{Rem:NoFenchel}, one can show that
%\begin{gather}\label{Eq:optimal_p}
%p^*_i = \max \{0, (\overline{u}^i)^Tv^{i,*} + \support{i} -f_{i,*}(x^*,v^{i,*}) - f_i(x^*, \overline{u}^i) - \theta^* \}
%\end{gather}
%%for an optimal solution $(x^*,p^*,\theta^*,v^{1,*}, \dots, v^{m,*})$ for all $i \in [m]$ and that of~\eqref{Prob:FenchelGammaCounterpart}. Inserting equation~\eqref{Eq:optimal_p} into the objective function of \eqref{Prob:FenchelGammaCounterpart} results in 
%%\begin{align}\label{Eq:piecewiselinear}
%% \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, (\overline{u}^i)^Tv^i + \support{i}-f_{i,*}(x,v) - f_i(x, \overline{u}^i) - \theta \}.
%%\end{align}
%%Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, 
%and that $\theta^*$ equals $0$ or there exists $k \in [m]$ such that
%\begin{gather}\label{Eq:OptimalTheta}
%\theta^* = (\overline{u}^k)^Tv^{k,*} + \support{k} - f_{k}(x^*
%,\overline{u}^k) - f_{k,*}(x^*,v^{k,*}).
%\end{gather}
%%for one $k \in [m]$. %Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, the minimum is furthermore obtained either at $0$ or 
%%Assume that $(x,v^1, \dots, v^m, \theta)$ is feasible and that $\theta$ is equal to 0 nor does it fulfill equation~\eqref{Eq:OptimalTheta} for any $k \in [m]$. Thus, the sets
%%\begin{align*}
%%S^{<}&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k)  < \theta\} \text{ and } \\
%%S^>&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) > \theta\}
%%\end{align*}
%%are a partition of $[m]$, i.e., $S^< \cup S^> = [m]$ and $S^< \cap S^> = \emptyset$. The objective can be rewritten as:
%%\begin{alignat*}{2}
%%&\Gamma\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} \left( -f_k(x,v^k) + \support{k} - \theta \right) \\
%%&= (\Gamma - |S^>|)\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} -f_k(x,v^k) + \support{k}. 
%%\end{alignat*}
%%We consider different cases for $S^>$:
%%\begin{itemize}
%%\item[\underline{First case:}] $S^> = \emptyset$. \\
%%In this case, $S^< = [m]$. The solution $(x,v^1, \dots, v^m, \overline{\theta})$ with
%%\begin{gather*}
%%\overline{\theta} := \max_{k \in [m]} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) 
%%\end{gather*}
%%has a better objective value than $(x,v^1, \dots, v^m, \theta)$, since $\overline{\theta} < \theta$.
%%\item[\underline{Second case:}] $S^> = [m]$.\\
%%In this case, 
%%\begin{gather*}
%%0 \leq \theta < f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) \ \forall k \in [m].
%%\end{gather*}
%%We set $
%%\overline{\theta} := \min_{k \in [m]} (\overline{u}^k)^Tv^k + \delta^*({A^k}^Tv^k \mid \mathcal{Z}_k) - f_k(x,\overline{u}^k) - f_k(x,v^k) $
%%
%%and since $\Gamma \in [m]$, the objective value of $(x,v^1, \dots, v^m, \overline{\theta})$ is at most the objective value of $(x,v^1, \dots, v^m, \theta)$. 
%%\item[\underline{Third case:}] $S^> \neq \emptyset, [m]$. \\
%%In this case, there exist $k,l \in [m]$, such that \begin{align*}
%%&f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k} < \theta \\
%%&< f_l(x,\overline{u}^l) - f_l(x,\overline{u}^l) - f_l(x,v^l) + \support{l}.
%%\end{align*}
%%In particular, it can be assumed without loss of generality that 
%%\begin{gather*}
%%k= \mathrm{argmax}_{i \in S^<} \theta - f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i}, \\
%%l= \mathrm{argmin}_{i \in S^>} f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i} - \theta.
%%\end{gather*} 
%%We set 
%%\begin{gather*}
%%\overline{\theta}:= \begin{cases} f_l(x,\overline{u}^l) + \support{l} - f_l(x,\overline{u}^l) - f_l(x,v^l), & \text{if $|S^>| > \Gamma$,} \\
%%\max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}, & \text{otherwise.}
%%\end{cases}
%%\end{gather*} 
%%%and otherwise, set
%%%\begin{gather*}
%%%\overline{\theta}:= \max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}.
%%%\end{gather*}
%%In both cases, we obtain a feasible solution with a better objective.
%%\end{itemize} 
%%We define
%%\begin{gather*}
%%\theta^k(x,v^k) := f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k - f_k(x,\overline{u}^k) - f_l(x,v^k) + \support{k}
%%\end{gather*}
%%for $k \in [m]$ and $\theta^0 := 0$. 
%Thus, the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%\begin{alignat*}{2}
%\min_{k \in [m]_0} & \min_{\substack{x \in \mathcal{X}, v^1 \in \R^{L_1}, \\  \dots, v^m \in \R^{L_m}}} \Gamma \theta^k(x,v^k) + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, \theta^i(x,v^i)- \theta^k(x,v^k) \}, \\
%& \ \ \mathrm{s.t.} \ \theta^i(x,v^i) \geq 0 \ \forall i \in [m]. 
%\end{alignat*}
%%By application of Fenchel's inequality (cf. \cite{ConvexAnalysis}, Chapter 12) and since Assumption~\ref{Ass:General}, (iii) holds, $\theta^i(x,v^i) \geq 0$ is redundant since 
%%%$\theta^0(x,v^0) = 0$ by definition and for $k \in [m]$, 
%%\begin{gather*}
%%\support{i} \geq 0 \Leftrightarrow \exists \zeta \in \mathcal{Z}_i: \ \zeta^T({A^i})^Tv^i \geq 0
%%\end{gather*}
%%and the first statement follows.
%Since $f_i$ is linear in the uncertainty, $f_{i,*}(x,v^k) \neq -\infty$ is equivalent to $v^i = l_i(x)$ and since $l_k$ is non-negative, $\support{k} = \Delta u_k^T l_k(x)$ and the equivalence of \eqref{Prob:GeneralGammaCounterpart} and \eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear} follows. 

%
%The second part follows from the observation that, for $l_k(x) = 0$, 
%%the objective of \eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear} is equal to and the equivalence of \eqref{Prob:GeneralGammaCounterpart} and \eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear} follows. %we obtain $\support{i} = \Delta u_i l_i(x)$ and the claim follows.
%%%Since $l_k$ is non-negative, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} does not change when one replaces $\mathcal{U}_k$ with $\mathcal{U}^\varepsilon_k := [\overline{u}_k - \varepsilon 1_{L_k}, \overline{u}_k + \Delta u_k]$ for any $\varepsilon > 0$ that is sufficiently small. Thus, Assumption~\ref{Ass:General} is fulfilled and \eqref{Prob:GeneralGammaCounterpart} is equivalent to~\eqref{Prob:GeneralGammaCounterpartWithoutDualLinear}. Since $l_k$ is non-negative, $\support{k} = \Delta u_k^T l_k(x)$ and the first part of the claim follows. The second part of the claim follows from the observation that, for $l_k(x) = 0$, the objective of \eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear} is equal to
%\begin{gather*}
%\min_{x \in \mathcal{X}, l_k(x) = 0} \sum_{i \in [m]} \overline{u}_il_i(x) + \max \{0, \Delta u_i l_i(x) \} = \min_{x \in \mathcal{X}, l_k(x) = 0} \sum_{i \in [m]} \overline{u}_il_i(x) + \Delta u_i l_i(x)
%\end{gather*}
%since $\Delta u_i \geq 0$ and $l_i(x) \in \{0,1\}$ which is the objective of \eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear} for $k=0$ and for $l_k(x) = 1$, it is equal to 
%\begin{alignat*}{2}
%& \min_{x \in \mathcal{X}} \Gamma \Delta u_k + \sum_{i \in [m]} \overline{u}_i l_i(x) + \max \{0, \Delta u_i l_i(x) - \Delta u_k \} = \\
%& \Gamma \Delta u_k + \min_{x \in \mathcal{X}} \sum_{i \in [m]} (\overline{u}_i + \max \{0, \Delta u_i - \Delta u_k\})l_i(x),
%\end{alignat*}
%since $l_i(x)$ is binary. 
\endproof
Theorem~\ref{Cor:LinInt} states that the $\Gamma$--counterpart under said theorem's assumptions can be 'almost' solved by an optimization oracle for solving~\eqref{Prob:GeneralNomOpt}, assuming that one can extend the oracle from $\mathcal{X}$ to $\mathcal{X}_\mathcal{Q}$. However, the number of calls is in $O(m2^m)$, i.e., exponential in the number of uncertain functions (even if $m$ is part of the input). To the best of our knowledge, there is no 'black box' that can go from $\mathcal{X}$ to $\mathcal{X}_\mathcal{Q}$ in the nonlinear combinatorial context which would certainly be an interesting research avenue. Thus, to be able to solve the $\Gamma$--counterpart with an optimization oracle as of now, one requires further assumptions. However, in Section~\ref{Sec:Reformulations}, we show that this is possible for programs 'underlying an assignment structure'. As a tool, we require the following result for models of the form $\min_{x \in \mathcal{X}} u^TBg(x)$ underlying said structure. 

%Similarly to Corollary~\ref{Prop:FenchelGammaCounterpart}, its tractability depends on the tractability of the support functions and the concave conjugates. \todo{hier konkav zu linear nochmal erwähnen}
%Note that, due to the difficulty with the max--term, it seems unlikely that this formulation is more beneficial than the one provided in Corollary~\ref{Prop:FenchelGammaCounterpart}. %and that, if $f_k$ is linear in the uncertainty, $v^k$ is fixed and $\theta^k(x,v^k) = \support{k}$. 
%Note that, for combinatorial optimization problems, one would like to obtain a reformulation over $\mathcal{X}$ with an objective with a 'similar' structure (e.g., if the objective is quadratic, the reformulated objective should be quadratic as well). A possibility to get rid of the max-term would be performing a distinction of cases for all $k \in [m]_0$ and $i \in [m]$ by adding the inequality
%\begin{gather*}
%\theta^i(x,v^i) \geq \theta^k(x,v^k) \text{ or } \theta^i(x,v^i) \leq \theta^k(x,v^k)
%\end{gather*}
%to the inner problem and optimizating over all possibilities. One can think of branch--and--bound-procedures to avoid enumerating the exponential number of possibilities, also in Theorem~\ref{Cor:LinInt}. 
%\end{remark}
%\begin{remark}
%We note that the constraint $l_k(x) = 1$ is in general not critical since $l_k(x)$ is a binary function. If $l_k(x)$ is the product of binary variables, $l_k(x) = 1$ fixes these variables to one and if it is the sum of binary variables, it is 'only' another linear constraint. We demonstrate in Section 5 that, for some applications, the additional constraint does not change the underlying structure. If it would, one can use that the $\Gamma$--counterpart of $\min_{x\in \mathcal{X}} u^Tl(x)$ under interval uncertainty and $l(x) \in \{0,1\}^m$ for all $x \in \mathcal{X}$ is also equivalent to 
%\begin{align}\label{Prob:CombinatorialGammaCounterPartWithoutDualLinearBinaryTwo}
%\begin{split}
%\min_{k \in [m]_0} & \Gamma \Delta u_k + \min_{x \in \mathcal{X}} \sum_{i \in [m]} (\overline{u}_i + \max \{0, \Delta u_i - \Delta u_k\})l_i(x),
%\end{split}
%\end{align}
%which is implied by the original results of Bertsimas and Sim applied to $\min_{(x,y) \in \mathcal{X}_y} u^Ty$ where $\mathcal{X}_y := \{(x,y) \in \mathcal{X} \times \{0,1\}^m:  \ l(x) = y \text{ for one } x \in \mathcal{X}\}$. Thus, depending on the underlying nominal problem, one can choose between reformulations~\eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinearBinary} and~\eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinearBinaryTwo}.
%\end{remark}
%Additionally, in the second setting of Theorem~\ref{Cor:LinInt}, one can reduce the number of nominal problems one has to solve and can determine $\alpha$-approximations (for $\alpha \geq 1$), if the underlying nominal problems are $\alpha$--approximable. The proofs are very similar to the ones for the original $\Gamma$--counterpart of Bertsimas and Sim and thus ommitted to Appendix B. 
%\begin{theorem}\label{Theo:Approx}
%Let $\Gamma \in [m]$ and consider the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} under interval uncertainty, i.e., for all $k \in [m]$ exist $\overline{u}_k, \Delta u_k \in \R_{>0}$, such that $\mathcal{U}_k = [\overline{u}_k, \overline{u}_k + \Delta u_k]$. If $f_k$ is linear in the uncertainty and binary for all $k \in [m]$, i.e., $f_k(x,u_k) = u_kl_k(x)$ for a function $l_k(x) \in \{0,1\}$ and the nominal problem is $\alpha$-approximable for one $\alpha \geq 1$, then \eqref{Prob:GeneralGammaCounterpart} is $\alpha$--approximable, too.
%%equivalent to
%%\begin{gather*}
%%\min_{k \in \mathcal{L}} \Gamma \Delta u_k + \min_{x \in \mathcal{X}} f(x,\overline{u}) + \sum_{i \in [k]} \left(\Delta u_i - \Delta u_k \right)l_i(x)
%%\end{gather*}
%%for $\mathcal{L} := \{\Gamma + 1, \dots, \Gamma + \gamma, m + 1\}$ with $\gamma$ being the biggest odd integer smaller than $(m + 1) - \Gamma$ and $\Delta_{m+1}:=0$.
%%\end{theorem}
%\end{theorem}
%\begin{theorem}\label{Theo:RedNumber}
%Let $\Gamma \in [m]$ and consider the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} under interval uncertainty, i.e., for all $k \in [m]$ exist $\overline{u}_k, \Delta u_k \in \R_{>0}$, such that $\mathcal{U}_k = [\overline{u}_k, \overline{u}_k + \Delta u_k]$. Without loss of generality, we assume $\Delta u_1 \geq \dots \geq \Delta u_m$. If $f_k$ is linear in the uncertainty and binary for all $k \in [m]$, i.e., $f_k(x,u_k) = u_kl_k(x)$ for a function $l_k(x) \in \{0,1\}$, then \eqref{Prob:GeneralGammaCounterpart} is equivalent to
%\begin{gather*}
%\min_{k \in \mathcal{L}} \Gamma \Delta u_k + \min_{x \in \mathcal{X}} f(x,\overline{u}) + \sum_{i \in [k]} \left(\Delta u_i - \Delta u_k \right)l_i(x)
%\end{gather*}
%for $\mathcal{L} := \{\Gamma + 1, \dots, \Gamma + \gamma, m + 1\}$ with $\gamma$ being the biggest odd integer smaller than $(m + 1) - \Gamma$ and $\Delta_{m+1}:=0$.
%\end{theorem}
%\todo[inline]{Theoreme auf unsere Version anpassen -- darauf achten, dass zulässige Mengen für die Sub-Probleme sogar disjunkt sein können!}
%\todo[inline]{Anwendung auf das QAP}
%
%This reduction is particulary important since, instead of solving $m + 1$ nominal problems, we only need to solve $\lceil \tfrac{m - \Gamma}{2} \rceil + 1$ problems. Especially for $\Gamma$ close to $m$, this reduction will prove substential.

%As an application of Theorem~\ref{Cor:LinInt}, we discuss a special structure under interval uncertainty: In the case of Examples~\ref{Ex:Scheduling} and \ref{Ex:QAP}, we have given interval uncertainties and an objective $u^TBg(x)$. We show that its $\Gamma$--counterpart is equivalent to the $\Gamma$--counterpart $y^Tg(x)$ for uncertain $y$ in a special case:
\begin{theorem}\label{Theo:CorrDoNotCare}
Let $B  \in \R_{\geq 0}^{m \times (m n)}$ be a block diagonal matrix where each block consists of a single row and let $g \colon \R^r \to \R_{\geq 0}^{mn}$ be an arbitrary nonnegative function. Consider program 
\begin{gather}\label{Prob:nom_LP_under_unc}
\inf_{x \in \mathcal{X}} u^TBg(x),
\end{gather}
under interval uncertainty, i.e., $u_i \in \mathcal{U}^i := [\overline{u}_i, \overline{u}_i + \Delta u_i] \subseteq \R_{\geq 0}$ for all $i \in [m]$. Furthermore, we assume that
\begin{gather}\label{Set:Assignment}
\mathcal{X} \subseteq \{x \in \R^r\colon \ \forall i \in [m] \exists ! j \in [n]: \ g_{i,j}(x) \text{ is not constant $0$}\}.
\end{gather} 
Let $\Gamma \in [m]$. Then the $\Gamma$--counterparts of program~\eqref{Prob:nom_LP_under_unc} and program
\begin{gather}
\label{Prob:nom_LP_under_unc_not_cor}
\inf_{x \in \mathcal{X}} y^Tg(x),
\end{gather}
under interval uncertainty $y_{(i,j)}\in \mathcal{Y}^{(i,j)} := [\overline{u}_i B_{i,(i,j)}, (\overline{u}_i + \Delta u_i) B_{i,(i,j)}]$ for all $(i,j) \in [m] \times [n]$ are equivalent.
\end{theorem}
\proof{Proof.}
We begin by introducing some notation: We set $B_{.,(0,0)} := \Delta y_{0,0}:= \overline{y}_{0,0}:=0$ (note that this is a slight abuse of notation and we mean the zero vector or the number $0$, depending on the dimension), $\Delta y:= (\Delta y_{a,b})_{(a,b) \in [m] \times [n]} := (\Delta u_a B_{a,(a,b)})_{(a,b) \in [m] \times [n]}$,  $\overline{y}:=(\overline{y}_{(a,b)})_{(a,b) \in [m] \times [n]} = (\overline{u}_a B_{a,(a,b)})_{(a,b) \in [m] \times [n]}$ and with $B_{k,.}$, we denote the $k$--th row of $B$. By applying Theorem~\ref{Cor:LinInt}, we obtain that the $\Gamma$--counterpart of program~\eqref{Prob:nom_LP_under_unc} is equivalent to
\begin{align}\label{Model:GammaCounterPartCor}
\inf_{k \in [m]_0} & \left\{ \inf_{\mathcal{Q} \subseteq [m]} \left\{ \inf_{x \in \mathcal{X_\mathcal{Q}}} \left\{ \Gamma \Delta u_k B_{k,.}g(x) + \sum_{i \in [m]} \overline{u}_iB_{i,.}g(x) + \sum_{q \in \mathcal{Q}} \Delta u_q B_{q,.}g(x) - \Delta u_k B_{k,.}g(x) \right\} \right\} \right\}.
\end{align}
Since $B$ is a block--diagonal matrix where each block contains exactly one row, one obtains $B_{i,(r,s)} = 0$ for $i \neq r$. Furthermore, since for all $i \in [m]$, $g_{i,j}(x) \neq 0$ for exactly one $j \in [n]$ (which will we be denoted by $j(i)$) we obtain 
\begin{gather*}
B_{q,.}g(x) = \sum_{i \in [m], j \in [n]} B_{q,(i,j)} g_{i,j}(x) = \sum_{i \in [m]} B_{q,(i,j(i))} g_{i,j(i)}(x) = B_{q,(q,j(q))} g_{q,j(q)}(x).
\end{gather*}
%Thus, for fixed $q \in \mathcal{Q}$, we obtain
%\begin{alignat}{2}\label{Eq:Help3}
%%\Delta u_q B_{q,.}g(x) - \Delta u_k B_{k,.}g(x) \geq 0 &\Longleftrightarrow\\
%\Delta u_q B_{q,(q,j(q))} g_{q,j(q)}(x) \geq  \Delta u_k B_{k,(k,j(k))} g_{k,j(k)}(x). &
%\end{alignat}
%we can further reformulate model~\eqref{Model:GammaCounterPartCor}:
%\begin{align}\label{Model_GammaCounterPartCorII}
%\begin{split}
%& \inf_{(k,l) \in [m] \times [n] \cup \{(0,0)\}}  \inf_{x \in \mathcal{X}} \ \Gamma \Delta u_k B_{k,(k,l)} g_{(k,l)}(x) + \overline{u}^TBg(x) \\
%& \sum_{(i,j) \in [m] \times [n]}   \max\{0, \Delta u_i B_{i,(i,j)} g_{(i,j)}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x)\}.
%\end{split}
%\end{align}
%Note that the case of $k = 0$ has only been changed by notation to $(k,l) = (0,0)$.
The $\Gamma$--counterpart of program~\eqref{Prob:nom_LP_under_unc_not_cor} is equivalent to (again by applying Theorem~\ref{Cor:LinInt} -- note that $l(x) = g(x)$ here and we replace $\mathcal{Q}$ by $\mathcal{Y}$ for the sake of notation):
\begin{align}\label{Model_GammaCounterPartUnCor}
\inf_{(a,b) \in [m] \times [n] \cup \{(0,0)\}} & \left\{ \inf_{\mathcal{Y} \subseteq [m] \times [n]} \left\{ \inf_{x \in \mathcal{X_\mathcal{Y}}} \left\{ \Gamma \Delta y_{(a,b)}g_{(a,b)}(x) +F_{\mathcal{Y},a,b}(x) \right\}  \right\} \right\}
\end{align}
with
\begin{align}\label{Eq:Help}
\begin{split}
F_{\mathcal{Y},a,b}(x) &:= \sum_{(i,j) \in [m] \times [n]} \overline{y}_{(i,j)}g_{(i,j)}x + \sum_{(q,p) \in \mathcal{Y}} \Delta y_{(q,p)}g_{(q,p)}(x) - \Delta y_{(a,b)}g_{(a,b)}(x).
\end{split}
\end{align}
In the following, we show that one can reduce the number of subproblems of program~\eqref{Model:GammaCounterPartCor} from $(m\cdot n+1) \cdot 2^{mn}$ to $(m+1)\cdot 2^m$ and that the resulting program is exactly~\eqref{Model_GammaCounterPartUnCor}. On the one hand, if $b \neq b(a)$, then $g_{(a,b)}(x) = 0$ for all $x \in \mathcal{X}$ by assumption and equation~\eqref{Eq:Help} results in
\begin{align}\label{Eq:Help2}
F_{\mathcal{Y},a,b}(x) = \sum_{(i,j) \in [m] \times [n]} \overline{y}_{(i,j)}g_{(i,j)}(x) + \sum_{(q,p) \in \mathcal{Y}} \Delta y_{(q,p)}g_{(q,p)}(x) = F_{\mathcal{Y},0,0}(x).
\end{align}
Thus, instead of $b \in [n]$, we can fix $b = b(a)$ in program~\eqref{Model_GammaCounterPartUnCor} and only have $m+1$ 'outer problems'. On the other hand, for each $\mathcal{Y} \subseteq [m] \times [n]$, $x \in \mathcal{X}_{\mathcal{Y}}$ only holds if
\begin{align*}
\Delta y_{q,p}g_{q,p}(x) \geq \Delta y_{a,b(a)}g_{a,b(a)}(x) > 0 \ \forall (q,p) \in \mathcal{Y}.
%% \Delta y_{q,p}g_{q,p}(x) \leq \Delta y_{a,b(a)}g_{a,b(a)}(x) \ %%%\forall (q,p) \in ([m] \times [n]) \setminus \mathcal{Y}.
\end{align*}
However, $g_{q,p}(x)$ is not equal to $0$ for some $x$ only if $p=p(q)$. Thus, $\mathcal{X}_\mathcal{Y} = \emptyset$ if $(q,p) \in \mathcal{Y}$ for some $p \neq p(q)$. Thus, program~\eqref{Model_GammaCounterPartUnCor} is equivalent to
\begin{align}\label{Model_GammaCounterPartUnCor2}
\inf_{a \in [m]_0} & \left\{ \inf_{\overline{\mathcal{Y}} \subseteq [m]} \left\{ \inf_{x \in \mathcal{X}_{\overline{\mathcal{Y}}}} \left\{\Gamma \Delta y_{(a,b(a))}g_{(a,b(a))}(x) + F_{\overline{\mathcal{Y}},a}(x) \right\} \right\} \right\}
\end{align}
where 
\begin{align*}
\mathcal{X}_{\overline{\mathcal{Y}}} := \{ x \in \mathcal{X}\colon & \Delta y_{q,p(q)}g_{q,p(q)}(x) \geq \Delta y_{a,b(a)}g_{a,b(a)}(x) \ \forall q \in \overline{\mathcal{Y}}, \\
& \Delta y_{q,p(q)}g_{q,p(q)}(x) \leq \Delta y_{a,b(a)}g_{a,b(a)}(x) \ \forall q \in [m]  \setminus \overline{\mathcal{Y}} \},
\end{align*}
$b(0) := 0$ and
\begin{align*}
F_{\overline{\mathcal{Y}},a}(x) &:=  \sum_{(i,j) \in [m] \times [n]} \overline{y}_{(i,j)}g_{(i,j)}(x) + \sum_{(q,p) \in \overline{\mathcal{Y}}} \Delta y_{(q,p(q))}g_{(q,p(q))}(x) - \Delta y_{(a,b(a))}g_{(a,b(a))}(x).
\end{align*}
By inserting the definition of $\overline{y}$ and $\Delta y$ into program~\eqref{Model_GammaCounterPartUnCor2} and by replacing all indices, one obtains program~\eqref{Model:GammaCounterPartCor}.
%However, since  Now, we assume that $b=a(b)$
%Note that the final equation holds since $\mathcal{X}_{\mathcal{Y}} = \mathcal{X}$ (the right--hand side of inequality~\eqref{Eq:Help3} is $0$ and the left--hand side is non--negative). Furthermore
\endproof
%%%%&= \Gamma \Delta u_a B_{a,(a,b)}g_{(a,b)}(x) + \sum_{(i,j) \in [m] \times [n]} \overline{y}_{(i,j)}g_{(i,j)}x + \sum_{(q,p) \in \mathcal{Y}} \Delta u_q B_{q,(q,p)}g_{(q,p)}(x) - \Delta y_{(a,b)}g_{(a,b)}(x) \\
%%%%&= \Gamma \Delta u_a B_{a,(a,b)}g_{(a,b)}(x) + \sum_{(i,j) \in [m] \times [n]} \overline{y}_{(i,j)}g_{(i,j)}x + \sum_{(q,p) \in \mathcal{Y}} \Delta u_q B_{q,(q,p)}g_{(q,p)}(x) - \Delta y_{(a,b)}g_{(a,b)}(x).

%%%%We recall that $(q,p) \in \mathcal{Y}$ implies
%\begin{alignat*}{2}
%\Delta y_{(q,p)}g_{(q,p)}(x) - \Delta y_{(a,b)}g_{(a,b)}(x)\geq 0 & \Longleftrightarrow 
%\Delta u_q B_{q,(q,p)}g_{(q,p)}(x) \geq	& \Delta y_{(a,b)}g_{(a,b)}(x)
%\end{alignat*}

% Inserting this into For fixed  Models~\eqref{Model_GammaCounterPartCorII} and \eqref{Model_GammaCounterPartUnCor} are equivalent,
%since $
%\Delta u^T B_{.,(k,l)} g_{(k,l)}(x) = \Delta u_k B_{k,(k,l)} g_{(k,l)}(x)$ for all $(k,l) \in [m] \times [n]$ and 
%\begin{alignat*}{2}
%&\sum_{i \in [m]} \max \{0, \Delta u_i B_{i,.} g_{i,.}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x) \} \\
%&=\sum_{i \in [m]} \max \{0, \Delta u_i \sum_{j \in [n]} B_{i,j} g_{(i,j)}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x)  \} \\
% &=\sum_{(i,j) \in [m] \times [n]} \underbrace{\max   \{0, \Delta u_i B_{i,(i,j)} g_{(i,j)}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x) \}}_{\neq 0 \text{ for exactly one $j \in [n]$}}. 
%\end{alignat*}

%By application of Theorem~\ref{Cor:LinInt} to the $\Gamma$--counterpart of model~\eqref{Prob:nom_LP_under_unc}, we obtain
%\begin{align}\label{Model:GammaCounterPartCor}
%\inf_{k \in [m]_0} \inf_{x \in \mathcal{X}} \Gamma \Delta u_k B_{k,.}g(x) + \overline{u}^TBg(x) + \sum_{i \in [m]}  \max\{0, \Delta u_i B_{i,.}g(x) - \Delta u_k B_{k,.}g(x) \}, 
%\end{align}
%with $B_{0,.} := \Delta u_0 := 0$. Since $B_{i,(r,s)} = 0$ for $i \neq r$ and since for all $i \in [m]$, $g_{(i,j)}(x) \neq 0$ for exactly one $j \in [n]$ by assumption, we can further reformulate model~\eqref{Model:GammaCounterPartCor}:
%\begin{align}\label{Model_GammaCounterPartCorII}
%\begin{split}
%& \inf_{(k,l) \in [m] \times [n] \cup \{(0,0)\}}  \inf_{x \in \mathcal{X}} \ \Gamma \Delta u_k B_{k,(k,l)} g_{(k,l)}(x) + \overline{u}^TBg(x) \\
%& \sum_{(i,j) \in [m] \times [n]}   \max\{0, \Delta u_i B_{i,(i,j)} g_{(i,j)}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x)\}.
%\end{split}
%\end{align}
%Note that the case of $k = 0$ has only been changed by notation to $(k,l) = (0,0)$. Next, we determine the $\Gamma$--counterpart of model~\eqref{Prob:nom_LP_under_unc_not_cor}, again by applying Theorem~\ref{Cor:LinInt}:
%\begin{align}\label{Model_GammaCounterPartUnCor}
%\begin{split}
%&\inf_{(k,l) \in [m] \times [n] \cup \{(0,0)\}}  \inf_{x \in \mathcal{X}} \ \Gamma \Delta u^T B_{.,(k,l)} g_{(k,l)}(x) + \\
%&\sum_{(i,j) \in [m] \times [n]} \overline{u}^T B_{.,(i,j)} g_{(i,j)}(x) + \max\{0, \Delta u^T B_{.,(i,j)} g_{(i,j)}(x) - \Delta u^TB_{.,(k,l)} g_{(k,l)}(x)\},
%\end{split}
%\end{align}
%where $B_{.,(0,0)} := 0$, $\Delta u:= (\Delta u_i)_{i \in [m]}$ and $\overline{u}:=(\overline{u}_i)_{i \in [m]}$. Models~\eqref{Model_GammaCounterPartCorII} and \eqref{Model_GammaCounterPartUnCor} are equivalent,
%since $
%\Delta u^T B_{.,(k,l)} g_{(k,l)}(x) = \Delta u_k B_{k,(k,l)} g_{(k,l)}(x)$ for all $(k,l) \in [m] \times [n]$ and 
%\begin{alignat*}{2}
%&\sum_{i \in [m]} \max \{0, \Delta u_i B_{i,.} g_{i,.}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x) \} \\
%&=\sum_{i \in [m]} \max \{0, \Delta u_i \sum_{j \in [n]} B_{i,j} g_{(i,j)}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x)  \} \\
% &=\sum_{(i,j) \in [m] \times [n]} \underbrace{\max   \{0, \Delta u_i B_{i,(i,j)} g_{(i,j)}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x) \}}_{\neq 0 \text{ for exactly one $j \in [n]$}}. 
%\end{alignat*}

%In the setting of the previous theorem, each part of the objective is influenced by exactly one uncertain parameter as in Example~\ref{Ex:Scheduling}. The theorem states that, under certain conditions for $g$, one can shift the linear combinations of the partial functions of $g$ into a modified uncertainty set. This is especially important in the linear case, where one can then straight-forwardly apply the original results of Bertsimas and Sim:
% when $g(x)$ is a binary function, one can then apply the results of Theorem~\ref{Cor:LinInt} to obtain tractable counterparts. Furthermore, by applying Theorem~\ref{Theo:CorrDoNotCare}, we prove that, for linear programs of the form $\min_{x\in\mathcal{X}} u^TLx$ with $u$ underlying interval uncertainty, the correlations imposed by the matrix $L$ linear problems can be 'ignored', if $\mathcal{X}$ underlies an assignment structure:

%:
%\begin{theorem}\label{Theo:CombinatorialGammaCounterPartWithoutDualLinear}
%Let $\Gamma \in [m]$. For all $i \in [m]$ assume that, there is a function $l_i\colon \R^n \to \R^{L_i} $, such that $f_i(x,u^i) = (u^i)^Tl_i(x)$, i.e., $f_i$ is linear in the uncertainty. Under Assumption~\ref{Ass:General}, problem~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
%\begin{align}\label{Prob:GeneralGammaCounterpartWithoutDualLinear}
%\begin{split}
%\min_{k \in \{0, \dots, m\}} & \min_{x \in \mathcal{X}} \Gamma \theta^k(x) + \sum_{i \in [m]} (\overline{u}^i)^Tl_i(x) + \max \{0, \theta^i(x) - \theta^k(x) \}, \\
%%\text{s.t.} & x \in \mathcal{X} \\
%%& \theta^k \geq 0. \\
%%& \theta^k = \overline{u^k}^Tv^k - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k) + \support{k}).
%\end{split}
%\end{align}
%where $\theta^0(x) = 0$ and $\theta^k(x) = \supportx{k}$. Furthermore, if all uncertainty sets are intervals, i.e., $\mathcal{U}_k = [\overline{u}_k, \overline{u}_k + \Delta u_k] \subseteq \R$ and $l_k(x) \geq 0$ for all $k \in [m]$, problem~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%\begin{align}\label{Prob:CombinatorialGammaCounterPartWithoutDualLinear}
%\begin{split}
%\min_{k \in \{0, \dots, m\}} & \min_{x \in \mathcal{X}} \Gamma \Delta u_k l_k(x) + \sum_{i \in [m]} \overline{u}_il_i(x) + \max \{0, \Delta u_i l_i(x) - \Delta u_k l_k(x) \},
%\end{split}
%\end{align}
%with $\Delta u_0 := l_0(x) := 0$.
%\end{theorem}
%\proof{Proof.}
%The proof for
%reformulation~\eqref{Prob:GeneralGammaCounterpartWithoutDual} follows the same outline as the proof of
%Proposition~\ref{Prop:FenchelGammaCounterpart} and is therefore omitted. In the case of interval uncertainty for all $k \in [m]$, i.e., $\mathcal{U}_k:=[\overline{u}^k,\overline{u}^k + \Delta u^k]$ for a perturbation $\Delta u_k$, one obtains $\theta^k(x) = \Delta u_k  l_k(x)$, since $l_k$ is non-negative on $\mathcal{X}$. 
%%In this case, applying Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} results in 
%%\begin{gather*}
%%\theta^k(x) = \Delta u_k l_k(x), \ k \in [m], 
%%\end{gather*} 
%\endproof
%Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear}
%implies that, in the case of linearity, we obtain a reformulation over the feasible set $\mathcal{X}$ without variables $v^i$, and that in the case of interval uncertainty, the required support functions can be determined.
% It is straightforward to show that
%Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} is a generalization of Proposition~\ref{Prop:Tractable_Gamma_Comb}.\\ %, thus we omit the proof.\\

%While the reformulation given in Example~\ref{ex:QAP_genau} is, to our knowledge, new in literature, there are already studies for solving the $\Gamma$--counterpart of a QAP. E.g. in \citep{QAP2015} the techniques of \cite{IntroGamma} where applied. Afterwards the authors used linearizing techniqes from \cite{QAP_lin} to linearizte the resulting MIQP. In our numerical study in Section 5, we compare our reformulation with linearizations in which one linearizes all quadratic terms with standart linearizations and applies the reformulations of \cite{IntroGamma}. 
%For all $i,j,r,s \in [n]$, we will apply a standard linearization of $x_{ir}x_{js}$ and introduce auxiliary variables $z_{ijrs}$, such that
%%We need a linear objective function to apply the reformulation of \citep{IntroGamma} to Problem~\eqref{Prob:QAP_RobCP}. Therefore, we linearizing the products $x_{ir}x_{js}$ in Problem~\eqref{Prob:QAP_RobCP} for $(i,j,r,s) \in [n]^4$ with
%\begin{align*}
%& z_{irjs} \ge x_{ir} +x_{js} -1, \quad \forall (i,j,r,s) \in [n]^4,\\
%&z_{irjs} \le x_{ir} , \quad \forall (i,j,r,s) \in [n]^4,\\
% & z_{irjs} \le  x_{js}, \quad \forall (i,j,r,s) \in [n]^4,\\
%& z_{irjs} \in [0,1], \quad \forall (i,j,r,s) \in [n]^4.
%\end{align*}
%The variables $z_{ijrs}$ are subject to the uncertain 'coefficients' $c_{ij}d_{rs} \in [d_{rs}\overline{c}_{ij}, d_{rs}(\overline{c}_{ij} + \Delta c_{ij})]$. The linearized model and our reformulation are equivalent while ot
%%\begin{align}
%%\begin{split}
%%\min_{z,x} & \sum_{(i,j,r,s) \in [n]^4}\left(\bar{c}_{ij}d_{rs}z_{ijrs} + \max_{\mathcal{S} \subseteq [n]^4: |S| \le \Gamma} \Delta c_{ij} d_{rs} z_{ijrs}\right)\\
%%\text{s.t. } & z_{irjs} \ge x_{ir} +x_{js} -1, \quad \forall (i,j,r,s) \in [n]^4,\\
%%& z_{irjs} \le x_{ir} , \quad \forall (i,j,r,s) \in [n]^4,\\
%% & z_{irjs} \le  x_{js}, \quad \forall (i,j,r,s) \in [n]^4,\\
%%& z_{irjs} \in [0,1], \quad \forall (i,j,r,s) \in [n]^4\\
%%&x\in \mathcal{X}.
%%\end{split}
%%\end{align} 
%We set for our uncertainty set
%\[c_{ij}d_{rs} \in  \mathcal{U}_{ijrs}=[d_{rs}\bar{c}_{ij},d_{rs}(\bar{c}_{ij}+\Delta c_{ij})] \quad \forall(i,j,r,s)\in [n]^4.\]
%%\todo[inline]{man sollte statt auf prop. 2.1 zu verweisen sagen dass das imgrunde bertsimas - sim ist, ansonsten wirkt es so als sei prop 2.1schon unser resultat...}
%With that we have a MIP and can use the standard $\Gamma$-approach of Proposition~\ref{Prop:Gamma_MIP} (see \cite{IntroGamma} Theorem 1). We denote the resulting MIP as $QAP_\text{MIP}$. Because of the linearization we get $n^4$ more variables but we have to solve only one MIP.
%If we further define $z_{ijrs} \in \{0,1\}$ we can apply Proposition~\ref{Prop:Tractable_Gamma_Comb} (see \cite{IntroGamma} Theorem 3). 
%The resulting binary problem is denoted as $QAP_\text{BP}$. In that case we also have $n^4$ more variables like with $QAP_\text{MIP}$ but we also have to solve the same amount of single BPs like with problem $QAP$ and compare them.

%\todo[inline][inline]{Dennis: Quelle!}


%\begin{example}
%For combinatorial problems of the form \eqref{Prob:Gamma_Comb} with uncertainty set $\mathcal{U}_i := [\overline{c}_i, \overline{c}_i + \Delta c_i]$, we define (as in the notation of Problem~\eqref{Prob:GeneralNomOpt}) 
%\begin{gather*}
%\overline{u}^i := \overline{c}^i, \ f_i(x,c_i) = c_ix_i, \ \mathcal{U}_i = \{ c_i = \overline{c^i} + \alpha \Delta c_i \mid \alpha \in [0,1]\}, \ \mathcal{Z}_i := [0,1].
%\end{gather*}
%Since $f_i$ is linear in the uncertainty, we obtain $v^k = l_k(x) = x_k$ and \begin{gather*}
%\theta^k = \delta^*(\Delta c_kx_k \mid \mathcal{Z}^k) = \sup_{\zeta \in [0,1]} \zeta \Delta c_k x_k = \Delta c_k x_k
%\end{gather*}
%for $k \in [m]$, since $x_k \in \{0,1\}$ and $\Delta c_k \geq 0$. Hence we need to solve 
%\begin{alignat*}{2}
%\min_{k \in \{0, \dots, m\}} & \min_{x} \Gamma \Delta c_k x_k + \sum_{i \in [m]} \overline{c_i} x_i + \max \{0, \Delta c_i x_i - \Delta c_k x_k\}, \\
%\text{s.t.} & x \in \mathcal{X}
%\end{alignat*}
%where $\Delta c_0 := x_0 := 0$. Now, if we assume without loss of generality that $\Delta c_1 \geq \Delta c_2 \geq \dots \geq \Delta c_m \geq 0$, one obtains the result of Proposition~\ref{Prop:Tractable_Gamma_Comb}: If $x_k = 0$, the inner problem is 
%\begin{gather*}
%\min_{x} \sum_{i \in [m]} \overline{c}_i x_i + \max \{0, \Delta c_i x_i \} = \min_x \sum_{i \in [m]} \overline{c}_i x_i + \Delta c_i x_i. 
%\end{gather*}
%It can easily be seen that this is exactly the model from Proposition~\ref{Prop:Tractable_Gamma_Comb}. %for $k = n+1$. If $x_k = 1$, one obtains 
%%\begin{alignat*}{2}
%%\min_{x} \Gamma \Delta c_k + \sum_{i \in [m]} \overline{c}_i x_i + \max \{0, \Delta c_i x_i - \Delta c_k\} &= \Gamma \Delta c_k + \min_{x} \overline{c}^Tx + \sum_{i \in [m]} \max \{0, \Delta c_i - \Delta c_k\} x_i \\ &= \Gamma \Delta c_k + \min_{x} \overline{c}^Tx + \sum_{i \in [m]} (\Delta c_i - \Delta c_k) x_i.
%%\end{alignat*}
%%which are the inner problems for $k = 1, \dots, n$ in Proposition~\ref{Prop:Tractable_Gamma_Comb}.
%\end{example}
%%\begin{example}[Linear in the uncertainty]
%%Easy to prove (see \cite{Fenchel}): $\theta^k = \delta^*({A^k}^Tv^k \mid Z^k)$, if 
%%\begin{gather*}
%%f_k(x, u^k) = {u^k}^Tl_k(x) 
%%\end{gather*}
%%for a (affine-)linear function $l_k \colon \R^n \to \R^m$. In particular, this implies that, for $k > 0$, we obtain (as an inner problem)
%%\begin{alignat*}{2}
%%\min_{x} \ & \Gamma \delta^*({A^k}^Tl_k(x)|Z_k) + \sum_{i \in [m]} f_i(x,\overline{u^i}) + \max \{0, \delta^*({A^i}^Tl_i(x)|Z_i)- \delta^*({A^k}^Tl_k(x)|Z_k) \} \\
%%\text{s.t.} & x \in \mathcal{X} 
%%\end{alignat*}
%%\end{example}
%%\todo[inline][inline]{Jana: Abschnitt zu MINLP-Kombinatorik schreiben. SpezialfÃ¤lle in denen man direkt ablesen kann, was passiert?}
%Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} implies that for combinatorial optimization problems, even if the functions $f_i$ are linear, obtaining a computationally tractable version for the $\Gamma$--counterpart is not easy. % The structure of the objective function is non-linear and more difficult due to
%%\begin{gather*}
%%\max\{0, \theta^i(x) - \theta^k(x)\}
%%\end{gather*}
%%which is in general, in combination with optimizing, a very hard optimization problem. 
%However, for many combinatorial optimization problems, the functions
%$f_i(x,u^i)$ are linear in the uncertainty %- i.e., $f_i(x,u^i) =
%                                %(u^i)^Tl_i(x)$ for some function
%%$l_i$ -
%and the uncertainty set for a parameter $u^i$ is an interval, i.e., $\mathcal{U}_i:=[\overline{u}^i,\overline{u}^i + \Delta u^i]$. In this case, applying Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} results in 
%\begin{gather*}
%\theta^k(x) = \Delta u_k l_k(x), \ k \in [m], 
%\end{gather*} 
%and thus in the optimization problem
%\begin{align}\label{Prob:CombGammaCounterPartFenchelStandard}
%\begin{split}
%\min_{k \in \{0, \dots, m\}} & \min_{x} \Gamma \Delta u_k l_k(x) + \sum_{i \in [m]} (\overline{u}^i)^Tl_i(x) + \max \{0, \Delta u_i l_i(x) - \Delta u_k l_k(x) \} \\
%\text{s.t.} & x \in \mathcal{X} \\
%%& \theta^k \geq 0. \\
%%& \theta^k = \overline{u^k}^Tv^k - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k) + \support{k}).
%\end{split}
%\end{align}

%Example~\ref{ex:QAP_genau} demonstrates that the exploitation of the combinatorial structure can result in a computationally tractable reformulation of a non-linear combinatorial optimization problem based on Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} and more generally on Theorem~\ref{Theo:GeneralGammaCounterPartWithoutDual} without losing the combinatorial structure. In general, the tractability of model~\eqref{Prob:GammaCombCounterpartWithoutFenchel} still heavily depends on the actual objective function of the nominal problem, the geometry of the uncertainty set and the combinatorial structure of $\mathcal{X}$. \\


%Theorem~\ref{Theo:CorrDoNotCare} shows that, at least in a special
%assignment structure of $B$ and $g$, it is possible to perform an affine transformation of the uncertainty set 
%'linearly
%combine'\todo[inline]{ist das nicht eher ein kreuzprodukt von intervallen?}
%\todo[inline]{Ich konstruiere ja die Menge $[\overline{u}^TB_{.,(i,j)}, (\overline{u}_i, \overline{u}_i + \Delta u_i)^TB_{.,(i,j)}]$, also Matrix mit ner Box multiplifiziert. Hab das ganze jetzt mit ner affinen Transformation umformuliert.}
Thus, if $g(x)$ is a $0/1$--function, then one can apply Theorem~\ref{Theo:CorrDoNotCare} to obtain an equivalent $\Gamma$--counterpart where the uncertainty is linear and no matrix $B$ is involved. The following corollary demonstrates this for $g(x) = x$:
\begin{corollary}\label{Cor:LPsAssigment}
Consider program \begin{gather}\label{Prob:nom_LP_under_unc:ASSIGN}
\min_{x \in \mathcal{X}} u^TBx
\end{gather}
as in the setting of Theorem~\ref{Theo:CorrDoNotCare} and assume that $
\mathcal{X} \subseteq \{x \in \{0,1\}^{[m] \times [n]}: \sum_{j \in [n]} x_{i,j} = 1 \ \forall i \in [m]\}$.
Let $\Gamma \in [m]$. Then the $\Gamma$--counterpart of \eqref{Prob:nom_LP_under_unc:ASSIGN} is equivalent to
\begin{align*}
\min_{(k,l) \in [m] \times [n] \cup \{(0,0)\}} \left\{ \Gamma \Delta u_k B_{k,(k,l)}  +
\min_{x \in \mathcal{X}} \left\{ \overline{u}^TBx + \sum_{(i,j) \in [m] \times [n]} F_{i,j,k,l}(x) \right\} \right\}
\end{align*}
where $B_{0,.} := \Delta u_0 := 0$ (the first one being a row vector of zeros and the latter being the number $0$) and 
\begin{gather*}
F_{i,j,k,l}(x):=\max\{0, \Delta u_i B_{i,(i,j)} - \Delta u_k B_{k,(k,l)}\}x_{i,j}.
\end{gather*}
\end{corollary}
%\begin{align*} %\label{Prob:RobustCounterpartSuperComb}
%\begin{split}
%\min_{\substack{(k,l) \in [m] \times [n] \\ \lor k = l = 0 }} \left\{\Gamma \Delta u^T B_{.,(k,l)} + 
% \min_{x \in \mathcal{X}}  \overline{u}^TBx + \sum_{(i,j) \in [m] \times [n]} \max \left\{0,\Delta u^T\left( B_{.,(i,j)} - B_{.,(k,l)}\right)\right\}x_{i,j} \right\}.
%\end{split} 
%\end{align*}
%$\min_{x Assume that for all $i \in [m]$, there is a function $l_i\colon \R^n \to \R^{L_i} $, such that $f_i(x,u^i) = (u^i)^Tl_i(x)$, i.e., $f_i$ is linear in the uncertainty and in the decision. Assume that the uncertainty set is $\mathcal{U}^i := [\overline{u}^\overline{u}^i + \Delta u^i
\proof{Proof.}
This follows from Theorem~\ref{Theo:CorrDoNotCare} and Proposition~\ref{Prop:Tractable_Gamma_Comb} by setting $g(x) = x$.
\endproof


%\subsection{Computational complexity}
%In this subsection, we make some remarks about the difficulty of solving $\Gamma$--counterparts.
%%Before we show some computational exampled, we would like to give some
%%thoughts about the computational complexity of
%%$\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart}.
%In the case of a pure combinatorial optimization problem with a linear objective and binary variables under interval uncertainty, the $\Gamma$--counterpart is solvable in oracle-polynomial time with a linear number of oracle calls \cite{IntroGamma}. Thus, if the nominal problem is solvable in polynomial time, this is also the case for the $\Gamma$--counterpart. This also holds in the setting of Theorem~\ref{Theo:PseudoLin}. The same does hold for $\alpha$-approximability: If the nominal problem is $\alpha$-approximable, the problem stays $\alpha$-approximable, see Theorem~\ref{Theo:Approx}. \\
%In the more general concave setting, $
%\supportx{k} $ needs to be determined
%for each $k \in [m]$, i.e., an additional
%optimization problem needs to be solved. This can result in more than linearly many optimization problems: Even in Example~\ref{Ex:Scheduling}, a quadratic number of problems need to be solved, although the problem is a binary, linear optimization problem. \\
%Furthermore, in \cite{RobustScheduling} the authors showed that not only the number of nominal optimization problems in the computationally tractable formulation that can increase not linearly but quadratically, they showed that the complexity class itself can change: Given a single-machine scheduling problem with a finite set of jobs $\mathcal{J}$, they considered the optimization problem
%\begin{gather}\label{Prob:WeightedCompletionTimeScheduling}
%\min_{x \in \mathcal{X}} \sum_{j \in \mathcal{J}} w_jC_j(x,p),
%\end{gather}
%see Example~\ref{Ex:Scheduling}. Problem~\eqref{Prob:WeightedCompletionTimeScheduling} is known to be polynomial because Smith's Rule can be applied \cite{Smith}. \\
%For $w_j = 1 \ \forall j \in \mathcal{J}$, the application of the
%$\Gamma$-flexible approach under uncertain processing times $p_j$
%stays polynomially solvable, while otherwise, solving the $\Gamma$--counterpart of problem~\eqref{Prob:WeightedCompletionTimeScheduling} is an $NP$-hard problem (if
%$\Gamma > 1$, it is strongly $NP$-hard). 
%This demonstrates that in general, the complexity of a combinatorial
%optimization problem under uncorrelated interval uncertainty can
%change for non-linear optimization problems, even if the
%objective is linear in the uncertainty and the decision. This is a crucial difference when compared to the setting of problem~\eqref{Prob:Gamma_Comb}, where the complexity class of the robust problem and the nominal problem are the sam.

\paragraph*{The special case of $0/1$--functions.}
Before we apply our theory in Section~\ref{Sec:Reformulations}, we discuss one more case, namely the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} under linear one--dimensional interval uncertainty with $0/1$--functions:
\begin{assumption}\label{Ass:GeneralLinear01}
For the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} and for all $i \in [m]$ we assume:
\begin{itemize}
\item[(i)] The uncertainty set $\mathcal{U}_i$ is a 1--dimensional interval, i.e., $\mathcal{U}_i = [\overline{u}_i, \overline{u}_i + \Delta u_i] \subseteq \R_{> 0}$ and $\Delta u_i > 0$.
\item[(ii)] There is a $0/1$--function $l_i\colon \mathcal{X} \to \{0,1\}$ such that $f_i(x,u_i) = u_il_i(x)$ for all $u_i \in \mathcal{U}_i$.
\end{itemize}
\end{assumption}
%\begin{align}\label{Prob:Non-LinearBin}
%\min_{x \in \mathcal{X}} u^T l(x)
%\end{align}
%where $u \in \R^n$ is uncertain under interval uncertainty and $l(x) \in \{0,1\}^m$ for all $x \in \mathcal{X}$ and $\mathcal{X} \subseteq \{0,1\}^n$. This is a special case of model~\eqref{Prob:GeneralNomOpt} which is still non-linear since there are no assumptions for $l$ (expect that on $\mathcal{X}$, its image is a subset of $\{0,1\}^m$). 
Although Assumption~\ref{Ass:GeneralLinear01} seems restrictive, it covers many combinatorial programs under uncertainty, e.g. the quadratic knapsack problem or the quadratic matching problem. By applying Proposition~\ref{Prop:Tractable_Gamma_Comb}, we obtain the following:
\begin{theorem}\label{Theo:PseudoLin}
Let $\Gamma \in [m]$ and assume that Assumption~\ref{Ass:GeneralLinear01} holds. Then $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
\begin{gather}\label{Prog:PseudoLin}
\inf_{k \in [m]_0} \left\{ \Gamma \Delta u_k + \inf_{x \in \mathcal{X}} \left\{\overline{u}^Tl(x) + \sum_{j \in [m]} \max\{0,\Delta u_j - \Delta u_k\}l_j(x) \right\} \right\}.
\end{gather}
\end{theorem}
\proof{Proof.}
Under Assumption~\ref{Ass:GeneralLinear01}, program~\eqref{Prob:GeneralNomOpt} is equivalent to $\inf_{(x,y) \in \mathcal{X}_y} u^Ty$ with $\mathcal{X}_y := \mathcal{X} \times l(\mathcal{X}) \subseteq \R^n \times \{0,1\}^{m}$. Then Proposition~\ref{Prop:Tractable_Gamma_Comb} implies that the modified program's $\Gamma$--counterpart is equivalent to
\begin{gather*}
\inf_{k \in [m]_0} \left\{ \Gamma \Delta u_k + \inf_{x \in \mathcal{X}_y} \left\{\overline{u}^Ty + \sum_{j \in [m]} \max\{0,\Delta u_j - \Delta u_k\}y_j \right\} \right\}
\end{gather*}
where $\Delta u_0 := 0$. Since $y_j = l_j(x)$, the claim follows.
\endproof
%Naturally, since we applied Bertsimas' and Sim's original result, assuming that $l(x) \in \{0,1\}^m$ is binary is essential. Therefore, the previous theorem does not cover Examples~\ref{Ex:Scheduling} and \ref{Ex:QAP}. However, it does cover cases where $l_i(x)$ is a product of binary variables for each $i \in [m]$ which is the case for example, quadratic combinatorial optimization problems with objective \begin{gather*}
%\sum_{i \in [n]} p_i x_i + \sum_{i \in [n], j \in [n] \setminus \{i\}} p_{i,j}x_{i}x_{j}
%\end{gather*}
%for binary variables $x_i$ and uncertain coefficients. We demonstrate that in Section~\ref{Sec:Reformulations}.
Theorem~\ref{Theo:PseudoLin} demonstrates that one can solve the $\Gamma$--counterpart with an optimization oracle of program~\eqref{Prob:GeneralNomOpt}. This result only implies that additionally, one can reduce the number of oracle calls one has to solve and can determine $\alpha$-approximations (for $\alpha \geq 1$), if program~\eqref{Prob:GeneralNomOpt} is $\alpha$--approximable (the following definition is not formal and is usually applied for combinatorial programs: Assume that $f^* \in$~$(-\infty,\infty)$ is the optimal value of program~\eqref{Prob:GeneralNomOpt}. Then program~\eqref{Prob:GeneralNomOpt} is called $\alpha$--approximable when there exists a real number $\alpha \geq 1$ and an algorithm $\texttt{ALG}$ with input $(f,\mathcal{X})$, output $\tilde{x}$, the inequality $\alpha f^* \geq f(\tilde{x})$ holds for every instance $(f,\mathcal{X})$ and the running time of algorithm $\texttt{ALG}$ is polynomial in the encoding length of $(f, \mathcal{X})$). The proofs are both heavily inspired by the resp. proofs in \cite{IntroGamma} and \cite{Lee2014}:
\begin{theorem}\label{Theo:Approx}
Let $\Gamma \in [m]$. If Assumption~\ref{Ass:GeneralLinear01} holds and program~\eqref{Prob:GeneralNomOpt} is $\alpha$-approximable, then \eqref{Prob:GeneralGammaCounterpart} is $\alpha$--approximable. 
%equivalent to
%\begin{gather*}
%\min_{k \in \mathcal{L}} \Gamma \Delta u_k + \min_{x \in \mathcal{X}} f(x,\overline{u}) + \sum_{i \in [k]} \left(\Delta u_i - \Delta u_k \right)l_i(x)
%\end{gather*}
%for $\mathcal{L} := \{\Gamma + 1, \dots, \Gamma + \gamma, m + 1\}$ with $\gamma$ being the biggest odd integer smaller than $(m + 1) - \Gamma$ and $\Delta_{m+1}:=0$.
%\end{theorem}
\end{theorem}
\proof{Proof.}
For $k \in [m]_0$, we denote the objective of the $k$--th inner problem of program~\eqref{Prog:PseudoLin} with $G^k(x)$, i.e.,
\begin{gather*}
G^k(x) := \sum_{j \in [m]} (\overline{u}_j + \max\{0,\Delta u_j - \Delta u_k\})l_j(x). 
\end{gather*}
Naturally, one can $\alpha$--approximate program $\inf_{x\in \mathcal{X}} G^k(x)$ for each $k \in [m]_0$ by assumption. Let $x^k$ be the output of the given approximation algorithm with objective value $z^k$ and $Z^*$ be the optimal value of program~\eqref{Prog:PseudoLin}, which is equivalent to $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} since Assumption~\ref{Ass:GeneralLinear01} holds. Then we obtain
\begin{alignat*}{2}
Z^* & \leq \left( \sum_{i \in [m]} l_i(x^k)\overline{u}_i \right) +
\sup_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \sum_{i \in \mathcal{S}}  \Delta u_i l_i(x^k) \\
    & = \left( \sum_{i \in [m]} l_i(x^k)\overline{u}_i \right) + \inf_{\theta \geq 0} \sum_{j \in [m]} \max \{0, \Delta u_i l_i(x^k) -  \theta\} + \Gamma \theta \\
    & \overset{l_i(x^k) \in \{0,1\}}{=} \left(\sum_{i \in [m]} l_i(x^k)\overline{u}_i \right) + \inf_{\theta \geq 0} \sum_{j \in [m]} \max\{0, \Delta u_i  -  \theta \}l_i(x^k) + \Gamma \theta \\
    & \leq \Gamma \Delta u_k + \sum_{i \in [m]} (\overline{u}_i + \max \{0, \Delta u_i  -  \Delta u_k\})l_i(x^k)   \\
    & = \Gamma \Delta u_k + G^k(x^k) \\
    & \leq \alpha(z_k^* - \Gamma \Delta u_k) + \Gamma \Delta u_k \\
    & \overset{\alpha \geq 1}{\leq} \alpha z_k^* \\
    & = \alpha Z^*
\end{alignat*}
which proves the claim since it is sufficient to apply the given $\alpha$--approximation to $\inf_{x\in \mathcal{X}} G^k(x)$ for every $k \in [m]_0$ and to solve $\min_{k \in [m]_0} z_k$.
\endproof
\begin{theorem}\label{Theo:RedNumber}
Let $\Gamma \in [m]$ and assume that $\Delta u_1 \geq \Delta u_2 \geq \dots \geq \Delta u_m \geq 0$. If Assumption~\ref{Ass:GeneralLinear01} holds, then the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
\begin{gather*}
\inf_{k \in \mathcal{L}} \left\{ \Gamma \Delta u_k + \inf_{x \in \mathcal{X}} \left\{ f(x,\overline{u}) + \sum_{i \in [k]} \left(\Delta u_i - \Delta u_k \right)l_i(x) \right\} \right\}
\end{gather*}
for $\mathcal{L} := \{\Gamma + 1, \dots, \Gamma + \gamma, m + 1\}$ with $\gamma$ being the largest odd integer smaller than $(m + 1) - \Gamma$ and $\Delta_{m+1}:=0$. Furthermore, if the optimal value of the $k$--th inner program is smaller than $\Gamma \Delta u_l$ for $l \in \mathcal{L}$, one can replace $\mathcal{L}$ with $\mathcal{L}^* := \{k \in \mathcal{L}: \ k > l\}$.
\end{theorem}
\proof{Proof.}
Since Assumption~\ref{Ass:GeneralLinear01} holds, this statement is a consequence of Theorem 1 in \cite{Lee2014} by introducing binary variables $y_i$, $i \in [m]$, with $y_i = l_i(x)$ (as in the proof of Theorem~\ref{Theo:PseudoLin}).
\endproof
In particular, Theorem~\ref{Theo:RedNumber} implies that, instead of solving $m+1$ nominal programs, one only needs to solve $\lceil \frac{m - \Gamma}{2} \rceil + 1$ subproblems instead of $m+1$, as in the case of Theorem~\ref{Theo:PseudoLin}. \cite{Lee2014} demonstrates that this significantly reduces the number of subproblems one needs to solve for the linear case. %We apply Theorem~\ref{Theo:RedNumber} in our numerical study in Section~\ref{Sec:App}. \\
\\
Before we conclude this section, for the sake of completeness, we note the following: 
\begin{remark}\label{Rem:Concave}
%\begin{enumerate}
%\item[i)] In the setting of Theorem~\ref{Theo:CorrDoNotCare}, one can also show that for the case of $k = 0$, exactly one subproblem needs to be solved, since (in program~\eqref{Model:GammaCounterPartCor}) $x \in \mathcal{X}_\mathcal{Q}$ only holds if and only if
%\begin{alignat*}{2}
%\Delta u_qB_{q,(q,j(q))}g_{q,j(q)}(x)&\geq 0 \ \forall q \in \mathcal{Q},\\
%\Delta u_qB_{q,(q,j(q))}g_{q,j(q)}(x)&\leq 0 \ \forall q \in [m] \setminus \mathcal{Q}
%%% \Delta y_{q,p}g_{q,p}(x) \leq \Delta y_{a,b(a)}g_{a,b(a)}(x) \ %%%\forall (q,p) \in ([m] \times [n]) \setminus \mathcal{Y}.
%\end{alignat*}
%which can only hold for $[m] = \mathcal{Q}$. Since it was not important for our theory, we only mention it here but for the reduction of the number of subproblems, this observation can be crucial. 
With respect to concave uncertainties under Assumption~\ref{Ass:General}, one can show that $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
\begin{alignat}{2}\label{Reform:Concave}
\min_{k \in [m]_0} & \left\{ \min_{\substack{x \in \mathcal{X}, v^1 \in \R^{L_1}, \\  \dots, v^m \in \R^{L_m}}} \left\{ \Gamma \theta^k(x,v^k) + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, \theta^i(x,v^i)- \theta^k(x,v^k) \} \right\} \right\}
\end{alignat}
where
\begin{gather*}
\theta^k(x,v^k) := (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k)  \ \forall k \in [m].
\end{gather*}
In this context, however, it seems unlikely that one would use this formulation over the one given in Corollary~\ref{Prop:FenchelGammaCounterpart} since the objective is very different from the one of program~\eqref{Prob:GeneralNomOpt}, the feasible set was altered, rendering oracles not applicable.
\end{remark}


\section{Practical examples}\label{Sec:Reformulations}
In this section, we demonstrate some examples of the reformulations of Section~\ref{sec:Rev}. We note that some are maximization programs for which our theory naturally applies as well.
%\begin{example}
%We consider an optimization problem with a quadratic objective:
%\begin{align}\label{Prob:NomQuad}
%\min_{x \in \mathcal{X}} \sum_{i \in [m]} (x_i - u_i)^2.
%\end{align}
%For every $i \in [m]$, $u_i$ is subject to uncertainty $\mathcal{U}_i := [\overline{u}_i, \overline{u}_i + \Delta u_i]$. For $\Gamma \in [m]$, the $\Gamma$--counterpart of model~\eqref{Prob:NomQuad} after applying Lemma~\ref{Lem:ReModel} is given by
%\begin{align}\label{Prob:FirstQuad}
%\begin{split}
%\min_{x, p, \theta} & \ \Gamma \theta + \sum_{i \in [m]} (x_i - \overline{u}_i)^2 + p_i, \\
%\mathrm{s.t.} & \ x \in \mathcal{X}, \\
%& (x_i - u_i)^2 - (x_i - \overline{u}_i)^2 \leq p_i + \theta \ \forall u_i \in \mathcal{U}_i, \ \forall i \in [m].
%\end{split}
%\end{align}
%The inequalities of model~\eqref{Prob:FirstQuad} are equivalent to
%\begin{gather}\label{Ineq:ReformedQuad}
%-2x_i u_i + u_i^2 \leq p_i + \theta - 2x_i \overline{u}_i + \overline{u}_i^2 \ \forall u_i \in \mathcal{U}_i
%\end{gather}
%for each $i \in [m]$. The left-hand side of \eqref{Ineq:ReformedQuad} is not concave in $u_i$ and thus, we cannot apply the reformulations of Subsection~\ref{subsec:Concave}. However, \eqref{Ineq:ReformedQuad} is of the form \eqref{Ineq:SecondApproach}. We set
%\begin{gather*}
%g_1(x) = -2x, \ g_2(x) = 1, \ h(u_i) = u_i^2
%\end{gather*}
%and re-write the uncertainty set:
%\begin{gather*}
%[\overline{u}_i, \overline{u}_i + \Delta u_i] = \{u_i \in \R\colon (-2 \overline{u}_i - \Delta u_i)u_i + u_i^2 \leq -\overline{u}_i^2 - \overline{u}_i \cdot \Delta u_i\}.
%\end{gather*}
%Inequality~\eqref{Ineq:SecondApproach} is obtained by setting
%\begin{gather*}
%\alpha = -2\overline{u}_i - \Delta u_i, \ \beta = 1, \ \gamma = -\overline{u}_i^2 - \overline{u}_i \Delta u_i. \
%\end{gather*}
%Since $\alpha$ and $\beta$ are scalars, they are clearly term-wise parallel. Thus, we can set $b_i:=h(u_i):= u_i^2$ and \eqref{Ineq:ReformedQuad} is satisfied for $(x, p, \theta)$ if and only if there exists $v \in \R$, such that
%\begin{align*}
%&(1 + v)h_i^*\left(\frac{2x + 2 \overline{u}_iv + \Delta u_iv}{1+v}\right) - \overline{u}_i^2v - \overline{u}_iv \Delta u_iv \le p_i + \theta -2x_i \overline{u}_i + \overline{u}_i^2,\\
%&1 + v \ge 0,\\
%&v\ge 0.
%\end{align*}
%Clearly, the second inequality is redundant. Furthermore, since
%$h_i^*(z) = \frac{z^2}{4}$, the first inequality is convex in $(x,v)$ if it is assumed that $x \geq 0$. This is a valid assumption for many problems, for example in logistics. Thus, assuming that $\mathcal{X}$ is a convex set, the $\Gamma$--counterpart of problem~\eqref{Prob:NomQuad} is a convex optimization problem, although it is not concave in the uncertainty.
%\end{example}
\paragraph*{Linear programs under uncertainty.}
Here, we cover the case of $\min_{x \in \mathcal{X}} u^TBx$. If $B$ is the unit matrix and $u$ is subject to interval uncertainty, we obtain the original setting of Bertsimas and Sim. We have already shown with Corollary~\ref{Cor:LPsAssigment} that there is a case where one can 'shift' $B$ into the uncertainty set and that one can solve the $\Gamma$--counterpart with a polynomial number of oracle calls. This is a generalization of a result in \cite{RobustScheduling} which has been applied to the single--machine scheduling problem under uncertainty:
%\begin{corollary}\label{Cor:LPsAssigment}
%Consider the optimization problem \begin{gather}\label{Prob:nom_LP_under_unc:ASSIGN}
%\min_{x \in \mathcal{X}} u^TBx
%\end{gather}
%as in the setting of Theorem~\ref{Theo:CorrDoNotCare} and assume that $
%\mathcal{X} \subseteq \{x \in \{0,1\}^{[m] \times [n]}: \sum_{j \in [n]} x_{i,j} = 1 \ \forall i \in [m]\}$.
%Let $\Gamma \in [m]$. Then the $\Gamma$--counterpart of \eqref{Prob:nom_LP_under_unc:ASSIGN} is equivalent to
%\begin{align*}
%\min_{(k,l) \in [m] \times [n] \cup \{(0,0)\}}  \Gamma \Delta u_k B_{k,(k,l)}+ 
%\min_{x \in \mathcal{X}} \overline{u}^TBx + \sum_{(i,j) \in [m] \times [n]} \max\{0, \Delta u_i B_{i,(i,j)} - \Delta u_k B_{k,(k,l)}\}x_{i,j},
%\end{align*}
%where $B_{0,.} := \Delta u_0 := 0$.
%\end{corollary}
%%\begin{align*} %\label{Prob:RobustCounterpartSuperComb}
%%\begin{split}
%%\min_{\substack{(k,l) \in [m] \times [n] \\ \lor k = l = 0 }} \left\{\Gamma \Delta u^T B_{.,(k,l)} + 
%% \min_{x \in \mathcal{X}}  \overline{u}^TBx + \sum_{(i,j) \in [m] \times [n]} \max \left\{0,\Delta u^T\left( B_{.,(i,j)} - B_{.,(k,l)}\right)\right\}x_{i,j} \right\}.
%%\end{split} 
%%\end{align*}
%%$\min_{x Assume that for all $i \in [m]$, there is a function $l_i\colon \R^n \to \R^{L_i} $, such that $f_i(x,u^i) = (u^i)^Tl_i(x)$, i.e., $f_i$ is linear in the uncertainty and in the decision. Assume that the uncertainty set is $\mathcal{U}^i := [\overline{u}^\overline{u}^i + \Delta u^i
%\proof{Proof.}
%This follows from Theorem~\ref{Theo:CorrDoNotCare} and Proposition~\ref{Prop:Tractable_Gamma_Comb} by setting $g(x) = x$.
%\endproof
%Now, regarding Example~\ref{Ex:Scheduling}, one can apply Corollary~\ref{Cor:LPsAssigment}:
%Corollary~\ref{Cor:LPsAssigment} 
\begin{example}\label{Ex:SchedulingGeneral}
We recall that in Section~\ref{sec:Rev}, we considered an instance of the program %problems of the form
\begin{align}\label{Prob:NomScheduling}
\begin{split}
\min_{x} & \ \sum_{i,j \in \mathcal{I}, \mathcal{J}} u_i q_j x_{i,j}, \\
\mathrm{s.t.} & \ x \in \mathcal{X} \subseteq \left\{x \in \{0,1\}^{|\mathcal{I}|\cdot|\mathcal{J}|}:
\sum_{j \in \mathcal{J}} x_{i,j} = 1 \ \forall i \in \mathcal{I}\right\}
\end{split}
\end{align}
where $u_i$ is subject to uncertainty $[\overline{u}_i, \overline{u}_i + \Delta u_i]$ in the context of single--machine scheduling. By applying Corollary~\ref{Cor:LPsAssigment}, one can show that the $\Gamma$--counterpart of program~\eqref{Prob:NomScheduling} is equivalent to taking the minimum of
\begin{align*}
\min_{(k,l) \in \mathcal{I} \times \mathcal{J}} \left\{ \Gamma q_k \Delta u_l + \min_{x \in \mathcal{X}} \left\{ \sum_{i,j \in \mathcal{I}, \mathcal{J}} (\overline{u}_i + \max\{0, \Delta u_i - \frac{\Delta u_k q_l}{q_j}\})q_jx_{i,j} \right\} \right\}
\end{align*}
and 
\begin{align*}
\min_{x \in \mathcal{X}} \sum_{i,j \in \mathcal{I}, \mathcal{J}} (\overline{u}_i + \Delta u_i)q_jx_{i,j}.
\end{align*}
In \cite{RobustScheduling}, this has been shown by algebraic means.
%This was established through algebraic manipulations and reformulations which were used to prove
%Proposition~\ref{Prop:Tractable_Gamma_Comb}. We establish the same result through Corollary~\ref{Cor:LPsAssigment}: By setting
%\begin{gather*}
%B:= \begin{pmatrix}
%q_1   \dots q_{|\mathcal{J}|} & 0_{\mathcal{J}} & \dots & 0_{\mathcal{J}} \\
%0_{\mathcal{J}} & q_1   \dots q_{|\mathcal{J}|} & 0_{\mathcal{J}} \dots & 0_{\mathcal{J}} \\
%\vdots & \vdots & \vdots & \vdots \\
%0_{\mathcal{J}} & 0_{\mathcal{J}} & 0_{\mathcal{J}} & q_1   \dots q_{|\mathcal{J}|} 
%\end{pmatrix} \in \R^{|\mathcal{I}| \times |\mathcal{I}| |\mathcal{J}|},
%\end{gather*}
%and inserting this into~\eqref{Prob:RobustCounterpartSuperComb}, we obtain the same reformulation.
\end{example}

\paragraph*{Quadratic programs under uncertainty.}
As an application of Corollary~\ref{Cor:LinInt}, we reformulate the QAP under uncertainty given in Section~\ref{sec:Rev}. 
\begin{example}\label{ex:QAP_genau}
We consider the QAP under interval uncertainty
\begin{align}\label{Prob:QAP_Nom}
\begin{split}
\min_{x} & \ \sum_{(i,j,r,s) \in [n]^4} c_{i,j}d_{r,s}x_{i,r}x_{j,s} \\
\mathrm{s.t.} & \ x \in \mathcal{X} = \{x \in \{0,1\}^{[n]^2}: \sum_{i \in [n]} x_{i,r} = 1 \ \forall r \in [n], \ \sum_{r \in [n]} x_{i,r} = 1 \ \forall i \in [n]\}
\end{split}
\end{align}
with uncertain coefficients $c_{i,j} \in \mathcal{U}_{i,j} := [\overline{c}_{i,j}, \overline{c}_{i,j} + \Delta c_{i,j}] \subseteq \R_{\geq 0}$ for all $i,j \in [n]$ and $d_{r,s} \geq 0$ for all $r,s \in [n]$. Let $\Gamma \in [n^2]$.
The objective of ~\eqref{Prob:QAP_Nom} equals $u^TBg(x)$ where $B \in \R^{n^2 \times n^4}$ is a block diagonal matrix with $n^2$ copies of $d^T$, $u = c$ and $g_{(i,j),(r,s)}(x):= x_{i,r}x_{j,s}
$ for $(i,j,r,s) \in [n]^4$. Then Theorem~\ref{Theo:CorrDoNotCare} implies that the $\Gamma$--counterpart of program~\eqref{Prob:QAP_Nom} is equivalent to the $\Gamma$--counterpart of
\begin{gather*}
\min_{x \in \mathcal{X}} y^Tg(x)
\end{gather*}
with $y \in \R^{n^4}$ being subject to interval uncertainty, in particular $y_{i,j,r,s} \in [\overline{c}_{i,j}d_{r,s}, (\overline{c}_{i,j} + \Delta c_{i,j})d_{r,s}]$ for $i,j,r,s \in [n]$. Now, we can apply Theorem~\ref{Theo:PseudoLin} and we obtain the reformulation
%\begin{align}\label{Prob:QAP_Reform_One}
%\min_{(k_1,k_2,k_3,k_4) \in [n]^4 \cup \{(0,0,0,0)\}} & \min_{x \in \mathcal{X}} \Gamma \Delta (\overline{c}_{k_1,k_2} + \Delta c_{k_1,k_2})d_{k_3,k_4} x_{k_1,k_3}x_{k_2,k_4} + \sum_{(i,j) \in [n]^2} \overline{c}_{i,j}d_{r,s}x_{i,r}x_{j,s} + \max \{0, \Delta {c}_{i,j}d_{r,s}x_{i,r}x_{j,s} - \Delta c_{k_1,k_2}d_{k_3,k_4} x_{k_1,k_3}x_{k_2,k_4} \}
%\end{align}
%where $\bar{c}_{0,0} := \Delta c_{0, 0} := d_{0,0} := x_{0,0} = 0$. We assume that $x_{k_1,k_3}x_{k_2,k_4} = 1$ for $(k_1,k_2,k_3,k_4)\in [n]^4$ (otherwise the term would be $0$ and we would be in the case $k_i = 0$ for $i \in [4]$). Then, 
%\begin{alignat*}{2}
%\max \{0, \Delta {c}_{i,j}d_{r,s}x_{i,r}x_{j,s} - \Delta c_{k_1,k_2}d_{k_3,k_4} x_{k_1,k_3}x_{k_2,k_4} \} &= 
%\max \{0, \Delta {c}_{i,j}d_{r,s}x_{i,r}x_{j,s} - \Delta c_{k_1,k_2}d_{k_3,k_4}  \} =  \\
%&=\max \{0, \Delta {c}_{i,j}d_{r,s} - \Delta c_{k_1,k_2}d_{k_3,k_4}\}x_{i,r}x_{j,s},
%\end{alignat*} 
%since all involved numbers are non-negative. 
%
%Thus, problem~\eqref{Prob:QAP_Reform_One} is equivalent to
\begin{align}\label{Prob:QAP_Reform_Two}
\min_{\substack{(k_1,k_2,k_3,k_4) \in [n]^4 \\ \cup \{(0,0,0,0)\}}} & \left\{ \Gamma (\Delta c_{k_1,k_2})d_{k_3,k_4} + \min_{x \in \mathcal{X}} \left\{ F_{k_1,k_2,k_3,k_4}(x) \right\} \right\}
\end{align}
where 
\begin{gather*}
F_{k_1,k_2,k_3,k_4}(x) = \sum_{(i,j,r,s) \in [n]^4} (\overline{c}_{i,j}d_{r,s} + \max \{0, \Delta {c}_{i,j} d_{r,s} - \Delta c_{k_1,k_2}d_{k_3,k_4} \})x_{i,r}x_{j,s} 
\end{gather*}
for $(k_1,k_2,k_3,k_4) \in [n]^4$, $F_{0,0,0,0}(x) := \sum_{(i,j,r,s) \in [n]^4}  (\overline{c}_{i,j}d_{r,s} + \Delta {c}_{i,j} d_{r,s})x_{i,r}x_{j,s}$, and $\Delta c_{0,0} := d_{0,0} := 0$.
%\begin{align}\label{Prob:QAP_Reform_Two}
%\min_{(k_1,k_2,k_3,k_4) \in [n]^4 \cup \{(0,0,0,0)\}} & \Gamma (\Delta c_{k_1,k_2})d_{k_3,k_4} + \min_{x \in \mathcal{X}, \ x_{k_1 k_3} x_{k_2 k_4} = 1} \sum_{(i,j,r,s) \in [n]^4} (\overline{c}_{i,j}d_{r,s} + \max \{0, \Delta {c}_{i,j} d_{r,s} - \Delta c_{k_1,k_2}d_{k_3,k_4} \})x_{i,r}x_{j,s}.
%\end{align}
%%%Since $x_{k_1 k_3} x_{k_2 k_4} = 1$ is equivalent to $x_{k_1 k_3} = x_{k_2 k_4}= 1$, facilities $k_1$ and $k_2$ are assigned to locations $k_3$ and $k_4$, respectively. Thus, the variables $x_{k_1 j}$, $x_{k_2 j}$, $x_{i k_3}$ and $x_{i k_4}$ are fixed for all $j \in [n]$ and we can neglect those variables. Thus, we can replace the feasible set with 
%%%\begin{gather*}
%%%\mathcal{X}_{k_1,k_2,k_3,k_4} := \left\{x \in \{0,1\}^{[n]_{\setminus k_1,k_2} \times [n]_{\setminus k_3,k_4}}: \ \sum_{i \in [n]_{\setminus k_1,k_2}} x_{i,r} = 1 \ \forall r \in [n]_{\setminus k_3,k_4}, \ \sum_{r \in [n]_{\setminus k_3,k_4}} x_{i,r} = 1 \ \forall i \in [n]_{\setminus k_1,k_2} \right\}.
%%%%\begin{gather*}
%%%%\tilde{\mathcal{X}} := \left\{ x \in \{0,1\}^{([n]\setminus \{k_1,k_2\}) \times ([n] \setminus \{k_3,k_4\})}: \ \sum_{i \in [n]\setminus \{k_1,k_2\}} x_{i,r} = 1 \ \forall r \in [n] \setminus \{k_3,k_4\}, \ \sum_{r \in [n]\setminus \{k_3,k_4\}} x_{i,r} = 1 \ \forall i \in [n] \setminus \{k_1,k_2\} \right\}. 
%%%%
%%%\end{gather*} 
%The inner problems are infeasible, if exactly one of the equations $k_1 = k_2$ or $k_3 = k_4$ holds (for $k_1,k_2,k_3,k_4 \in [n]$). 
If we assume that the flow and the distance coefficients are symmetrical, i.e., $\Delta c_{i,j} = \Delta c_{j,i}$ and $d_{r,s} = d_{s,r}$ for all $i,j,r,s \in [n]$, then we only have to solve inner problems of the set
\begin{gather*}
\mathcal{M}:=\{(k_1,k_2,k_3,k_4) \in [n]^4: \ k_1 < k_2, k_3 < k_4\} \cup \{(0,0,0,0)\}.
\end{gather*}
Thus, one needs to solve $1 + (\frac{n(n-1)}{2})^2 = \frac{n^4 - n^3}{2} + 1$ QAPs to solve program~\eqref{Prob:QAP_Reform_Two}.
%, in particular
%\begin{align}\label{Prob:QAP_Reform_Three}
%\min_{(k_1,k_2,k_3,k_4) \in \mathcal{M}} & \Gamma (\Delta c_{k_1,k_2})d_{k_3,k_4}  + \min_{x \in \mathcal{X}} \sum_{(i,j,r,s) \in [n]^4} (\overline{c}_{i,j}d_{r,s} + \max \{0, \Delta {c}_{i,j} d_{r,s} - \Delta c_{k_1,k_2} d_{k_3,k_4} \})x_{i,r}x_{j,s}.
%\end{align}
By application of Theorem~\ref{Theo:RedNumber}, we can reduce the number of subproblems to $\lceil \frac{n^4 - n^3}{4}  + \frac12 - \frac{\Gamma}{2} \rceil + 1$. In our electronic companion, we demonstrate how the application of Theorem~\ref{Theo:RedNumber} significantly speeds up the the optimization process.
%Furthermore, since $d_{r,s}$ is the distance between locations $r$ and $s$, $d_{r,s} = d_{s,r}$  for all $r,s \in [n]$.  Thus, we only have to consider already covered by the cases in $\mathcal{M}_1:=\{(i,j,r,s) \in [n]^4: r < s \}$. Similarly, the flows are symmetrical in the sense that $\Delta u_{i,j} = \Delta u_{j,i}$ and it is sufficient to cover the cases in $\mathcal{M}_2:= \{(i,j,r,s) \in [n]^4: i \leq j \}$. Finally, $\Delta c_{i,i} = 0 = d_{i,i}$ for $i \in [n]$ (since there is no flow from a facility to itself) and these cases are covered by $(k_1,k_2,k_3,k_4) = (0,0,0,0)$. With $\mathcal{M}_3:= \{(i,j,r,s) \in [n]^4: i \neq j \land r \neq s\}$, one finally obtains the following scenarios:
%\begin{gather*}
%\mathcal{M} := \mathcal{M}_1  \cap \mathcal{M}_2 \cap \mathcal{M}_3 = \{(i,j,r,s) \in [n]^4: i < j, \ r < s\}
%\end{gather*}
%and $(k_1,k_2,k_3,k_4) = (0,0,0,0)$ -- thus, one needs to solve $n^4 + 1$ nominal problems.
%
%\todo[inline][inline]{Fehler??}
%%If we take the definition of the QAP into account, i.e., $d_{r,r} = 0$ for $r \in [n]$ and $d_{r,s} = d_{s,r}$ for $r,s \in [n]$, we can neglect the cases of $k_3=k_4$ and need to solve $1 + n^4 - n^2(\frac{n(n+1)}{2}) = n^4 - \frac{n^4 + n^3}{2} + 1 = \frac{n^4 - n^3}{2} + 1$  QAPs without uncertainty in \eqref{Prob:QAP_Reform_Two}.
%%the minimum 
%  A QAP with uncertain flow coefficients under interval uncertainty  has been solved by linearizing the non-linearities and applying the original results of Bertsimas and Sim. We aim to apply Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear}  and set
%\begin{gather*}
%f_{k_1k_2}(x,c_{k_1k_2})= c_{k_1k_2} \sum_{(r,s)\in [n]^2} d_{rs}x_{k_1r}x_{k_2s} =: c_{k_1k_2}l_{k_1k_2}(x) \ \forall k_1, k_2 \in [n],
%\end{gather*}
%with the interval uncertainty set $
%\mathcal{U}_{k_1k_2} := [\overline{c}_{k_1k_2}, \overline{c}_{k_1k_2} + \Delta c_{k_1k_2}]$ for all $k_1, k_2 \in [n]$, and recall that $\mathcal{X} = \{x \in \{0,1\}^{[n]^2}: \sum_{i \in [n]} x_{ir} = 1 \ \forall r \in [n], \ \sum_{r \in [n]} x_{ir} = 1 \ \forall i \in [n]\}$.

%\begin{align}\label{Prob:QAPRC}
%\begin{split}
%&\min_{x\in \mathcal{X}}  \max_{\mathcal{S} \subseteq [n]^2: |\mathcal{S}| \le \Gamma} %\left\{ \sum_{(i,j)\in \mathcal{S}}^n \max_{c_{ij}\in \mathcal{U}_{ij}} \sum_{(r,s)\in [n]^2} c_{ij} d_{rs}x_{ir}x_{js} + \sum_{(i,j) \in [n]^2 \setminus \mathcal{S}} \sum_{(r,s)\in [n]^2} \bar{c}_{ij} d_{rs}x_{ir}x_{js} \right\} 
%\end{split}
%\end{align} 
%\[\mathcal{U}_{ij}= [\bar{c}_{ij}, \bar{c}_{ij}+ \Delta c_{ij}], \quad \forall (i,j) \in [n]^2.\]
%By application of Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear}: 
%\[\bar{u}_{k_1k_2} = \bar{c}_{k_1k_2}, \quad l_{k_1k_2}(x)= \sum_{(r,s)\in [n]^2} d_{rs}x_{k_1r}x_{k_2s}\] and
%\[f_{k_1k_2}(x,c_{k_1k_2}) = c_{k_1k_2}\sum_{(r,s)\in [n]^2} d_{rs} x_{k_1r}x_{k_2s}\]with $ (k_1,k_2)\in [n]^2$. The uncertainty set can be expressed as box uncertainty 
%\[\mathcal{U}_{k_1k_2} = \left\{ c_{k_1k_2}|c_{k_1k_2} = \bar{c}_{k_1k_2} + \alpha \Delta c_{k_1k_2}, \alpha \in \mathcal{Z}_{k_1k_2} \right\}\]  with $\mathcal{Z}_{k_1k_2}=[0,1]$.  
%We apply
%reformulation~\eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear},
%which implies that \eqref{Prob:QAP_RobCP} is equivalent to the minimum
%of
%\[\theta_{k_1k_2}(x) = \delta^*(\Delta c_{k_1k_2} l_{k_1k_2}(x)|\mathcal{Z}_{k_1k_2})= \Delta c_{k_1k_2}\sum_{(r,s)\in [n]^2} d_{rs}x_{k_1r}x_{k_2s} = f_{k_1k_2}(x,\Delta c_{k_1k_2}) \ \forall k_1,k_2 \in [n]\]
%and $\theta_{0,0}(x)=0$,
%the reformulation of $\Gamma$--counterpart~\eqref{Prob:QAP_RobCP} is given by the minimum of
%\begin{align}\label{Prob:QAP_Gen}
%\begin{split}
%&\min_{ k_1,k_2 \in [n]} \min_{x\in \mathcal{X}} \ \Gamma \sum_{r,s \in [n]} d_{rs}\Delta c_{k_1 k_2}x_{k_1r}x_{k_2s} +\\
% & \sum_{i,j\in [n]} \left(\sum_{r,s\in [n]} \bar{c}_{ij}d_{rs}x_{ir}x_{js} + \max\left\{0, \sum_{r,s\in [n]} d_{rs}\left(\Delta c_{ij} x_{ir}x_{js}-\Delta c_{k_1 k_2} x_{k_1r}x_{k_2s}\right)\right\}\right)
% \end{split}
%\end{align}
%%\begin{align}\label{Prob:QAP_Gen}
%%\min_{ (k_1,k_2) \in [n]^2} \min_{x\in \mathcal{X}} \Gamma f_{k_1k_2}(x,\Delta c_{k_1k_2}) 
%%+ \sum_{(i,j)\in [n]^2} \left(f_{k_1k_2}(x, \overline{c}_{ij})+ \max\left\{0, f_{ij}(x, \Delta c_{i,j}) -f_{k_1k_2}(x, \Delta c_{k_1k_2})\right\}\right).
%%\end{align}
%and
%\begin{align}\label{Prob:thetanull}
%\min_{x\in\mathcal{X}} \sum_{i,j\in [n]} \sum_{r,s \in [n]} ( c_{ij} + \Delta c_{ij})d_{rs} x_{ir}x_{js}.
%\end{align}
%%\begin{align*}
%%\min_{x\in \mathcal{X}} 
%%\sum_{(i,j)\in [n]^2} f_{k_1k_2}(x, \overline{c}_{ij})+ f_{i,j}(x, \Delta c_{i,j}).
%%\end{align*}
%Since the inner minimization problems of model~\eqref{Prob:QAP_Gen} are not QAPs, we reformulate the objective: As $x \in \mathcal{X}$,
%the equation $\sum_{s \in [n]} x_{js} = 1$ holds for all $j \in [n]$. We obtain
%%since
%%\[\theta_{k_1k_2}(x) = \delta^*(\Delta c_{k_1k_2} l_{k_1k_2}(x)|\mathcal{Z}_{k_1k_2})= \Delta c_{k_1k_2}\sum_{(r,s)\in [n]^2} d_{rs}x_{k_1r}x_{k_2s} = f_{k_1k_2}(x,\Delta c_{k_1k_2})\]
%%and $\theta_0(x)=0$.
%%$x_{\theta}$ is the $x\in \mathcal{X}$ minimal for $\theta$. The optimal solution of \eqref{Prob:QAP_RobCP} is the minimum of all $(\theta, x_{\theta})$. Therefore, we reformulate the objective as
%%The inner minimization-problem is not a quadratic assignment problem due to the maximum in the objective. To keep the structure of a QAP we have to reformulate the objective:\\
%\begin{align}\label{Prob:OneSum}
%\sum_{r\in[n]} \sum_{s\in[n]} x_{ir}x_{js}= \sum_{r\in[n]} x_{ir} \sum_{s \in [n]} x_{js} =1 \ \forall i,j \in [n].
%\end{align} 
%Therefore, $x_{k_1r}x_{k_2s} = 1 $ for exactly one pair $(r,s)\in
%[n]^2$  for every $k_1,k_2\in [n]$, i.e., $x_{k_1r}x_{k_2s} = 1$
%only holds in exactly one case. Thus, instead of optimizing over
%$(k_1,k_2) \in [n]^2 $ in model~\eqref{Prob:QAP_Gen}, we optimize over
%$(k_1, k_2, k_3, k_4) \in [n]^4$ to fix all indices of
%$c_{k_1k_2}d_{k_3k_4}$. Then, model~\eqref{Prob:QAP_Gen} is equivalent to
%\begin{align*}
%\begin{split}
%&\min_{ k_1,k_2,k_3,k_4 \in [n]}\ \Gamma \Delta c_{k_1 k_2} d_{k_3 k_4} + \\
% & \min_{x \in \mathcal{X}} \sum_{i,j,r,s \in [n]}  d_{rs}c_{ij}x_{ir}x_{js} + \max \left\{0, \left( \sum_{r,s \in [n]} d_{rs}\Delta c_{ij} x_{ir}x_{js} \right)-\Delta c_{k_1 k_2} d_{k_3 k_4} \right\}.
% \end{split}
%\end{align*}
%
%%We note, that in our setting for all $r\in [n]$ the distance between a location and itself equals 0. Hence, $d_{rr}c_{ij}x_{ir}x_{jr} = 0$ for $(i,j)\in [n]^2$ due to $d_{rr}=0$. To avoid later division by zero we only sum up factors with $d_{rs}\neq 0$ e.g. $r \neq s$. 
%%Then, the inner optimization problem of Problem~\eqref{Prob:QAP_Gen} is equivalent to:
%% \[\min_{x \in \mathcal{X}} \sum_{(i,j)\in [n]^2} \sum_{(r,s)\in [n]^2, r \neq s} d_{rs}c_{ij}x_{ir}x_{js} + \max \left\{0, \sum_{(r,s)\in [n]^2, r \neq s} d_{rs}\left(\Delta c_{ij} x_{ir}x_{js}\right)-\Delta c_{k_1 k_2} d_{k_3 k_4} \right\}.\]
%%To omit the decision variable in the maximum we reformulate:
%We note here, that we do not demand $x_{k_1k_3}x_{k_2k_4} = 1 $ within the feasible set. If this equation is not fulfilled, there is another tuple $(\bar{k}_1,\bar{k}_2,\bar{k}_3,\bar{k}_4)$ with a higher objective for the same $x$, since for a fixed $x$ the objective is piecewise linear in $\Delta c_{k_1 k_2} d_{k_3 k_4}$ and the optimal $\Delta c_{k_1 k_2} d_{k_3 k_4}$ is always met if $x_{k_1k_3}x_{k_2k_4}=1$ for the optimal $x$ (since those are the changepoints of the objective). Thus, if we minimize over all tuple $(i,j,r,s)\in [n]^4$ an infeasible solution can not be optimal. 
%Since $d_{r,s}$ denotes the distance between two locations $r$ and $s$, we can assume $d_{rr} = 0$ for all $r \in [n]$ and $d_{rs} > 0$ for $r \neq s$. Hence
%\begin{align*}
%\begin{split}
%\max & \left\{0, \sum_{ r,s \in [n]} \Delta c_{ij} d_{rs} x_{ir}x_{js}-\Delta c_{k_1 k_2} d_{k_3 k_4}\right\}\overset{(*)}{=}\\
%\max& \left\{0, \left(\sum_{r,s \in [n], r \neq s} d_{rs} x_{ir}x_{js}\right) \left(\Delta c_{ij}-\frac{\Delta c_{k_1 k_2} d_{k_3 k_4}}{ \sum_{r,s\in [n], r \neq s} d_{rs} x_{ir}x_{js}}\right)\right\} \overset{x \in \mathcal{X}}{=}\\
%\max &\left\{0, \Delta c_{ij}-\frac{\Delta c_{k_1 k_2} d_{k_3 k_4}}{d_{rs}}\right\}d_{rs} x_{ir}x_{js}.
%\end{split}
%\end{align*}
%In $(*)$ we factorized $\sum_{r,s \in [n], r \neq s} d_{rs}x_{ir}x_{js}$ for a better understanding of the next reformulation.
%%We apply equality~\eqref{Prob:OneSum} to remove the sum from the maximum and obtain as equivalent reformulation for the inner optimization problem of \eqref{Prob:QAP_Gen}:
%%\[\Gamma \left( d_{k_3 k_4}\Delta c_{k_1 k_2}\right) +
%% \min_{x \in \mathcal{X}}\sum_{(i,j,r, s)\in [n]^4, r \neq s} d_{rs}c_{ij}x_{ir}x_{js} + \max\left\{0,\Delta c_{ij}-\frac{\Delta c_{k_1 k_2} d_{k_3 k_4}}{d_{rs}}\right\}d_{rs}x_{ir}x_{js}.\]
%%We obtain
%%\[\max\left\{0, \sum_{(r,s)\in [n]^2} \underbrace{d_{rs} x_{ir}x_{js} \Delta c_{ij}}_{\ge 0}\right\}= \sum_{(r,s)\in [n]^2} d_{rs} x_{ir}x_{js} \Delta c_{ij}\]
%%for $\theta_0(x) =0$.
%In sum, solving the robust counterpart \eqref{Prob:QAP_RobCP} is equivalent to 
%determining the minimum of
%\begin{align}\label{Prob:thetanichtnull}
%\begin{split}
%&\min_{ (k_1,k_2,k_3,k_4)\in [n]^4} \Gamma \left( \Delta c_{k_1 k_2}d_{k_3 k_4}\right) + \\
%& \min_{x\in \mathcal{X}} 
% \sum_{(i,j)\in [n]^2} \sum_{(r,s)\in [n]^2, r \neq s} d_{rs}\left(c_{ij} + \max\left\{0,\Delta c_{ij}-\frac{\Delta c_{k_1 k_2} d_{k_3 k_4}}{d_{rs}}\right\}\right)x_{ir}x_{js}
%\end{split}
%\end{align}
%and model~\eqref{Prob:thetanull}. This means that the robust
%counterpart can be solved by determining the minimum of $n^4 + 1$
%nominal QAPs. 
%\begin{align}\label{Prob:thetanull}
%\min_{x\in\mathcal{X}} \sum_{(i,j)\in [n]^2} \sum_{(r,s)\in [n]^2} d_{rs} x_{ir}x_{js}( c_{ij} + \Delta c_{ij}).
%\end{align}
%The inner optimization problem of \eqref{Prob:thetanichtnull} and
%\eqref{Prob:thetanull} are both QAPs again. Hence, obtaining an optimal
%solution of Problem~\eqref{Prob:QAP_RobCP} can be achieved by solving
%$\mathcal{O}(n^4)$ QAPs and taking the minimum of the objective values. Therefore, with our reformulation it is possible to keep the structure of the nominal Problem. We therefore denote that reformulation $QAP$.\\
\end{example}


%\begin{remark}\label{Rem:QAPLinearizations}
%In Example~\ref{ex:QAP_genau}, we established models~\eqref{Prob:thetanull} and \eqref{Prob:thetanichtnull} as a valid reformulation without uncertainty of the $\Gamma$--counterpart of a QAP under flow uncertainty. It is not by chance that the proof structure of Theorem~\ref{Theo:CorrDoNotCare} and the determination of  reformulation~\eqref{Prob:thetanull} are similar: Theorem~\ref{Theo:CorrDoNotCare} implies that the $\Gamma$--counterpart of the QAP~\eqref{Prob:QAP_RobCP} and the $\Gamma$--counterpart of
%\begin{gather}\label{Model:AlmostLinQAP}
%\min_{x \in \mathcal{X}} \sum_{i,j,r,s \in [n]} y_{ijrs} x_{ij} x_{rs} 
%\end{gather}
%with uncertain coefficients $y_{ijrs} \in \mathcal{Y}^{ijrs} := [\overline{c}_{ij} d_{rs}, \overline{c}_{ij} d_{rs} + \Delta c_{ij} d_{rs}]$ are equivalent. In terms of application, this results in another tool to solve the $\Gamma$--counterpart: By linearizing $x_{ij}x_{rs}$ in \eqref{Model:AlmostLinQAP}, we obtain the original setting of Bertsimas and Sim, i.e., \eqref{Prob:Gamma_Comb}, and can apply Propositions~\ref{Prop:Tractable_Gamma_Comb} or \ref{Prop:Gamma_MIP} and apply techniques for solving MIPs. There are already studies addressing how to solve the $\Gamma$--counterpart of a QAP with these linearized models, we refer the reader to \citep{QAP2015} and \cite{QAP_lin}. In Section~\ref{Sec:App}, we compare these linearized models (applying standard linearizations) with our new reformulation~\eqref{Prob:thetanull} and \eqref{Prob:thetanichtnull}. 
%\end{remark}
%By applying Theorem~\ref{Theo:CorrDoNotCare}, we finally consider linear problems of the form $u^TLx$ under interval uncertainty in the coefficients $u_i$, with underlying assignment structure:
%\begin{corollary}\label{Cor:LPsAssigment}
%Consider the optimization problem \begin{gather}\label{Prob:nom_LP_under_unc:ASSIGN}
%\min_{x \in \mathcal{X}} u^TBx
%\end{gather}
%as in the setting of Theorem~\ref{Theo:CorrDoNotCare} and assume $\mathcal{X} \subseteq \{0,1\}^{[m] \times [n]}$. Let $\Gamma \in [m]$. Furthermore, assume $B_{i,(r,s)} = 0$ for $i \neq r$, and for all $i \in [m]$ and for all $x \in \mathcal{X}$, there is exactly one $j \in [n]$, such that $x_{i,j} = 1$. Then the $\Gamma$--counterpart of \eqref{Prob:nom_LP_under_unc:ASSIGN} is equivalent to
%\begin{align}\label{Prob:RobustCounterpartSuperComb}
%\begin{split}
%&\min_{(k,l) \in [m] \times [n] \cup \{(0,0)\}} \Gamma \Delta u^T B_{.,(k,l)} + \\
%&\min_{x \in \mathcal{X}} \overline{u}^TBx + \sum_{(i,j) \in [m] \times [n]} \max\{0,\Delta u^TB_{.,(i,j)} - \Delta u^TB_{.,(k,l)}\}x_{i,j}.
%\end{split}
%\end{align}
%%$\min_{x Assume that for all $i \in [m]$, there is a function $l_i\colon \R^n \to \R^{L_i} $, such that $f_i(x,u^i) = (u^i)^Tl_i(x)$, i.e., $f_i$ is linear in the uncertainty and in the decision. Assume that the uncertainty set is $\mathcal{U}^i := [\overline{u}^\overline{u}^i + \Delta u^i
%\end{corollary}
%\proof{Proof.}
%This follows from Theorem~\ref{Theo:CorrDoNotCare} and Proposition~\ref{Prop:Tractable_Gamma_Comb} by setting $g(x) = x$.
%\endproof

\begin{example}
We consider the following quadratic combinatorial program under interval uncertainty:
\begin{align}\label{Prob:QuadUnc}
\begin{split}
\min_{x \in \mathcal{X} \subseteq \{0,1\}^n} & \sum_{i \in[n]} \sum_{j\in [i]} p_{i,j} x_ix_j
%%\mathrm{s.t} & \ x \in \mathcal{X} := \{x \in \{0,1\}^n: \ \sum_{j\in [n]} \omega_j x_j \le c\}
%\mathrm{s.t} & \ x \in \mathcal{X} \subseteq \{0,1\}^n
\end{split}
\end{align}
with uncertain coefficients $p_{i,j} \in [\bar{p}_{i,j}, \bar{p}_{i,j} + \Delta p_{i,j}]$. Let $m:= n^2 - \frac{n(n+1)}{2} = \frac{n^2 - n}{2}$ be the number of uncertain coefficients and let $\mathcal{M}:=\{(k,l) \in [n]^2: \ l \leq k\}$. For $\Gamma \in [m]$, its $\Gamma$--counterpart is given by
%\begin{align*}
%\max_{x \in \mathcal{X}} & \left\{ \min_{\mathcal{S} \subseteq \mathcal{M}: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{(i,j) \in \mathcal{S}} \min_{p_{i,j} \in [\bar{p}_{ij} - \Delta p_{i,j}, \bar{p}_{ij}]} p_{i,j} x_ix_j + \sum_{(i,j) \in \mathcal{M} \setminus \mathcal{S}} \bar{p}_{i,j} x_ix_j \right\} \right\}
%\end{align*}
%or, equivalently,
\begin{align}\label{Prob:RobQP}
\min_{x \in \mathcal{X}} & \left\{ \sum_{(i,j) \in \mathcal{M} } \bar{p}_{i,j} x_ix_j + \max_{\mathcal{S} \subseteq \mathcal{M}: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{(i,j) \in \mathcal{S}} \Delta p_{i,j}x_ix_j \right\} \right\}
\end{align}
By applying Theorem~\ref{Theo:PseudoLin}, we obtain that program~\eqref{Prob:RobQP} is equivalent to
%-> $f_i(x,u_i) = p_{ij}l_{ij}(x)$ mit $l_{ij} = x_ix_j \ge 0 $ 
%Dann ist gilt mit Theorem 4.10 für das robuste Gegenstück:
%\begin{align*}
%\min_{k,l \in [n]} \min_{x \in \{0,1\}^n} & \Gamma \Delta p_{kl} + \sum_{i \in[n]} \sum_{j\in [n]} \bar{p}_{ij} x_ix_j + \max \{0, \Delta p_{ij}x_i x_j - \Delta p_{ij}x_k x_l\}\\
%\text{s.t} &\sum_{j\in n} \omega_j x_j \le c
%\end{align*}
%\todo[inline][inline]{Du meinst schon immer $p_{i,j}x_kx_l$, oder?}
%Wir nehmen an $x_lx_k = 1$ mit der gleichen Argumentation wie beim QAP. \todo[inline][inline]{Wieso geht das hier? Die Bedingungen für das QAP sind hier ja nicht da, also dass man für alle $j$ ein $i$ braucht -- können nicht auch $k$ und $l$ in der Optimallösung nicht eingepackt werden?}
%Dann wird aus dem maximum   
%\[\max \{0, \Delta p_{ij}x_i x_j - \Delta p_{ij}\}:\]
%Da $x_ix_j = 1 \vee 0$ kann man die $x$ aus dem Maximum ziehen denn:\\
%$x_ix_j = 1$
%\[\max \{0, \Delta p_{ij}\cdot 1 - \Delta p_{ij}\} = \max \{0, \Delta p_{ij} - \Delta p_{ij}\} \cdot 1\]
%$x_ix_j = $
%\[\max \{0, \underbrace{\Delta p_{ij} \cdot0 - \Delta p_{ij}}_{\le 0}\} = 0 =\max \{0, \Delta p_{ij} - \Delta p_{ij}\} \cdot 0\]
%\todo[inline][inline][inline]{Ich würde auhc nicht erwarten, dass es genauso funktioniert wie beim QAP: Unser Theorem 4.12 sagt in Prinzip "sobald wir Assignment-Strukturen haben, können wir alle Korrelatoinen ignorieren" und wir haben hier keine Assignment-Struktur. Wenn ich mich nicht vertue, müsste es irgendwie so sein:}
%{\color{red} Forme $\max \{0, \Delta p_{i,j} x_ix_j - \Delta p_{k,l}x_kx_l\}$ um. Ohne weitere Voraussetzungen führen wir folgende Fallunterscheidung durch: \\
%1. Fall: $x_k = 0 \vee x_l = 0$. Dann ist $\max \{0, \Delta p_{i,j} x_ix_j - \Delta p_{k,l}x_kx_l\} = \\ \max \{0, \Delta p_{i,j}\}x_ix_j $.\\
%2. Fall: $x_k = x_l = 1$. Dann ist $\max \{0, \Delta p_{i,j} x_ix_j - \Delta p_{k,l}x_kx_l\} = max \{0, \Delta p_{i,j} - - \Delta p_{k,l}\}x_ix_j $. \\
%Nun glaube ich schon, dass es so geht, dass man annehmen kann, dass im Optimum irgendwo mal der 2. Fall auftritt -- wäre das nicht so, wäre $x_{k}x_l = 0$ für alle $k,l \in [n]$ und es wäre optimal, gar nichts mit zunehmen. Dann wäre das Budget aber kleiner als alle Gewichte, und sobald du irgendwas einpackst, gibt es ein $x_kx_l = 1$, da $k=l$ gelten kann (richtig?)... Was ich damit sagen will: ich glaube schon, dass es geht, die Argumentationsstruktur läuft nur anders als beim QAP, wo wir wussten, dass die Nullösung nicht funktioniert.}
%Damit müssen $n\times n$ Knapsacks gelöst werden
\begin{align*}
\min_{(k,l) \in \mathcal{M} \cup \{(0,0)\}} \left\{ \Gamma \Delta p_{k,l} + \min_{x \in \mathcal{X}}   \left\{ \sum_{i \in[n]} \sum_{j\in [i]} (\bar{p}_{ij} + \max \{0, \Delta p_{i,j} - \Delta p_{k,l}\}) x_ix_j  \right\} \right\}
\end{align*}
where $\Delta p_{0,0} := 0$ and we can solve the robust counterpart with $m+1$ calls of an optimization oracle of program~\eqref{Prob:QuadUnc}.

%Linearisierung: Standart
%\begin{align*}
% \min_{x \in \{0,1\}^n, y\in \{0,1\}^{n\cdot n}}& \sum_{i \in[n]} \sum_{j\in [n]} p_{ij} y_{ij}\\
%\text{s.t} &\sum_{j\in n} \omega_j x_j \le c\\
%&y_{ij} \ge x_i +x_j -1\\
%&y_{ij} \le x_i \\
%&y_{ij} \le x_j
%\end{align*}
%Reformuliert dann zu
%\begin{align*}
% \min_{x \in \{0,1\}^n, y\in \{0,1\}^{n\cdot n}}& \sum_{i \in[n]} \sum_{j\in [n]} p_{ij} y_{ij} +\max_{S\subseteqeq [n]\times [n]:|S|\le \Gamma}  \sum_{(i,j) \in S}  \Delta p_{ij} y_{ij}\\
%\text{s.t} &\sum_{j\in n} \omega_j x_j \le c\\
%&y_{ij} \ge x_i +x_j -1\\
%&y_{ij} \le x_i \\
%&y_{ij} \le x_j
%\end{align*}
%
%\begin{align*}
% \min_{x \in \{0,1\}^n, y\in \{0,1\}^{n\cdot n}, z}& \sum_{i \in[n]} \sum_{j\in [n]} p_{ij} y_{ij} +\Gamma z_0 + \sum_{i,j \in [n]} z_{ij}\\
%\text{s.t} &\sum_{j\in n} \omega_j x_j \le c\\
%&y_{ij} \ge x_i +x_j -1\\
%&y_{ij} \le x_i \\
%&y_{ij} \le x_j\\
%& z_{ij}+z_0 \ge \Delta p_{ij} y_{ij}\\
%& z_{ij} \ge 0
%\end{align*}
%\todo[inline][inline]{Da vertraue ich dir mal, dass das passt :P Erstmal klären, ob das mit dem Knapsack wirlkich alles passt.}
\end{example}
To conclude the discussion of quadratic programs under uncertainty, we demonstrate the  approach of applying the notion of term--wise parallel vectors and hidden concavity \cite{TermWise} for interval uncertainty. 
\begin{example}
Let $\mathcal{X}$ be a convex set. We consider the following program:
\begin{align}\label{Prob:NomQuad}
\inf_{x \in \mathcal{X}} \sum_{i \in [m]} (x_i - u_i)^2.
\end{align}
For every $i \in [m]$, $u_i$ is subject to uncertainty $\mathcal{U}_i := [\overline{u}_i, \overline{u}_i + \Delta u_i]$. For $\Gamma \in [m]$, the $\Gamma$--counterpart of program~\eqref{Prob:NomQuad} after applying Lemma~\ref{Lem:ReModel} is given by
\begin{align}\label{Prob:FirstQuad}
\begin{split}
\inf_{x, p, \theta} & \ \Gamma \theta + \sum_{i \in [m]} (x_i - \overline{u}_i)^2 + p_i, \\
\mathrm{s.t.} & \ x \in \mathcal{X}, \\
& \max_{u_i \in \mathcal{U}_i} (x_i - u_i)^2 - (x_i - \overline{u}_i)^2 \leq p_i + \theta \ \forall i \in [m].
\end{split}
\end{align}
The inequalities of program~\eqref{Prob:FirstQuad} are equivalent to
\begin{gather}\label{Ineq:ReformedQuad}
-2x_i u_i + u_i^2 \leq p_i + \theta - 2x_i \overline{u}_i + \overline{u}_i^2 \ \forall u_i \in \mathcal{U}_i
\end{gather}
for each $i \in [m]$. The left--hand side of \eqref{Ineq:ReformedQuad} is not concave in $u_i$ and thus, we cannot apply the reformulations of Subsection~\ref{subsec:Concave}. We set $h(y) := y^2$ for all $y \in \R$  
%\eqref{Ineq:ReformedQuad} is of the form \eqref{Ineq:SecondApproach}: We set
and consider the following formulation of the uncertainty set:
\begin{gather*}
[\overline{u}_i, \overline{u}_i + \Delta u_i] = \{u_i \in \R\colon (-2 \overline{u}_i - \Delta u_i)u_i + u_i^2 \leq -\overline{u}_i^2 - \overline{u}_i \cdot \Delta u_i\}.
\end{gather*}
Finally, define
\begin{gather*}
\alpha := -2\overline{u}_i - \Delta u_i, \ \beta := 1, \ \gamma = -\overline{u}_i^2 - \overline{u}_i \Delta u_i. \
\end{gather*}
Since $\alpha$ and $\beta$ are scalars, they are clearly term--wise parallel \cite{TermWise}. Thus, we obtain that \eqref{Ineq:ReformedQuad} is satisfied for $(x, p, \theta)$ if and only if there exist $v_1, \dots, v_m \in \R$, such that
\begin{align*}
&(1 + v)h_i^*\left(\frac{2x + 2 \overline{u}_iv_i + \Delta u_iv_i}{1+v_i}\right) - \overline{u}_i^2v_i - \overline{u}_iv_i \Delta u_iv_i + 2x_i \overline{u}_i\le p_i + \theta  + \overline{u}_i^2,\\
&1 + v_i \ge 0,\\
&v_i\ge 0,
\end{align*}
see \cite{Fenchel}, Subsection 4.3, for details. Clearly, the second inequality is redundant. Furthermore, since
$h_i^*(z) = \frac{z^2}{4}$, the first inequality is convex in $(x,v_i)$ if it is assumed that $x \geq 0$. If $\mathcal{X} \subseteq \R^n_{\geq \overline{u}}$, then the $\Gamma$--counterpart of program~\eqref{Prob:NomQuad} is a convex optimization problem, although the uncertainty is not concave.
\end{example}

\paragraph*{Deadline uncertainties in a piecewise linear setting.}
%A piecewise linear function is a function $f$ with domain $\mathcal{D}$ and that there exists a finite number of polyhedra $\mathcal{P}_i$ and $(m_{\mathcal{P}_i}, c_{\mathcal{P}_i})$, such that $\cup_{i=1}^m \mathcal{P}_i = \mathcal{X}$ and $f(x) = m_{\mathcal{P}_i}^Tx + c_{\mathcal{P}_i}$ for $x \in \mathcal{P}_i$. We assume that $f$ is continuous and that the interior of the polyhedra are pairwise disjoint. Furthermore, we assume that $f$ is subject to uncertaintyWe employ our reformulations for a fixed number of reformulations, e.g. for cases of Example~\ref{Ex:UncertainBounds}. 
%We consider continuous piecewise linear functions as considered in XXX:
%\begin{definition}
%Let $\mathcal{X}$ be the domain of a function $f \colon \mathcal{X} \to \R$. $f$ is called \emph{piecewise linear}, if there is a finite number of polyhedra $\mathcal{P}_i$ and $(m_{\mathcal{P}_i}, c_{\mathcal{P}_i})$, such that $\cup_{i=1}^m \mathcal{P}_i = \mathcal{X}$ and $f(x) = m_{\mathcal{P}_i}^Tx + c_{\mathcal{P}_i}$ for $x \in \mathcal{P}_i$. The definition already implies that $f$ is continuous. W.l.o.g. we assume that the relative interior of the polyhedra are pairwise disjoint.
%%\end{definition}
%we consider model~\eqref{Prob:GeneralStrictOpt} 
%where each function $f_i$ is continuous piecewise linear. We start by the assumption that $f_i$ is concave in the uncertainty.
%\paragraph*{Concavity in the uncertainty} 
%As pointed out in Remark~\ref{Rem:Concave}, under Assumption~\ref{Ass:General} one can state a reformulation. In the following, we furthermore assume that $f_i(x,u_i) = \min_{j \in \mathcal{I}_i} \{a_jx_i - b_j + u_i\}$.
%
%\paragraph*{Application: Deadline Uncertainty}
%Since those are in general neither convex nor concave, thus, if the underlying vectors $(m_{\mathcal{P}_i}, c_{\mathcal{P}_i})$ are subject to uncertainty, we can in general not apply reformulations of Subsection~\ref{subsec:Concave}. 
%\todo[inline][inline]{Beispiel, so dass sich auch die Polyeder ändern?}. 
%Furthermore, because of the inherent definition, it is not clear how a robust counterpart can be formulated algebrically. However, applying our recent results, we obtain the following result:
%\begin{theorem}
%For $i \in [m]$, let $f_i \colon \mathcal{X}$ be a continuous piecewise linear function...
%\end{theorem}
%% Therein, a continuous function $f$ is called piecewise linear on its domain $\mathcal{D}\subseteq \R^n$, if there exists a set $\mathcal{P}$ that contains polyhedra and for each $P \in \mathcal{P}$, there is a vector $m_P$ and a scalar $c_P$, such that for all $x \in D$ there exists a polyhedron $P$, such that $f(x) = m_p^Tx + c_p$. Without loss of generality, we can assume that the polyhedra are pairwise disjoint. In practice... \todo[inline][inline]{Drauf eingehen wieso $\Gamma$ hier nicht einfach über MIP anwendbar ist}. In this definition of a function, there are many ways uncertainty can appear:
%\begin{itemize}
%\item The polyhedra are subject to change, i.e., $\mathcal{P}$
%\item The polyhedra 
%\item 
%\end{itemize}

%We show next that with
%Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear},
%Proposition~\ref{Prop:Tractable_Gamma_Comb} can be applied as well: If we consider $u_{i,j} := p_i q_j$ with uncertainty set $\mathcal{U}_{i,j} := [\overline{p}_i q_j, \overline{p}_iq_j + \Delta p_i q_j]$ for each $(i,j) \in \mathcal{I} \times \mathcal{J}$, the $\Gamma$--counterpart of $\min_{x \in \mathcal{X}} u^Tx$ is given by
%\begin{gather*}
%\min_{x \in \mathcal{X}} \left\{ \sum_{(i,j) \in \mathcal{I} \times \mathcal{J}} \overline{p}_iq_j x_{i,j} + \max_{\mathcal{S} \subseteq \mathcal{I} \times \mathcal{J}, |\mathcal{S}| \leq \Gamma} \sum_{(i,j) \in \mathcal{S}} u_{i,j} \Delta p_i q_j x_{i,j} \right\}.
%\end{gather*}
%Technically, we applied that the uncertainty of the coefficients of $x_{i,j}$ are not correlated although they are in the original setting. However, applying Proposition~\ref{Prop:Tractable_Gamma_Comb} results exactly in the problems~\eqref{Prob:SchedulingFamily} and ~\eqref{Prob:Scheduling0}. This is a consequence of the worst-cases of the two settings being equivalent: In the first setting, a coefficient $p_i$ realizes its worst case when $p_i = \overline{p}_i + \Delta p_i$ and in the second setting, a coefficient $u_i = p_i q_j$ realizes its worst case when $u_{i,j} = \overline{p}_iq_j + \Delta p_i q_j = (\overline{p}_i + \Delta p_i)q_j$. Thus, for every $j \in \mathcal{J}$, the worst-case of $u_{i,j}$ realizes if and only if the worst-case of $q_i$ realizes. Since we only consider worst-case scenarios in our $\Gamma$--counterparts, the reformulations of Proposition~\ref{Prop:Tractable_Gamma_Comb} and \cite{RobustScheduling} are identical.
%has been determined, namely in Proposition 1 in \cite{RobustScheduling}. 
%This setting covers e.g. the single-machine scheduling of Example~\ref{Ex:Scheduling}:\\ The authors assumed that, for every $i \in \mathcal{I}$, the parameter $\overline{p}_i$ is uncertain and lies in the uncertainty set $\mathcal{U}_i := [\overline{p}_i, \overline{p}_i + \Delta p_i]$. Although Problem~\eqref{Prob:NomScheduling} is linear in the uncertainty and the decision variables, one can not simply apply Proposition~\ref{Prop:Tractable_Gamma_Comb} since the number of uncertain parameters and decision variables do not match, as the authors of \cite{RobustScheduling} have pointed out. They explicitly stated the $\Gamma$--counterpart
%\begin{gather*}
%\min_{x \in \mathcal{X}} \sum_{i \in \mathcal{I}} \overline{p}_i \sum_{j \in \mathcal{J}} q_j x_{ij} + \max_{\mathcal{S} \subseteq \mathcal{I}: |\mathcal{S}| \leq \Gamma} \sum_{i \in \mathcal{S}} \Delta p_i \sum_{j \in \mathcal{J}} q_i x_{ij} 
%\end{gather*} 
%is equivalent to obtaining the minimum of 
%\begin{align}\label{Prob:SchedulingFamily}
%\min_{(k,l) \in \mathcal{I} \times \mathcal{J}} \Gamma q_k \Delta p_l + \min_{x \in \mathcal{X}} \sum_{i,j \in \mathcal{I}, \mathcal{J}} (\overline{p}_i + \max\{0, \Delta p_i - \frac{\Delta p_k q_l}{q_j}\})q_jx_{i,j}
%\end{align}
%and 
%\begin{align}\label{Prob:Scheduling0}
%\begin{split}
%\min_{x \in \mathcal{X}} \sum_{i,j \in \mathcal{I}, \mathcal{J}} (\overline{p}_i + \Delta p_i)q_jx_{i,j}.
%\end{split}
%\end{align}
%We can prove this with Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear}: We set
%\begin{gather*}
%\overline{u}^i := \overline{p}^i, \ l_i(x) = \sum_{j \in \mathcal{J}} q_j x_{i,j}, \ f_i(x,u^i) = p_i l_i(x), \ \mathcal{U}_i = \{p_i = \overline{p}_i + \alpha \Delta p_i \mid \alpha \in [0,1]\}, \mathcal{Z}_i = [0,1]
%\end{gather*}
%and obtain 
%\begin{gather*}
%\theta^k := \delta^*(\Delta p_k l_k(x) \mid \mathcal{Z}_k) = \Delta p_k \sum_{j \in \mathcal{J}} q_j x_{k,j}.
%\end{gather*}
%Thus, applying Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} results in 
%\begin{align}\label{Prob:GeneralGammaCounterpartWithoutDualScheduling}
%\begin{split}
%\min_{k \in \{1, \dots, m\}} & \min_{x} \Gamma \Delta p_k \sum_{j \in \mathcal{J}} q_j x_{k,j} + \sum_{i \in [m]} \overline{p}_i\sum_{j \in \mathcal{J}} q_j x_{i,j} + \max \{0, \Delta p_i \sum_{j \in \mathcal{J}} q_j x_{i,j} - \Delta p_k \sum_{j \in \mathcal{J}} q_j x_{k,j} \} \\
%\text{s.t.} & x \in \mathcal{X} \\
%%& \theta^k \geq 0. \\
%%& \theta^k = \overline{u^k}^Tv^k - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k) + \support{k}).
%\end{split}
%\end{align}
%For obtaining a computationally tractable counterpart which a linear objective function, we use that for each $k \in \mathcal{I}$, $\sum_{j \in \mathcal{J}} x_{k,j} = 1$, i.e., for each $k \in \mathcal{I}$, there exists exactly one $l \in \mathcal{J}$, such that $x_{k,l} = 1$. Thus, we minimize over $(k,l) \in \mathcal{I} \times \mathcal{J}$ instead of only $k \in \mathcal{I}$ and obtain as an objective, for fixed $(k,l)$,
%\begin{align*}
%\Gamma \Delta p_k q_l + \sum_{i \in [m]} \overline{p}_i \sum_{j \in \mathcal{J}} q_j x_{i,j} + \max\{0, \Delta p_i \sum_{j \in \mathcal{J}} q_j x_{i,j} - \Delta p_k q_l \}= \\
% \Gamma \Delta p_k q_l + \sum_{i \in [m]} \overline{p}_i \sum_{j \in \mathcal{J}} q_j x_{i,j} + \sum_{j \in \mathcal{J}} \max\{0, \Delta p_i - \frac{\Delta p_k q_l}{q_j}\} q_j x_{i,j}
%\end{align*}
%due to $\sum_{j \in \mathcal{J}} x_{i,j} = 1.$ This results in Problem~\eqref{Prob:SchedulingFamily}. For $\theta^0 := 0$, we easily obtain Problem~\eqref{Prob:Scheduling0}: Applying Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear}, this results in
%\begin{gather*}
%\min_{x \in \mathcal{X}} \sum_{i \in \mathcal{I}} \overline{p}_i \sum_{j \in \mathcal{J}} q_j x_{i,j} + \max\{0, \Delta p_i \sum_{j \in \mathcal{J}} q_j x_{i,j}\}
%\end{gather*}
%which is, due to $\Delta p_i \sum_{j \in \mathcal{J}} q_j x_{i,j} \geq 0$, exactly Problem~\eqref{Prob:Scheduling0}.
%\end{example}
%%Example~\ref{Ex:Scheduling} shows that there exist cases where, although the objective is linear in the uncertainty and the decision variable, one can not apply Proposition~\ref{Prop:Tractable_Gamma_Comb}. This is due to uncertainty and decision vector not having the same dimension.\\
%
%We note that for Example~\ref{Ex:SchedulingGeneral}, one could have applied a similar proof to obtain the computationally tractable counterpart. \\
We conclude our discussion of applications with the deadline uncertainty setting we introduced in Section~\ref{sec:Rev}.
%This concludes our discussion of concavity in the uncertainty. In the next subsection, we propose methods to tackle the general case.

%Looking at \ref{Prob:GeneralReModel}, we try to compute with Fenchel duality a tractable formulation for $p_i+\theta \ge \max_{u^i \in \mathcal{U}_i} f_i(x,u^i) -f_i(x, \bar{u}^i)$. This equals $ p_i+\theta - \max_{u^i \in \mathcal{U}_i} f_i(x,u^i) +f_i(x, \bar{u}^i)\ge 0$. Here it is possible to replace the maximum with a for all condition. We also assume that $f_i(x,u)$ is separable:
%\[-p_i - \theta - f_i(x, \bar{u}^i) + \bar{f}_i(u^i)^Tg_i(x)\le 0\]
%Following approach on we replace $\bar{f}_(u)=b$. With this we obtain:
%\[b_i^T\bar{g}_i(x) \le 0, \qquad \forall (u_i,b_i) \in \bar{U}^i=\{(u,b): u \in \mathcal{U}^i, \bar{f}_i(u^i)=b_i\} \}.\]
%Now we have to obtain $conv(\bar{U}^i)$. However, this depends strongly on the structure of $\mathcal{U}_i$. For a general $conv(\bar{U}_i)$ the resulting robust counterpart can be determined as:
%\begin{align*}
%\min_{x,p,\theta} & \Gamma \theta + \sum_{i \in [m]} f_i(x, \bar{u}^i +p_i\\
%\text{s.t} & x \in \mathcal{X}\\
%& a^{0T}\bar{g}_i(x)+\delta^*(A^T\bar{g}_i(x)|Z_i)\le 0\\
%&p,\theta \ge 0
%\end{align*} 
%%Apart from these approaches, there are cases that enable a formula for $\max_{u^i \in \mathcal{U}_i}
%%f_i(x,\overline{u}^i)$ analytically. We apply this approach to the problem introduced in
%%Example~\ref{Ex:VRP}:
\begin{example}\label{Ex:UncertainBounds}
Consider the $\Gamma$--counterpart of program~\eqref{Prob:BoundNom} as introduced in Section~\ref{sec:Rev}:%Example~\ref{Ex:VRP}:
\begin{align*}
\inf_{x \in \mathcal{X}}  \left\{ \sup_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} \max\{0,x_i - \overline{b}_i + \Delta b_i\} + \sum_{i \in [m] \setminus \mathcal{S}} \max\{0, x_i - \overline{b}_i\} \right\} \right\}.
\end{align*}
An equivalent reformulation, given in Remark~\ref{Rem:NoFenchel} as program~\eqref{Prob:GammaCombCounterpartWithoutFenchel}, is
\begin{align}\label{Prob:PiecewiseLinearFirstStep}
\begin{split}
\inf_{k \in [m]_0} \left\{ \inf_{x \in \mathcal{X}} \left\{  \Gamma \theta^k(x) + 
\sum_{i \in [m]}  \max \{0, x_i - \overline{b}_i, \max\{0,x_i - \overline{b}_i + \Delta b_i\} - \theta^k(x)\} \right\} \right\}
\end{split}
\end{align}
with $\theta^k(x) := \max \{0, x_k - \overline{b}_k + \Delta b_k\} - \max\{0,x_k - \overline{b}_k\}$ and $\theta^0(x) := 0$. Thus, for $k = 0$, it is necessary to solve
%We apply 
%\begin{gather*}
%\max_{u^i \in \mathcal{U}_i} f_i(x,u^i) := \max_{u^i \in \mathcal{U}_i} \max \{0,x_i-u^i\} = \max \{0,x_i - \min_{u^i \in \mathcal{U}_i} u^i \} = \max \{0,x_i - \overline{b}_i + \Delta b_i\}
%\end{gather*}
%for $\mathcal{U}_i := [\overline{b}_i, \overline{b}_i + \Delta b_i]$.
%%Note that in this problem, technically only additive terms are uncertain. This was, to the best of our knowledge, first studied in \cite{RobCombOpt}.\\
%gztfzu \begin{alignat}{2}
%p_i + \max\{0, x_i - u_i\} &= \max\{0, x_i - u_i, x_i - u_i + \Delta u_i - (x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\})\} \\
%&= \max\{0, x_i - u_i, x_i - u_i + \Delta u_i - (x_l - u_l + \Delta u_l), x_i - u_i + \Delta u_i - \Delta u_l \}\label{Eq:p}
%\end{alignat}
%We set $\theta^k(x) := \max \{0, x_k - \overline{b}_k + \Delta b_k\} - \max\{0,x_k - \overline{b}_k\}$. Since $\Gamma$ is integral and with Remark~\ref{Rem:NoFenchel}, one obtains
%\begin{align}\label{Prob:PiecewiseLinearFirstStep}
%\begin{split}
%\min_{k \in \{0, \dots, m\}} & \min_{x} \Gamma \theta^k + \sum_{i \in [n]} \max \{0,x_i - \overline{b}_i\} + \max \{0, \theta^i(x) - \theta^k(x) \}, \\
%\text{s.t.} & x \in \mathcal{X}
%\end{split}
%\end{align}
%with $\theta^0(x) = 0$ and 
%\begin{align}\label{Eq:Bound_Piecewiselinear}
%\begin{split}
%\theta^k(x) &= \max\{0,x_k - \overline{b}_k + \Delta \overline{b}_k\} - \max \{0, x_k - \overline{b}_k\}. \\
%%&= \max\{0, x_k - \overline{b}_k + \Delta \overline{b}_k, \Delta b_k\}. \\
%%&= \max\{x_k - \overline{b}_k + \Delta b_k, \Delta b_k\} \\
%%&= \Delta b_k + \max\{0, x_k - \overline{b}_k\}.
%\end{split}
%\end{align}
%Thus,
%\begin{align}\label{Eq:ObjBounds}
%\begin{split}
%\max \{0,x_i - \overline{b}_i\} + \max \{0, \theta^i(x) - \theta^k(x) \} %&= \max \{\max \{0,x_i - \overline{b}_i\}, \max \{0,x_i - \overline{b}_i\} + \theta^i(x) - \theta^k(x)\} \\
%&= \max \{0, x_i - \overline{b}_i, \max \{0,x_i - \overline{b}_i + \Delta b_i\} - \theta^k(x)\}\\
%%&= \max \{0, x_i - b_i, \Delta b_i - \max\{0, x_k - b_k + \Delta b_k, \Delta b_k\}\} - \max\{0, x_i - b_i + \Delta b_i, \Delta b_i - \max\{0, x_k - b_k + \Delta b_k, \Delta b_k\}\}
%&=\max \{0, x_i - \overline{b}_i, x_i - \overline{b}_i + \Delta b_i- \theta^k(x)\}
%\end{split}
%\end{align}
$ \min_{x \in \mathcal{X}} \sum_{i \in [m]} \max \{0, x_i - \overline{b}_i + \Delta b_i\}$. For $k > 0$, we distinguish between three cases:
\begin{enumerate}
\item[i)] $x_k \geq \overline{b}_k$, i.e., $\theta^k(x) = \Delta b_k$ and
\begin{gather}\label{Eq:Case1}
\max \{0, x_i - \overline{b}_i, \max \{0,x_i - \overline{b}_i + \Delta b_i\} - \theta^k(x)\} = \max\{0, x_i - \overline{b}_i, x_i - \overline{b}_i + \Delta b_i -\Delta b_k\}.
\end{gather}
\item[ii)] $x_k \in [\overline{b}_k- \Delta b_k, \overline{b}_k]$, i.e., $\theta^k(x)  = x_k - \overline{b}_k + \Delta b_k$ and
%Continuing with \eqref{Eq:ObjBounds} results in 
\begin{align}\label{Eq:Case2}
\begin{split}
&\max \{0, x_i - \overline{b}_i, \max \{0,x_i - \overline{b}_i + \Delta b_i\} - \theta^k(x)\} =\\ & \max\{0, x_i - \overline{b}_i, x_i - \overline{b}_i + \Delta b_i - x_k + \overline{b}_k - \Delta b_k\}.
\end{split}
\end{align}
\item[iii)] $x_k \leq \overline{b}_k - \Delta b_k$, i.e., $\max \{0, x_k - \overline{b}_k\} = \max \{0, x_k - \overline{b}_k + \Delta b_k\}=0$. Thus, $\theta^k(x) = 0$ and we refer to the case of $k = 0$.
\end{enumerate}
For each $k \in [m]$, by applying equations~\eqref{Eq:Case1} and \eqref{Eq:Case2}, we solve 
\begin{align}\label{Prob:SubProbVRPNOTRec}
\begin{split}
\inf_{x \in \mathcal{X}} & \ \sum_{i \in [m]} \max\{0, x_i - \overline{b}_i, x_i - \overline{b}_i + \Delta b_i - \Delta b_k \} + \Gamma \Delta b_k \\
\mathrm{s.t.} & \ x_k \in [\overline{b}_k - \Delta b_k, \overline{b}_k]
\end{split}
\end{align}
and
\begin{align}\label{Prob:SubProbVRPRec}
\begin{split}
\inf_{x \in \mathcal{X}} & \ \sum_{i \in [m]} \max\{0, x_i - \overline{b}_i, x_i - \overline{b}_i + \Delta b_i - x_k + \overline{b}_k -\Delta b_k \} + \Gamma (x_k - \overline{b}_k + \Delta b_k) \\
\mathrm{s.t.} & \ x_k \geq b_k.
\end{split}
\end{align}
%For $k = 0$, we need to solve
%\begin{align*}
%\min_{x \in \mathcal{X}} & \ \sum_{i \in [m]} \max \{0,x_i - \overline{b}_i + \Delta b_i\}.
%\end{align*}
Therefore, in total, we need to solve $2m + 1$ optimization programs with a piecewise linear objective with the addition of one additional hard bound for exactly one variable for $k \in [m]$. In the electric companion, we apply this reformulation to a special case of the vehicle routing problem with general time windows.
%Applying the example of logistics, one can interpret this in the following way: For $k \in [m]$, we solve two optimization problems: we distinct between the nominal bound $\overline{b}_k$ being satisfied and not being satisfied. In both cases, one compares the violations for $x_i$ and $x_k$ and adds $\Gamma$ times the violation of bound $x_k$. For $k = 0$, $\Gamma$ is multiplied and $0$ and vanished but all bounds realize their worst-case scenario. So basically, it is a trade-off between worst-case scenarios and the impact of bound $\overline{b}_k$ being not satisfied.
%We note that (except for $k = 0$), the number of pieces doubles ($2$ instead of $4$). For piecewise linear optimization it is crucial that the number of pieces does not rise exponentially.
\end{example}
%Example~\ref{Ex:UncertainBounds} shows that, even without concavity in the uncertainty, one can directly give a robust counterpart for some examples. \\
%A more detailed discussion of this topic can be found in Appendix A.
%Next, we discuss the case of uncertainty in the constraints.
%In this section, we show that the $\Gamma$-flexible approach can be applied to problems of the form
%\begin{alignat*}{2}
%\min & \ \sum_{i \in [n]} \max\{0,x_i - u_i\}\\
%\text{s.t.} & x \in \mathcal{X}. \\
%\end{alignat*} 
%As already discussed, problems of this form can occur whenever the bounds of the problem are increasing the complexity of the problem from polynomial complexity to being NP-hard and when it is actually beneficial to shift the bonds into the objective function, see e.g. Chapter 4 in \cite{Probust}.
%Now, it is possible that one wants again that these soft bounds can be subject to uncertainty with not every bound allowing to change. This results in the $\Gamma$-robust counterpart
%\begin{alignat*}{2}
%\min_{x \in \mathcal{X}} & \ \max_{S \subseteq [n]: |S| \leq \Gamma} \sum_{i \in S} \max\{0,x_i - u_i + \Delta u_i\} + \sum_{i \in [n] \setminus S} \max\{0, x_i - u_i\}\\
%\text{s.t.} & x \in \mathcal{X}. \\
%\end{alignat*}
%%\textbf{TO DO: Looking up: Buchheim, !!!!}\\
%Note that this is a problem with uncertainty in a \emph{constant} of the objective function and not in a coefficient. To the best of our knowledge, this has first been introduced in \cite{RobCombOpt}. \\
%In the following, we will denote a problem over the set $\mathcal{X}$ as \emph{nominal}, if its objective function is a piecewise-linear function. The following theorem shows that we can, similar to the combinatorial case, reformulate the $\Gamma$-Robust counterpart to such a nominal problem:
%\begin{theorem}\label{Theo:GammaBounds}
%The $\Gamma$-robust counterpart can be solved by solving $2n + 1$ problems in nominal form.
%\end{theorem}
%%\proof{Proof.}
%%Similar to the combinatorial case, we introduce binary variables $y_i \in \{0,1\}$ to re-model the inner optimization problem:
%%\begin{alignat*}{3}
%%\max_{y} & \sum_{i \in [n]} \max\{0, x_i - u_i\} + (\max\{0, x_i - u_i + \Delta u_i\} - \max\{0, x_i - u_i\})y_i & \\
%%\text{s.t.} & \sum_{i \in [n]} y_i \leq \Gamma & \\
%%& y_i \in \{0,1\} & \forall i \in [n]. 
%%\end{alignat*}
%%Since $\Gamma$ is a positive integer, the knapsack constraint is TDI and we can substitute this binary programm with a linear programm: 
%%\begin{alignat*}{3}
%%\max_{y} & \sum_{i \in [n]} \max\{0, x_i - u_i\} + (\max\{0, x_i - u_i + \Delta u_i\} - \max\{0, x_i - u_i\})y_i & \\
%%\text{s.t.} & \sum_{i \in [n]} y_i \leq \Gamma & \\
%%& y_i \in [0,1] & \forall i \in [n]. 
%%\end{alignat*}
%%By neglecting the first additive term and by strong duality for linear programs, we obtain
%%\begin{alignat*}{3}
%%\min_{p,\theta} & \ \sum_{i \in [n]} p_i + \Gamma \theta & \\
%%\text{s.t.} & p_i + \theta \geq \max\{0, x_i - u_i + \Delta u_i\} - \max\{0, x_i - u_i\} & \\
%%& p, \theta \geq 0 . 
%%\end{alignat*}
%%Inserting this equivalent form of the inner optimization problem in the original problem results in
%%\begin{alignat*}{2}
%%\min_{x,p,\theta} & \ \sum_{i \in [n]} \max\{0, x_i - u_i\} + p_i + \Gamma \theta &\\
%%\text{s.t.} & x \in \mathcal{X}, \\
%%& p_i + \theta \geq \max\{0, x_i - u_i + \Delta u_i\} - \max\{0, x_i - u_i\} & \forall i \in [n], \\
%%& p, \theta \geq 0.
%%\end{alignat*}
%%Since $p_i + \theta \geq 0$, we can re-write the above constraint to 
%%\begin{gather*}
%%p_i + \theta \geq x_i - u_i + \Delta u_i - \max \{0, x_i - u_i\} 
%%\end{gather*} 
%%The next step is eliminating the new variables $p_i$ and $\theta$. First, we will give a formula for the optimal value of $\theta$:\\
%%Assume that $(x^*,p^*,\theta^*)$ is feasible. We assume \begin{gather*}
%%\theta^* \neq x_j^* - u_j + \Delta u_j - \max \{0, x^*_j - u_j\} =: b_j \text{ for $j = 0, \dots, n$.}
%%\end{gather*} 
%%We note that we defined $b_0 := 0$.
%%Then, with $b_{n+1} := \infty$ (after a possible re-ordering), there is $j$, such that $\theta^* \in (b_j, b_{j+1})$. We consider, two cases:
%%\begin{enumerate}
%%\item[i)] $n - j \leq \Gamma$: Set \begin{gather*}
%%\overline{\theta} := b_j - p_j^*, \ \overline{p_i} := \begin{cases} p_i^*, i \leq j - 1, \\ p_i^* + (\theta^* - \overline{\theta}), i \geq j \end{cases}
%%\end{gather*}
%%Then, $(x^*, \overline{p}, \overline{\theta})$ is obviously still feasible. Furthermore, the objective value does not increase: \begin{alignat*}{2}
%%\sum_{i=1}^n \overline{p_i} + \Gamma \overline{\theta} &= \sum_{i=1}^n p_i^* + (n-j)(\theta^* - \overline{\theta}) + \Gamma \overline{\theta} \\
%%&= \sum_{i=1}^n p_i^* + \Gamma \theta^* + (\theta^* - \overline{\theta})(n-j-\Gamma) \\
%%&\leq \sum_{i=1}^n p_i^* + \Gamma \theta^*.
%%\end{alignat*}
%%\item[ii)] $\Gamma \leq n-j + 1$: Set 
%%\begin{gather*}
%%\overline{\theta} := b_{j+1} - p_{j+1}^*, \ \overline{p_i} := \begin{cases} p_i^*, i \leq j , \\ p_i^* + \theta^* - \overline{\theta}, i \geq j + 1 \end{cases}
%%\end{gather*}
%%Then, like in the first case, $(x^*, \overline{p}, \overline{\theta})$ is obviously still feasible and the objective value does not increase: \begin{alignat*}{2}
%%\sum_{i=1}^n \overline{p_i} + \Gamma \overline{\theta} &= \sum_{i=1}^n p_i^* - (n-(j+1))(\overline{\theta} - \theta^*) + \Gamma \overline{\theta} \\
%%&= \sum_{i=1}^n p_i^* + \Gamma \theta^* + (\overline{\theta} - \theta^*)(\Gamma - (n-(j+1)) \\
%%&\leq \sum_{i=1}^n p_i^* + \Gamma \theta^*.
%%\end{alignat*} 
%%\end{enumerate} 
%%Since we have chosen an arbitrary feasible point, an optimal $\theta$ is, for any optimal $x$, an element of $\{0\} \cup \bigcup_{l \in [n]} \{ x_i - u_i + \Delta u_i - \max \{0, x_i - u_i\} \}$. In other words, the optimization problem is 
%%\begin{alignat*}{3} 
%%\min_{l\in [n+1] }\min_{x,p} & \ \sum_{i \in [n]} \max\{0, x_i - u_i\} + p_i + \Gamma (x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\}) &\\
%%\text{s.t.} & x \in \mathcal{X}, \\
%%& p_i + x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\} \geq x_i - u_i + \Delta u_i - \max \{0, x_i - u_i\} & \ \forall i \in [n], \\
%%%& \theta^l = \Delta u_l + \max\{0, u_l - x_l\} , \\
%%& p \geq 0, \\
%%& x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\} \geq 0.
%%\end{alignat*}
%%(note that we defined $\Delta u_{n+1} := u_{n+1} := x_{n+1} := 0$).
%%To finish the proof of part (a), we will eliminate $p$: It is obvious that an optimal $p_i$ is
%%\begin{gather*}
%%p_i = \max\{0, x_i - u_i + \Delta u_i - \max \{0, x_i - u_i\} - (x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\})\}.
%%\end{gather*}
%%and that 
%%\begin{alignat*}{3} 
%%\min_{l\in [n+1] } \min_{x} & \ \sum_{i \in [n]} \max\{0, x_i - u_i, x_i - u_i + \Delta u_i - (x_l - u_l + \Delta u_l), x_i - u_i + \Delta u_i - \Delta u_l \}+ \Gamma (x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\}) &\\
%%\text{s.t.} & x \in \mathcal{X}, \\
%%& x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\} \geq 0.
%%\end{alignat*}
%%However, due to $\theta^l \geq 0$, $\max\{0, u_l - x_l\} = 0$ and thus, 
%%\begin{gather*}
%%p_i = \max\{0, \Delta u_i - \max \{0, u_i - x_i\} - \Delta u_l\}
%%\end{gather*}
%%Inserting $p_i$ into the objective function finally results in
%%\begin{align*}
%%\sum_{i \in [n]} \max\{0, x_i - u_i\} + \max\{0, x_i - u_i + \Delta u_i - \max \{0, x_i - u_i\} - (x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\})\} - \Gamma (x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\}) \= \sum_{i \in [n]} + \max\{\max \{0, x_i - u_i\}, x_i - u_i + \Delta u_i - \Delta u_l\} + \Gamma (\Delta u_l)\\
%%&= \max \{0, x_i - u_i, x_i - u_i + \Delta u_i - \Delta u_l\} + \Gamma (\Delta u_l).
%%\end{align*}
%%which proves part (a).
%%\endproof
%%Note that there was no point in this proof in which we required the structure of the optimization problem, i.e., there was no point in which it was important if the underlying problem is a discrete, continuous, convex, linear or non-convex optimization problem. \\
%%\paragraph{Generalization for convex, piecewise linear functions}
%\begin{theorem}
%Let $f(x,u) := \sum_{i=1}^n f_i(x_i, u_i)$ be a separable, piecewise linear, convex function with uncertainty $u$. Then the $\Gamma$-robust counterpart
%\begin{alignat}{2}
%\min_x & \max_{S \subseteq [n]: |S| \leq \Gamma} \{ \sum_{i \in S} \max_{u_i \in \mathcal{U}_i} f_i(x_i, u_i) + \sum_{i \in [n] \setminus S} f_i(x_i, \overline{u}_i) \} \\
%\text{s.t.} & x \in \mathcal{X}
%\end{alignat}
%is equivalent to...
%\end{theorem}
%\proof{Proof.}
%Since $f_i(x_i)$ is a convex, piecewise linear function in $x_i$, there is a finite index set $\mathcal{I}^i$ and $(a_1^i, b_1^i), \dots, (a_j^i, b_j^i)$, such that
%\begin{gather*}
%f_i(x_i) = \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\}.
%\end{gather*}
%For the sake of technical issues, we avoid the superscript $i$ unless necessary. \\
%The proof is analogous to the one of Theorem~\ref{Theo:GammaBounds}. Firstly, we have to reformulate the inner optimization problem:
%\begin{alignat*}{2}
%\max_y & \sum_{i \in [n]} \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} + (\max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j + \Delta b^i_j\} - \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\})y_i \\
%\text{s.t.} & \sum_{i \in [n]} y_i \leq \Gamma \\
%& y_i \in \{0,1\} \ \forall i \in [n].
%\end{alignat*}
%Once again, the inequality is TDI and the binary problem is equivalent to its LP relaxation:
%\begin{alignat*}{2}
%\max_y & \sum_{i \in [n]} \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} + (\max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j + \Delta b^i_j\} - \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\})y_i \\
%\text{s.t.} & \sum_{i \in [n]} y_i \leq \Gamma \\
%& y_i \in [0,1] \ \forall i \in [n]
%\end{alignat*}
%and we dualize:
%\begin{alignat*}{3}
%\min_{p,\theta} & \ \sum_{i \in [n]} p_i + \Gamma \theta & \\
%\text{s.t.} & p_i + \theta \geq \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j + \Delta b^i_j\} - \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} \ \forall i \in [n] & \\
%& p, \theta \geq 0 . 
%\end{alignat*}
%Inserting this into our optimization problem leads to
%\begin{alignat*}{2}
%\min_{x,p,\theta} & \ \sum_{i \in [n]} \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} + p_i + \Gamma \theta &\\
%\text{s.t.} & x \in \mathcal{X}, \\
%& p_i + \theta \geq \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j + \Delta b^i_j\} - \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} & \forall i \in [n], \\
%& p, \theta \geq 0.
%\end{alignat*}
%To obtain a tractable formula, we reformulate the right-hand-side of the inequalities (and for the sake of simplicity, neglect the script $i$). \\
%Since $f_i$ is piecewise linear, we can re-write $f_i$ as
%\begin{gather*}
%f_i(x) = \begin{cases}
%a_1x - b_1, x \leq k_1, \\
%a_2x - b_2, x \in [k_1,k_2], \\
%\dots, \\
%a_mx - b_m, x \geq k_m
%\end{cases}
%\end{gather*}
%and $\Delta f_i(x) := \max_{j \in \mathcal{I}} \{a_j x - b_j + \Delta b_j\}$ as 
%\begin{gather*}
%\Delta f_i(x) = \begin{cases}
%a_1x - b_1 + \Delta b_1, x \leq k_1 + \tfrac{\Delta b_2 - \Delta b_1}{a_1 - a_2}, \\
%a_2x - b_2 + \Delta b_2, x \in [k_1 + \tfrac{\Delta b_2 - \Delta b_1}{a_1 - a_2},k_2 + \tfrac{\Delta b_3 - \Delta b_2}{a_2 - a_3}], \\
%\dots, \\
%a_mx - b_m + \Delta b_m, x \geq k_m + \tfrac{\Delta b_m - \Delta b_{m-1}}{a_{m-1} - a_m}
%\end{cases}
%\end{gather*}
%Hence
%\begin{gather*}
%\Delta f_i(x_i) - f_i(x_i) = \begin{cases}
%\Delta b_1, & x \leq k_1, \\
%(a_1-a_2)x - b_1 + \Delta b_1 + b_2, & x \in [k_1, k_1 + \tfrac{\Delta b_2 - \Delta b_1}{a_1 - a_2}], \\
%\Delta b_2, & x \in [k_1 + \tfrac{\Delta b_2 - \Delta b_1}{a_1 - a_2}, k_2],\\
%(a_2-a_3)x - b_2 + \Delta b_2 + b_3, & x \in [k_2, k_2 + \tfrac{\Delta b_3 - \Delta b_2}{a_2 - a_3}], \\
%\dots, \\
%\Delta b_m, & x \geq k_m + \tfrac{\Delta b_m - \Delta b_{m-1}}{a_{m-1} - a_m}
%\end{cases} 
%\end{gather*}
%$\Delta f_i(x_i) - f_i(x_i)$ is a continuous, piecewise linear function which is in general not convex or concave, i.e., for a fitting and finite $\Pi \subseteq \R^2$,
%\begin{alignat*}{2}
%\Delta f(x) - f(x) &= \max_{j \in \mathcal{I}} \{a_j x - b_j + 								\Delta b_j\} - \max_{j \in \mathcal{I}} \{a_jx - b_j\} \\
%& = \max_{j \in \mathcal{I}} \{a_j x - b_j + \Delta b_j - \max_{k \in \mathcal{I}} \{a_kx - b_k\}\} \\
%& = - \min_{j \in \mathcal{I}} \{-a_jx + b_j - \Delta b_j + \max_{k \in \mathcal{I}} \{a_kx - b_k\} \} \\
%&= - \min_{j \in \mathcal{I}} \{\max_{k \in \mathcal{I}} \{(a_k - a_j)x + b_j - b_k - \Delta b_j\} \}\\
%&= \max_{j \in \mathcal{I}} \{\min_{k \in \mathcal{I}} \{(a_j - a_k)x - b_j + b_k + \Delta b_j\}\}
%% {\Sigma \in \Pi} \max_{(a,b) \in \Sigma} \{ax_i - b\}
%\end{alignat*}
%In other words, with \begin{gather*}
%\Pi := \bigcup_{j \in \mathcal{I}} \{\{(a_j - a_1)x - b_j + b_1 + \Delta b_j, \dots, (a_j - a_{|\mathcal{I}|} )x - b_j + b_{|\mathcal{I}|} + \Delta b_j\}\},
%\end{gather*}
%one can re-write 
%\begin{gather*}
%\Delta f(x) - f(x) = \max_{\Sigma \in \Pi} \min_{(a,b) \in \Sigma} \{ax + b\} =: \overline{f}(x)
%\end{gather*}
%%\overline{f_i}(x_i):= 
%%\textcolor{red}{Vermutung: In jedem StÃ¼ck $j = 1, \dots, m$ hat $\Delta f_i - f_i$ die Form
%%\begin{gather*}
%%\Delta f_i(x) - f_i(x) = 
%%\begin{cases} 
%%\begin{cases} 
%%\Delta b_j, & \text{ if } x \leq k_j + \frac{\Delta b_{j+1} - \Delta b_j}{a_j - a_{j+1}},\\
%%(a_{j+1} - a_j)x - b_{j+1} + \Delta b_j + b_j, & \text{ if } x \in [k_j + \frac{\Delta b_{j+1} - \Delta b_j}{a_j - a_{j+1}}, \min \{k_{j+1} + \frac{\Delta b_{j+2} - \Delta b_{j+1}}{a_{j+1} - a_{j+2}},k_j]
%%\end{cases}, \\
%%\begin{cases} 
%%\Delta b_j, & \text{ if } x \leq k_j ,\\
%%(a_{j} - a_{j+1})x + b_{j+1} - \Delta b_j - b_j, & \text{ if } x \in [k_j , \min \{k_{j} + \frac{\Delta b_{j+2} - \Delta b_{j+1}}{a_{j+1} - a_{j+2}},k_{j+1} + \frac{\Delta b_{j+2} - \Delta b_{j+1}}{a_{j+1}-a_{j+2}}\}]
%%\end{cases}
%%\end{cases}
%%\end{gather*}
%%abhÃ¤ngig davon, ob $\Delta b_j \leq \Delta b_{j+1}$ gilt.\\
%%}
%with $\overline{f}$ being a continuous, piecewise linear function (which is general and very likely not convex anymore!). Hence, the optimization problem is equivalent to
%\begin{alignat*}{2}
%\min_{x,p,\theta} & \ \sum_{i \in [n]} \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} + p_i + \Gamma \theta &\\
%\text{s.t.} & x \in \mathcal{X}, \\
%&
%p_i + \theta \geq \overline{f_i}(x_i) & \forall i \in [n], \\
%& p, \theta \geq 0.
%\end{alignat*}
%Once again, it is easy to show that an optimal $\theta^*$ is an element of
%\begin{gather*}
%\{0, \overline{f_1}(x_1^*), \dots, \overline{f_n}(x_n^*)\}.
%\end{gather*}
%Therefore, to solve the $\Gamma$-robust counterpart, one has to solve (we define $\overline{f_0}:= 0 =: x_0$)
%\begin{alignat*}{3} 
%\min_{l\in [n+1] }\min_{x,p} & \ \sum_{i \in [n]} \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} + p_i + \Gamma \overline{f_l}(x_l) &\\
%\text{s.t.} & x \in \mathcal{X}, \\
%& p_i + \overline{f_l}(x_l) \geq \overline{f_i}(x_i) & \ \forall i \in [n], \\
%%& \theta^l = \Delta u_l + \max\{0, u_l - x_l\} , \\
%& p \geq 0, \\
%\end{alignat*}
%Again, for fixed $l$, \begin{gather*}
%p^*_i = \max\{0, \overline{f_i}(x^*_i) - \overline{f_l}(x^*_l)\} \ \forall i \in [n] 
%\end{gather*}
%which can be re-written... \textcolor{red}{TO BE CONTINUED!}
%$\rightarrow$ idea: Splitting the $\overline{f_l}$ into minimum and solving even more inner problems. Re-writing as easy as possible!
%\textcolor{red}{Till this point separability is not necessary. It is possible to define $f_i(x)= \max_{j \in \mathcal{I}^i} \{a_j^T x - b^i_j\} $ }\\
%$\rightarrow$ idea: Splitting the $\overline{f_l}$ into minimum and solving even more inner problems. Re-writing as easy as possible!
%\endproof


==> Non_Linear_Objective_Functions_Preprint.tex <==
%!TEX root = main.tex

\section{Reformulations for programs with uncertain objectives} \label{sec:Non_Linear_Objective_Functions} 
In this section, we present equivalent reformulations for the
$\Gamma$--counterpart introduced in Section~\ref{Sec:General}. Several of the proofs are inspired by those in \cite{IntroGamma}. It turns out that it is possible to obtain first reformulations of $\Gamma$-- counterpart~\eqref{Prob:GeneralGammaCounterpart} without any assumptions on the functions $f_i$ or the uncertainty sets $\mathcal{U}^i$.  % It also turns out that the bottleneck in solving the $\Gamma$--counterpart is solving $\max_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x,\overline{u}^i)$ for each $i \in [m]$: 
\begin{lemma}\label{Lem:ReModel}
Let $\Gamma \in [m]$. Then $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
\begin{align}\label{Prob:GeneralReModel}
\begin{split}
\inf_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
\mathrm{s.t.\;} & x \in \mathcal{X}, \\
& p_i + \theta \geq \sup_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i) \ \forall i \in [m], \\
& p \in \R^m_{\geq 0}, \theta \in \R_{\geq 0}.
\end{split}
\end{align}
\end{lemma}
\begin{proof}
The structure of the proof is similar to the proof of Theorem 3 in \cite{IntroGamma}. With the binary variables
\begin{gather*}
s_i := \begin{cases} 1, \text{ if $i \in \mathcal{S}$,}\\ 
0, \text{ otherwise,} \\
\end{cases} 
\end{gather*}
$i \in [m]$, the inner maximization program of $\Gamma$--counterpart \eqref{Prob:GeneralGammaCounterpart} is equivalent to
\begin{align}\label{Prob:LinearOrdering}
\begin{split}
\sup_{s} & \ \sum_{i \in [m]} f_i(x, \overline{u}^i) + s_i(\sup_{u^i \in \mathcal{U}_i} f_i(x, u^i) - f_i(x, \overline{u}^i)), \\
\text{s.t.} & \ \sum_{i \in [m]} s_i \leq \Gamma, \\
& \ s \in \{0,1\}^m.
\end{split}
\end{align}
%This is a binary program with $\sum_{i \in [m]} f_i(x,
%\overline{u}^i)$ being independent of the decision variable $s$ and a
%knapsack constraint with equal, unit weights and integral
%capacity. Thus,
%we can recycle the proof of
%Proposition~\ref{Prop:Tractable_Gamma_Comb}:
Clearly, program~\eqref{Prob:LinearOrdering} is equivalent to its LP
relaxation. Inserting its dual into $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} proves the claim.
%Its dual is
%\begin{alignat*}{2}
%\min_{p, \theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x, \overline{u}^i) + \sum_{i \in [m]} p_i, \\
%\text{s.t.} & \ p_i + \theta \geq \max_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i) \ \forall i \in [m], \\
%& p, \theta \geq 0.
%\end{alignat*} 
\end{proof}
In Lemma~\ref{Lem:ReModel}, to obtain a tractable formulation, it is necessary to reformulate the inequality
%obtain a tractable formula for $\sup_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i),$ i.e. to solve a maximization problem over the uncertainty set. In the following subsection, we assume that the uncertainty is concave to apply results of \cite{Fenchel}. In \cite{Fenchel}, the authors proposed various ways of reformulating inequality
\begin{gather}\label{Ineq:RobustNonCon}
p_i + \theta \geq \sup_{u^i \in \mathcal{U}_i} f(x,u^i) - f(x, \overline{u}^i)
\end{gather}
for all $i \in [m]$. In \cite{Fenchel}, the authors proposed various approaches, especially for linear/concave uncertainties which will be discussed in the subsequent subsections. We demonstrate one approach for the non--concave case that uses the notion of term--wise parallel vectors for a non--convex quadratic program in Section~\ref{Sec:Reformulations}. For other approaches, we refer to \cite{Fenchel} and \cite{NonlinearRO}. \\

%even if $f$ is \emph{not} concave in the uncertainty (we note that, since we concentrate on single inequalities, we neglect the indices of the inequalities in model~\eqref{Prob:GeneralReModel} for better readibility). We briefly discuss two of their stated approaches (for more details, see \cite{Fenchel}): \\
%On the one hand, if $f(x,u) = h(u)^Tg(x)$ for all $u \in \mathcal{U}$ and $x \in \mathcal{X}$, one can attempt to compute the uncertainty set's convex hull and reformulate inequality 
%%Set $b := h(u)$ and $\overline{\mathcal{U}} :=\mathcal{U} \times h(\mathcal{U})$. Clearly, inequality~\eqref{Ineq:RobustNonCon} is equivalent to $
%\begin{gather*}
%p + \theta \geq \max_{(u,b) \in \mathrm{conv}(\mathcal{U} \times h(\mathcal{U}))} {b}^Tg(x) - f(x, \overline{u}).
%\end{gather*}
%which is 'easier' since the uncertainty is linear instead of non-concave. On the other hand, 
%%Since $b^Tg(x)$ is linear in $b$ -- and thus concave -- $\overline{\mathcal{U}}$ can be replaced with its convex hull and the
%%reformulations of Subsection~\ref{subsec:Concave} can be applied. However, finding the convex hull of a
%%given set is generally NP-hard. 
%% In this case $f(u)$ does not have to be concave and $g(x)$ may attain negative values.
%%Through parameterization $b=f(u)$ we obtain as robust counterpart
%%\[b^Tg(x)\le 0 \qquad \forall (u,b) \in \bar{U},\]
%%with $\bar{U}=\{(u,b)| b=f(u), u \in \mathcal{U}\}$.
%%Now the lefthand side is linear in the uncertainty, so we can replace the uncertainty set with its convex hull. 
%%If we can determine $conv(\bar{U})$ Fenchel duality can be applied. \\
%%The second approach was introduced in \cite{TermWise} and was discussed for robust optimization in \cite{Fenchel}:
%under the assumption that inequality~\eqref{Ineq:RobustNonCon} can be formulated as
%\begin{align}\label{Ineq:SecondApproach}
%u^Tg_1(x)+h(u)^Tg_2(x)\le p + \theta + f(x,u) \qquad \forall u: \ \alpha_k^Tu+\beta_k^Th(u) \le \gamma_k, k \in [K],
%\end{align}
%% Another approach assumes it is possible tor write the robust counterpart as \[u^Tg_1(x)+f(u)^Tg_2(x)\le 0 \qquad \forall u \alpha_k^Tu+\beta_k^Tf(a) \le \gamma_k, k \in [K].\]
%one can attempt to apply the notion of \emph{term-wise parallel vectors} \cite{TermWise}: After setting $b:=h(u)$, inequality~\eqref{Ineq:SecondApproach} is equivalent to 
%\begin{align}\label{Ineq:Parametrizing}
%u^Tg_1(x)+b^Tg_2(x)\le 0 \qquad \forall (u,b): \ \alpha_k^Tu+\beta_k^Tb \le \gamma_k, k \in [K], b=h(u).
%\end{align}
%While the left-hand side of the inequalities are clearly linear -- and thus, concave -- in $u$, the lifted uncertainty set $
%\mathcal{V} := \{(u,b): \alpha_k^Tu+\beta_k^Tb \le \gamma_k, k \in [K], \ b = h(u)\}
%$
%is generally not convex and thus, the theory of Subsection~\ref{subsec:Concave} cannot be applied for reformulating \eqref{Ineq:Parametrizing}. However, if $\mathcal{V}$ is replaced with  
%$
%\mathcal{V}^{\mathrm{rel}} := \{(u,b): \alpha_k^Tu+\beta_k^Tb \le \gamma_k, k \in [K], \ b \leq h(u)\}
%$
%in \eqref{Ineq:Parametrizing}, one can apply said theory since $\mathcal{V}^{\mathrm{rel}}$ is convex. If $\alpha_k$ and $\beta_k$ are term-wise parallel and $\max_{(u,b) \in \mathcal{V}^{\mathrm{rel}}} u^Tg_1(x)+b^Tg_2(x)$ exists and is finite for every $x \in \mathcal{X}$,
%\eqref{Ineq:Parametrizing} and
%\begin{gather}\label{Ineq:Relax}
%u^Tg_1(x)+b^Tg_2(x)\le p + \theta + f(x,u) \qquad \forall (u,b) \in \mathcal{V}^{\mathrm{rel}}
%\end{gather} 
%are equivalent. 
%%However, this changes when $\alpha_k$ and $\beta_k$ are \emph{term-wise parallel} \cite{TermWise, Fenchel}:
%%\begin{definition}
%%Consider a family of $K$ inequalities, given by
%%\begin{gather*}
%%\alpha_k^T u + \beta_k^T b \leq \gamma_k \ \forall k \in [K],
%%\end{gather*}
%%where $\alpha_k, \beta_k \in \R^L, \gamma_k \in \R$ for all $k \in [K]$. The vectors $\alpha_k,\ \beta_k$ are called \emph{term-wise parallel} if 
%%\begin{gather*}
%%\mathrm{rank}\{(\alpha_{kl},\beta_{kl}), \ k \in [K]\} \leq 1 \ \forall l \in [L].
%%\end{gather*}
%%\end{definition}
%%With this notion, inequalities~\eqref{Ineq:Parametrizing} and \eqref{Ineq:Relax} are equivalent if $\alpha_k$ and $\beta_k$ are term-wise parallel and if $\max_{(u,b) \in \mathcal{V}^{\mathrm{rel}}} u^Tg_1(x)+b^Tg_2(x)$ exists and is finite for every $x \in \mathcal{X}$.
%Then $x$ satisfies inequality~\eqref{Ineq:RobustNonCon} if and only if for all $k \in [K]$ there exist vectors $v^k \in \R^n$, such that
%% If $b \ge f(\bar{u})$ it has been proven that there is another optimal solution for $u$ that satisfies $b=f(u)$. Because of that both robust counterparts are equivalent and we can use Fenchel duality for the latter. The final counterpart is then:
%\begin{align*}
%&\sum_{l\in[L]} \left(g_{2l}(x)+\sum_{k\in[K]} \beta_{kl}v_k\right)h^*\left(-\frac{g_{1l}(x)+\sum_{k\in[K]}\alpha_{ki}v_k}{g_{2l}(x)+\sum_{k\in[K]} \beta_{kl}v_k}\right)+\sum_{k\in[K]} \gamma_kv_k \le p + \theta + f(x,\overline{u}),\\
%&g_{2l}(x)+\sum_{k\in[K]} \beta_{kl}v_k \ge 0 \ \forall l \in [L],\\
%&v\ge 0,
%\end{align*}
%see \cite{Fenchel}, Subsection 4.3. We demonstrate an application in Section~\ref{Sec:Reformulations}. Otherwise, one can still attempt to obtain reformulations, although it is less straightforward. We show a 1--dimensional example where this is possible in Section~\ref{Sec:Reformulations}. 
Furthermore, one can reformulate program~\eqref{Prob:GeneralReModel} to obtain a program with feasible set $\mathcal{X}$ and without variables $p$ and $\theta$:
\begin{lemma}\label{Rem:NoFenchel}
If $\Gamma \in [m]$, then $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%Theorem~\ref{Theo:GeneralGammaCounterPartWithoutDual} also holds in a more general version: By Lemma~\ref{Lem:ReModel},
%the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to model~\eqref{Prob:GeneralReModel} and by applying the proof of Theorem~\ref{Theo:GeneralGammaCounterPartWithoutDual} to model~\eqref{Prob:GeneralReModel} we obtain
\begin{align}\label{Prob:GammaCombCounterpartWithoutFenchel}
\begin{split}
\inf_{k \in [m]_0} & \left\{ \inf_{x \in \mathcal{X}} \left\{ \Gamma \theta^k(x) + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \sup\{0, \theta^i(x) - \theta^k(x) \} \right\} \right\}, \\
\end{split}
\end{align}
where $\theta^k(x) := \sup_{u^k \in \mathcal{U}_k} f_k(x,u^k) - f_k(x,\overline{u}^k)$ and $\theta^0(x) := 0$. 
%Note that % The only difference between problems~\eqref{Prob:GammaCombCounterpartWithoutFenchel} and \eqref{Prob:GeneralGammaCounterpartWithoutDual} is that one can not apply Fenchel's Inequality. However, due to definition, $\theta^k(x) \geq 0$. In other words: 
%the only difference between \eqref{Prob:GeneralGammaCounterpartWithoutDual} and \eqref{Prob:GammaCombCounterpartWithoutFenchel} is that in the general case, Proposition~\ref{Prop:GeneralPrinciple} could not be applied (which results in the lack of variables $v^i$) and $\max_{u^k \in \mathcal{U}_k} f_k(x,u^k) - f_k(x, \overline{u}^k)$ still needs to be solved. We include an example of this case in Subsection~\ref{Subsec:Non-Concave}.
\end{lemma}
\begin{proof}
Since $\Gamma \in [m]$, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to \eqref{Prob:GeneralReModel}. Since for all $i \in [m]$, $p_i$ only occurs in exactly one inequality, we obtain
\begin{gather}\label{Eq:optimal_p}
p^*_i = \sup \{0, \sup_{u^i \in \mathcal{U}_i} f_i(x^*,u^i) - f_i(x^*, \overline{u}^i) )- \theta^* \} \ \forall i \in [m]
\end{gather}
for an optimal solution $(x^*,p^*,\theta^*)$ of~\eqref{Prob:GeneralReModel}. Inserting equation~\eqref{Eq:optimal_p} into the objective function of \eqref{Prob:GeneralReModel} results in 
\begin{align}\label{Eq:piecewiselinearlem}
 \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \sup \{0, \sup_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i) ) - \theta \}.
\end{align}
Since $\eqref{Eq:piecewiselinearlem}$ is convex and piecewise linear in $\theta$, either $\theta^*=0$ or %Next, we prove that either $\theta^* = 0$ or there exists $k \in [m]$ such that
%\begin{gather}\label{Eq:OptimalTheta}
$\theta^* = \theta^k(x)$ %\max_{u^k \in \mathcal{U}_k} f_k(x^*,u^k) - f_k(x^*,\overline{u}^k)$
%\end{gather}
for one $k \in [m]$.  %Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, the minimum is furthermore obtained either at $0$ or 
%Assume that $(x,v^1, \dots, v^m, \theta)$ is feasible and that $\theta$ is equal to 0 nor does it fulfill equation~\eqref{Eq:OptimalTheta} for any $k \in [m]$. Thus, the sets
%\begin{align*}
%S^{<}&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k)  < \theta\} \text{ and } \\
%S^>&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) > \theta\}
%\end{align*}
%are a partition of $[m]$, i.e., $S^< \cup S^> = [m]$ and $S^< \cap S^> = \emptyset$. The objective can be rewritten as:
%\begin{alignat*}{2}
%&\Gamma\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} \left( -f_k(x,v^k) + \support{k} - \theta \right) \\
%&= (\Gamma - |S^>|)\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} -f_k(x,v^k) + \support{k}. 
%\end{alignat*}
%We consider different cases for $S^>$:
%\begin{itemize}
%\item[\underline{First case:}] $S^> = \emptyset$. \\
%In this case, $S^< = [m]$. The solution $(x,v^1, \dots, v^m, \overline{\theta})$ with
%\begin{gather*}
%\overline{\theta} := \max_{k \in [m]} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) 
%\end{gather*}
%has a better objective value than $(x,v^1, \dots, v^m, \theta)$, since $\overline{\theta} < \theta$.
%\item[\underline{Second case:}] $S^> = [m]$.\\
%In this case, 
%\begin{gather*}
%0 \leq \theta < f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) \ \forall k \in [m].
%\end{gather*}
%We set $
%\overline{\theta} := \min_{k \in [m]} (\overline{u}^k)^Tv^k + \delta^*({A^k}^Tv^k \mid \mathcal{Z}_k) - f_k(x,\overline{u}^k) - f_k(x,v^k) $
%
%and since $\Gamma \in [m]$, the objective value of $(x,v^1, \dots, v^m, \overline{\theta})$ is at most the objective value of $(x,v^1, \dots, v^m, \theta)$. 
%\item[\underline{Third case:}] $S^> \neq \emptyset, [m]$. \\
%In this case, there exist $k,l \in [m]$, such that \begin{align*}
%&f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k} < \theta \\
%&< f_l(x,\overline{u}^l) - f_l(x,\overline{u}^l) - f_l(x,v^l) + \support{l}.
%\end{align*}
%In particular, it can be assumed without loss of generality that 
%\begin{gather*}
%k= \mathrm{argmax}_{i \in S^<} \theta - f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i}, \\
%l= \mathrm{argmin}_{i \in S^>} f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i} - \theta.
%\end{gather*} 
%We set 
%\begin{gather*}
%\overline{\theta}:= \begin{cases} f_l(x,\overline{u}^l) + \support{l} - f_l(x,\overline{u}^l) - f_l(x,v^l), & \text{if $|S^>| > \Gamma$,} \\
%\max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}, & \text{otherwise.}
%\end{cases}
%\end{gather*} 
%%and otherwise, set
%%\begin{gather*}
%%\overline{\theta}:= \max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}.
%%\end{gather*}
%In both cases, we obtain a feasible solution with a better objective.
%\end{itemize} 
%We define
%\begin{gather*}
%\theta^k(x,v^k) := f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k - f_k(x,\overline{u}^k) - f_l(x,v^k) + \support{k}
%\end{gather*}
%for $k \in [m]$ and $\theta^0 := 0$. 
%Thus, the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%\begin{alignat*}{2}
%\min_{k \in \{0, \dots, m\}} & \min_{x \in \mathcal{X}} \Gamma \theta^k(x) + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, \theta^i(x)- \theta^k(x) \}. 
%%\text{s.t.} & x \in \mathcal{X}. \\
%\end{alignat*}
%Finally, by application of Fenchel's inequality (cf. \cite{ConvexAnalysis}, Chapter 12) and Assumption~\ref{Ass:General}, (iii) $\theta^k(x,v^k) \geq 0$ is redundant since 
%%$\theta^0(x,v^0) = 0$ by definition and for $k \in [m]$, 
%\begin{gather*}
%\support{k} \geq 0 \Leftrightarrow \exists \zeta \in \mathcal{Z}_k: \ \zeta^T({A^k})^Tv^k \geq 0.
%\end{gather*}
\end{proof}
%As an application, we demonstrate the formulation of Lemma~\ref{Rem:NoFenchel} for Example~\ref{Ex:VRP}. 
\subsection{Concave Uncertainties} \label{subsec:Concave}
%Until now, we have made no assumptions about $f_i$ or
%$\mathcal{U}_i$. 
In this subsection, we will focus on programs that fulfill the following assumptions:
\begin{assumption}\label{Ass:General}
For $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} and for all $i \in [m]$ we assume:
\begin{itemize}
\item[(i)] There is a nominal scenario $\overline{u}^i \in \R^{L_i}$, a matrix $A^i \in \R^{L_i \times m_i}$ and a convex set $\mathcal{Z}_i \subseteq \R^{m_i}$, such that $
\mathcal{U}_i = \{\overline{u}^i + A^i \zeta^i\mid \ \zeta^i \in
\mathcal{Z}_i\}$, i.e., $\mathcal{U}_i$ is an affine transformation of a convex set (and thus, convex).
\item[(ii)] The uncertainty of $f_i$ is concave (we recall that this definition implies that $f_i(x,\cdot): \mathcal{U}^i \to \R$ is concave for every $x \in \mathcal{X}$).
\item[(iii)] The nominal scenario $\overline{u}^i$ is contained in the relative interior of $\mathcal{U}_i$.
\end{itemize}
\end{assumption}
%Since convex sets stay convex under affine-linear transformations,
%(i) implies that $\mathcal{U}^i$ is convex.
Convexity of the uncertainty set (i) is a typical assumption in robust optimization, see \cite{RobustBook}. 
%Furthermore, we note that $0 \in \mathcal{Z}_i$ implies $\overline{u}^i \in \mathcal{U}^i$ which is, again, a straight-forward assumption. 
%We note that, iwf $f_i(x,u^i)$ is \emph{convex} in $x$, (i) can be assumed without loss of generality; for more details, see 
%\todo[inline][inline]{Dennis: Ben-Tal nachlesen}
Assumptions (ii) and (iii) are required to apply the techniques from \cite{Fenchel}. To this end, we need some tools of convex analysis:
\begin{definition}
Let $\mathcal{X} \subseteq \R^n$ and $\mathcal{A} \subseteq \R^m$ be a convex set. Let $f \colon \mathcal{X} \times \mathcal{A} \to \R, \ (x,a) \mapsto f(x,a)$ be a function that is concave in $a$ for every $x \in \mathcal{X}$. For an arbitrary, but fixed $x \in \mathcal{X}$, the function
\begin{alignat*}{4}
f_{*}(x, \cdot) \colon & \R^n & \to & \ \R \cup \{-\infty\}, \\
& a & \mapsto & \inf_{y \in \mathcal{A}} \{a^Ty - f(x,y)\}
\end{alignat*}
is called the (partial) concave conjugate with respect to $a$. For a non--empty set $\mathcal{S} \subseteq \R^n$, the function
\begin{alignat*}{4}
\delta^*(\cdot \mid \mathcal{S})  \colon & \R^n & \to & \ \R \cup \{\infty\}, \\
& x & \mapsto & \sup_{y \in \mathcal{S}} y^Tx
\end{alignat*}
is called the support function of $\mathcal{S}$.
\end{definition}
%\begin{remark}
%With our notation, we aim to stay close to the notation of \cite{Fenchel}. For example, $\delta^*(\cdot \mid \mathcal{S})$ is the \emph{convex conjugate} of the indicator function. Since we do not require the exact definition of convex conjugates or indicator functions, we neglect them in this paper. For more details, see \cite{Fenchel} or \cite{ConvexAnalysis}.
%\end{remark}
%\todo[inline][inline]{Dennis: Proper definitions...}
The main result of \cite{Fenchel} is the following reformulation:
\begin{prop}(\cite{Fenchel}, Theorem 2)\label{Prop:GeneralPrinciple}
Under Assumption~\ref{Ass:General}, inequality
\begin{gather*}
\sup_{u^i \in \mathcal{U}_i} f_i(x,u^i) \leq 0
\end{gather*}
is satisfied if and only if there is a vector $v^i \in \R^{L_i}$, such that
\begin{gather}\label{Ineq:GeneralPrinciple}
\left(\overline{u}^i\right)^T v^i + \delta^*((A^i)^Tv^i \mid \mathcal{Z}_i) - f_{i,*}(x,v^i) \leq 0.
\end{gather}
\end{prop}
%\begin{proof}
%See Theorem 2 in \cite{Fenchel}.
%\end{proof}
%Proposition~\ref{Prop:GeneralPrinciple} implies that we can verify
%whether a given $x$ satisfies a given inequality under uncertainty by
%solving a deterministic inequality without uncertainty. Furthermore,
We note that convexity of $f_i$ in $x$ implies that the left-hand side of inequality~\eqref{Ineq:GeneralPrinciple} is also convex, since $\delta^*$ is convex in $v^i$ and $f_{i,*}$ is concave in $(x,v^i)$, see \cite{Fenchel}.\\ By applying Proposition~\ref{Prop:GeneralPrinciple} to
program~\eqref{Prob:GeneralReModel}, we obtain an equivalent reformulation of $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart}: %which is deterministic: 
\begin{corollary}\label{Prop:FenchelGammaCounterpart}
Let $\Gamma \in [m]$. Under Assumption~\ref{Ass:General}, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to %Problem~\eqref{Prob:GeneralReModel} 
\begin{align}\label{Prob:FenchelGammaCounterpart}
\begin{split}
\inf_{x,p,\theta,v^1, \dots, v^m} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i \\
\mathrm{s.t.}\; & x \in \mathcal{X} \\
& p_i + \theta \geq (\overline{u}^i)^Tv^i + \support{i} - f_{i,*}(x,v^i) - f_i(x, \overline{u}^i) \ \forall i \in [m] \\
& p, \theta \geq 0.
\end{split}
\end{align}
%%Furthermore, if $f_i$ is linear in the uncertainty for some $i \in [m]$, i.e., $f_i(x,u^i)={(u^i)}^Tl_i(x)$ for a function $l_i \colon \R^n \to \R^{L_i}$, the inequality constraints of problem~\eqref{Prob:FenchelGammaCounterpart} are equivalent to 
%%\begin{align}\label{Prob:FenchelGammaCounterpartLinear}
%%\begin{split}
%%%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%%%\text{s.t.} & x \in \mathcal{X}, \\
%% p_i + \theta \geq  \supportx{i}\\
%%%& p, \theta \geq 0.
%%\end{split}
%%\end{align}
%%for each $i \in [m]$.
\end{corollary}
\begin{proof}
Since $\Gamma$ is integral, Lemma~\ref{Lem:ReModel} holds. Proposition~\ref{Prop:GeneralPrinciple} implies that for each $i
\in [m]$, 
\begin{gather*}
p_i + \theta \geq ({\overline{u}^i})^Tv^i + \support{i} - f_{i,*}(x,v^i) - f_i(x, \overline{u}^i)
\end{gather*}
is satisfied for $v \in \R^{L_i}$ if and only if 
%\begin{gather*}
$p_i + \theta \geq \sup_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i).$
%\end{gather*}
%which proves the first part of the claim. In the case where $f_i$ is linear in $u^i$, we have
%\begin{gather*}
%f_{i,*}(x,v^i) \neq -\infty \Leftrightarrow v^i = l_i(x),
%\end{gather*} 
%which implies $f_{i,*}(x,l_i(x)) = 0$ \cite{Fenchel}. Since inequality~\eqref{Ineq:GeneralPrinciple} is not fulfilled for $f_{i,*}(x,v^i) = - \infty$, $v^i = l_i(x)$ holds. Inserting this into the inequality constraints of problem~\eqref{Prob:FenchelGammaCounterpart} results in the claim, since $f_i(x, \overline{u}^i) = (\overline{u}^i)^Tl_i(x)$.
%\begin{align*}
%%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%%\text{s.t.} & x \in \mathcal{X}, \\
%p_i + \theta \geq (\overline{u}^i)^Tl_i(x) + \supportx{i} - f_i(x,\overline{u}^i) \ \forall i \in [m]. 
%%& p, \theta \geq 0.
%\end{align*} 
%Since $f_i(x, \overline{u}^i) = (\overline{u}^i)^Tl_i(x)$, the claim follows.
\end{proof}
%\todo{Remark einfädeln als Korollar.}
%\todo{Bemerkung machen, wie sich viele konkave Settings zu linear umformulieren lassen.}
In general, program~\eqref{Prob:FenchelGammaCounterpart} is not compuationally tractable. The support function and the concave conjugate with respect to $v^i$ are optimization programs themselves that depend on a new decision variable $v^i$. In \cite{Fenchel}, the authors derived finite reformulations for various uncertainty sets $\mathcal{U}_i$, including geometries like ellipsoids, polyhedra, cones, boxes, Minkowski sums or their intersections and uncertainty sets that are described by various functions, e.g. convex functions or separable functions and. Their findings can also be applied here. For details, we refer to Tables 1, 2 and 3 in \cite{Fenchel}. 
%In this section, we extend
%Propositions~\ref{Prop:Tractable_Gamma_Comb} and \ref{Prop:Gamma_MIP}
%to more general classes of optimization problems which are subject to
%uncertainty in the objective. For the case of uncertainty in the constraints, we refer to Appendix B. \\
%We first consider 
%\emph{nominal} optimization problems that are of the form
%\begin{align}\label{Prob:GeneralNomOpt}
%\begin{split}
%\min_x & \sum_{i \in [m]} \ \overline{f}_i(x),\\
%\text{s.t.} & \ x \in \mathcal{X}
%\end{split} 
%\end{align}
%where $\overline{f}_i \colon \R^n \to \R$ is an arbitrary, but fixed function for every $i \in [m]$. %In the following, we call problem~\eqref{Prob:GeneralNomOpt} the \emph{nominal problem}. \\
%We assume that every function $\overline{f}_i$ is subject to an
%uncertainty set $\mathcal{U}_i$, i.e., we set %extend $\overline{f}_i$ to 
%\begin{gather*}
%f_i \colon \R^n \times \mathcal{U}_i \to \R
%\end{gather*} 
%with $f_i(x,\overline{u}^i):= \overline{f}_i(x)$ for a nominal
%scenario $\overline{u}^i \in \mathcal{U}_i$. Like in Section 2, we focus on the
%uncorrelated case by assuming that uncertainties of different functions $f_i$ are uncorrelated, i.e., the uncertainty set of $f(x,u) := \sum_{i \in [m]} f_i(x, u^i)$ is $\mathcal{U} := \bigtimes_{i \in [m]} \mathcal{U}_i$.
%Hence the robust counterpart of problem~\eqref{Prob:GeneralNomOpt} reads
%\begin{align}\label{Prob:GeneralStrictOpt}
%\begin{split}
%\min_x & \sum_{i \in [m]} \ \max_{u^i \in \mathcal{U}_i} f_i(x,u^i),\\
%\text{s.t.} & \ x \in \mathcal{X}.
%\end{split} 
%\end{align} 
%An overview over methods for tackling
%problem~\eqref{Prob:GeneralStrictOpt} can be found e.g. in
%\cite{NonlinearRO}. 
%%Future research could consider generalizations of problem~\eqref{Prob:GeneralStrictOpt}
%%by taking correlated uncertainties into
%%account %of each
%%%function $f_i$
%%%are correlated, i.e.,
%%so that the objective under uncertainty reads $\max_{u \in
%% \mathcal{U}} \sum_{i \in [m]} f_i(x,u^i)$.\\ %Here, we aim at
%%generalizing the flexible $\Gamma$-approach for uncorrelated
%%interval uncertainties and leave the correlated case
%%subject to future research. \\
%%In the linear case in Section 2, one attempted to be robust against
%%$\Gamma$ changing coefficients.
%Generalizing the setting from the previous section, we aim to be protected against at most $\Gamma$ functions deviating from their nominal scenario:
%\begin{alignat}{2}\label{Prob:GeneralGammaCounterpart}
%\min_{x \in \mathcal{X}} & \left\{ \max_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} \max_{u^i \in \mathcal{U}_i} f_i(x,u^i) + \sum_{i \in [m] \setminus \mathcal{S}} f_i(x, \overline{u}^i) \right\} \right\}.
%\end{alignat}
%This problem is henceforth called \emph{$\Gamma$--counterpart}. To demonstrate that this generalization is natural, we start by showing that it
%generalizes the linear version \eqref{Prob:Gamma_Comb}.
%% state some applications for which this $\Gamma$--counterpart is a
%%natural robustification, and briefly discuss another possible
%%generalization. 
%\begin{example}\label{Rem:GeneralizeComb}
%For functions $f(x,c) = c^Tx$ with interval uncertainty for every coefficient $c_i$,
%problem~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
%problem~\eqref{Prob:Gamma_Comb}: inserting $ %\begin{gather*}
%n = m, \ \mathcal{U}_i := [\overline{c}_i, \overline{c}_i + \Delta c_i] \ \forall i \in [n], \ f_i(x,c_i) := c_i \cdot x_i \ \forall i \in [n]$ into \eqref{Prob:GeneralGammaCounterpart}, %\end{gather*} 
%one obtains 
%\begin{alignat*}{2}
%\min_{x \in \mathcal{X}} & \left\{ \max_{\mathcal{S} \subseteq [n]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} \max_{c_i \in [\overline{c}_i, \overline{c}_i + \Delta c_i]} c_ix_i + \sum_{i \in [n] \setminus \mathcal{S}} \overline{c}_ix_i \right\} \right\}.
%\end{alignat*}
%If $\mathcal{X} \subseteq \{0,1\}^n$, then
%$\max_{c_i \in [\overline{c}_i, \overline{c}_i + \Delta c_i]} c_ix_i = \overline{c}_i x_i + \Delta c_i x_i
%$  
%and one obtains formulation~\eqref{Prob:Gamma_Comb}.
%\end{example}
%\begin{example}
%The next example covers a case for which the objective is linear but the uncertainty is not only contained in intervals. Let $G = (V,E)$ be an undirected graph with $4$ nodes, i.e., $V = (1,2,3,4)$, and $E=(e, f, g, h)$ with 
%\begin{gather*}
%e := \{1,2\}, \ f := \{2,3\}, \ g:= \{3,4\} \text{ and } h:= \{4,1\}.
%\end{gather*} 
%We aim to obtain a minimal spanning tree of $G$. The nominal cost of the edges is given by $\overline{c}_e = 1- \varepsilon,  \overline{c}_h = 1$, $ \overline{c}_f = 1 - \varepsilon$, $\overline{c}_g = 1$ for a sufficiently small $\varepsilon > 0$ and the nominal problem is $\min_{x \in \mathcal{X}} \overline{c}^Tx$.
%with $x$ denoting the incidence vectors of the resp. spanning tree and $\mathcal{X}:=\{(1,1,1,0)^T, (1,0,1,1)^T, (1,1,0,1)^T, (0,1,1,1)^T\}$ denoting the set of spanning trees of $G$. %It is easy to see that $x^*=(1,1,0,1)$ is the nominal optimum. \\
%The coefficients are assumed to be subject to uncertainty: The costs of $e$ and $f$ are correlated within the ellipsoidal uncertainty set% While the costs for $g$ are $\mathcal{U}_g := [1,1.5]$, the costs for $e$ and $f$ are correlated:
%\begin{gather*}
%\mathcal{U}^{e,f}:= \begin{pmatrix} 1 - \varepsilon,  1-\varepsilon \end{pmatrix}^T + \{c \in \R^2: \ c_e^2 + c_f^2 \leq 1\}.
%\end{gather*}
%The costs of $g$ and $h$ are uncorrelated and within the interval uncertainty set $\mathcal{U}^{g} = \mathcal{U}^h:= [1,2]$.
%The $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is  given by
%\begin{gather}\label{Prob:GammaSpanningTree}
%\min_{x \in \mathcal{X}} \left\{ \max_{\mathcal{S} \subseteq \{\{e,f\}, g,h\}, |\mathcal{S}| \leq \Gamma} \left\{ \sum_{I \in \mathcal{S}} \max_{(c_{I_1}, c_{I_2}) \in \mathcal{U}^I} c_{I_1}x_{I_1} + c_{I_2}x_{I_2} + \sum_{I \in \{\{e,f\}, g,h\} \setminus \mathcal{S}} {\overline{c}_{I_1}}x_{I_1} + {\overline{c}_{I_2}}x_{I_2} \right\} \right\}.
%\end{gather}
%Application of Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} results in $x^* = (1,1,0,1)$ being the robust optimal solution for $\Gamma = 1,2$ in the unique optimal solution $(e,g)$ for both $\Gamma = 1$ and $\Gamma = 2$. \\
%For $\Gamma = 1$, the objective values of the incidence vectors are given in Table~\ref{TableSpanningTree}. The optimal solutions are thus given by $(1,1,1,0)$ and $(0,1,1,1)$.
%\begin{table}[H]
%\centering
%\caption{Objective values for the feasible solutions problem~\eqref{Prob:GammaSpanningTree} for $\Gamma = 1.$\label{TableSpanningTree}}
%\begin{tabular}[c]{|l|l|}
%\hline
%Incidence vector & Objective Value \\ \hline
%$(1,1,1,0)$ & $4 - \varepsilon$\\ \hline
%$(1,1,0,1)$ & $3 - 2 \varepsilon + \sqrt{2}$\\ \hline
%$(1,0,1,1)$ & $3 - 2 \varepsilon + \sqrt{2}$ \\ \hline
%$(0,1,1,1)$ & $4 - \varepsilon$ \\ \hline
%\end{tabular}
%\end{table}
%robust optimal solutions would be
%$(1,0,1,1)$ and $(0,1,1,1)$ with optimal value $4 - \varepsilon$. However, $(1,1,0,1)$ or $(1,1,1,0)$ would be strictly worse, because
%\begin{gather*}
%\max_{(c_e,c_f) \in \mathcal{U}^{e,f}} c_e + c_f = \sqrt{2}.
%\end{gather*}
%and thus, the objective value is $3 - 2 \varepsilon + \sqrt{2} > 4 - \varepsilon$ for $\varepsilon \in (\sqrt{2} - 1, 1)$. 
%Since the uncertainty set is not a pure interval uncertainty set, one can not apply Proposition~\ref{Prop:Tractable_Gamma_Comb}.  However, if we replace $\mathcal{U}^{e,f}$ with the uncertainty sets $\mathcal{U}^e = \mathcal{U}^f := [1-\varepsilon,2 - \varepsilon]$ for $c_e$ and $c_f$, one obtains that for each $\Gamma = 1,2,3,4$, the optimal solution of problem~\eqref{Prob:Gamma_Comb} would be $(1,1,1,0)$ and $(1,1,0,1)$. However, these are exactly the solutions which are \emph{not} optimal for problem~\eqref{Prob:GammaSpanningTree} for $\Gamma = 1$. Consequently, in general, ignoring correlations can lead to too conservative solutions.
%\todo[inline]{Die genauen Berechnungen könnte man in den Appendix stecken oder dem Lesen überlassen. Ich finde nicht, dass das hier einen Mehrwert darstellt. Man könnte hier noch graphisch den Baum und die Unsicherheitsmengen darstellen zum besseren verständnis.}
%\end{example}
%\begin{example}\label{Ex:Scheduling}
%We consider a single-machine scheduling problem: A set of $m$ jobs
%$\mathcal{J}$ has to be scheduled on a single machine. The machine
%requires a \emph{processing time} $\overline{p}_j \in \R_{\geq 0}$ for finishing job $j \in \mathcal{J}$ without preemption. With $C_j(x,\overline{p})$ we denote the completion time of job $j$ which depends on the actual schedule $x$ and on the processing time $\overline{p}:=(\overline{p}_j)_{j \in \mathcal{J}}$. With $\mathcal{X}$, we the
%set of feasible schedules:
%\begin{gather*}
%\mathcal{X} := \{x \in \{0,1\}^{[m] \times \mathcal{J}}: \sum_{i \in [m]} x_{i,j} = 1 \ \forall j \in \mathcal{J}, \ \sum_{j \in \mathcal{J}} x_{i,j} = 1 \ \forall i \in [m] \}.
%\end{gather*}
%Assuming that every job $j$ is weighted with a weight $w_j \in \R_{\geq 0}$, we aim to minimize the weighted total completion time:
%\begin{gather}\label{Prob:WeightedScheduling}
%\min_{x \in \mathcal{X}} \sum_{j \in \mathcal{J}} w_j C_j(x,\overline{p}).
%\end{gather} 
%If $w_j = 1 \ \forall j \in \mathcal{J}$, 
%problem~\eqref{Prob:WeightedScheduling} is equivalent to
%\begin{gather}\label{Prob:UnWeightedScheduling}
%\min_{x \in \mathcal{X}} \sum_{j \in \mathcal{J}} \overline{p}_j \sum_{i \in [m]} (m+1-i)x_{i,j},
%\end{gather}
%where
%\begin{gather*}
%x_{i,j} = \begin{cases} 1, & \text{job $j$ is scheduled at position $i$},\\
%0, & \text{otherwise}. \end{cases}
%\end{gather*}
%Now, we assume for each job $j$ that the processing time $p_j$ is subject to
%uncorrelated uncertainty $\mathcal{U}_j=[\overline{p}_j,
% \overline{p}_j + \Delta p_j]$. Although the objective of
%\eqref{Prob:UnWeightedScheduling} is linear in $p$ and in $x$, one
%cannot simply apply Proposition~\ref{Prop:Tractable_Gamma_Comb}: While the uncertainties are not correlated for the different jobs $j \in \mathcal{J}$, they are correlated for the schedules: If $\overline{p}_j$ is subject to uncertainty, the variables $x_{i,j}$ are influenced for all $i \in [m]$, while in the setting of
%Proposition~\ref{Prop:Tractable_Gamma_Comb}, an uncertainty influences exactly one variable. Applying Proposition~\ref{Prop:Tractable_Gamma_Comb} that assumes uncorrelated
%uncertainties, could therefore result in an overly conservative reformulation. 
%\\
%The $\Gamma$--counterpart introduced in this section can be applied,
%and reads 
%\begin{gather*}
%\min_{x \in \mathcal{X}} \sum_{j \in \mathcal{J}} \overline{p}_j \sum_{i \in [m]} (m+1-i)x_{i,j} + \max_{\mathcal{S} \subseteq \mathcal{J}: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{j \in \mathcal{S}} \Delta p_j \sum_{i \in [m]} (m+1-i)x_{i,j} \right\}.
%\end{gather*}
%\end{example}
%
%\begin{example}\label{Ex:VRP}
%Logistics problems involving deliveries within given time windows can be modeled as combinatorial optimization problems with non-linear objective functions. As an example, consider taxi routing, delivery of goods or patient transports. These three cases have in common that on the one
%hand, being on time is important for the satisfaction of the customers.
%On the other hand, it usually is not problematic if a
%vehicle arrives too early for a pick-up. \\
%Therefore, by ignoring earliest arrival times, a job $i$ shall be
%finished until a point in time $b_i \in \R$.
%If it is finished after $b_i$, penalty costs occur. A
%model for (unweighted) penalty cost that are linear in the distance
%from $b_i$ is given by
%\begin{align}\label{Prob:BoundNom}
%\begin{split}
%\min_{x \in \mathcal{X}} & \ \sum_{i \in [m]} \max\{0,x_i - b_i\}.
%\end{split}
%\end{align} 
%We note that such tasks may arise in transportation logistics, for
%example as a special case of Vehicle
%Routing Problems with Soft Time Windows, see \cite{VRPSTW}. They
%also occur in energy contexts, see e.g. Chapter 4 in
%\cite{Probust}. \\
%We now assume that the time windows are uncertain. %, i.e., $b$ is
%subject to uncertainty.
%Assuming that $b_i \in \mathcal{U}_i := [\overline{b}_i - \Delta b_i, \overline{b}_i + \Delta b_i]$ for some nominal scenario $\overline{b}_i$ and a perturbation $\Delta b_i$, the $\Gamma$--counterpart is given by
%\begin{align}\label{Prob:UncertainBounds}
%\begin{split}
%\min_{x \in \mathcal{X}} & \ \max_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \sum_{i \in \mathcal{S}} \max\{0,x_i - \overline{b}_i + \Delta b_i\} + \sum_{i \in [m] \setminus \mathcal{S}} \max\{0, x_i - \overline{b}_i\}. 
%\end{split}
%\end{align}
%\end{example}
%\begin{example}\label{Ex:QAP}
%The Quadratic Assignment Problem as considered in \cite{QAP2015}
%models the process of assigning $n \in \mathbb{N}$ facilities to $n$
%locations. For each pair of facilities $i$
%and $j$, $(i,j) \in [n]^2$, the amount $c_{ij}$ of exchanged goods
%between $i$ and $j$ is given. Furthermore, the distance $d_{rs}$ between
%two locations $r, s \in [n]$, is given as well. %The material handling costs between the facilities, given the flow i.e., the amount of goods transported between two facilities and the distance between two locations should be minimized.
%$c_{ij}$ is the flow between the facilities $i$ and $j$, $(i,j) \in [n]^2$ and $d_{rs}$ is the distance between the locations $r$ and $s$, $(r,s) \in [n]^2$.
%
%The task is to minimize the cost for transportation which is defined as the product of the amount of material which is transported between two facilities and the distance between the corresponding locations.
%We introduce binary variables $x_{ir}$ to indicate whether facility $i$ is positioned at location $r$:
%\begin{align*}
%x_{ir} = \left\{
%\begin{array}{ll}
%1, & \text{if facility } i \text{ is located at }r, \\
%0, & \, \text{otherwise.} \\
%\end{array}
%\right.
%\end{align*}
%To ensure that each facility is assigned to exactly one location and that for every location, exactly one facility is assigned, we define the feasible region $\mathcal{X}$ as:
% \[\mathcal{X} = \left\{x \in \{0,1\}^{[n]^2}: \sum_{i\in [n]} x_{ir}= 1 \quad \forall r \in [n], \sum_{r \in [n]} x_{ir}=1 \quad \forall i \in [n]\right\}.\]
%We seek protection against uncertainties in $c_{ij}$ for all $(i,j)\in [n]^2$ that is modeled by a perturbation of at most $\Delta c_{ij}$, e.g. $c_{ij} \in \mathcal{U}_{ij} = [\bar{c}_{ij}, \bar{c}_{ij}+ \Delta c_{ij}]$.
%With the uncertainty set $\mathcal{U} := \bigtimes_{(i,j)\in [n]^2} \mathcal{U}_{ij}$ the %resulting optimization problem can be modeled as
%\begin{align*}
%\min_{x\in \mathcal{X}} \max_{c \in \mathcal{U}}  \sum_{i=1}^n \sum_{j=1}^n \sum_{r=1}^n \sum_{s=1}^n c_{ij} d_{rs}x_{ir}x_{js}.
%\end{align*}
%Using the flexible $\Gamma$-approach as in the setting of Problem~\eqref{Prob:GeneralGammaCounterpart} the $\Gamma$--counterpart is given by:
%\begin{align}\label{Prob:QAP_RobCP}
%\begin{split}
%&\min_{x\in \mathcal{X}} \sum_{(i,j,r,s) \in [n]^4} \bar{c}_{ij}d_{rs}x_{ir}x_{js} + \max_{\mathcal{S} \subseteq [n]^2:|\mathcal{S}|\le \Gamma}  \sum_{(i,j)\in \mathcal{S}}  \sum_{(r,s)\in [n]^2} \Delta \bar{c}_{ij} d_{rs}x_{ir}x_{js} .
%\end{split}
%\end{align}
%We note, that since the objective is quadratic the reformulations from \cite{IntroGamma} can not be used.
%\end{example}
%
%\begin{example}\label{SFB}
%Assume that for a set of $m$ objects $O_1, \dots, O_m$, e.g., particles, each shall be characterized by an $n$-dimensional data set comprised of attributes $A_1,A_2,\dots,A_n, n \geq 2$, that are measured in
%practical experiments. 
%\begin{table}[H]
%    \centering
%    \begin{tabular}{l|c|c}
%         & Object $O_1$ & Object $O_2$  \\
%     $A_1$   &  & \\
%     $A_2$ (weight)     & & 
%    \end{tabular}
%    \caption{Values of attributes of objects}
%    \label{tab:my_label}
%\end{table}
%%Attributes may for example be weights or different diameters \todo[inline][inline]{Durchmesser von...?}. 
%\todo[inline][inline]{...Goal: TABELLE FÜLLEN!!! Problemaufzählung: Warum geht das nicht so einfach? Simultane Messung und nur k Attribute und Messungenauigkeiten. Was ist das nominalle Problem? [HYPERGRAPHEN] (Formulierung der Tabellenfüllung). Was ist das robuste Problem, also wo kommt die Unsicherheit mit rein?} 
%However, often one cannot measure all
%attributes simultaneously, but only a limited number $k < n$ of these. \todo[inline][inline]{Beispiel: Referenz?}
%The goal is the reconstruction of the values of $A_1, A_2, \dots, A_n$ for each object from these $k$-dimensional measurements. We assume that we conduct $N \in \mathbb{Z}_{\geq 0}$ measurements. %Through one measurement the values of $k$ attributes are determined. \todo[inline]{immer die gleichen?}
%The result of measurement $j \in [N]$ are $m$ $k$-tuples of values, one for each object $o$, denoted as $a^o_j \in \R^k$. We note that this is a slight abuse of notation, we note that due to the simultaneous measurement, we do not know which tuple $a^o_j$ belongs to which of the objects $O_1, \dots, O_m$. %w%hile $a^i_j$ has $m$ entries, after a measurement we do not know which value for attribute $i$ belongs to which object. But for one measurement $j \in [N]$  %$A_i$ For measurement $M_i$, the  We order the measurements so that $A_i, \ldots, A_{i+k}$ are determined at measurement $M_i$ for $i \in [n]$. \todo[inline]{Was ist denn Attribut $A_{n+k}$? Sollte man hier nicht vielleicht besser mit Subindizes arbeiten, also $A_{i_k}$?}
%%For each attribute $A_i$ we denote the vector that contains all
%%values of $A_i$ as $a^i$. 
%%\todo[inline]{koennen wir hier nicht
%%  noch in k Messungen arbeiten? Es muss auch noch erklaert werden dass wir hier der Einfachheit halber annehmen dass keine Messung doppelt vorkommt, oder? Warum werden hier die Hypergraphen genannt? Spielen spaeter keine Rolle mehr... ich faende es gut wenn es hier im Text noch in k-Tupeln erklaert waere, und bei den Formeln reduziert man es auf k=2. welches Optiierungsproblem steckt dahinter wenn man k Messungen hat, ist es ein Hypergraph Matching in einem Graphen der jeweils Hyperkanten aus k Knoten hat? das sollte auch so erklaert werden, finde ich. es sollte dann auch am Ende dazugesagt werden was bei k > 2 das Optimierungsproblem ist. Ich hatte schon gemutmasst dass
%%es sich um ein polynomiales Optimierungsproblem mit Monomen der Laenge k handelt - ist das korrekt? sollte auch mit gesagt werden, am schluss koenntest du wieder allgemeiner werden und sagen (im Text) dass im Allgemeinen bei k > 2 ein XYZ Optimierungsproblem entsteht.}
%If two measurements $j_1, j_2 \in [N]$ determine the same attribute $A_i$, $i  \in [n]$ and if two tuples $a^{(o_1,j_1)}$ and $a^{(o_2,j_2)}$ share the value of an attribute $A_i$, the tuples belong to the same particle. Thus, the values of the shared attribute are the same. Therefore, we aim to combine these tuples. % that contain the same or an equal value for the common attribute. 
%%Note that we need to conduct at least $N \geq \frac{n-1}{k-1}$ to ensure that there exists a relation through these tuples between all measurement. 
%%However, if a measurement determines attributes that in no other measurement are determined no relation can be found.% Therefore we need at least $\frac{n-1}{k-1}$ measurements to find a tuple of all $n$ attributes. 
%% For a better understanding, we want to model the problem as a matching on a
%%hypergraph. Each node of the graph represents a tuple of values that are determined in a measurement. An edge between those nodes only exists if both tuples 
%%belong to the same object. We aim to find edges that connect $\frac{n-1}{k-1}$
%%nodes. Two connected nodes cannot be output
%%of the same measurement.
%%If $n=2$ and $k=1$ the resulting optimization problem is an assignment problem. \todo[inline][inline]{Referenz auf die assignment Struktur des Schedulings und des Assignment Problems?}
%%For $n>2$ a multidimensional assignment problem has to be
%%solved. 
%\todo[inline][inline]{WAS IST DAS OPTIMIERUNGSPROBLEM??? NOMINELL????}
%For avoiding issues regarding notation, we formulate the resulting optimization problem for $m=5$ objects with $n=4$ attributes for which we conduct $N = 3$ measurements which measure $k = 2$ attributes. 
%From each measurement we obtain a binary vector, indicating if two values belong to the same particle. \todo[inline][inline]{aber gehören nicht Attribute zu einem Partikel....?} %Those vectors are given through the measurements and are no decision variables.  \todo[inline][inline]{Der Satz kann weg. Man muss den Text glaub ich nur verständlicher aufschreiben. Du schreibst an vielen Stellen etwas von Knoten/Kanten/Tupeln/Vektoren ohne die Strukturen notatiostechnisch wirklich zu benutzen. Das sollten wir mal diskutieren.}
%%\begin{align*}
%%&\nu^1_{ij} = \left\{
%%\begin{array}{ll}
%%1, & \text{if in }M_1\text{ a pair } \ a^1_{i} \in a^1 \text{ and }a^{2}_{j} \in a^{2}, (o_1,o_2)\in [m]^2 \text{ was determined}, \\
%%0, & \, \text{otherwise} \\
%%\end{array}
%%\right.
%%\end{align*} \todo[inline][inline]{Hier stimmt was nicht: oben sind die $a^i$ noch Vektoren und hier haben die Vektoren auf einmal elemente?}
%%\begin{align*}
%%&\nu^2_{jk} = \left\{
%%\begin{array}{ll}
%%1, & \text{if in }M_2\text{ a pair } \ a^2_{j} \in a^2 \text{ and }a^{3}_{k} \in a^{3}, (j,k)\in [m]^2 \text{ was determined}, \\
%%0, & \, \text{otherwise} \\
%%\end{array}
%%\right.
%%\end{align*}
%%\begin{align*}
%%nu^3_{kr} = \left\{
%%\begin{array}{ll}
%%1, & \text{if in }M_3\text{ a pair } \ a^3_{k} \in a^k \text{ and }a^{4}_{r} \in a^{4}, (k,r)\in [m]^2 \text{ was determined}, \\
%%0, & \, \text{otherwise} \\
%%\end{array}
%%\right.
%%\end{align*}
%%\todo[inline][inline]{Ich finde es unschön, wenn $k=4$ und dann $k$ auf einmal ein Laufindex ist...}
%%The aim is to find tuples of values $(a_i^1, a_j^2, a_k^3, a_r^4)$ that belong to one object. 
%Our decision variables are binary variables indicating which
%values belong to the same particle: 
%\todo[inline][inline]{$x_{(o_j, l_i),....} \in j \in [m] \times [N]$}
%\begin{align*}
%&x_{(o_1,j_1), \dots, (o_n,j_n)} = \left\{
%\begin{array}{ll}
%1, & \text{if there is an object with } (a^1_{i}, a^2_{j},a^3_k, a^4_{r}),(i,j,k,r)\in[m]^4 \\
%0, & \, \text{otherwise}. \\
%\end{array}
%\right.
%\end{align*}
%\todo[inline][inline]{Dann kann man die Variable schon direkt bei der Def. der Tupel definieren? Wenn dann schon klar ist, was wir eigentlich optimieren wollen...}
%%For ease of exposition, we assume that if for two particles the same value of an attribute is measured this value is listed two times in the vector. So no tuple has to be assigned to two particles.
% We thus determine $x \in
%\mathcal{X}$ with 
%\begin{align*}
%\mathcal{X}=\left\{x \in \{0,1\}^{4m}: \right. & \left. \sum_{(j,k,r) \in [m]^3} x_{ijkr} =1 \quad \forall i \in [m],
% \sum_{(i,k,r) \in [m]^3} x_{ijkr} =1 \quad \forall j \in [m],\right.\\
%&\left. \sum_{(i,j,r) \in [m]^3} x_{ijkr} =1 \quad \forall k \in [m], \sum_{(i,j,k) \in [m]^3} x_{ijkr} =1 \quad \forall r \in [m] \right\}.
%\end{align*} 
%\todo[inline][inline]{ab hier stiege ich leider komplett aus....}
%If we want to assign the values $(a_i^1, a_j^2, a_k^3, a_r^4)$ to one particles we have to make sure the pair $(a^1_i,a^2_j)$ was determined in $M_1$, $(a^2_j,a^3_k)$ was determined in $M_2$ and $(a^3_k,a^4_r)$ was determined in $M_3$.
%The deviation of $a_j^2$ and its measured values in $M_1$ and $M_2$ for one tuple $(a_i^1, a_j^2, a_k^3, a_r^4)$ can be determined through the binary vectors $y^1$ and $y^2$ as:
%\[ \left|a^{2}_{j}-\sum_{l \in [m]}a^{2}_{l}y^1_{il}\right|+\left|a^{2}_{j}-\sum_{l \in [m]}a^{2}_{l}y^{2}_{lk}\right|.\]
%Note that $\sum_{l \in [m]}y^{s}_{lk} = 1 \ \forall s \in [1,2,3], k \in [m]$.
%Since we have to consider this difference also for $a^3_k$ we define
%the sum of the differences of $a^2_j$ and $a^3_k$:
%\[c_{ijkr} = \left|a^{2}_{j}-\sum_{l \in [m]}a^{2}_{l}y^1_{il}\right|+\left|a^{2}_{j}-\sum_{l \in [m]}a^{2}_{l}y^{2}_{lk}\right|+ \left|a^{3}_{k}-\sum_{l \in [m]}a^{3}_{l}y^3_{jl}\right|+\left|a^{3}_{k}-\sum_{l \in [m]}a^{3}_{l}y^{4}_{lr}\right|. \]
%This difference should be minimized.
%We also assume that there might be inaccuracies in the measurement. So
%it is possible that the measured values of the attributes might
%vary. Therefore $c_{ijkr}$ is uncertain with $c_{ijkr} \in \mathcal{U}_{ijkr} = [\bar{c}_{ijkr}, \bar{c}_{ijkr} + \Delta c_{ijkr}]$. The resulting robust counterpart can be written as:
%% \todo[inline]{von was?hier steht ja noch gar nichts von robustheit...} problem is a multidimensional assignment problem: 
%\begin{align*}
%\min_{x\in \mathcal{X}} \sum_{(i,j,k,r) \in [m]^4} x_{ijkr} +
%\max_{\mathcal{S}\subseteq [m]^4: |\mathcal{S}|\le \Gamma} \left\{\sum_{(i,j,k,r) \in \mathcal{S}} \max_{c_{ijkr} \in\mathcal{U}_{ijkr}} c_{ijkr} + \sum_{(i,j,k,r) \in [m]^4 \setminus \mathcal{S}} \bar{c}_{ijkr} \right\}.
%\end{align*}
%\todo[inline][inline]{Das Optimierungsproblem, kann das so stimmen? 1. Ist das innerste Maximum klar und du hast das glaube ich bei der leztten Summe schon verwendet. Zweitens, wenn sich die Koeffizienten deterministich aus den $a_{blubb}$ zusammensetzen, 3. Warum minimieren wir über die $x$? Deine zulässige Menge heißt doch: Für jede Messung muss es ein Objekt geben, was diese Attrbute hat, oder nicht? 4. Das x und das c haben keinen Zusammenhang, man könnte das große Maximierungsproblem direkt rausziehen! Also müssten doch die $a_i$ unsicher sicher sein? Da ist irgendwo ein Wurm drin. Oder das Problem ist doch ne Spur zu konstruiert....}
%With that we can find correlations for different attributes, even if
%the measurements might be inaccurate.
%\end{example}
%
%%%Example~\ref{Rem:GeneralizeComb} shows that the $\Gamma$--counterpart
%%is a possibility for generalizing model~\eqref{Prob:Gamma_Comb} to
%%mixed-integer nonlinear optimization problems. We furthermore would like to point out that Proposition~\ref{Prop:Tractable_Gamma_Comb} is only applicable in the case of interval uncertainty and, in particular, uncorrelated uncertainty - for more details, see Appendix A.
%\begin{remark}
%Our application of the flexible $\Gamma$-approach is only one possible
%extension of the approach of \citep{IntroGamma}. One could also assume
%that, for each function $f_i(x,u^i)$ with $u^i \in \R^{L_i}$, we would
%like to be robust against at most $\Gamma_i$ many uncertain
%coefficients. In formulas, this corresponds to 
%\begin{gather}\label{Prob:GeneralizationII}
%\min_{x \in \mathcal{X}} \sum_{i \in [m]} \max_{\mathcal{S} \subseteq [L_i], |\mathcal{S}| \leq \Gamma_i} \max_{u^i \in \mathcal{U}_{\mathcal{S}^{i}}} f_i(x,u^i)
%\end{gather}
%where 
%\begin{gather*}
%\mathcal{U}_S^{i}:= \{u^i \in \mathcal{U}^i: \ u_j^i = \overline{u}_j^i \ \forall j \notin S\}.
%\end{gather*}
%This approach would only technically be a generalization of the
%$\Gamma$--counterpart introduced in \cite{IntroGamma} as well, since in
%this case, one could set for the special case $f_i(x,u) = u^Tx$, i.e., $m = 1$ and $L_1 = n$ with only one $\Gamma$. 
%%Furthermore, for separable functions
%%$f_i(x,u^i) = g_i(u^i)h_i(x)$ for some functions $g_i\colon
%%\mathcal{U}_i \to \R$ and $h_i \colon \mathcal{X} \to \R$, it is
%%straightforward to solve the maximization problems, since 
%%\begin{gather*}
%%\max_{S \subseteq [L_i], |S| \leq \Gamma_i} \max_{u^i \in \mathcal{U}_S^{i}} f_i(x,u^i) = \max_{S \subseteq [L_i], |S| \leq \Gamma_i} h_i(x) \max_{u^i \in \mathcal{U}_S^{i}} g_i(u^i).
%%\end{gather*}
%%where the inner maximization problem can be solved
%%analytically\todo[inline]{wer sagt dass das analytisch geloest werden kann,
%%  stimmt das fuer alle fkt g?}.
%Thus, we stay with the
%$\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart}, and a
%discussion about models generalized from~\eqref{Prob:GeneralizationII}
%is possible subject to future research.%only be applicable, when the $f_i(x,u^i)$ are not separable in $x$ and $u^i$, i.e., there are no real-valued functions $g_i$ and $h_i$, such that $f_i(x,u^i) =g_i(u^i)^Th_i(x)$, because in this case, one could assume that..
%%While this approach would still a generalization of the linear case %of Problem~\eqref{Prob:Gamma_Comb} we want to note that $\Gamma_i \in \{0,1\}$  However, if one assumes $f_i(x,u_i) = u_i \cdot x_i$, uneeds to set $m = 1$ and $\Gamma_1 = \Gamma$). However, our $\Gamma$--counterpart seems to be more natural, especially in terms of combinatorial optimization. 
%\end{remark} 
%After having introduced several different applications that motivate the robust counterpart defined here, we next present algorithmically
%tractable reformulations. It turns out that a bottleneck of
%solving~\eqref{Prob:GeneralGammaCounterpart} consists in solving
%\begin{gather*}
%\max_{u^i \in \mathcal{U}_i} f_i(x,u^i)
%\end{gather*} 
%for each $i \in [m]$.
%\begin{lemma}\label{Lem:ReModel}
%If $\Gamma$ is integral, the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%\begin{align}\label{Prob:GeneralReModel}
%\begin{split}
%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%\text{s.t.} & x \in \mathcal{X}, \\
%& p_i + \theta \geq \max_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i) \ \forall i \in [m], \\
%& p \in \R^m_+, \theta \in \R_+.
%\end{split}
%\end{align}
%\end{lemma}
%\begin{proof}
%With the binary variables
%\begin{gather*}
%s_i := \begin{cases} 1, \text{ if $i \in \mathcal{S}$,}\\ 
%0, \text{ otherwise,} \\
%\end{cases} 
%\end{gather*}
%for $i \in [m]$, the inner maximization problem of \eqref{Prob:GeneralGammaCounterpart} is equivalent to
%\begin{align}\label{Prob:LinearOrdering}
%\begin{split}
%\max_{s} & \ \sum_{i \in [m]} f_i(x, \overline{u}^i) + s_i(\max_{u^i \in \mathcal{U}_i} f_i(x, u^i) - f_i(x, \overline{u}^i)), \\
%\text{s.t.} & \ \sum_{i = 1}^m s_i \leq \Gamma, \\
%& s \in \{0,1\}^m.
%\end{split}
%\end{align}
%%This is a binary program with $\sum_{i \in [m]} f_i(x,
%%\overline{u}^i)$ being independent of the decision variable $s$ and a
%%knapsack constraint with equal, unit weights and integral
%%capacity. Thus,
%%we can recycle the proof of
%%Proposition~\ref{Prop:Tractable_Gamma_Comb}:
%Clearly, problem~\eqref{Prob:LinearOrdering} is equivalent to its LP
%relaxation. Its dual is
%\begin{alignat*}{2}
%\min_{p, \theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x, \overline{u}^i) + \sum_{i=1}^m p_i \\
%\text{s.t.} & p_i + \theta \geq \max_{u^i \in \mathcal{U}_i} f_i(x,u^i) - f_i(x, \overline{u}^i) \ \forall i \in [m] \\
%& p, \theta \geq 0.
%\end{alignat*} 
%Inserting this equivalent reformulation into problem~\eqref{Prob:GeneralGammaCounterpart} proves the claim.
%\end{proof}
%\todo[inline]{Reformulierung über die optimalen Werte, aber vielleicht nicht die gleichen optimalen Lösungen?} 

%We note that for the rest of this section, we assume that all minima or maxima are well-defined, which is the case in combinatorial settings since the feasible sets are usually compact or finite.

%\subsection{Reformulations of robust counterparts with assumptions}

\subsection{Linear Uncertainties} \label{subsec:Linear}
%Until now, we have made no assumptions about $f_i$ or
%$\mathcal{U}_i$. 
During the last decades, research has been focused on linear uncertainties and they are well--studied. Thus, in this subsection, we will show how one can deal with linear uncertainties in the context of MINLPs under uncertainty, noting that many combinatorial programs are dealing with linear uncertainty (as we will also demonstrate in Section~\ref{Sec:Reformulations}):
\begin{assumption}\label{Ass:GeneralLinear}
For $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} and for all $i \in [m]$, Assumption~\ref{Ass:General} holds with the following modification:
\begin{itemize}
%\item[(i)] There is a nominal scenario $\overline{u}^i \in \R^{L_i}$, a matrix $A^i \in \R^{L_i \times m_i}$ and a convex set $\mathcal{Z}_i \subseteq \R^{m_i}$, such that $
%\mathcal{U}_i = \{\overline{u}^i + A^i \zeta^i\mid \ \zeta^i \in
%\mathcal{Z}_i\}$, i.e., $\mathcal{U}_i$ is an affine transformation of a convex set (and thus, convex).
\item[$\text{(ii)}^*$] The uncertainty is linear, i.e., there exists a function $l_i \colon \mathcal{X} \to \R^{L_i}$ such that 
\begin{gather*}
f_i(x,u^i) = (u^i)^Tl_i(x)\  \forall u^i \in \mathcal{U}_i, \ x \in \mathcal{X}.
\end{gather*}
%\item[(iii)] The nominal scenario $\overline{u}^i$ is contained in the relative interior of $\mathcal{U}_i$.
\end{itemize}
\end{assumption}
%Since convex sets stay convex under affine-linear transformations,
%(i) implies that $\mathcal{U}^i$ is convex.
We start by formulating Corollary~\ref{Prop:FenchelGammaCounterpart} under Assumption~\ref{Ass:GeneralLinear}:
\begin{corollary}\label{Prop:FenchelGammaCounterpartLinear}
Let $\Gamma \in [m]$. Under Assumption~\ref{Ass:GeneralLinear}, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to %Problem~\eqref{Prob:GeneralReModel} 
\begin{align}\label{Prob:FenchelGammaCounterpartLin}
\begin{split}
\inf_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} (\overline{u}^i)^Tl_i(x) + p_i, \\
\mathrm{s.t.}\; & x \in \mathcal{X}, \\
& p_i + \theta \geq  \supportx{i} \ \forall i \in [m], \\
& p, \theta \geq 0.
\end{split}
\end{align}
\end{corollary}
\begin{proof}
Since $\Gamma$ is integral, Corollary~\ref{Prop:FenchelGammaCounterpart} holds. Since the uncertainty is linear, we have
\begin{gather*}
f_{i,*}(x,v^i) \neq -\infty \Leftrightarrow v^i = l_i(x),
\end{gather*} 
see \cite{Fenchel}. Since inequality~\eqref{Ineq:GeneralPrinciple} is naturally not fulfilled for $f_{i,*}(x,v^i) = - \infty$, $v^i = l_i(x)$ holds. Inserting this into program~\eqref{Prob:FenchelGammaCounterpart} proves the claim, since $f_i(x, \overline{u}^i) = (\overline{u}^i)^Tl_i(x)$.
%\begin{align*}
%%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%%\text{s.t.} & x \in \mathcal{X}, \\
%p_i + \theta \geq (\overline{u}^i)^Tl_i(x) + \supportx{i} - f_i(x,\overline{u}^i) \ \forall i \in [m]. 
%%& p, \theta \geq 0.
%\end{align*} 
%Since $f_i(x, \overline{u}^i) = (\overline{u}^i)^Tl_i(x)$, the claim follows.
\end{proof}
 
\begin{remark}
We note that naturally, similar to $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} being a generalization of program~\eqref{Prob:Gamma_Comb}, Corollary~\ref{Prop:FenchelGammaCounterpartLinear} is a generalization of Theorem~1 in \cite{IntroGamma}.
\end{remark}



%\begin{example} %For illustrative purposes, we study the case $\mathcal{Z}_i := \{\zeta^i \mid || \zeta_i ||_p \leq \rho\},$ where $f_i$ is linear in the uncertainty.
% We also show that the second part of Theorem~\ref{Theo:FenchelGammaCounterpart} is a generalization of Proposition~\ref{Prop:Gamma_MIP}. 
%In \cite{Fenchel}, several examples for the support function and the concave conjugate have been determined and given explicitly which is, of course, possible here as well. We will come back to that later in this section. In a first step, we show what happens when $f_i(x,\overline{u}^i)$ is not only concave but linear in $\overline{u}^i$:
%\begin{theorem}\label{Theo:GeneralLinearUncertainty}
%Let $\Gamma$ be integral and assume that Assumptions (i), (ii) and (iii) hold. Assume that for all $i \in [m]$, there is a function $l_i(x)\colon \R^n \to \R^n $, such that $f_i(x,u^i) = (u^i)^Tl_i(x)$, i.e., $f_i$ is linear in the uncertainty. Then Problem~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
%\begin{align}\label{Prob:FenchelGammaCounterpartLinear}
%\begin{split}
%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i \\
%\text{s.t.} & x \in \mathcal{X} \\
%& p_i + \theta \geq  \supportx{i} \ \forall i \in [m] \\
%& p, \theta \geq 0.
%\end{split}
%\end{align}
%\end{theorem}
%\begin{proof}
%Since Assumptions (i), (ii) and (iii) hold and since $\Gamma$ is integral, Theorem~\ref{Theo:FenchelGammaCounterpart} holds and Problem~\eqref{Prob:GeneralGammaCounterpart} is Problem~\eqref{Prob:FenchelGammaCounterpart}. In \cite{Fenchel}, the authors showed that in the case $f_i$ being linear in $u^i$, 
%\begin{gather*}
%f_{i,*}(x,v^i) \neq -\infty \Leftrightarrow v^i = l_i(x)
%\end{gather*} 
%and that $f_{i,*}(x,l_i(x)) = 0$. Since $f_{i,*}(x,v^i) = - \infty$ would lead to infeasibility of Problem~\eqref{Prob:FenchelGammaCounterpartLinear}, $v^i = l_i(x) \ \forall i \in [m]$. \\
%Inserting this into Problem~\eqref{Prob:FenchelGammaCounterpart} results in
%\begin{align*}
%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%\text{s.t.} & x \in \mathcal{X}, \\
%& p_i + \theta \geq (\overline{u}^i)^Tl_i(x) + \supportx{i} - f_i(x,\overline{u}^i) \ \forall i \in [m], \\
%& p, \theta \geq 0.
%\end{align*} 
%Since $f_i(x, \overline{u}^i) = (\overline{u}^i)^Tl_i(x)$, the claim follows.
%\end{proof}
%Theorem~\ref{Theo:GeneralLinearUncertainty} implies that in the case
%of linearity in the uncertainty, the problem of solving the robust
%counterpart mainly reduced to determining $\supportx{i}$ for all $i
%\in [m]$. In \cite{Fenchel}, the authors did that for various
%uncertainty sets $\mathcal{U}_i$, including explicit geometries like
%ellipsoids, polyhedra, cones, boxes, Miskowski sums or their
%intersections and uncertainty sets which are describes by various
%functions, e.g. convex functions or separable functions. For
%illustrative purposes, we show two examples: the cases of
%$\mathcal{Z}_i$ being a polyhedron for all $i \in [m]$ and
%$\mathcal{Z}_i$ being defined by the $p$-norm for all $i \in [m]$.
%\begin{example}\label{Ex:Polyhedra}
%As it was shown in \cite{Fenchel} and in \cite{RobustBook}, when $\mathcal{U}_i = \{\overline{u}^i + A^i \zeta^i \mid C^i \zeta^i \leq d^i\}$, i.e., $\mathcal{Z}^i = \{\zeta^i \mid C^i \zeta^i \leq d^i\}$ being a non-empty, full-dimensional polyhedron,
%\begin{gather*}
%\supportx{i} = \max_{\zeta^i: C^i \zeta^i \leq d^i } (\zeta^i)^T(A^i)^Tl_i(x) 
%\end{gather*}
%and thus by strong duality
%\begin{gather*}
%\supportx{i} = \min_{y^i: (C^i)^Ty^i = (A^i)^Tl_i(x), y \geq 0} (d^i)^T y^i
%\end{gather*}
%Hence problem~\eqref{Prob:FenchelGammaCounterpartLinear} is equivalent to
%\begin{align}\label{Prob:FenchelGammaCounterpartLinearPolyhedra}
%\begin{split}
%\min_{x,p,\theta,y^i} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%\text{s.t.} & x \in \mathcal{X}, \\
%& p_i + \theta \geq (d^i)^Ty^i \ \forall i \in [m], \\
%& (C^i)^Ty^i = (A^i)^Tl_i(x) \ \forall i \in [m], \\
%& p, \theta, y^1, \dots, y^m \geq 0.
%\end{split}
%\end{align}
%\end{example}
%\todo[inline][inline]{ich habe das Label vom ursprÃ¼nglichen Beispiel 3.14 Ã¼bernommen. Der Querverweis fuktioniert genauso}
%\begin{example}\label{Ex:Norm}
%Let $p \in [1, \infty]$. If we assume that $\mathcal{Z}_i := \{\zeta^i \mid || \zeta_i ||_p \leq \rho\}$ for an arbitrary $\rho \in \R_{\geq 0}$, then (we again refer to \cite{Fenchel} and \cite{RobustBook}) 
%\begin{gather*}
%\supportx{i} = \rho || (A^i)^Tl_i(x) ||_q,
%\end{gather*}
%where $q$ satisfies $\frac1p + \frac1q = 1$ for $p \neq \infty$ and $q = 1$ otherwise. Then problem~\eqref{Prob:FenchelGammaCounterpartLinear} is equivalent to problem~\eqref{Prob:GeneralReModel}: 
%\begin{align}\label{Prob:FenchelGammaCounterpartLinearPolyhedra}
%\begin{split}
%\min_{x,p,\theta} & \ \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + p_i, \\
%\mathrm{s.t.} &  \ x \in \mathcal{X}, \\
%& p_i + \theta \geq \rho || (A^i)^Tl_i(x) ||_q \ \forall i \in [m], \\
%& p, \theta \geq 0. 
%\end{split}
%\end{align}
%\end{example}
%We also show that the second part of Proposition~\ref{Prop:FenchelGammaCounterpart} is a generalization of Proposition~\ref{Prop:Gamma_MIP}.
%\begin{example}
%Consider an MIP with an uncertain objective under interval uncertainty.
%% Similar to Example~\ref{Rem:GeneralizeComb}, we set the various parameters and insert them into problem~\eqref{Prob:FenchelGammaCounterpartLinearPolyhedra}:
%%\begin{gather*}
%%\mathcal{U}_i := [\overline{c}_i - \Delta c_i, \overline{c}_i + \Delta c_i], \ \overline{u}^i := \overline{c}_i, \ f_i(x,u^i) := u^i \cdot x_i, \ \mathcal{X}:=\{x \in \Z^{r} \times \R^{n-r} \mid Ax \leq b\}.
%%\end{gather*}
%%Thus, the uncertainty set is as an affine
%The uncertainty set for each coefficient can be rewritten as an affine
%transformation of a (one-dimensional) box:
%\begin{gather*}
%\mathcal{U}_i := \{\overline{c}_i + \Delta c_i\zeta_i \mid |\zeta_i| \leq 1\}, 
%\end{gather*}
%i.e., $\mathcal{Z}_i := \{\zeta_i \in \R: \ |\zeta_i| \leq 1\}.$ With the notation
%from Example~\ref{Ex:Norm}, $p= \rho = 1$ and $A^i = \Delta
%c_i$. After linearizing constraints that contain absolute values, inserting this into model~\eqref{Prob:FenchelGammaCounterpartLinearPolyhedra} results in
%\begin{align*}
%\min_{x,p,\theta,z} & \ \Gamma \theta + \sum_{i \in [n]} \overline{c}_ix_i + p_i, \\
%\mathrm{s.t.} & \ x \in \mathcal{X}, \\
%& p_i + \theta \geq \Delta c_i z_i  \ \forall i \in [n], \\
%& x_i \in [-z_i, z_i] \ \forall i \in [n], \\
%& p, \theta \geq 0.
%\end{align*}
%%i.e., problem~\eqref{Prob:RobCounterpartMIP}. 
%\end{example}
%For more details on other uncertainty set geometries, we refer to Section 3 and
%to Table 1 in \cite{Fenchel}. \\
%While one can now give a reformulation for MINLPs without
%uncertainty,
For combinatorial optimization under interval uncertainty, it is usually essential to obtain a tractable reformulation for which the feasible set is not altered, as oracles for program~\eqref{Prob:GeneralNomOpt} can then be used to solve the resp. $\Gamma$--counterpart. In the case of linear uncertainty, this can be achieved by adding the additional assumption of $l_i$, $i \in [m]$, being non--negative on $\mathcal{X}$ and altering $\mathcal{X}$:
%%\todo[inline]{Thm 4.8 leistet
%%das aber noch nicht, weil da noch die v Werte dabeisind, oder? Das
%%muesste man dann noch dazusagen, dass das naechste thm a step towards
%%reaching this goal darstellt, oder sowas in der art.}
%%\todo[inline]{Dennis: da kommen wir auch nur im Linearen hin, ich hab das jetzt danach kommentiert. Man kann die PArameter $v^i$ aber eigentlich frei bestimmen, so dass es von der allgemeinen Struktur abhängt, was man mit dem Problem macht (zum Beispiel mehr Fallunterscheidungen, bei denen man $\theta^k$ bestimmen kann).}
%%\begin{theorem}\label{Theo:GeneralGammaCounterPartWithoutDual}
%%Let $\Gamma \in [m]$. Under Assumption~\ref{Ass:General}, the $\Gamma$--counterpart \eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%%\begin{align}\label{Prob:GeneralGammaCounterpartWithoutDual}
%%\begin{split}
%%\min_{k \in [m]_0} & \min_{\substack{x \in \mathcal{X}, v^1 \in \R^{L_1}, \\  \dots, v^m \in \R^{L_m}}} \Gamma \theta^k(x,v^k) + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, \theta^i(x,v^i) - \theta^k(x,v^k) \}, \\
%%%\text{s.t.} & \ x \in \mathcal{X} \\
%%%& \theta^k \geq 0. \\
%%%& \theta^k = \overline{u^k}^Tv^k - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k) + \support{k}).
%%\end{split}
%%\end{align}
%%with $\theta^0(x,v^0):=0 \text{ and }$
%%\begin{gather*}
%%\theta^k(x,v^k) := (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k)  \ \forall k \in [m].
%%\end{gather*}
%%If $f_i$ is linear in the uncertainty, i.e., $f_i(x,u^i) = (u^i)^Tl_i(x),$ for $l_i\colon \R^n \to \R^{L_i}, $ problem~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
%%\begin{align}\label{Prob:GeneralGammaCounterpartWithoutDualLinear}
%%\begin{split}
%%\min_{k \in [m]_0} & \min_{x \in \mathcal{X}} \Gamma \theta^k(x) + \sum_{i \in [m]} (\overline{u}^i)^Tl_i(x) + \max \{0, \theta^i(x) - \theta^k(x) \}, \\
%%%\text{s.t.} & x \in \mathcal{X} \\
%%%& \theta^k \geq 0. \\
%%%& \theta^k = \overline{u^k}^Tv^k - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k) + \support{k})
%%\end{split}
%%\end{align}
%%where $\theta^0(x) = 0$ and $\theta^k(x) = \supportx{k}$. 
%%\end{theorem}
%%\begin{proof}
%Since Assumption~\ref{Ass:General} holds and $\Gamma \in [m]$, the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
%\eqref{Prob:FenchelGammaCounterpart}. Analogously to the proof in Lemma~\ref{Rem:GeneralizeComb}, one can show that
%\begin{gather}\label{Eq:optimal_p}
%p^*_i = \max \{0, (\overline{u}^i)^Tv^{i,*} + \support{i} -f_{i,*}(x^*,v^{i,*}) - f_i(x^*, \overline{u}^i) - \theta^* \}
%\end{gather}
%%for an optimal solution $(x^*,p^*,\theta^*,v^{1,*}, \dots, v^{m,*})$ for all $i \in [m]$ and that of~\eqref{Prob:FenchelGammaCounterpart}. Inserting equation~\eqref{Eq:optimal_p} into the objective function of \eqref{Prob:FenchelGammaCounterpart} results in 
%%\begin{align}\label{Eq:piecewiselinear}
%% \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, (\overline{u}^i)^Tv^i + \support{i}-f_{i,*}(x,v) - f_i(x, \overline{u}^i) - \theta \}.
%%\end{align}
%%Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, 
%and that $\theta^*$ equals $0$ or there exists $k \in [m]$ such that
%\begin{gather}\label{Eq:OptimalTheta}
%\theta^* = (\overline{u}^k)^Tv^{k,*} + \support{k} - f_{k}(x^*
%,\overline{u}^k) - f_{k,*}(x^*,v^{k,*}).
%\end{gather}
%%for one $k \in [m]$. %Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, the minimum is furthermore obtained either at $0$ or 
%%Assume that $(x,v^1, \dots, v^m, \theta)$ is feasible and that $\theta$ is equal to 0 nor does it fulfill equation~\eqref{Eq:OptimalTheta} for any $k \in [m]$. Thus, the sets
%%\begin{align*}
%%S^{<}&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k)  < \theta\} \text{ and } \\
%%S^>&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) > \theta\}
%%\end{align*}
%%are a partition of $[m]$, i.e., $S^< \cup S^> = [m]$ and $S^< \cap S^> = \emptyset$. The objective can be rewritten as:
%%\begin{alignat*}{2}
%%&\Gamma\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} \left( -f_k(x,v^k) + \support{k} - \theta \right) \\
%%&= (\Gamma - |S^>|)\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} -f_k(x,v^k) + \support{k}. 
%%\end{alignat*}
%%We consider different cases for $S^>$:
%%\begin{itemize}
%%\item[\underline{First case:}] $S^> = \emptyset$. \\
%%In this case, $S^< = [m]$. The solution $(x,v^1, \dots, v^m, \overline{\theta})$ with
%%\begin{gather*}
%%\overline{\theta} := \max_{k \in [m]} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) 
%%\end{gather*}
%%has a better objective value than $(x,v^1, \dots, v^m, \theta)$, since $\overline{\theta} < \theta$.
%%\item[\underline{Second case:}] $S^> = [m]$.\\
%%In this case, 
%%\begin{gather*}
%%0 \leq \theta < f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) \ \forall k \in [m].
%%\end{gather*}
%%We set $
%%\overline{\theta} := \min_{k \in [m]} (\overline{u}^k)^Tv^k + \delta^*({A^k}^Tv^k \mid \mathcal{Z}_k) - f_k(x,\overline{u}^k) - f_k(x,v^k) $
%%
%%and since $\Gamma \in [m]$, the objective value of $(x,v^1, \dots, v^m, \overline{\theta})$ is at most the objective value of $(x,v^1, \dots, v^m, \theta)$. 
%%\item[\underline{Third case:}] $S^> \neq \emptyset, [m]$. \\
%%In this case, there exist $k,l \in [m]$, such that \begin{align*}
%%&f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k} < \theta \\
%%&< f_l(x,\overline{u}^l) - f_l(x,\overline{u}^l) - f_l(x,v^l) + \support{l}.
%%\end{align*}
%%In particular, it can be assumed without loss of generality that 
%%\begin{gather*}
%%k= \mathrm{argmax}_{i \in S^<} \theta - f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i}, \\
%%l= \mathrm{argmin}_{i \in S^>} f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i} - \theta.
%%\end{gather*} 
%%We set 
%%\begin{gather*}
%%\overline{\theta}:= \begin{cases} f_l(x,\overline{u}^l) + \support{l} - f_l(x,\overline{u}^l) - f_l(x,v^l), & \text{if $|S^>| > \Gamma$,} \\
%%\max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}, & \text{otherwise.}
%%\end{cases}
%%\end{gather*} 
%%%and otherwise, set
%%%\begin{gather*}
%%%\overline{\theta}:= \max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}.
%%%\end{gather*}
%%In both cases, we obtain a feasible solution with a better objective.
%%\end{itemize} 
%%We define
%%\begin{gather*}
%%\theta^k(x,v^k) := f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k - f_k(x,\overline{u}^k) - f_l(x,v^k) + \support{k}
%%\end{gather*}
%%for $k \in [m]$ and $\theta^0 := 0$. 
%Thus, the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%\begin{alignat*}{2}
%\min_{k \in [m]_0} & \min_{\substack{x \in \mathcal{X}, v^1 \in \R^{L_1}, \\  \dots, v^m \in \R^{L_m}}} \Gamma \theta^k(x,v^k) + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, \theta^i(x,v^i)- \theta^k(x,v^k) \}, \\
%& \ \ \mathrm{s.t.} \ \theta^i(x,v^i) \geq 0 \ \forall i \in [m]. \\
%\end{alignat*}
%Finally, by application of Fenchel's inequality (cf. \cite{ConvexAnalysis}, Chapter 12) and Assumption~\ref{Ass:General}, (iii) $\theta^i(x,v^i) \geq 0$ is redundant since 
%%$\theta^0(x,v^0) = 0$ by definition and for $k \in [m]$, 
%\begin{gather*}
%\support{i} \geq 0 \Leftrightarrow \exists \zeta \in \mathcal{Z}_i: \ \zeta^T({A^i})^Tv^i \geq 0
%\end{gather*}
%and the first statement follows. If $f_i$ is linear in the uncertainty, $f_{i,*}(x,v^k) \neq -\infty$ is equivalent to $v^i = l_i(x)$ and the equivalence of \eqref{Prob:GeneralGammaCounterpart} and \eqref{Prob:GeneralGammaCounterpartWithoutDualLinear} follows. %we obtain $\support{i} = \Delta u_i l_i(x)$ and the claim follows.
%\end{proof}
%Due to the fact that we also need to optimize over the variables $v^i$, the first part of  Theorem~\ref{Theo:GeneralGammaCounterPartWithoutDual} is not an exact analogon to Proposition~\ref{Prop:Tractable_Gamma_Comb}.\todo[inline]{Remark und Vergleich mit Lemma 4.2?} However, we have obtained a reformulation of non-linear (combinatorial) optimization problems under uncertainty for which the constraints of the decision variables $x$ does not change. In addition, in the case of linearity in the uncertainty, another step can be taken and the variables $v^i$ can be determined on the spot. 

\begin{theorem}\label{Cor:LinInt}
Let $\Gamma \in [m]$ and consider the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} under interval uncertainty $\mathcal{U}_k = [\overline{u}_k, \overline{u}_k + \Delta u_k]$ for some $\overline{u}_k, \Delta u_k \in \R_{\geq 0}^{L_k}$ for all $k \in [m]$. If the uncertainty is linear with $f(x,u_k) = u_k^Tl_k(x)$ and $l_k(x) \geq 0$ holds for all $x \in \mathcal{X}$ and all $k \in [m]$, then program~\eqref{Prob:GeneralGammaCounterpart} is equivalent to   %, $\theta^k(x) = \Delta u_k l_k(x)$, resulting in %%problem~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
\begin{align}\label{Prob:CombinatorialGammaCounterPartWithoutDualLinear}
\begin{split}
\inf_{k \in [m]_0} & \left\{ \inf_{\mathcal{Q} \subseteq [m]} \left\{ \inf_{x \in \mathcal{X_\mathcal{Q}}} \left\{ \Gamma \Delta u_k^T l_k(x) + \sum_{i \in [m]} \overline{u}_i^Tl_i(x) + \sum_{q \in \mathcal{Q}} \Delta u_q^T l_q(x) - \Delta u_k^T l_k(x) \right\} \right\} \right\},
\end{split}
\end{align}
with $\Delta u_0 := l_0(x) := 0$ and 
\begin{gather*}
\mathcal{X}_\mathcal{Q} := \{x \in \mathcal{X}: \Delta u_q^T l_q(x) - \Delta u_k^T l_k(x) \geq 0 \ \forall q \in \mathcal{Q}, \ \Delta u_q^T l_q(x) - \Delta u_k^T l_k(x) \leq 0 \ \forall q \in [m] \setminus \mathcal{Q}\}.
\end{gather*}
%  If the uncertainty is 1-dimensional and $l_k$ is binary for all $k \in [m]$, i.e., $u_k \in \R$ and $l_k(x) \in \{0,1\}$ for all $x \in \mathcal{X}$, \eqref{Prob:GeneralGammaCounterpart} is equivalent to
%\begin{align}\label{Prob:CombinatorialGammaCounterPartWithoutDualLinearBinary}
%\begin{split}
%\min_{k \in [m]_0} & \Gamma \Delta u_k + \min_{\substack{x \in \mathcal{X},\\ l_k(x) = 1}} \sum_{i \in [m]} (\overline{u}_i + \max \{0, \Delta u_i - \Delta u_k\})l_i(x),
%\end{split}
%\end{align}
%i.e., the $\Gamma$--counterpart is equivalent to the minimum of $m+1$ nominal problems and an additional constraint.
\end{theorem}
%\todo[inline]{Auch hier: Können wir nicht über exponentiell viele Probleme gehen?}
\begin{proof}
Let $e^j$ be the vector of only ones in $\R^j$. Since $l_k$ is non--negative, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} does not change when one replaces $\mathcal{U}_k$ with $\mathcal{U}^\varepsilon_k := [\overline{u}_k - \varepsilon e^{L_k}, \overline{u}_k + \Delta u_k]$ for any $\varepsilon > 0$ and Assumption~\ref{Ass:GeneralLinear} holds. Thus, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to \eqref{Prob:FenchelGammaCounterpart}. Analogously to the proof of Lemma~\ref{Rem:NoFenchel}, one can show that
\begin{gather}\label{Eq:lin_optimal_p}
p^*_i = \max \{0, \supportx{i} - \theta^* \}
\end{gather}
%for an optimal solution $(x^*,p^*,\theta^*,v^{1,*}, \dots, v^{m,*})$ for all $i \in [m]$ and that of~\eqref{Prob:FenchelGammaCounterpart}. Inserting equation~\eqref{Eq:optimal_p} into the objective function of \eqref{Prob:FenchelGammaCounterpart} results in 
%\begin{align}\label{Eq:piecewiselinear}
% \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, (\overline{u}^i)^Tv^i + \support{i}-f_{i,*}(x,v) - f_i(x, \overline{u}^i) - \theta \}.
%\end{align}
%Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, 
and that $\theta^*$ equals $0$ or there exists $k \in [m]$ such that
\begin{gather}\label{Eq:lin_OptimalTheta}
\theta^* = \supportx{k} = \Delta u_k^Tl_k(x)
\end{gather}
for optimal $p^*$ and $\theta^*$. Note that the last equation in \eqref{Eq:lin_OptimalTheta} holds since $l_k$ is non--negative.
%for one $k \in [m]$. %Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, the minimum is furthermore obtained either at $0$ or 
%Assume that $(x,v^1, \dots, v^m, \theta)$ is feasible and that $\theta$ is equal to 0 nor does it fulfill equation~\eqref{Eq:OptimalTheta} for any $k \in [m]$. Thus, the sets
%\begin{align*}
%S^{<}&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k)  < \theta\} \text{ and } \\
%S^>&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) > \theta\}
%\end{align*}
%are a partition of $[m]$, i.e., $S^< \cup S^> = [m]$ and $S^< \cap S^> = \emptyset$. The objective can be rewritten as:
%\begin{alignat*}{2}
%&\Gamma\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} \left( -f_k(x,v^k) + \support{k} - \theta \right) \\
%&= (\Gamma - |S^>|)\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} -f_k(x,v^k) + \support{k}. 
%\end{alignat*}
%We consider different cases for $S^>$:
%\begin{itemize}
%\item[\underline{First case:}] $S^> = \emptyset$. \\
%In this case, $S^< = [m]$. The solution $(x,v^1, \dots, v^m, \overline{\theta})$ with
%\begin{gather*}
%\overline{\theta} := \max_{k \in [m]} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) 
%\end{gather*}
%has a better objective value than $(x,v^1, \dots, v^m, \theta)$, since $\overline{\theta} < \theta$.
%\item[\underline{Second case:}] $S^> = [m]$.\\
%In this case, 
%\begin{gather*}
%0 \leq \theta < f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) \ \forall k \in [m].
%\end{gather*}
%We set $
%\overline{\theta} := \min_{k \in [m]} (\overline{u}^k)^Tv^k + \delta^*({A^k}^Tv^k \mid \mathcal{Z}_k) - f_k(x,\overline{u}^k) - f_k(x,v^k) $
%
%and since $\Gamma \in [m]$, the objective value of $(x,v^1, \dots, v^m, \overline{\theta})$ is at most the objective value of $(x,v^1, \dots, v^m, \theta)$. 
%\item[\underline{Third case:}] $S^> \neq \emptyset, [m]$. \\
%In this case, there exist $k,l \in [m]$, such that \begin{align*}
%&f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k} < \theta \\
%&< f_l(x,\overline{u}^l) - f_l(x,\overline{u}^l) - f_l(x,v^l) + \support{l}.
%\end{align*}
%In particular, it can be assumed without loss of generality that 
%\begin{gather*}
%k= \mathrm{argmax}_{i \in S^<} \theta - f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i}, \\
%l= \mathrm{argmin}_{i \in S^>} f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i} - \theta.
%\end{gather*} 
%We set 
%\begin{gather*}
%\overline{\theta}:= \begin{cases} f_l(x,\overline{u}^l) + \support{l} - f_l(x,\overline{u}^l) - f_l(x,v^l), & \text{if $|S^>| > \Gamma$,} \\
%\max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}, & \text{otherwise.}
%\end{cases}
%\end{gather*} 
%%and otherwise, set
%%\begin{gather*}
%%\overline{\theta}:= \max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}.
%%\end{gather*}
%In both cases, we obtain a feasible solution with a better objective.
%\end{itemize} 
%We define
%\begin{gather*}
%\theta^k(x,v^k) := f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k - f_k(x,\overline{u}^k) - f_l(x,v^k) + \support{k}
%\end{gather*}
%for $k \in [m]$ and $\theta^0 := 0$. 
 Thus, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
\begin{alignat*}{2}
\inf_{k \in [m]_0} & \left\{ \inf_{\substack{x \in \mathcal{X}}} \left\{ \Gamma u_k^Tl_k(x) + \sum_{i \in [m]} (\overline{u}^i)^Tl_i(x) + \max \{0, \Delta u_i^Tl_i(x) - \Delta u_k^Tl_k(x)\} \right\} \right\}.
%& \ \ \mathrm{s.t.} \ \theta^i(x) \geq 0 \ \forall i \in [m]. 
\end{alignat*}
This proves the claim since $\mathcal{Q}$ encodes which maximization terms are non--negative.
%By application of Fenchel's inequality (cf. \cite{ConvexAnalysis}, Chapter 12) and since Assumption~\ref{Ass:General}, (iii) holds, $\theta^i(x,v^i) \geq 0$ is redundant since 
%%$\theta^0(x,v^0) = 0$ by definition and for $k \in [m]$, 
%\begin{gather*}
%\support{i} \geq 0 \Leftrightarrow \exists \zeta \in \mathcal{Z}_i: \ \zeta^T({A^i})^Tv^i \geq 0
%\end{gather*}
%and the first statement follows.
%Since $f_i$ is linear in the uncertainty, $f_{i,*}(x,v^k) \neq -\infty$ is equivalent to $v^i = l_i(x)$ and since $l_k$ is non-negative, $\support{k} = \Delta u_k^T l_k(x)$ and the equivalence of \eqref{Prob:GeneralGammaCounterpart} and \eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear} follows. 

%Since $l_k$ is non-negative, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} does not change when one replaces $\mathcal{U}_k$ with $\mathcal{U}^\varepsilon_k := [\overline{u}_k - \varepsilon e^{L_k}, \overline{u}_k + \Delta u_k]$ for any $\varepsilon > 0$ that is sufficiently small and Assumption~\ref{Ass:General} is fulfilled. Thus, the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to \eqref{Prob:FenchelGammaCounterpart}. Analogously to the proof of Lemma~\ref{Rem:NoFenchel}, one can show that
%\begin{gather}\label{Eq:optimal_p}
%p^*_i = \max \{0, (\overline{u}^i)^Tv^{i,*} + \support{i} -f_{i,*}(x^*,v^{i,*}) - f_i(x^*, \overline{u}^i) - \theta^* \}
%\end{gather}
%%for an optimal solution $(x^*,p^*,\theta^*,v^{1,*}, \dots, v^{m,*})$ for all $i \in [m]$ and that of~\eqref{Prob:FenchelGammaCounterpart}. Inserting equation~\eqref{Eq:optimal_p} into the objective function of \eqref{Prob:FenchelGammaCounterpart} results in 
%%\begin{align}\label{Eq:piecewiselinear}
%% \Gamma \theta + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, (\overline{u}^i)^Tv^i + \support{i}-f_{i,*}(x,v) - f_i(x, \overline{u}^i) - \theta \}.
%%\end{align}
%%Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, 
%and that $\theta^*$ equals $0$ or there exists $k \in [m]$ such that
%\begin{gather}\label{Eq:OptimalTheta}
%\theta^* = (\overline{u}^k)^Tv^{k,*} + \support{k} - f_{k}(x^*
%,\overline{u}^k) - f_{k,*}(x^*,v^{k,*}).
%\end{gather}
%%for one $k \in [m]$. %Since $\eqref{Eq:piecewiselinear}$ is piecewise linear and convex in $\theta$, the minimum is furthermore obtained either at $0$ or 
%%Assume that $(x,v^1, \dots, v^m, \theta)$ is feasible and that $\theta$ is equal to 0 nor does it fulfill equation~\eqref{Eq:OptimalTheta} for any $k \in [m]$. Thus, the sets
%%\begin{align*}
%%S^{<}&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k)  < \theta\} \text{ and } \\
%%S^>&:= \{k \in [m]: (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) > \theta\}
%%\end{align*}
%%are a partition of $[m]$, i.e., $S^< \cup S^> = [m]$ and $S^< \cap S^> = \emptyset$. The objective can be rewritten as:
%%\begin{alignat*}{2}
%%&\Gamma\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} \left( -f_k(x,v^k) + \support{k} - \theta \right) \\
%%&= (\Gamma - |S^>|)\theta + \sum_{k \in S^<} f_k(x,\overline{u}^k) + \sum_{k \in S^>} -f_k(x,v^k) + \support{k}. 
%%\end{alignat*}
%%We consider different cases for $S^>$:
%%\begin{itemize}
%%\item[\underline{First case:}] $S^> = \emptyset$. \\
%%In this case, $S^< = [m]$. The solution $(x,v^1, \dots, v^m, \overline{\theta})$ with
%%\begin{gather*}
%%\overline{\theta} := \max_{k \in [m]} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) 
%%\end{gather*}
%%has a better objective value than $(x,v^1, \dots, v^m, \theta)$, since $\overline{\theta} < \theta$.
%%\item[\underline{Second case:}] $S^> = [m]$.\\
%%In this case, 
%%\begin{gather*}
%%0 \leq \theta < f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_k(x,v^k) \ \forall k \in [m].
%%\end{gather*}
%%We set $
%%\overline{\theta} := \min_{k \in [m]} (\overline{u}^k)^Tv^k + \delta^*({A^k}^Tv^k \mid \mathcal{Z}_k) - f_k(x,\overline{u}^k) - f_k(x,v^k) $
%%
%%and since $\Gamma \in [m]$, the objective value of $(x,v^1, \dots, v^m, \overline{\theta})$ is at most the objective value of $(x,v^1, \dots, v^m, \theta)$. 
%%\item[\underline{Third case:}] $S^> \neq \emptyset, [m]$. \\
%%In this case, there exist $k,l \in [m]$, such that \begin{align*}
%%&f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k} < \theta \\
%%&< f_l(x,\overline{u}^l) - f_l(x,\overline{u}^l) - f_l(x,v^l) + \support{l}.
%%\end{align*}
%%In particular, it can be assumed without loss of generality that 
%%\begin{gather*}
%%k= \mathrm{argmax}_{i \in S^<} \theta - f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i}, \\
%%l= \mathrm{argmin}_{i \in S^>} f_i(x,\overline{u}^i) - f_i(x,\overline{u}^i) - f_i(x,v^i) + \support{i} - \theta.
%%\end{gather*} 
%%We set 
%%\begin{gather*}
%%\overline{\theta}:= \begin{cases} f_l(x,\overline{u}^l) + \support{l} - f_l(x,\overline{u}^l) - f_l(x,v^l), & \text{if $|S^>| > \Gamma$,} \\
%%\max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}, & \text{otherwise.}
%%\end{cases}
%%\end{gather*} 
%%%and otherwise, set
%%%\begin{gather*}
%%%\overline{\theta}:= \max\{0,f_k(x,\overline{u}^k) - f_k(x,\overline{u}^k) - f_k(x,v^k) + \support{k}\}.
%%%\end{gather*}
%%In both cases, we obtain a feasible solution with a better objective.
%%\end{itemize} 
%%We define
%%\begin{gather*}
%%\theta^k(x,v^k) := f_k(x,\overline{u}^k) + \sum_{k \in S^>} (\overline{u}^k)^Tv^k - f_k(x,\overline{u}^k) - f_l(x,v^k) + \support{k}
%%\end{gather*}
%%for $k \in [m]$ and $\theta^0 := 0$. 
%Thus, the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%\begin{alignat*}{2}
%\min_{k \in [m]_0} & \min_{\substack{x \in \mathcal{X}, v^1 \in \R^{L_1}, \\  \dots, v^m \in \R^{L_m}}} \Gamma \theta^k(x,v^k) + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, \theta^i(x,v^i)- \theta^k(x,v^k) \}, \\
%& \ \ \mathrm{s.t.} \ \theta^i(x,v^i) \geq 0 \ \forall i \in [m]. 
%\end{alignat*}
%%By application of Fenchel's inequality (cf. \cite{ConvexAnalysis}, Chapter 12) and since Assumption~\ref{Ass:General}, (iii) holds, $\theta^i(x,v^i) \geq 0$ is redundant since 
%%%$\theta^0(x,v^0) = 0$ by definition and for $k \in [m]$, 
%%\begin{gather*}
%%\support{i} \geq 0 \Leftrightarrow \exists \zeta \in \mathcal{Z}_i: \ \zeta^T({A^i})^Tv^i \geq 0
%%\end{gather*}
%%and the first statement follows.
%Since $f_i$ is linear in the uncertainty, $f_{i,*}(x,v^k) \neq -\infty$ is equivalent to $v^i = l_i(x)$ and since $l_k$ is non-negative, $\support{k} = \Delta u_k^T l_k(x)$ and the equivalence of \eqref{Prob:GeneralGammaCounterpart} and \eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear} follows. 

%
%The second part follows from the observation that, for $l_k(x) = 0$, 
%%the objective of \eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear} is equal to and the equivalence of \eqref{Prob:GeneralGammaCounterpart} and \eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear} follows. %we obtain $\support{i} = \Delta u_i l_i(x)$ and the claim follows.
%%%Since $l_k$ is non-negative, $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} does not change when one replaces $\mathcal{U}_k$ with $\mathcal{U}^\varepsilon_k := [\overline{u}_k - \varepsilon 1_{L_k}, \overline{u}_k + \Delta u_k]$ for any $\varepsilon > 0$ that is sufficiently small. Thus, Assumption~\ref{Ass:General} is fulfilled and \eqref{Prob:GeneralGammaCounterpart} is equivalent to~\eqref{Prob:GeneralGammaCounterpartWithoutDualLinear}. Since $l_k$ is non-negative, $\support{k} = \Delta u_k^T l_k(x)$ and the first part of the claim follows. The second part of the claim follows from the observation that, for $l_k(x) = 0$, the objective of \eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear} is equal to
%\begin{gather*}
%\min_{x \in \mathcal{X}, l_k(x) = 0} \sum_{i \in [m]} \overline{u}_il_i(x) + \max \{0, \Delta u_i l_i(x) \} = \min_{x \in \mathcal{X}, l_k(x) = 0} \sum_{i \in [m]} \overline{u}_il_i(x) + \Delta u_i l_i(x)
%\end{gather*}
%since $\Delta u_i \geq 0$ and $l_i(x) \in \{0,1\}$ which is the objective of \eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear} for $k=0$ and for $l_k(x) = 1$, it is equal to 
%\begin{alignat*}{2}
%& \min_{x \in \mathcal{X}} \Gamma \Delta u_k + \sum_{i \in [m]} \overline{u}_i l_i(x) + \max \{0, \Delta u_i l_i(x) - \Delta u_k \} = \\
%& \Gamma \Delta u_k + \min_{x \in \mathcal{X}} \sum_{i \in [m]} (\overline{u}_i + \max \{0, \Delta u_i - \Delta u_k\})l_i(x),
%\end{alignat*}
%since $l_i(x)$ is binary. 
\end{proof}
Theorem~\ref{Cor:LinInt} states that the $\Gamma$--counterpart under said theorem's assumptions can be 'almost' solved by an optimization oracle for solving~\eqref{Prob:GeneralNomOpt}, assuming that one can extend the oracle from $\mathcal{X}$ to $\mathcal{X}_\mathcal{Q}$. However, the number of calls is in $O(m2^m)$, i.e., exponential in the number of uncertain functions (even if $m$ is part of the input). To the best of our knowledge, there is no 'black box' that can go from $\mathcal{X}$ to $\mathcal{X}_\mathcal{Q}$ in the nonlinear combinatorial context which would certainly be an interesting research avenue. Thus, to be able to solve the $\Gamma$--counterpart with an optimization oracle as of now, one requires further assumptions. However, in Section~\ref{Sec:Reformulations}, we show that this is possible for programs 'underlying an assignment structure'. As a tool, we require the following result for models of the form $\min_{x \in \mathcal{X}} u^TBg(x)$ underlying said structure. 

%Similarly to Corollary~\ref{Prop:FenchelGammaCounterpart}, its tractability depends on the tractability of the support functions and the concave conjugates. \todo{hier konkav zu linear nochmal erwähnen}
%Note that, due to the difficulty with the max--term, it seems unlikely that this formulation is more beneficial than the one provided in Corollary~\ref{Prop:FenchelGammaCounterpart}. %and that, if $f_k$ is linear in the uncertainty, $v^k$ is fixed and $\theta^k(x,v^k) = \support{k}$. 
%Note that, for combinatorial optimization problems, one would like to obtain a reformulation over $\mathcal{X}$ with an objective with a 'similar' structure (e.g., if the objective is quadratic, the reformulated objective should be quadratic as well). A possibility to get rid of the max-term would be performing a distinction of cases for all $k \in [m]_0$ and $i \in [m]$ by adding the inequality
%\begin{gather*}
%\theta^i(x,v^i) \geq \theta^k(x,v^k) \text{ or } \theta^i(x,v^i) \leq \theta^k(x,v^k)
%\end{gather*}
%to the inner problem and optimizating over all possibilities. One can think of branch--and--bound-procedures to avoid enumerating the exponential number of possibilities, also in Theorem~\ref{Cor:LinInt}. 
%\end{remark}
%\begin{remark}
%We note that the constraint $l_k(x) = 1$ is in general not critical since $l_k(x)$ is a binary function. If $l_k(x)$ is the product of binary variables, $l_k(x) = 1$ fixes these variables to one and if it is the sum of binary variables, it is 'only' another linear constraint. We demonstrate in Section 5 that, for some applications, the additional constraint does not change the underlying structure. If it would, one can use that the $\Gamma$--counterpart of $\min_{x\in \mathcal{X}} u^Tl(x)$ under interval uncertainty and $l(x) \in \{0,1\}^m$ for all $x \in \mathcal{X}$ is also equivalent to 
%\begin{align}\label{Prob:CombinatorialGammaCounterPartWithoutDualLinearBinaryTwo}
%\begin{split}
%\min_{k \in [m]_0} & \Gamma \Delta u_k + \min_{x \in \mathcal{X}} \sum_{i \in [m]} (\overline{u}_i + \max \{0, \Delta u_i - \Delta u_k\})l_i(x),
%\end{split}
%\end{align}
%which is implied by the original results of Bertsimas and Sim applied to $\min_{(x,y) \in \mathcal{X}_y} u^Ty$ where $\mathcal{X}_y := \{(x,y) \in \mathcal{X} \times \{0,1\}^m:  \ l(x) = y \text{ for one } x \in \mathcal{X}\}$. Thus, depending on the underlying nominal problem, one can choose between reformulations~\eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinearBinary} and~\eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinearBinaryTwo}.
%\end{remark}
%Additionally, in the second setting of Theorem~\ref{Cor:LinInt}, one can reduce the number of nominal problems one has to solve and can determine $\alpha$-approximations (for $\alpha \geq 1$), if the underlying nominal problems are $\alpha$--approximable. The proofs are very similar to the ones for the original $\Gamma$--counterpart of Bertsimas and Sim and thus ommitted to Appendix B. 
%\begin{theorem}\label{Theo:Approx}
%Let $\Gamma \in [m]$ and consider the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} under interval uncertainty, i.e., for all $k \in [m]$ exist $\overline{u}_k, \Delta u_k \in \R_{>0}$, such that $\mathcal{U}_k = [\overline{u}_k, \overline{u}_k + \Delta u_k]$. If $f_k$ is linear in the uncertainty and binary for all $k \in [m]$, i.e., $f_k(x,u_k) = u_kl_k(x)$ for a function $l_k(x) \in \{0,1\}$ and the nominal problem is $\alpha$-approximable for one $\alpha \geq 1$, then \eqref{Prob:GeneralGammaCounterpart} is $\alpha$--approximable, too.
%%equivalent to
%%\begin{gather*}
%%\min_{k \in \mathcal{L}} \Gamma \Delta u_k + \min_{x \in \mathcal{X}} f(x,\overline{u}) + \sum_{i \in [k]} \left(\Delta u_i - \Delta u_k \right)l_i(x)
%%\end{gather*}
%%for $\mathcal{L} := \{\Gamma + 1, \dots, \Gamma + \gamma, m + 1\}$ with $\gamma$ being the biggest odd integer smaller than $(m + 1) - \Gamma$ and $\Delta_{m+1}:=0$.
%%\end{theorem}
%\end{theorem}
%\begin{theorem}\label{Theo:RedNumber}
%Let $\Gamma \in [m]$ and consider the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} under interval uncertainty, i.e., for all $k \in [m]$ exist $\overline{u}_k, \Delta u_k \in \R_{>0}$, such that $\mathcal{U}_k = [\overline{u}_k, \overline{u}_k + \Delta u_k]$. Without loss of generality, we assume $\Delta u_1 \geq \dots \geq \Delta u_m$. If $f_k$ is linear in the uncertainty and binary for all $k \in [m]$, i.e., $f_k(x,u_k) = u_kl_k(x)$ for a function $l_k(x) \in \{0,1\}$, then \eqref{Prob:GeneralGammaCounterpart} is equivalent to
%\begin{gather*}
%\min_{k \in \mathcal{L}} \Gamma \Delta u_k + \min_{x \in \mathcal{X}} f(x,\overline{u}) + \sum_{i \in [k]} \left(\Delta u_i - \Delta u_k \right)l_i(x)
%\end{gather*}
%for $\mathcal{L} := \{\Gamma + 1, \dots, \Gamma + \gamma, m + 1\}$ with $\gamma$ being the biggest odd integer smaller than $(m + 1) - \Gamma$ and $\Delta_{m+1}:=0$.
%\end{theorem}
%\todo[inline]{Theoreme auf unsere Version anpassen -- darauf achten, dass zulässige Mengen für die Sub-Probleme sogar disjunkt sein können!}
%\todo[inline]{Anwendung auf das QAP}
%
%This reduction is particulary important since, instead of solving $m + 1$ nominal problems, we only need to solve $\lceil \tfrac{m - \Gamma}{2} \rceil + 1$ problems. Especially for $\Gamma$ close to $m$, this reduction will prove substential.

%As an application of Theorem~\ref{Cor:LinInt}, we discuss a special structure under interval uncertainty: In the case of Examples~\ref{Ex:Scheduling} and \ref{Ex:QAP}, we have given interval uncertainties and an objective $u^TBg(x)$. We show that its $\Gamma$--counterpart is equivalent to the $\Gamma$--counterpart $y^Tg(x)$ for uncertain $y$ in a special case:
\begin{theorem}\label{Theo:CorrDoNotCare}
Let $B  \in \R_{\geq 0}^{m \times (m n)}$ be a block diagonal matrix where each block consists of a single row and let $g \colon \R^r \to \R_{\geq 0}^{mn}$ be an arbitrary nonnegative function. Consider program 
\begin{gather}\label{Prob:nom_LP_under_unc}
\inf_{x \in \mathcal{X}} u^TBg(x),
\end{gather}
under interval uncertainty, i.e., $u_i \in \mathcal{U}^i := [\overline{u}_i, \overline{u}_i + \Delta u_i] \subseteq \R_{\geq 0}$ for all $i \in [m]$. Furthermore, we assume that
\begin{gather}\label{Set:Assignment}
\mathcal{X} \subseteq \{x \in \R^r\colon \ \forall i \in [m] \exists ! j \in [n]: \ g_{i,j}(x) \text{ is not constant $0$}\}.
\end{gather} 
Let $\Gamma \in [m]$. Then the $\Gamma$--counterparts of program~\eqref{Prob:nom_LP_under_unc} and program
\begin{gather}
\label{Prob:nom_LP_under_unc_not_cor}
\inf_{x \in \mathcal{X}} y^Tg(x),
\end{gather}
under interval uncertainty $y_{(i,j)}\in \mathcal{Y}^{(i,j)} := [\overline{u}_i B_{i,(i,j)}, (\overline{u}_i + \Delta u_i) B_{i,(i,j)}]$ for all $(i,j) \in [m] \times [n]$ are equivalent.
\end{theorem}
\begin{proof}
We begin by introducing some notation: We set $B_{.,(0,0)} := \Delta y_{0,0}:= \overline{y}_{0,0}:=0$ (note that this is a slight abuse of notation and we mean the zero vector or the number $0$, depending on the dimension), $\Delta y:= (\Delta y_{a,b})_{(a,b) \in [m] \times [n]} := (\Delta u_a B_{a,(a,b)})_{(a,b) \in [m] \times [n]}$,  $\overline{y}:=(\overline{y}_{(a,b)})_{(a,b) \in [m] \times [n]} = (\overline{u}_a B_{a,(a,b)})_{(a,b) \in [m] \times [n]}$ and with $B_{k,.}$, we denote the $k$--th row of $B$. By applying Theorem~\ref{Cor:LinInt}, we obtain that the $\Gamma$--counterpart of program~\eqref{Prob:nom_LP_under_unc} is equivalent to
\begin{align}\label{Model:GammaCounterPartCor}
\inf_{k \in [m]_0} & \left\{ \inf_{\mathcal{Q} \subseteq [m]} \left\{ \inf_{x \in \mathcal{X_\mathcal{Q}}} \left\{ \Gamma \Delta u_k B_{k,.}g(x) + \sum_{i \in [m]} \overline{u}_iB_{i,.}g(x) + \sum_{q \in \mathcal{Q}} \Delta u_q B_{q,.}g(x) - \Delta u_k B_{k,.}g(x) \right\} \right\} \right\}.
\end{align}
Since $B$ is a block--diagonal matrix where each block contains exactly one row, one obtains $B_{i,(r,s)} = 0$ for $i \neq r$. Furthermore, since for all $i \in [m]$, $g_{i,j}(x) \neq 0$ for exactly one $j \in [n]$ (which will we be denoted by $j(i)$) we obtain 
\begin{gather*}
B_{q,.}g(x) = \sum_{i \in [m], j \in [n]} B_{q,(i,j)} g_{i,j}(x) = \sum_{i \in [m]} B_{q,(i,j(i))} g_{i,j(i)}(x) = B_{q,(q,j(q))} g_{q,j(q)}(x).
\end{gather*}
%Thus, for fixed $q \in \mathcal{Q}$, we obtain
%\begin{alignat}{2}\label{Eq:Help3}
%%\Delta u_q B_{q,.}g(x) - \Delta u_k B_{k,.}g(x) \geq 0 &\Longleftrightarrow\\
%\Delta u_q B_{q,(q,j(q))} g_{q,j(q)}(x) \geq  \Delta u_k B_{k,(k,j(k))} g_{k,j(k)}(x). &
%\end{alignat}
%we can further reformulate model~\eqref{Model:GammaCounterPartCor}:
%\begin{align}\label{Model_GammaCounterPartCorII}
%\begin{split}
%& \inf_{(k,l) \in [m] \times [n] \cup \{(0,0)\}}  \inf_{x \in \mathcal{X}} \ \Gamma \Delta u_k B_{k,(k,l)} g_{(k,l)}(x) + \overline{u}^TBg(x) \\
%& \sum_{(i,j) \in [m] \times [n]}   \max\{0, \Delta u_i B_{i,(i,j)} g_{(i,j)}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x)\}.
%\end{split}
%\end{align}
%Note that the case of $k = 0$ has only been changed by notation to $(k,l) = (0,0)$.
The $\Gamma$--counterpart of program~\eqref{Prob:nom_LP_under_unc_not_cor} is equivalent to (again by applying Theorem~\ref{Cor:LinInt} -- note that $l(x) = g(x)$ here and we replace $\mathcal{Q}$ by $\mathcal{Y}$ for the sake of notation):
\begin{align}\label{Model_GammaCounterPartUnCor}
\inf_{(a,b) \in [m] \times [n] \cup \{(0,0)\}} & \left\{ \inf_{\mathcal{Y} \subseteq [m] \times [n]} \left\{ \inf_{x \in \mathcal{X_\mathcal{Y}}} \left\{ \Gamma \Delta y_{(a,b)}g_{(a,b)}(x) +F_{\mathcal{Y},a,b}(x) \right\}  \right\} \right\}
\end{align}
with
\begin{align}\label{Eq:Help}
\begin{split}
F_{\mathcal{Y},a,b}(x) &:= \sum_{(i,j) \in [m] \times [n]} \overline{y}_{(i,j)}g_{(i,j)}x + \sum_{(q,p) \in \mathcal{Y}} \Delta y_{(q,p)}g_{(q,p)}(x) - \Delta y_{(a,b)}g_{(a,b)}(x).
\end{split}
\end{align}
In the following, we show that one can reduce the number of subproblems of program~\eqref{Model:GammaCounterPartCor} from $(m\cdot n+1) \cdot 2^{mn}$ to $(m+1)\cdot 2^m$ and that the resulting program is exactly~\eqref{Model_GammaCounterPartUnCor}. On the one hand, if $b \neq b(a)$, then $g_{(a,b)}(x) = 0$ for all $x \in \mathcal{X}$ by assumption and equation~\eqref{Eq:Help} results in
\begin{align}\label{Eq:Help2}
F_{\mathcal{Y},a,b}(x) = \sum_{(i,j) \in [m] \times [n]} \overline{y}_{(i,j)}g_{(i,j)}(x) + \sum_{(q,p) \in \mathcal{Y}} \Delta y_{(q,p)}g_{(q,p)}(x) = F_{\mathcal{Y},0,0}(x).
\end{align}
Thus, instead of $b \in [n]$, we can fix $b = b(a)$ in program~\eqref{Model_GammaCounterPartUnCor} and only have $m+1$ 'outer problems'. On the other hand, for each $\mathcal{Y} \subseteq [m] \times [n]$, $x \in \mathcal{X}_{\mathcal{Y}}$ only holds if
\begin{align*}
\Delta y_{q,p}g_{q,p}(x) \geq \Delta y_{a,b(a)}g_{a,b(a)}(x) > 0 \ \forall (q,p) \in \mathcal{Y}.
%% \Delta y_{q,p}g_{q,p}(x) \leq \Delta y_{a,b(a)}g_{a,b(a)}(x) \ %%%\forall (q,p) \in ([m] \times [n]) \setminus \mathcal{Y}.
\end{align*}
However, $g_{q,p}(x)$ is not equal to $0$ for some $x$ only if $p=p(q)$. Thus, $\mathcal{X}_\mathcal{Y} = \emptyset$ if $(q,p) \in \mathcal{Y}$ for some $p \neq p(q)$. Thus, program~\eqref{Model_GammaCounterPartUnCor} is equivalent to
\begin{align}\label{Model_GammaCounterPartUnCor2}
\inf_{a \in [m]_0} & \left\{ \inf_{\overline{\mathcal{Y}} \subseteq [m]} \left\{ \inf_{x \in \mathcal{X}_{\overline{\mathcal{Y}}}} \left\{\Gamma \Delta y_{(a,b(a))}g_{(a,b(a))}(x) + F_{\overline{\mathcal{Y}},a}(x) \right\} \right\} \right\}
\end{align}
where 
\begin{align*}
\mathcal{X}_{\overline{\mathcal{Y}}} := \{ x \in \mathcal{X}\colon & \Delta y_{q,p(q)}g_{q,p(q)}(x) \geq \Delta y_{a,b(a)}g_{a,b(a)}(x) \ \forall q \in \overline{\mathcal{Y}}, \\
& \Delta y_{q,p(q)}g_{q,p(q)}(x) \leq \Delta y_{a,b(a)}g_{a,b(a)}(x) \ \forall q \in [m]  \setminus \overline{\mathcal{Y}} \},
\end{align*}
$b(0) := 0$ and
\begin{align*}
F_{\overline{\mathcal{Y}},a}(x) &:=  \sum_{(i,j) \in [m] \times [n]} \overline{y}_{(i,j)}g_{(i,j)}(x) + \sum_{(q,p) \in \overline{\mathcal{Y}}} \Delta y_{(q,p(q))}g_{(q,p(q))}(x) - \Delta y_{(a,b(a))}g_{(a,b(a))}(x).
\end{align*}
By inserting the definition of $\overline{y}$ and $\Delta y$ into program~\eqref{Model_GammaCounterPartUnCor2} and by replacing all indices, one obtains program~\eqref{Model:GammaCounterPartCor}.
%However, since  Now, we assume that $b=a(b)$
%Note that the final equation holds since $\mathcal{X}_{\mathcal{Y}} = \mathcal{X}$ (the right--hand side of inequality~\eqref{Eq:Help3} is $0$ and the left--hand side is non--negative). Furthermore
\end{proof}
%%%%&= \Gamma \Delta u_a B_{a,(a,b)}g_{(a,b)}(x) + \sum_{(i,j) \in [m] \times [n]} \overline{y}_{(i,j)}g_{(i,j)}x + \sum_{(q,p) \in \mathcal{Y}} \Delta u_q B_{q,(q,p)}g_{(q,p)}(x) - \Delta y_{(a,b)}g_{(a,b)}(x) \\
%%%%&= \Gamma \Delta u_a B_{a,(a,b)}g_{(a,b)}(x) + \sum_{(i,j) \in [m] \times [n]} \overline{y}_{(i,j)}g_{(i,j)}x + \sum_{(q,p) \in \mathcal{Y}} \Delta u_q B_{q,(q,p)}g_{(q,p)}(x) - \Delta y_{(a,b)}g_{(a,b)}(x).

%%%%We recall that $(q,p) \in \mathcal{Y}$ implies
%\begin{alignat*}{2}
%\Delta y_{(q,p)}g_{(q,p)}(x) - \Delta y_{(a,b)}g_{(a,b)}(x)\geq 0 & \Longleftrightarrow 
%\Delta u_q B_{q,(q,p)}g_{(q,p)}(x) \geq	& \Delta y_{(a,b)}g_{(a,b)}(x)
%\end{alignat*}

% Inserting this into For fixed  Models~\eqref{Model_GammaCounterPartCorII} and \eqref{Model_GammaCounterPartUnCor} are equivalent,
%since $
%\Delta u^T B_{.,(k,l)} g_{(k,l)}(x) = \Delta u_k B_{k,(k,l)} g_{(k,l)}(x)$ for all $(k,l) \in [m] \times [n]$ and 
%\begin{alignat*}{2}
%&\sum_{i \in [m]} \max \{0, \Delta u_i B_{i,.} g_{i,.}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x) \} \\
%&=\sum_{i \in [m]} \max \{0, \Delta u_i \sum_{j \in [n]} B_{i,j} g_{(i,j)}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x)  \} \\
% &=\sum_{(i,j) \in [m] \times [n]} \underbrace{\max   \{0, \Delta u_i B_{i,(i,j)} g_{(i,j)}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x) \}}_{\neq 0 \text{ for exactly one $j \in [n]$}}. 
%\end{alignat*}

%By application of Theorem~\ref{Cor:LinInt} to the $\Gamma$--counterpart of model~\eqref{Prob:nom_LP_under_unc}, we obtain
%\begin{align}\label{Model:GammaCounterPartCor}
%\inf_{k \in [m]_0} \inf_{x \in \mathcal{X}} \Gamma \Delta u_k B_{k,.}g(x) + \overline{u}^TBg(x) + \sum_{i \in [m]}  \max\{0, \Delta u_i B_{i,.}g(x) - \Delta u_k B_{k,.}g(x) \}, 
%\end{align}
%with $B_{0,.} := \Delta u_0 := 0$. Since $B_{i,(r,s)} = 0$ for $i \neq r$ and since for all $i \in [m]$, $g_{(i,j)}(x) \neq 0$ for exactly one $j \in [n]$ by assumption, we can further reformulate model~\eqref{Model:GammaCounterPartCor}:
%\begin{align}\label{Model_GammaCounterPartCorII}
%\begin{split}
%& \inf_{(k,l) \in [m] \times [n] \cup \{(0,0)\}}  \inf_{x \in \mathcal{X}} \ \Gamma \Delta u_k B_{k,(k,l)} g_{(k,l)}(x) + \overline{u}^TBg(x) \\
%& \sum_{(i,j) \in [m] \times [n]}   \max\{0, \Delta u_i B_{i,(i,j)} g_{(i,j)}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x)\}.
%\end{split}
%\end{align}
%Note that the case of $k = 0$ has only been changed by notation to $(k,l) = (0,0)$. Next, we determine the $\Gamma$--counterpart of model~\eqref{Prob:nom_LP_under_unc_not_cor}, again by applying Theorem~\ref{Cor:LinInt}:
%\begin{align}\label{Model_GammaCounterPartUnCor}
%\begin{split}
%&\inf_{(k,l) \in [m] \times [n] \cup \{(0,0)\}}  \inf_{x \in \mathcal{X}} \ \Gamma \Delta u^T B_{.,(k,l)} g_{(k,l)}(x) + \\
%&\sum_{(i,j) \in [m] \times [n]} \overline{u}^T B_{.,(i,j)} g_{(i,j)}(x) + \max\{0, \Delta u^T B_{.,(i,j)} g_{(i,j)}(x) - \Delta u^TB_{.,(k,l)} g_{(k,l)}(x)\},
%\end{split}
%\end{align}
%where $B_{.,(0,0)} := 0$, $\Delta u:= (\Delta u_i)_{i \in [m]}$ and $\overline{u}:=(\overline{u}_i)_{i \in [m]}$. Models~\eqref{Model_GammaCounterPartCorII} and \eqref{Model_GammaCounterPartUnCor} are equivalent,
%since $
%\Delta u^T B_{.,(k,l)} g_{(k,l)}(x) = \Delta u_k B_{k,(k,l)} g_{(k,l)}(x)$ for all $(k,l) \in [m] \times [n]$ and 
%\begin{alignat*}{2}
%&\sum_{i \in [m]} \max \{0, \Delta u_i B_{i,.} g_{i,.}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x) \} \\
%&=\sum_{i \in [m]} \max \{0, \Delta u_i \sum_{j \in [n]} B_{i,j} g_{(i,j)}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x)  \} \\
% &=\sum_{(i,j) \in [m] \times [n]} \underbrace{\max   \{0, \Delta u_i B_{i,(i,j)} g_{(i,j)}(x) - \Delta u_k B_{k,(k,l)} g_{(k,l)}(x) \}}_{\neq 0 \text{ for exactly one $j \in [n]$}}. 
%\end{alignat*}

%In the setting of the previous theorem, each part of the objective is influenced by exactly one uncertain parameter as in Example~\ref{Ex:Scheduling}. The theorem states that, under certain conditions for $g$, one can shift the linear combinations of the partial functions of $g$ into a modified uncertainty set. This is especially important in the linear case, where one can then straight-forwardly apply the original results of Bertsimas and Sim:
% when $g(x)$ is a binary function, one can then apply the results of Theorem~\ref{Cor:LinInt} to obtain tractable counterparts. Furthermore, by applying Theorem~\ref{Theo:CorrDoNotCare}, we prove that, for linear programs of the form $\min_{x\in\mathcal{X}} u^TLx$ with $u$ underlying interval uncertainty, the correlations imposed by the matrix $L$ linear problems can be 'ignored', if $\mathcal{X}$ underlies an assignment structure:

%:
%\begin{theorem}\label{Theo:CombinatorialGammaCounterPartWithoutDualLinear}
%Let $\Gamma \in [m]$. For all $i \in [m]$ assume that, there is a function $l_i\colon \R^n \to \R^{L_i} $, such that $f_i(x,u^i) = (u^i)^Tl_i(x)$, i.e., $f_i$ is linear in the uncertainty. Under Assumption~\ref{Ass:General}, problem~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
%\begin{align}\label{Prob:GeneralGammaCounterpartWithoutDualLinear}
%\begin{split}
%\min_{k \in \{0, \dots, m\}} & \min_{x \in \mathcal{X}} \Gamma \theta^k(x) + \sum_{i \in [m]} (\overline{u}^i)^Tl_i(x) + \max \{0, \theta^i(x) - \theta^k(x) \}, \\
%%\text{s.t.} & x \in \mathcal{X} \\
%%& \theta^k \geq 0. \\
%%& \theta^k = \overline{u^k}^Tv^k - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k) + \support{k}).
%\end{split}
%\end{align}
%where $\theta^0(x) = 0$ and $\theta^k(x) = \supportx{k}$. Furthermore, if all uncertainty sets are intervals, i.e., $\mathcal{U}_k = [\overline{u}_k, \overline{u}_k + \Delta u_k] \subseteq \R$ and $l_k(x) \geq 0$ for all $k \in [m]$, problem~\eqref{Prob:GeneralGammaCounterpart} is equivalent to 
%\begin{align}\label{Prob:CombinatorialGammaCounterPartWithoutDualLinear}
%\begin{split}
%\min_{k \in \{0, \dots, m\}} & \min_{x \in \mathcal{X}} \Gamma \Delta u_k l_k(x) + \sum_{i \in [m]} \overline{u}_il_i(x) + \max \{0, \Delta u_i l_i(x) - \Delta u_k l_k(x) \},
%\end{split}
%\end{align}
%with $\Delta u_0 := l_0(x) := 0$.
%\end{theorem}
%\begin{proof}
%The proof for
%reformulation~\eqref{Prob:GeneralGammaCounterpartWithoutDual} follows the same outline as the proof of
%Proposition~\ref{Prop:FenchelGammaCounterpart} and is therefore omitted. In the case of interval uncertainty for all $k \in [m]$, i.e., $\mathcal{U}_k:=[\overline{u}^k,\overline{u}^k + \Delta u^k]$ for a perturbation $\Delta u_k$, one obtains $\theta^k(x) = \Delta u_k  l_k(x)$, since $l_k$ is non-negative on $\mathcal{X}$. 
%%In this case, applying Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} results in 
%%\begin{gather*}
%%\theta^k(x) = \Delta u_k l_k(x), \ k \in [m], 
%%\end{gather*} 
%\end{proof}
%Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear}
%implies that, in the case of linearity, we obtain a reformulation over the feasible set $\mathcal{X}$ without variables $v^i$, and that in the case of interval uncertainty, the required support functions can be determined.
% It is straightforward to show that
%Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} is a generalization of Proposition~\ref{Prop:Tractable_Gamma_Comb}.\\ %, thus we omit the proof.\\

%While the reformulation given in Example~\ref{ex:QAP_genau} is, to our knowledge, new in literature, there are already studies for solving the $\Gamma$--counterpart of a QAP. E.g. in \citep{QAP2015} the techniques of \cite{IntroGamma} where applied. Afterwards the authors used linearizing techniqes from \cite{QAP_lin} to linearizte the resulting MIQP. In our numerical study in Section 5, we compare our reformulation with linearizations in which one linearizes all quadratic terms with standart linearizations and applies the reformulations of \cite{IntroGamma}. 
%For all $i,j,r,s \in [n]$, we will apply a standard linearization of $x_{ir}x_{js}$ and introduce auxiliary variables $z_{ijrs}$, such that
%%We need a linear objective function to apply the reformulation of \citep{IntroGamma} to Problem~\eqref{Prob:QAP_RobCP}. Therefore, we linearizing the products $x_{ir}x_{js}$ in Problem~\eqref{Prob:QAP_RobCP} for $(i,j,r,s) \in [n]^4$ with
%\begin{align*}
%& z_{irjs} \ge x_{ir} +x_{js} -1, \quad \forall (i,j,r,s) \in [n]^4,\\
%&z_{irjs} \le x_{ir} , \quad \forall (i,j,r,s) \in [n]^4,\\
% & z_{irjs} \le  x_{js}, \quad \forall (i,j,r,s) \in [n]^4,\\
%& z_{irjs} \in [0,1], \quad \forall (i,j,r,s) \in [n]^4.
%\end{align*}
%The variables $z_{ijrs}$ are subject to the uncertain 'coefficients' $c_{ij}d_{rs} \in [d_{rs}\overline{c}_{ij}, d_{rs}(\overline{c}_{ij} + \Delta c_{ij})]$. The linearized model and our reformulation are equivalent while ot
%%\begin{align}
%%\begin{split}
%%\min_{z,x} & \sum_{(i,j,r,s) \in [n]^4}\left(\bar{c}_{ij}d_{rs}z_{ijrs} + \max_{\mathcal{S} \subseteq [n]^4: |S| \le \Gamma} \Delta c_{ij} d_{rs} z_{ijrs}\right)\\
%%\text{s.t. } & z_{irjs} \ge x_{ir} +x_{js} -1, \quad \forall (i,j,r,s) \in [n]^4,\\
%%& z_{irjs} \le x_{ir} , \quad \forall (i,j,r,s) \in [n]^4,\\
%% & z_{irjs} \le  x_{js}, \quad \forall (i,j,r,s) \in [n]^4,\\
%%& z_{irjs} \in [0,1], \quad \forall (i,j,r,s) \in [n]^4\\
%%&x\in \mathcal{X}.
%%\end{split}
%%\end{align} 
%We set for our uncertainty set
%\[c_{ij}d_{rs} \in  \mathcal{U}_{ijrs}=[d_{rs}\bar{c}_{ij},d_{rs}(\bar{c}_{ij}+\Delta c_{ij})] \quad \forall(i,j,r,s)\in [n]^4.\]
%%\todo[inline]{man sollte statt auf prop. 2.1 zu verweisen sagen dass das imgrunde bertsimas - sim ist, ansonsten wirkt es so als sei prop 2.1schon unser resultat...}
%With that we have a MIP and can use the standard $\Gamma$-approach of Proposition~\ref{Prop:Gamma_MIP} (see \cite{IntroGamma} Theorem 1). We denote the resulting MIP as $QAP_\text{MIP}$. Because of the linearization we get $n^4$ more variables but we have to solve only one MIP.
%If we further define $z_{ijrs} \in \{0,1\}$ we can apply Proposition~\ref{Prop:Tractable_Gamma_Comb} (see \cite{IntroGamma} Theorem 3). 
%The resulting binary problem is denoted as $QAP_\text{BP}$. In that case we also have $n^4$ more variables like with $QAP_\text{MIP}$ but we also have to solve the same amount of single BPs like with problem $QAP$ and compare them.

%\todo[inline][inline]{Dennis: Quelle!}


%\begin{example}
%For combinatorial problems of the form \eqref{Prob:Gamma_Comb} with uncertainty set $\mathcal{U}_i := [\overline{c}_i, \overline{c}_i + \Delta c_i]$, we define (as in the notation of Problem~\eqref{Prob:GeneralNomOpt}) 
%\begin{gather*}
%\overline{u}^i := \overline{c}^i, \ f_i(x,c_i) = c_ix_i, \ \mathcal{U}_i = \{ c_i = \overline{c^i} + \alpha \Delta c_i \mid \alpha \in [0,1]\}, \ \mathcal{Z}_i := [0,1].
%\end{gather*}
%Since $f_i$ is linear in the uncertainty, we obtain $v^k = l_k(x) = x_k$ and \begin{gather*}
%\theta^k = \delta^*(\Delta c_kx_k \mid \mathcal{Z}^k) = \sup_{\zeta \in [0,1]} \zeta \Delta c_k x_k = \Delta c_k x_k
%\end{gather*}
%for $k \in [m]$, since $x_k \in \{0,1\}$ and $\Delta c_k \geq 0$. Hence we need to solve 
%\begin{alignat*}{2}
%\min_{k \in \{0, \dots, m\}} & \min_{x} \Gamma \Delta c_k x_k + \sum_{i \in [m]} \overline{c_i} x_i + \max \{0, \Delta c_i x_i - \Delta c_k x_k\}, \\
%\text{s.t.} & x \in \mathcal{X}
%\end{alignat*}
%where $\Delta c_0 := x_0 := 0$. Now, if we assume without loss of generality that $\Delta c_1 \geq \Delta c_2 \geq \dots \geq \Delta c_m \geq 0$, one obtains the result of Proposition~\ref{Prop:Tractable_Gamma_Comb}: If $x_k = 0$, the inner problem is 
%\begin{gather*}
%\min_{x} \sum_{i \in [m]} \overline{c}_i x_i + \max \{0, \Delta c_i x_i \} = \min_x \sum_{i \in [m]} \overline{c}_i x_i + \Delta c_i x_i. 
%\end{gather*}
%It can easily be seen that this is exactly the model from Proposition~\ref{Prop:Tractable_Gamma_Comb}. %for $k = n+1$. If $x_k = 1$, one obtains 
%%\begin{alignat*}{2}
%%\min_{x} \Gamma \Delta c_k + \sum_{i \in [m]} \overline{c}_i x_i + \max \{0, \Delta c_i x_i - \Delta c_k\} &= \Gamma \Delta c_k + \min_{x} \overline{c}^Tx + \sum_{i \in [m]} \max \{0, \Delta c_i - \Delta c_k\} x_i \\ &= \Gamma \Delta c_k + \min_{x} \overline{c}^Tx + \sum_{i \in [m]} (\Delta c_i - \Delta c_k) x_i.
%%\end{alignat*}
%%which are the inner problems for $k = 1, \dots, n$ in Proposition~\ref{Prop:Tractable_Gamma_Comb}.
%\end{example}
%%\begin{example}[Linear in the uncertainty]
%%Easy to prove (see \cite{Fenchel}): $\theta^k = \delta^*({A^k}^Tv^k \mid Z^k)$, if 
%%\begin{gather*}
%%f_k(x, u^k) = {u^k}^Tl_k(x) 
%%\end{gather*}
%%for a (affine-)linear function $l_k \colon \R^n \to \R^m$. In particular, this implies that, for $k > 0$, we obtain (as an inner problem)
%%\begin{alignat*}{2}
%%\min_{x} \ & \Gamma \delta^*({A^k}^Tl_k(x)|Z_k) + \sum_{i \in [m]} f_i(x,\overline{u^i}) + \max \{0, \delta^*({A^i}^Tl_i(x)|Z_i)- \delta^*({A^k}^Tl_k(x)|Z_k) \} \\
%%\text{s.t.} & x \in \mathcal{X} 
%%\end{alignat*}
%%\end{example}
%%\todo[inline][inline]{Jana: Abschnitt zu MINLP-Kombinatorik schreiben. SpezialfÃ¤lle in denen man direkt ablesen kann, was passiert?}
%Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} implies that for combinatorial optimization problems, even if the functions $f_i$ are linear, obtaining a computationally tractable version for the $\Gamma$--counterpart is not easy. % The structure of the objective function is non-linear and more difficult due to
%%\begin{gather*}
%%\max\{0, \theta^i(x) - \theta^k(x)\}
%%\end{gather*}
%%which is in general, in combination with optimizing, a very hard optimization problem. 
%However, for many combinatorial optimization problems, the functions
%$f_i(x,u^i)$ are linear in the uncertainty %- i.e., $f_i(x,u^i) =
%                                %(u^i)^Tl_i(x)$ for some function
%%$l_i$ -
%and the uncertainty set for a parameter $u^i$ is an interval, i.e., $\mathcal{U}_i:=[\overline{u}^i,\overline{u}^i + \Delta u^i]$. In this case, applying Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} results in 
%\begin{gather*}
%\theta^k(x) = \Delta u_k l_k(x), \ k \in [m], 
%\end{gather*} 
%and thus in the optimization problem
%\begin{align}\label{Prob:CombGammaCounterPartFenchelStandard}
%\begin{split}
%\min_{k \in \{0, \dots, m\}} & \min_{x} \Gamma \Delta u_k l_k(x) + \sum_{i \in [m]} (\overline{u}^i)^Tl_i(x) + \max \{0, \Delta u_i l_i(x) - \Delta u_k l_k(x) \} \\
%\text{s.t.} & x \in \mathcal{X} \\
%%& \theta^k \geq 0. \\
%%& \theta^k = \overline{u^k}^Tv^k - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k) + \support{k}).
%\end{split}
%\end{align}

%Example~\ref{ex:QAP_genau} demonstrates that the exploitation of the combinatorial structure can result in a computationally tractable reformulation of a non-linear combinatorial optimization problem based on Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} and more generally on Theorem~\ref{Theo:GeneralGammaCounterPartWithoutDual} without losing the combinatorial structure. In general, the tractability of model~\eqref{Prob:GammaCombCounterpartWithoutFenchel} still heavily depends on the actual objective function of the nominal problem, the geometry of the uncertainty set and the combinatorial structure of $\mathcal{X}$. \\


%Theorem~\ref{Theo:CorrDoNotCare} shows that, at least in a special
%assignment structure of $B$ and $g$, it is possible to perform an affine transformation of the uncertainty set 
%'linearly
%combine'\todo[inline]{ist das nicht eher ein kreuzprodukt von intervallen?}
%\todo[inline]{Ich konstruiere ja die Menge $[\overline{u}^TB_{.,(i,j)}, (\overline{u}_i, \overline{u}_i + \Delta u_i)^TB_{.,(i,j)}]$, also Matrix mit ner Box multiplifiziert. Hab das ganze jetzt mit ner affinen Transformation umformuliert.}
Thus, if $g(x)$ is a $0/1$--function, then one can apply Theorem~\ref{Theo:CorrDoNotCare} to obtain an equivalent $\Gamma$--counterpart where the uncertainty is linear and no matrix $B$ is involved. The following corollary demonstrates this for $g(x) = x$:
\begin{corollary}\label{Cor:LPsAssigment}
Consider program \begin{gather}\label{Prob:nom_LP_under_unc:ASSIGN}
\min_{x \in \mathcal{X}} u^TBx
\end{gather}
as in the setting of Theorem~\ref{Theo:CorrDoNotCare} and assume that $
\mathcal{X} \subseteq \{x \in \{0,1\}^{[m] \times [n]}: \sum_{j \in [n]} x_{i,j} = 1 \ \forall i \in [m]\}$.
Let $\Gamma \in [m]$. Then the $\Gamma$--counterpart of \eqref{Prob:nom_LP_under_unc:ASSIGN} is equivalent to
\begin{align*}
\min_{(k,l) \in [m] \times [n] \cup \{(0,0)\}} \left\{ \Gamma \Delta u_k B_{k,(k,l)}  +
\min_{x \in \mathcal{X}} \left\{ \overline{u}^TBx + \sum_{(i,j) \in [m] \times [n]} F_{i,j,k,l}(x) \right\} \right\}
\end{align*}
where $B_{0,.} := \Delta u_0 := 0$ (the first one being a row vector of zeros and the latter being the number $0$) and 
\begin{gather*}
F_{i,j,k,l}(x):=\max\{0, \Delta u_i B_{i,(i,j)} - \Delta u_k B_{k,(k,l)}\}x_{i,j}.
\end{gather*}
\end{corollary}
%\begin{align*} %\label{Prob:RobustCounterpartSuperComb}
%\begin{split}
%\min_{\substack{(k,l) \in [m] \times [n] \\ \lor k = l = 0 }} \left\{\Gamma \Delta u^T B_{.,(k,l)} + 
% \min_{x \in \mathcal{X}}  \overline{u}^TBx + \sum_{(i,j) \in [m] \times [n]} \max \left\{0,\Delta u^T\left( B_{.,(i,j)} - B_{.,(k,l)}\right)\right\}x_{i,j} \right\}.
%\end{split} 
%\end{align*}
%$\min_{x Assume that for all $i \in [m]$, there is a function $l_i\colon \R^n \to \R^{L_i} $, such that $f_i(x,u^i) = (u^i)^Tl_i(x)$, i.e., $f_i$ is linear in the uncertainty and in the decision. Assume that the uncertainty set is $\mathcal{U}^i := [\overline{u}^\overline{u}^i + \Delta u^i
\begin{proof}
This follows from Theorem~\ref{Theo:CorrDoNotCare} and Proposition~\ref{Prop:Tractable_Gamma_Comb} by setting $g(x) = x$.
\end{proof}


%\subsection{Computational complexity}
%In this subsection, we make some remarks about the difficulty of solving $\Gamma$--counterparts.
%%Before we show some computational exampled, we would like to give some
%%thoughts about the computational complexity of
%%$\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart}.
%In the case of a pure combinatorial optimization problem with a linear objective and binary variables under interval uncertainty, the $\Gamma$--counterpart is solvable in oracle-polynomial time with a linear number of oracle calls \cite{IntroGamma}. Thus, if the nominal problem is solvable in polynomial time, this is also the case for the $\Gamma$--counterpart. This also holds in the setting of Theorem~\ref{Theo:PseudoLin}. The same does hold for $\alpha$-approximability: If the nominal problem is $\alpha$-approximable, the problem stays $\alpha$-approximable, see Theorem~\ref{Theo:Approx}. \\
%In the more general concave setting, $
%\supportx{k} $ needs to be determined
%for each $k \in [m]$, i.e., an additional
%optimization problem needs to be solved. This can result in more than linearly many optimization problems: Even in Example~\ref{Ex:Scheduling}, a quadratic number of problems need to be solved, although the problem is a binary, linear optimization problem. \\
%Furthermore, in \cite{RobustScheduling} the authors showed that not only the number of nominal optimization problems in the computationally tractable formulation that can increase not linearly but quadratically, they showed that the complexity class itself can change: Given a single-machine scheduling problem with a finite set of jobs $\mathcal{J}$, they considered the optimization problem
%\begin{gather}\label{Prob:WeightedCompletionTimeScheduling}
%\min_{x \in \mathcal{X}} \sum_{j \in \mathcal{J}} w_jC_j(x,p),
%\end{gather}
%see Example~\ref{Ex:Scheduling}. Problem~\eqref{Prob:WeightedCompletionTimeScheduling} is known to be polynomial because Smith's Rule can be applied \cite{Smith}. \\
%For $w_j = 1 \ \forall j \in \mathcal{J}$, the application of the
%$\Gamma$-flexible approach under uncertain processing times $p_j$
%stays polynomially solvable, while otherwise, solving the $\Gamma$--counterpart of problem~\eqref{Prob:WeightedCompletionTimeScheduling} is an $NP$-hard problem (if
%$\Gamma > 1$, it is strongly $NP$-hard). 
%This demonstrates that in general, the complexity of a combinatorial
%optimization problem under uncorrelated interval uncertainty can
%change for non-linear optimization problems, even if the
%objective is linear in the uncertainty and the decision. This is a crucial difference when compared to the setting of problem~\eqref{Prob:Gamma_Comb}, where the complexity class of the robust problem and the nominal problem are the sam.

\paragraph*{The special case of $0/1$--functions}
Before we apply our theory in Section~\ref{Sec:Reformulations}, we discuss one more case, namely the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} under linear one--dimensional interval uncertainty with $0/1$--functions:
\begin{assumption}\label{Ass:GeneralLinear01}
For the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} and for all $i \in [m]$ we assume:
\begin{itemize}
\item[(i)] The uncertainty set $\mathcal{U}_i$ is a 1--dimensional interval, i.e., $\mathcal{U}_i = [\overline{u}_i, \overline{u}_i + \Delta u_i] \subseteq \R_{> 0}$ and $\Delta u_i > 0$.
\item[(ii)] There is a $0/1$--function $l_i\colon \mathcal{X} \to \{0,1\}$ such that $f_i(x,u_i) = u_il_i(x)$ for all $u_i \in \mathcal{U}_i$.
\end{itemize}
\end{assumption}
%\begin{align}\label{Prob:Non-LinearBin}
%\min_{x \in \mathcal{X}} u^T l(x)
%\end{align}
%where $u \in \R^n$ is uncertain under interval uncertainty and $l(x) \in \{0,1\}^m$ for all $x \in \mathcal{X}$ and $\mathcal{X} \subseteq \{0,1\}^n$. This is a special case of model~\eqref{Prob:GeneralNomOpt} which is still non-linear since there are no assumptions for $l$ (expect that on $\mathcal{X}$, its image is a subset of $\{0,1\}^m$). 
Although Assumption~\ref{Ass:GeneralLinear01} seems restrictive, it covers many combinatorial programs under uncertainty, e.g. the quadratic knapsack problem or the quadratic matching problem. By applying Proposition~\ref{Prop:Tractable_Gamma_Comb}, we obtain the following:
\begin{theorem}\label{Theo:PseudoLin}
Let $\Gamma \in [m]$ and assume that Assumption~\ref{Ass:GeneralLinear01} holds. Then $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
\begin{gather}\label{Prog:PseudoLin}
\inf_{k \in [m]_0} \left\{ \Gamma \Delta u_k + \inf_{x \in \mathcal{X}} \left\{\overline{u}^Tl(x) + \sum_{j \in [m]} \max\{0,\Delta u_j - \Delta u_k\}l_j(x) \right\} \right\}.
\end{gather}
\end{theorem}
\begin{proof}
Under Assumption~\ref{Ass:GeneralLinear01}, program~\eqref{Prob:GeneralNomOpt} is equivalent to $\inf_{(x,y) \in \mathcal{X}_y} u^Ty$ with $\mathcal{X}_y := \mathcal{X} \times l(\mathcal{X}) \subseteq \R^n \times \{0,1\}^{m}$. Then Proposition~\ref{Prop:Tractable_Gamma_Comb} implies that the modified program's $\Gamma$--counterpart is equivalent to
\begin{gather*}
\inf_{k \in [m]_0} \left\{ \Gamma \Delta u_k + \inf_{x \in \mathcal{X}_y} \left\{\overline{u}^Ty + \sum_{j \in [m]} \max\{0,\Delta u_j - \Delta u_k\}y_j \right\} \right\}
\end{gather*}
where $\Delta u_0 := 0$. Since $y_j = l_j(x)$, the claim follows.
\end{proof}
%Naturally, since we applied Bertsimas' and Sim's original result, assuming that $l(x) \in \{0,1\}^m$ is binary is essential. Therefore, the previous theorem does not cover Examples~\ref{Ex:Scheduling} and \ref{Ex:QAP}. However, it does cover cases where $l_i(x)$ is a product of binary variables for each $i \in [m]$ which is the case for example, quadratic combinatorial optimization problems with objective \begin{gather*}
%\sum_{i \in [n]} p_i x_i + \sum_{i \in [n], j \in [n] \setminus \{i\}} p_{i,j}x_{i}x_{j}
%\end{gather*}
%for binary variables $x_i$ and uncertain coefficients. We demonstrate that in Section~\ref{Sec:Reformulations}.
Theorem~\ref{Theo:PseudoLin} demonstrates that one can solve the $\Gamma$--counterpart with an optimization oracle of program~\eqref{Prob:GeneralNomOpt}. This result only implies that additionally, one can reduce the number of oracle calls one has to solve and can determine $\alpha$-approximations (for $\alpha \geq 1$), if program~\eqref{Prob:GeneralNomOpt} is $\alpha$--approximable\footnote{The following definition is not formal and is usually applied for combinatorial programs: Assume that $f^* \in$~$(-\infty,\infty)$ is the optimal value of program~\eqref{Prob:GeneralNomOpt}. Then program~\eqref{Prob:GeneralNomOpt} is called $\alpha$--approximable when there exists a real number $\alpha \geq 1$ and an algorithm $\texttt{ALG}$ with input $(f,\mathcal{X})$, output $\tilde{x}$, the inequality $\alpha f^* \geq f(\tilde{x})$ holds for every instance $(f,\mathcal{X})$ and the running time of algorithm $\texttt{ALG}$ is polynomial in the encoding length of $(f, \mathcal{X})$.}. The proofs are both heavily inspired by the resp. proofs in \cite{IntroGamma} and \cite{Lee2014}:
\begin{theorem}\label{Theo:Approx}
Let $\Gamma \in [m]$. If Assumption~\ref{Ass:GeneralLinear01} holds and program~\eqref{Prob:GeneralNomOpt} is $\alpha$-approximable, then \eqref{Prob:GeneralGammaCounterpart} is $\alpha$--approximable. 
%equivalent to
%\begin{gather*}
%\min_{k \in \mathcal{L}} \Gamma \Delta u_k + \min_{x \in \mathcal{X}} f(x,\overline{u}) + \sum_{i \in [k]} \left(\Delta u_i - \Delta u_k \right)l_i(x)
%\end{gather*}
%for $\mathcal{L} := \{\Gamma + 1, \dots, \Gamma + \gamma, m + 1\}$ with $\gamma$ being the biggest odd integer smaller than $(m + 1) - \Gamma$ and $\Delta_{m+1}:=0$.
%\end{theorem}
\end{theorem}
\begin{proof}
For $k \in [m]_0$, we denote the objective of the $k$--th inner problem of program~\eqref{Prog:PseudoLin} with $G^k(x)$, i.e.,
\begin{gather*}
G^k(x) := \sum_{j \in [m]} (\overline{u}_j + \max\{0,\Delta u_j - \Delta u_k\})l_j(x). 
\end{gather*}
Naturally, one can $\alpha$--approximate program $\inf_{x\in \mathcal{X}} G^k(x)$ for each $k \in [m]_0$ by assumption. Let $x^k$ be the output of the given approximation algorithm with objective value $z^k$ and $Z^*$ be the optimal value of program~\eqref{Prog:PseudoLin}, which is equivalent to $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} since Assumption~\ref{Ass:GeneralLinear01} holds. Then we obtain
\begin{alignat*}{2}
Z^* & \leq \left( \sum_{i \in [m]} l_i(x^k)\overline{u}_i \right) +
\sup_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \sum_{i \in \mathcal{S}}  \Delta u_i l_i(x^k) \\
    & = \left( \sum_{i \in [m]} l_i(x^k)\overline{u}_i \right) + \inf_{\theta \geq 0} \sum_{j \in [m]} \max \{0, \Delta u_i l_i(x^k) -  \theta\} + \Gamma \theta \\
    & \overset{l_i(x^k) \in \{0,1\}}{=} \left(\sum_{i \in [m]} l_i(x^k)\overline{u}_i \right) + \inf_{\theta \geq 0} \sum_{j \in [m]} \max\{0, \Delta u_i  -  \theta \}l_i(x^k) + \Gamma \theta \\
    & \leq \Gamma \Delta u_k + \sum_{i \in [m]} (\overline{u}_i + \max \{0, \Delta u_i  -  \Delta u_k\})l_i(x^k)   \\
    & = \Gamma \Delta u_k + G^k(x^k) \\
    & \leq \alpha(z_k^* - \Gamma \Delta u_k) + \Gamma \Delta u_k \\
    & \overset{\alpha \geq 1}{\leq} \alpha z_k^* \\
    & = \alpha Z^*
\end{alignat*}
which proves the claim since it is sufficient to apply the given $\alpha$--approximation to $\inf_{x\in \mathcal{X}} G^k(x)$ for every $k \in [m]_0$ and to solve $\min_{k \in [m]_0} z_k$.
\end{proof}
\begin{theorem}\label{Theo:RedNumber}
Let $\Gamma \in [m]$ and assume that $\Delta u_1 \geq \Delta u_2 \geq \dots \geq \Delta u_m \geq 0$. If Assumption~\ref{Ass:GeneralLinear01} holds, then the $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
\begin{gather*}
\inf_{k \in \mathcal{L}} \left\{ \Gamma \Delta u_k + \inf_{x \in \mathcal{X}} \left\{ f(x,\overline{u}) + \sum_{i \in [k]} \left(\Delta u_i - \Delta u_k \right)l_i(x) \right\} \right\}
\end{gather*}
for $\mathcal{L} := \{\Gamma + 1, \dots, \Gamma + \gamma, m + 1\}$ with $\gamma$ being the largest odd integer smaller than $(m + 1) - \Gamma$ and $\Delta_{m+1}:=0$. Furthermore, if the optimal value of the $k$--th inner program is smaller than $\Gamma \Delta u_l$ for $l \in \mathcal{L}$, one can replace $\mathcal{L}$ with $\mathcal{L}^* := \{k \in \mathcal{L}: \ k > l\}$.
\end{theorem}
\begin{proof}
Since Assumption~\ref{Ass:GeneralLinear01} holds, this statement is a consequence of Theorem 1 in \cite{Lee2014} by introducing binary variables $y_i$, $i \in [m]$, with $y_i = l_i(x)$ (as in the proof of Theorem~\ref{Theo:PseudoLin}).
\end{proof}
In particular, Theorem~\ref{Theo:RedNumber} implies that, instead of solving $m+1$ nominal programs, one only needs to solve $\lceil \frac{m - \Gamma}{2} \rceil + 1$ subproblems instead of $m+1$, as in the case of Theorem~\ref{Theo:PseudoLin}. \cite{Lee2014} demonstrates that this significantly reduces the number of subproblems one needs to solve for the linear case. %We apply Theorem~\ref{Theo:RedNumber} in our numerical study in Section~\ref{Sec:App}. \\
\\
Before we conclude this section, for the sake of completeness, we note the following: 
\begin{remark}\label{Rem:Concave}
%\begin{enumerate}
%\item[i)] In the setting of Theorem~\ref{Theo:CorrDoNotCare}, one can also show that for the case of $k = 0$, exactly one subproblem needs to be solved, since (in program~\eqref{Model:GammaCounterPartCor}) $x \in \mathcal{X}_\mathcal{Q}$ only holds if and only if
%\begin{alignat*}{2}
%\Delta u_qB_{q,(q,j(q))}g_{q,j(q)}(x)&\geq 0 \ \forall q \in \mathcal{Q},\\
%\Delta u_qB_{q,(q,j(q))}g_{q,j(q)}(x)&\leq 0 \ \forall q \in [m] \setminus \mathcal{Q}
%%% \Delta y_{q,p}g_{q,p}(x) \leq \Delta y_{a,b(a)}g_{a,b(a)}(x) \ %%%\forall (q,p) \in ([m] \times [n]) \setminus \mathcal{Y}.
%\end{alignat*}
%which can only hold for $[m] = \mathcal{Q}$. Since it was not important for our theory, we only mention it here but for the reduction of the number of subproblems, this observation can be crucial. 
With respect to concave uncertainties under Assumption~\ref{Ass:General}, one can show that $\Gamma$--counterpart~\eqref{Prob:GeneralGammaCounterpart} is equivalent to
\begin{alignat}{2}\label{Reform:Concave}
\min_{k \in [m]_0} & \left\{ \min_{\substack{x \in \mathcal{X}, v^1 \in \R^{L_1}, \\  \dots, v^m \in \R^{L_m}}} \left\{ \Gamma \theta^k(x,v^k) + \sum_{i \in [m]} f_i(x,\overline{u}^i) + \max \{0, \theta^i(x,v^i)- \theta^k(x,v^k) \} \right\} \right\}
\end{alignat}
where
\begin{gather*}
\theta^k(x,v^k) := (\overline{u}^k)^Tv^k + \support{k} - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k)  \ \forall k \in [m].
\end{gather*}
In this context, however, it seems unlikely that one would use this formulation over the one given in Corollary~\ref{Prop:FenchelGammaCounterpart} since the objective is very different from the one of program~\eqref{Prob:GeneralNomOpt}, the feasible set was altered, rendering oracles not applicable.
\end{remark}


\section{Practical examples}\label{Sec:Reformulations}
In this section, we demonstrate some examples of the reformulations of Section~\ref{sec:Rev}. We note that some are maximization programs for which our theory naturally applies as well.
%\begin{example}
%We consider an optimization problem with a quadratic objective:
%\begin{align}\label{Prob:NomQuad}
%\min_{x \in \mathcal{X}} \sum_{i \in [m]} (x_i - u_i)^2.
%\end{align}
%For every $i \in [m]$, $u_i$ is subject to uncertainty $\mathcal{U}_i := [\overline{u}_i, \overline{u}_i + \Delta u_i]$. For $\Gamma \in [m]$, the $\Gamma$--counterpart of model~\eqref{Prob:NomQuad} after applying Lemma~\ref{Lem:ReModel} is given by
%\begin{align}\label{Prob:FirstQuad}
%\begin{split}
%\min_{x, p, \theta} & \ \Gamma \theta + \sum_{i \in [m]} (x_i - \overline{u}_i)^2 + p_i, \\
%\mathrm{s.t.} & \ x \in \mathcal{X}, \\
%& (x_i - u_i)^2 - (x_i - \overline{u}_i)^2 \leq p_i + \theta \ \forall u_i \in \mathcal{U}_i, \ \forall i \in [m].
%\end{split}
%\end{align}
%The inequalities of model~\eqref{Prob:FirstQuad} are equivalent to
%\begin{gather}\label{Ineq:ReformedQuad}
%-2x_i u_i + u_i^2 \leq p_i + \theta - 2x_i \overline{u}_i + \overline{u}_i^2 \ \forall u_i \in \mathcal{U}_i
%\end{gather}
%for each $i \in [m]$. The left-hand side of \eqref{Ineq:ReformedQuad} is not concave in $u_i$ and thus, we cannot apply the reformulations of Subsection~\ref{subsec:Concave}. However, \eqref{Ineq:ReformedQuad} is of the form \eqref{Ineq:SecondApproach}. We set
%\begin{gather*}
%g_1(x) = -2x, \ g_2(x) = 1, \ h(u_i) = u_i^2
%\end{gather*}
%and re-write the uncertainty set:
%\begin{gather*}
%[\overline{u}_i, \overline{u}_i + \Delta u_i] = \{u_i \in \R\colon (-2 \overline{u}_i - \Delta u_i)u_i + u_i^2 \leq -\overline{u}_i^2 - \overline{u}_i \cdot \Delta u_i\}.
%\end{gather*}
%Inequality~\eqref{Ineq:SecondApproach} is obtained by setting
%\begin{gather*}
%\alpha = -2\overline{u}_i - \Delta u_i, \ \beta = 1, \ \gamma = -\overline{u}_i^2 - \overline{u}_i \Delta u_i. \
%\end{gather*}
%Since $\alpha$ and $\beta$ are scalars, they are clearly term-wise parallel. Thus, we can set $b_i:=h(u_i):= u_i^2$ and \eqref{Ineq:ReformedQuad} is satisfied for $(x, p, \theta)$ if and only if there exists $v \in \R$, such that
%\begin{align*}
%&(1 + v)h_i^*\left(\frac{2x + 2 \overline{u}_iv + \Delta u_iv}{1+v}\right) - \overline{u}_i^2v - \overline{u}_iv \Delta u_iv \le p_i + \theta -2x_i \overline{u}_i + \overline{u}_i^2,\\
%&1 + v \ge 0,\\
%&v\ge 0.
%\end{align*}
%Clearly, the second inequality is redundant. Furthermore, since
%$h_i^*(z) = \frac{z^2}{4}$, the first inequality is convex in $(x,v)$ if it is assumed that $x \geq 0$. This is a valid assumption for many problems, for example in logistics. Thus, assuming that $\mathcal{X}$ is a convex set, the $\Gamma$--counterpart of problem~\eqref{Prob:NomQuad} is a convex optimization problem, although it is not concave in the uncertainty.
%\end{example}
\paragraph*{Linear programs under uncertainty}
Here, we cover the case of $\min_{x \in \mathcal{X}} u^TBx$. If $B$ is the unit matrix and $u$ is subject to interval uncertainty, we obtain the original setting of Bertsimas and Sim. We have already shown with Corollary~\ref{Cor:LPsAssigment} that there is a case where one can 'shift' $B$ into the uncertainty set and that one can solve the $\Gamma$--counterpart with a polynomial number of oracle calls. This is a generalization of a result in \cite{RobustScheduling} which has been applied to the single--machine scheduling problem under uncertainty:
%\begin{corollary}\label{Cor:LPsAssigment}
%Consider the optimization problem \begin{gather}\label{Prob:nom_LP_under_unc:ASSIGN}
%\min_{x \in \mathcal{X}} u^TBx
%\end{gather}
%as in the setting of Theorem~\ref{Theo:CorrDoNotCare} and assume that $
%\mathcal{X} \subseteq \{x \in \{0,1\}^{[m] \times [n]}: \sum_{j \in [n]} x_{i,j} = 1 \ \forall i \in [m]\}$.
%Let $\Gamma \in [m]$. Then the $\Gamma$--counterpart of \eqref{Prob:nom_LP_under_unc:ASSIGN} is equivalent to
%\begin{align*}
%\min_{(k,l) \in [m] \times [n] \cup \{(0,0)\}}  \Gamma \Delta u_k B_{k,(k,l)}+ 
%\min_{x \in \mathcal{X}} \overline{u}^TBx + \sum_{(i,j) \in [m] \times [n]} \max\{0, \Delta u_i B_{i,(i,j)} - \Delta u_k B_{k,(k,l)}\}x_{i,j},
%\end{align*}
%where $B_{0,.} := \Delta u_0 := 0$.
%\end{corollary}
%%\begin{align*} %\label{Prob:RobustCounterpartSuperComb}
%%\begin{split}
%%\min_{\substack{(k,l) \in [m] \times [n] \\ \lor k = l = 0 }} \left\{\Gamma \Delta u^T B_{.,(k,l)} + 
%% \min_{x \in \mathcal{X}}  \overline{u}^TBx + \sum_{(i,j) \in [m] \times [n]} \max \left\{0,\Delta u^T\left( B_{.,(i,j)} - B_{.,(k,l)}\right)\right\}x_{i,j} \right\}.
%%\end{split} 
%%\end{align*}
%%$\min_{x Assume that for all $i \in [m]$, there is a function $l_i\colon \R^n \to \R^{L_i} $, such that $f_i(x,u^i) = (u^i)^Tl_i(x)$, i.e., $f_i$ is linear in the uncertainty and in the decision. Assume that the uncertainty set is $\mathcal{U}^i := [\overline{u}^\overline{u}^i + \Delta u^i
%\begin{proof}
%This follows from Theorem~\ref{Theo:CorrDoNotCare} and Proposition~\ref{Prop:Tractable_Gamma_Comb} by setting $g(x) = x$.
%\end{proof}
%Now, regarding Example~\ref{Ex:Scheduling}, one can apply Corollary~\ref{Cor:LPsAssigment}:
%Corollary~\ref{Cor:LPsAssigment} 
\begin{example}\label{Ex:SchedulingGeneral}
We recall that in Section~\ref{sec:Rev}, we considered an instance of the program %problems of the form
\begin{align}\label{Prob:NomScheduling}
\begin{split}
\min_{x} & \ \sum_{i,j \in \mathcal{I}, \mathcal{J}} u_i q_j x_{i,j}, \\
\mathrm{s.t.} & \ x \in \mathcal{X} \subseteq \left\{x \in \{0,1\}^{|\mathcal{I}|\cdot|\mathcal{J}|}:
\sum_{j \in \mathcal{J}} x_{i,j} = 1 \ \forall i \in \mathcal{I}\right\}
\end{split}
\end{align}
where $u_i$ is subject to uncertainty $[\overline{u}_i, \overline{u}_i + \Delta u_i]$ in the context of single--machine scheduling. By applying Corollary~\ref{Cor:LPsAssigment}, one can show that the $\Gamma$--counterpart of program~\eqref{Prob:NomScheduling} is equivalent to taking the minimum of
\begin{align*}
\min_{(k,l) \in \mathcal{I} \times \mathcal{J}} \left\{ \Gamma q_k \Delta u_l + \min_{x \in \mathcal{X}} \left\{ \sum_{i,j \in \mathcal{I}, \mathcal{J}} (\overline{u}_i + \max\{0, \Delta u_i - \frac{\Delta u_k q_l}{q_j}\})q_jx_{i,j} \right\} \right\}
\end{align*}
and 
\begin{align*}
\min_{x \in \mathcal{X}} \sum_{i,j \in \mathcal{I}, \mathcal{J}} (\overline{u}_i + \Delta u_i)q_jx_{i,j}.
\end{align*}
In \cite{RobustScheduling}, this has been shown by algebraic means.
%This was established through algebraic manipulations and reformulations which were used to prove
%Proposition~\ref{Prop:Tractable_Gamma_Comb}. We establish the same result through Corollary~\ref{Cor:LPsAssigment}: By setting
%\begin{gather*}
%B:= \begin{pmatrix}
%q_1   \dots q_{|\mathcal{J}|} & 0_{\mathcal{J}} & \dots & 0_{\mathcal{J}} \\
%0_{\mathcal{J}} & q_1   \dots q_{|\mathcal{J}|} & 0_{\mathcal{J}} \dots & 0_{\mathcal{J}} \\
%\vdots & \vdots & \vdots & \vdots \\
%0_{\mathcal{J}} & 0_{\mathcal{J}} & 0_{\mathcal{J}} & q_1   \dots q_{|\mathcal{J}|} 
%\end{pmatrix} \in \R^{|\mathcal{I}| \times |\mathcal{I}| |\mathcal{J}|},
%\end{gather*}
%and inserting this into~\eqref{Prob:RobustCounterpartSuperComb}, we obtain the same reformulation.
\end{example}

\paragraph*{Quadratic programs under uncertainty}
As an application of Corollary~\ref{Cor:LinInt}, we reformulate the QAP under uncertainty given in Section~\ref{sec:Rev}. 
\begin{example}\label{ex:QAP_genau}
We consider the QAP under interval uncertainty
\begin{align}\label{Prob:QAP_Nom}
\begin{split}
\min_{x} & \ \sum_{(i,j,r,s) \in [n]^4} c_{i,j}d_{r,s}x_{i,r}x_{j,s} \\
\mathrm{s.t.} & \ x \in \mathcal{X} = \{x \in \{0,1\}^{[n]^2}: \sum_{i \in [n]} x_{i,r} = 1 \ \forall r \in [n], \ \sum_{r \in [n]} x_{i,r} = 1 \ \forall i \in [n]\}
\end{split}
\end{align}
with uncertain coefficients $c_{i,j} \in \mathcal{U}_{i,j} := [\overline{c}_{i,j}, \overline{c}_{i,j} + \Delta c_{i,j}] \subseteq \R_{\geq 0}$ for all $i,j \in [n]$ and $d_{r,s} \geq 0$ for all $r,s \in [n]$. Let $\Gamma \in [n^2]$.
The objective of ~\eqref{Prob:QAP_Nom} equals $u^TBg(x)$ where $B \in \R^{n^2 \times n^4}$ is a block diagonal matrix with $n^2$ copies of $d^T$, $u = c$ and $g_{(i,j),(r,s)}(x):= x_{i,r}x_{j,s}
$ for $(i,j,r,s) \in [n]^4$. Then Theorem~\ref{Theo:CorrDoNotCare} implies that the $\Gamma$--counterpart of program~\eqref{Prob:QAP_Nom} is equivalent to the $\Gamma$--counterpart of
\begin{gather*}
\min_{x \in \mathcal{X}} y^Tg(x)
\end{gather*}
with $y \in \R^{n^4}$ being subject to interval uncertainty, in particular $y_{i,j,r,s} \in [\overline{c}_{i,j}d_{r,s}, (\overline{c}_{i,j} + \Delta c_{i,j})d_{r,s}]$ for $i,j,r,s \in [n]$. Now, we can apply Theorem~\ref{Theo:PseudoLin} and we obtain the reformulation
%\begin{align}\label{Prob:QAP_Reform_One}
%\min_{(k_1,k_2,k_3,k_4) \in [n]^4 \cup \{(0,0,0,0)\}} & \min_{x \in \mathcal{X}} \Gamma \Delta (\overline{c}_{k_1,k_2} + \Delta c_{k_1,k_2})d_{k_3,k_4} x_{k_1,k_3}x_{k_2,k_4} + \sum_{(i,j) \in [n]^2} \overline{c}_{i,j}d_{r,s}x_{i,r}x_{j,s} + \max \{0, \Delta {c}_{i,j}d_{r,s}x_{i,r}x_{j,s} - \Delta c_{k_1,k_2}d_{k_3,k_4} x_{k_1,k_3}x_{k_2,k_4} \}
%\end{align}
%where $\bar{c}_{0,0} := \Delta c_{0, 0} := d_{0,0} := x_{0,0} = 0$. We assume that $x_{k_1,k_3}x_{k_2,k_4} = 1$ for $(k_1,k_2,k_3,k_4)\in [n]^4$ (otherwise the term would be $0$ and we would be in the case $k_i = 0$ for $i \in [4]$). Then, 
%\begin{alignat*}{2}
%\max \{0, \Delta {c}_{i,j}d_{r,s}x_{i,r}x_{j,s} - \Delta c_{k_1,k_2}d_{k_3,k_4} x_{k_1,k_3}x_{k_2,k_4} \} &= 
%\max \{0, \Delta {c}_{i,j}d_{r,s}x_{i,r}x_{j,s} - \Delta c_{k_1,k_2}d_{k_3,k_4}  \} =  \\
%&=\max \{0, \Delta {c}_{i,j}d_{r,s} - \Delta c_{k_1,k_2}d_{k_3,k_4}\}x_{i,r}x_{j,s},
%\end{alignat*} 
%since all involved numbers are non-negative. 
%
%Thus, problem~\eqref{Prob:QAP_Reform_One} is equivalent to
\begin{align}\label{Prob:QAP_Reform_Two}
\min_{\substack{(k_1,k_2,k_3,k_4) \in [n]^4 \\ \cup \{(0,0,0,0)\}}} & \left\{ \Gamma (\Delta c_{k_1,k_2})d_{k_3,k_4} + \min_{x \in \mathcal{X}} \left\{ F_{k_1,k_2,k_3,k_4}(x) \right\} \right\}
\end{align}
where 
\begin{gather*}
F_{k_1,k_2,k_3,k_4}(x) = \sum_{(i,j,r,s) \in [n]^4} (\overline{c}_{i,j}d_{r,s} + \max \{0, \Delta {c}_{i,j} d_{r,s} - \Delta c_{k_1,k_2}d_{k_3,k_4} \})x_{i,r}x_{j,s} 
\end{gather*}
for $(k_1,k_2,k_3,k_4) \in [n]^4$, $F_{0,0,0,0}(x) := \sum_{(i,j,r,s) \in [n]^4}  (\overline{c}_{i,j}d_{r,s} + \Delta {c}_{i,j} d_{r,s})x_{i,r}x_{j,s}$, and $\Delta c_{0,0} := d_{0,0} := 0$.
%\begin{align}\label{Prob:QAP_Reform_Two}
%\min_{(k_1,k_2,k_3,k_4) \in [n]^4 \cup \{(0,0,0,0)\}} & \Gamma (\Delta c_{k_1,k_2})d_{k_3,k_4} + \min_{x \in \mathcal{X}, \ x_{k_1 k_3} x_{k_2 k_4} = 1} \sum_{(i,j,r,s) \in [n]^4} (\overline{c}_{i,j}d_{r,s} + \max \{0, \Delta {c}_{i,j} d_{r,s} - \Delta c_{k_1,k_2}d_{k_3,k_4} \})x_{i,r}x_{j,s}.
%\end{align}
%%%Since $x_{k_1 k_3} x_{k_2 k_4} = 1$ is equivalent to $x_{k_1 k_3} = x_{k_2 k_4}= 1$, facilities $k_1$ and $k_2$ are assigned to locations $k_3$ and $k_4$, respectively. Thus, the variables $x_{k_1 j}$, $x_{k_2 j}$, $x_{i k_3}$ and $x_{i k_4}$ are fixed for all $j \in [n]$ and we can neglect those variables. Thus, we can replace the feasible set with 
%%%\begin{gather*}
%%%\mathcal{X}_{k_1,k_2,k_3,k_4} := \left\{x \in \{0,1\}^{[n]_{\setminus k_1,k_2} \times [n]_{\setminus k_3,k_4}}: \ \sum_{i \in [n]_{\setminus k_1,k_2}} x_{i,r} = 1 \ \forall r \in [n]_{\setminus k_3,k_4}, \ \sum_{r \in [n]_{\setminus k_3,k_4}} x_{i,r} = 1 \ \forall i \in [n]_{\setminus k_1,k_2} \right\}.
%%%%\begin{gather*}
%%%%\tilde{\mathcal{X}} := \left\{ x \in \{0,1\}^{([n]\setminus \{k_1,k_2\}) \times ([n] \setminus \{k_3,k_4\})}: \ \sum_{i \in [n]\setminus \{k_1,k_2\}} x_{i,r} = 1 \ \forall r \in [n] \setminus \{k_3,k_4\}, \ \sum_{r \in [n]\setminus \{k_3,k_4\}} x_{i,r} = 1 \ \forall i \in [n] \setminus \{k_1,k_2\} \right\}. 
%%%%
%%%\end{gather*} 
%The inner problems are infeasible, if exactly one of the equations $k_1 = k_2$ or $k_3 = k_4$ holds (for $k_1,k_2,k_3,k_4 \in [n]$). 
If we assume that the flow and the distance coefficients are symmetrical, i.e., $\Delta c_{i,j} = \Delta c_{j,i}$ and $d_{r,s} = d_{s,r}$ for all $i,j,r,s \in [n]$, then we only have to solve inner problems of the set
\begin{gather*}
\mathcal{M}:=\{(k_1,k_2,k_3,k_4) \in [n]^4: \ k_1 < k_2, k_3 < k_4\} \cup \{(0,0,0,0)\}.
\end{gather*}
Thus, one needs to solve $1 + (\frac{n(n-1)}{2})^2 = \frac{n^4 - n^3}{2} + 1$ QAPs to solve program~\eqref{Prob:QAP_Reform_Two}.
%, in particular
%\begin{align}\label{Prob:QAP_Reform_Three}
%\min_{(k_1,k_2,k_3,k_4) \in \mathcal{M}} & \Gamma (\Delta c_{k_1,k_2})d_{k_3,k_4}  + \min_{x \in \mathcal{X}} \sum_{(i,j,r,s) \in [n]^4} (\overline{c}_{i,j}d_{r,s} + \max \{0, \Delta {c}_{i,j} d_{r,s} - \Delta c_{k_1,k_2} d_{k_3,k_4} \})x_{i,r}x_{j,s}.
%\end{align}
By application of Theorem~\ref{Theo:RedNumber}, we can reduce the number of subproblems to $\lceil \frac{n^4 - n^3}{4}  + \frac12 - \frac{\Gamma}{2} \rceil + 1$. In our electronic companion, we demonstrate how the application of Theorem~\ref{Theo:RedNumber} significantly speeds up the the optimization process.
%Furthermore, since $d_{r,s}$ is the distance between locations $r$ and $s$, $d_{r,s} = d_{s,r}$  for all $r,s \in [n]$.  Thus, we only have to consider already covered by the cases in $\mathcal{M}_1:=\{(i,j,r,s) \in [n]^4: r < s \}$. Similarly, the flows are symmetrical in the sense that $\Delta u_{i,j} = \Delta u_{j,i}$ and it is sufficient to cover the cases in $\mathcal{M}_2:= \{(i,j,r,s) \in [n]^4: i \leq j \}$. Finally, $\Delta c_{i,i} = 0 = d_{i,i}$ for $i \in [n]$ (since there is no flow from a facility to itself) and these cases are covered by $(k_1,k_2,k_3,k_4) = (0,0,0,0)$. With $\mathcal{M}_3:= \{(i,j,r,s) \in [n]^4: i \neq j \land r \neq s\}$, one finally obtains the following scenarios:
%\begin{gather*}
%\mathcal{M} := \mathcal{M}_1  \cap \mathcal{M}_2 \cap \mathcal{M}_3 = \{(i,j,r,s) \in [n]^4: i < j, \ r < s\}
%\end{gather*}
%and $(k_1,k_2,k_3,k_4) = (0,0,0,0)$ -- thus, one needs to solve $n^4 + 1$ nominal problems.
%
%\todo[inline][inline]{Fehler??}
%%If we take the definition of the QAP into account, i.e., $d_{r,r} = 0$ for $r \in [n]$ and $d_{r,s} = d_{s,r}$ for $r,s \in [n]$, we can neglect the cases of $k_3=k_4$ and need to solve $1 + n^4 - n^2(\frac{n(n+1)}{2}) = n^4 - \frac{n^4 + n^3}{2} + 1 = \frac{n^4 - n^3}{2} + 1$  QAPs without uncertainty in \eqref{Prob:QAP_Reform_Two}.
%%the minimum 
%  A QAP with uncertain flow coefficients under interval uncertainty  has been solved by linearizing the non-linearities and applying the original results of Bertsimas and Sim. We aim to apply Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear}  and set
%\begin{gather*}
%f_{k_1k_2}(x,c_{k_1k_2})= c_{k_1k_2} \sum_{(r,s)\in [n]^2} d_{rs}x_{k_1r}x_{k_2s} =: c_{k_1k_2}l_{k_1k_2}(x) \ \forall k_1, k_2 \in [n],
%\end{gather*}
%with the interval uncertainty set $
%\mathcal{U}_{k_1k_2} := [\overline{c}_{k_1k_2}, \overline{c}_{k_1k_2} + \Delta c_{k_1k_2}]$ for all $k_1, k_2 \in [n]$, and recall that $\mathcal{X} = \{x \in \{0,1\}^{[n]^2}: \sum_{i \in [n]} x_{ir} = 1 \ \forall r \in [n], \ \sum_{r \in [n]} x_{ir} = 1 \ \forall i \in [n]\}$.

%\begin{align}\label{Prob:QAPRC}
%\begin{split}
%&\min_{x\in \mathcal{X}}  \max_{\mathcal{S} \subseteq [n]^2: |\mathcal{S}| \le \Gamma} %\left\{ \sum_{(i,j)\in \mathcal{S}}^n \max_{c_{ij}\in \mathcal{U}_{ij}} \sum_{(r,s)\in [n]^2} c_{ij} d_{rs}x_{ir}x_{js} + \sum_{(i,j) \in [n]^2 \setminus \mathcal{S}} \sum_{(r,s)\in [n]^2} \bar{c}_{ij} d_{rs}x_{ir}x_{js} \right\} 
%\end{split}
%\end{align} 
%\[\mathcal{U}_{ij}= [\bar{c}_{ij}, \bar{c}_{ij}+ \Delta c_{ij}], \quad \forall (i,j) \in [n]^2.\]
%By application of Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear}: 
%\[\bar{u}_{k_1k_2} = \bar{c}_{k_1k_2}, \quad l_{k_1k_2}(x)= \sum_{(r,s)\in [n]^2} d_{rs}x_{k_1r}x_{k_2s}\] and
%\[f_{k_1k_2}(x,c_{k_1k_2}) = c_{k_1k_2}\sum_{(r,s)\in [n]^2} d_{rs} x_{k_1r}x_{k_2s}\]with $ (k_1,k_2)\in [n]^2$. The uncertainty set can be expressed as box uncertainty 
%\[\mathcal{U}_{k_1k_2} = \left\{ c_{k_1k_2}|c_{k_1k_2} = \bar{c}_{k_1k_2} + \alpha \Delta c_{k_1k_2}, \alpha \in \mathcal{Z}_{k_1k_2} \right\}\]  with $\mathcal{Z}_{k_1k_2}=[0,1]$.  
%We apply
%reformulation~\eqref{Prob:CombinatorialGammaCounterPartWithoutDualLinear},
%which implies that \eqref{Prob:QAP_RobCP} is equivalent to the minimum
%of
%\[\theta_{k_1k_2}(x) = \delta^*(\Delta c_{k_1k_2} l_{k_1k_2}(x)|\mathcal{Z}_{k_1k_2})= \Delta c_{k_1k_2}\sum_{(r,s)\in [n]^2} d_{rs}x_{k_1r}x_{k_2s} = f_{k_1k_2}(x,\Delta c_{k_1k_2}) \ \forall k_1,k_2 \in [n]\]
%and $\theta_{0,0}(x)=0$,
%the reformulation of $\Gamma$--counterpart~\eqref{Prob:QAP_RobCP} is given by the minimum of
%\begin{align}\label{Prob:QAP_Gen}
%\begin{split}
%&\min_{ k_1,k_2 \in [n]} \min_{x\in \mathcal{X}} \ \Gamma \sum_{r,s \in [n]} d_{rs}\Delta c_{k_1 k_2}x_{k_1r}x_{k_2s} +\\
% & \sum_{i,j\in [n]} \left(\sum_{r,s\in [n]} \bar{c}_{ij}d_{rs}x_{ir}x_{js} + \max\left\{0, \sum_{r,s\in [n]} d_{rs}\left(\Delta c_{ij} x_{ir}x_{js}-\Delta c_{k_1 k_2} x_{k_1r}x_{k_2s}\right)\right\}\right)
% \end{split}
%\end{align}
%%\begin{align}\label{Prob:QAP_Gen}
%%\min_{ (k_1,k_2) \in [n]^2} \min_{x\in \mathcal{X}} \Gamma f_{k_1k_2}(x,\Delta c_{k_1k_2}) 
%%+ \sum_{(i,j)\in [n]^2} \left(f_{k_1k_2}(x, \overline{c}_{ij})+ \max\left\{0, f_{ij}(x, \Delta c_{i,j}) -f_{k_1k_2}(x, \Delta c_{k_1k_2})\right\}\right).
%%\end{align}
%and
%\begin{align}\label{Prob:thetanull}
%\min_{x\in\mathcal{X}} \sum_{i,j\in [n]} \sum_{r,s \in [n]} ( c_{ij} + \Delta c_{ij})d_{rs} x_{ir}x_{js}.
%\end{align}
%%\begin{align*}
%%\min_{x\in \mathcal{X}} 
%%\sum_{(i,j)\in [n]^2} f_{k_1k_2}(x, \overline{c}_{ij})+ f_{i,j}(x, \Delta c_{i,j}).
%%\end{align*}
%Since the inner minimization problems of model~\eqref{Prob:QAP_Gen} are not QAPs, we reformulate the objective: As $x \in \mathcal{X}$,
%the equation $\sum_{s \in [n]} x_{js} = 1$ holds for all $j \in [n]$. We obtain
%%since
%%\[\theta_{k_1k_2}(x) = \delta^*(\Delta c_{k_1k_2} l_{k_1k_2}(x)|\mathcal{Z}_{k_1k_2})= \Delta c_{k_1k_2}\sum_{(r,s)\in [n]^2} d_{rs}x_{k_1r}x_{k_2s} = f_{k_1k_2}(x,\Delta c_{k_1k_2})\]
%%and $\theta_0(x)=0$.
%%$x_{\theta}$ is the $x\in \mathcal{X}$ minimal for $\theta$. The optimal solution of \eqref{Prob:QAP_RobCP} is the minimum of all $(\theta, x_{\theta})$. Therefore, we reformulate the objective as
%%The inner minimization-problem is not a quadratic assignment problem due to the maximum in the objective. To keep the structure of a QAP we have to reformulate the objective:\\
%\begin{align}\label{Prob:OneSum}
%\sum_{r\in[n]} \sum_{s\in[n]} x_{ir}x_{js}= \sum_{r\in[n]} x_{ir} \sum_{s \in [n]} x_{js} =1 \ \forall i,j \in [n].
%\end{align} 
%Therefore, $x_{k_1r}x_{k_2s} = 1 $ for exactly one pair $(r,s)\in
%[n]^2$  for every $k_1,k_2\in [n]$, i.e., $x_{k_1r}x_{k_2s} = 1$
%only holds in exactly one case. Thus, instead of optimizing over
%$(k_1,k_2) \in [n]^2 $ in model~\eqref{Prob:QAP_Gen}, we optimize over
%$(k_1, k_2, k_3, k_4) \in [n]^4$ to fix all indices of
%$c_{k_1k_2}d_{k_3k_4}$. Then, model~\eqref{Prob:QAP_Gen} is equivalent to
%\begin{align*}
%\begin{split}
%&\min_{ k_1,k_2,k_3,k_4 \in [n]}\ \Gamma \Delta c_{k_1 k_2} d_{k_3 k_4} + \\
% & \min_{x \in \mathcal{X}} \sum_{i,j,r,s \in [n]}  d_{rs}c_{ij}x_{ir}x_{js} + \max \left\{0, \left( \sum_{r,s \in [n]} d_{rs}\Delta c_{ij} x_{ir}x_{js} \right)-\Delta c_{k_1 k_2} d_{k_3 k_4} \right\}.
% \end{split}
%\end{align*}
%
%%We note, that in our setting for all $r\in [n]$ the distance between a location and itself equals 0. Hence, $d_{rr}c_{ij}x_{ir}x_{jr} = 0$ for $(i,j)\in [n]^2$ due to $d_{rr}=0$. To avoid later division by zero we only sum up factors with $d_{rs}\neq 0$ e.g. $r \neq s$. 
%%Then, the inner optimization problem of Problem~\eqref{Prob:QAP_Gen} is equivalent to:
%% \[\min_{x \in \mathcal{X}} \sum_{(i,j)\in [n]^2} \sum_{(r,s)\in [n]^2, r \neq s} d_{rs}c_{ij}x_{ir}x_{js} + \max \left\{0, \sum_{(r,s)\in [n]^2, r \neq s} d_{rs}\left(\Delta c_{ij} x_{ir}x_{js}\right)-\Delta c_{k_1 k_2} d_{k_3 k_4} \right\}.\]
%%To omit the decision variable in the maximum we reformulate:
%We note here, that we do not demand $x_{k_1k_3}x_{k_2k_4} = 1 $ within the feasible set. If this equation is not fulfilled, there is another tuple $(\bar{k}_1,\bar{k}_2,\bar{k}_3,\bar{k}_4)$ with a higher objective for the same $x$, since for a fixed $x$ the objective is piecewise linear in $\Delta c_{k_1 k_2} d_{k_3 k_4}$ and the optimal $\Delta c_{k_1 k_2} d_{k_3 k_4}$ is always met if $x_{k_1k_3}x_{k_2k_4}=1$ for the optimal $x$ (since those are the changepoints of the objective). Thus, if we minimize over all tuple $(i,j,r,s)\in [n]^4$ an infeasible solution can not be optimal. 
%Since $d_{r,s}$ denotes the distance between two locations $r$ and $s$, we can assume $d_{rr} = 0$ for all $r \in [n]$ and $d_{rs} > 0$ for $r \neq s$. Hence
%\begin{align*}
%\begin{split}
%\max & \left\{0, \sum_{ r,s \in [n]} \Delta c_{ij} d_{rs} x_{ir}x_{js}-\Delta c_{k_1 k_2} d_{k_3 k_4}\right\}\overset{(*)}{=}\\
%\max& \left\{0, \left(\sum_{r,s \in [n], r \neq s} d_{rs} x_{ir}x_{js}\right) \left(\Delta c_{ij}-\frac{\Delta c_{k_1 k_2} d_{k_3 k_4}}{ \sum_{r,s\in [n], r \neq s} d_{rs} x_{ir}x_{js}}\right)\right\} \overset{x \in \mathcal{X}}{=}\\
%\max &\left\{0, \Delta c_{ij}-\frac{\Delta c_{k_1 k_2} d_{k_3 k_4}}{d_{rs}}\right\}d_{rs} x_{ir}x_{js}.
%\end{split}
%\end{align*}
%In $(*)$ we factorized $\sum_{r,s \in [n], r \neq s} d_{rs}x_{ir}x_{js}$ for a better understanding of the next reformulation.
%%We apply equality~\eqref{Prob:OneSum} to remove the sum from the maximum and obtain as equivalent reformulation for the inner optimization problem of \eqref{Prob:QAP_Gen}:
%%\[\Gamma \left( d_{k_3 k_4}\Delta c_{k_1 k_2}\right) +
%% \min_{x \in \mathcal{X}}\sum_{(i,j,r, s)\in [n]^4, r \neq s} d_{rs}c_{ij}x_{ir}x_{js} + \max\left\{0,\Delta c_{ij}-\frac{\Delta c_{k_1 k_2} d_{k_3 k_4}}{d_{rs}}\right\}d_{rs}x_{ir}x_{js}.\]
%%We obtain
%%\[\max\left\{0, \sum_{(r,s)\in [n]^2} \underbrace{d_{rs} x_{ir}x_{js} \Delta c_{ij}}_{\ge 0}\right\}= \sum_{(r,s)\in [n]^2} d_{rs} x_{ir}x_{js} \Delta c_{ij}\]
%%for $\theta_0(x) =0$.
%In sum, solving the robust counterpart \eqref{Prob:QAP_RobCP} is equivalent to 
%determining the minimum of
%\begin{align}\label{Prob:thetanichtnull}
%\begin{split}
%&\min_{ (k_1,k_2,k_3,k_4)\in [n]^4} \Gamma \left( \Delta c_{k_1 k_2}d_{k_3 k_4}\right) + \\
%& \min_{x\in \mathcal{X}} 
% \sum_{(i,j)\in [n]^2} \sum_{(r,s)\in [n]^2, r \neq s} d_{rs}\left(c_{ij} + \max\left\{0,\Delta c_{ij}-\frac{\Delta c_{k_1 k_2} d_{k_3 k_4}}{d_{rs}}\right\}\right)x_{ir}x_{js}
%\end{split}
%\end{align}
%and model~\eqref{Prob:thetanull}. This means that the robust
%counterpart can be solved by determining the minimum of $n^4 + 1$
%nominal QAPs. 
%\begin{align}\label{Prob:thetanull}
%\min_{x\in\mathcal{X}} \sum_{(i,j)\in [n]^2} \sum_{(r,s)\in [n]^2} d_{rs} x_{ir}x_{js}( c_{ij} + \Delta c_{ij}).
%\end{align}
%The inner optimization problem of \eqref{Prob:thetanichtnull} and
%\eqref{Prob:thetanull} are both QAPs again. Hence, obtaining an optimal
%solution of Problem~\eqref{Prob:QAP_RobCP} can be achieved by solving
%$\mathcal{O}(n^4)$ QAPs and taking the minimum of the objective values. Therefore, with our reformulation it is possible to keep the structure of the nominal Problem. We therefore denote that reformulation $QAP$.\\
\end{example}


%\begin{remark}\label{Rem:QAPLinearizations}
%In Example~\ref{ex:QAP_genau}, we established models~\eqref{Prob:thetanull} and \eqref{Prob:thetanichtnull} as a valid reformulation without uncertainty of the $\Gamma$--counterpart of a QAP under flow uncertainty. It is not by chance that the proof structure of Theorem~\ref{Theo:CorrDoNotCare} and the determination of  reformulation~\eqref{Prob:thetanull} are similar: Theorem~\ref{Theo:CorrDoNotCare} implies that the $\Gamma$--counterpart of the QAP~\eqref{Prob:QAP_RobCP} and the $\Gamma$--counterpart of
%\begin{gather}\label{Model:AlmostLinQAP}
%\min_{x \in \mathcal{X}} \sum_{i,j,r,s \in [n]} y_{ijrs} x_{ij} x_{rs} 
%\end{gather}
%with uncertain coefficients $y_{ijrs} \in \mathcal{Y}^{ijrs} := [\overline{c}_{ij} d_{rs}, \overline{c}_{ij} d_{rs} + \Delta c_{ij} d_{rs}]$ are equivalent. In terms of application, this results in another tool to solve the $\Gamma$--counterpart: By linearizing $x_{ij}x_{rs}$ in \eqref{Model:AlmostLinQAP}, we obtain the original setting of Bertsimas and Sim, i.e., \eqref{Prob:Gamma_Comb}, and can apply Propositions~\ref{Prop:Tractable_Gamma_Comb} or \ref{Prop:Gamma_MIP} and apply techniques for solving MIPs. There are already studies addressing how to solve the $\Gamma$--counterpart of a QAP with these linearized models, we refer the reader to \citep{QAP2015} and \cite{QAP_lin}. In Section~\ref{Sec:App}, we compare these linearized models (applying standard linearizations) with our new reformulation~\eqref{Prob:thetanull} and \eqref{Prob:thetanichtnull}. 
%\end{remark}
%By applying Theorem~\ref{Theo:CorrDoNotCare}, we finally consider linear problems of the form $u^TLx$ under interval uncertainty in the coefficients $u_i$, with underlying assignment structure:
%\begin{corollary}\label{Cor:LPsAssigment}
%Consider the optimization problem \begin{gather}\label{Prob:nom_LP_under_unc:ASSIGN}
%\min_{x \in \mathcal{X}} u^TBx
%\end{gather}
%as in the setting of Theorem~\ref{Theo:CorrDoNotCare} and assume $\mathcal{X} \subseteq \{0,1\}^{[m] \times [n]}$. Let $\Gamma \in [m]$. Furthermore, assume $B_{i,(r,s)} = 0$ for $i \neq r$, and for all $i \in [m]$ and for all $x \in \mathcal{X}$, there is exactly one $j \in [n]$, such that $x_{i,j} = 1$. Then the $\Gamma$--counterpart of \eqref{Prob:nom_LP_under_unc:ASSIGN} is equivalent to
%\begin{align}\label{Prob:RobustCounterpartSuperComb}
%\begin{split}
%&\min_{(k,l) \in [m] \times [n] \cup \{(0,0)\}} \Gamma \Delta u^T B_{.,(k,l)} + \\
%&\min_{x \in \mathcal{X}} \overline{u}^TBx + \sum_{(i,j) \in [m] \times [n]} \max\{0,\Delta u^TB_{.,(i,j)} - \Delta u^TB_{.,(k,l)}\}x_{i,j}.
%\end{split}
%\end{align}
%%$\min_{x Assume that for all $i \in [m]$, there is a function $l_i\colon \R^n \to \R^{L_i} $, such that $f_i(x,u^i) = (u^i)^Tl_i(x)$, i.e., $f_i$ is linear in the uncertainty and in the decision. Assume that the uncertainty set is $\mathcal{U}^i := [\overline{u}^\overline{u}^i + \Delta u^i
%\end{corollary}
%\begin{proof}
%This follows from Theorem~\ref{Theo:CorrDoNotCare} and Proposition~\ref{Prop:Tractable_Gamma_Comb} by setting $g(x) = x$.
%\end{proof}

\begin{example}
We consider the following quadratic combinatorial program under interval uncertainty:
\begin{align}\label{Prob:QuadUnc}
\begin{split}
\min_{x \in \mathcal{X} \subseteq \{0,1\}^n} & \sum_{i \in[n]} \sum_{j\in [i]} p_{i,j} x_ix_j
%%\mathrm{s.t} & \ x \in \mathcal{X} := \{x \in \{0,1\}^n: \ \sum_{j\in [n]} \omega_j x_j \le c\}
%\mathrm{s.t} & \ x \in \mathcal{X} \subseteq \{0,1\}^n
\end{split}
\end{align}
with uncertain coefficients $p_{i,j} \in [\bar{p}_{i,j}, \bar{p}_{i,j} + \Delta p_{i,j}]$. Let $m:= n^2 - \frac{n(n+1)}{2} = \frac{n^2 - n}{2}$ be the number of uncertain coefficients and let $\mathcal{M}:=\{(k,l) \in [n]^2: \ l \leq k\}$. For $\Gamma \in [m]$, its $\Gamma$--counterpart is given by
%\begin{align*}
%\max_{x \in \mathcal{X}} & \left\{ \min_{\mathcal{S} \subseteq \mathcal{M}: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{(i,j) \in \mathcal{S}} \min_{p_{i,j} \in [\bar{p}_{ij} - \Delta p_{i,j}, \bar{p}_{ij}]} p_{i,j} x_ix_j + \sum_{(i,j) \in \mathcal{M} \setminus \mathcal{S}} \bar{p}_{i,j} x_ix_j \right\} \right\}
%\end{align*}
%or, equivalently,
\begin{align}\label{Prob:RobQP}
\min_{x \in \mathcal{X}} & \left\{ \sum_{(i,j) \in \mathcal{M} } \bar{p}_{i,j} x_ix_j + \max_{\mathcal{S} \subseteq \mathcal{M}: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{(i,j) \in \mathcal{S}} \Delta p_{i,j}x_ix_j \right\} \right\}
\end{align}
By applying Theorem~\ref{Theo:PseudoLin}, we obtain that program~\eqref{Prob:RobQP} is equivalent to
%-> $f_i(x,u_i) = p_{ij}l_{ij}(x)$ mit $l_{ij} = x_ix_j \ge 0 $ 
%Dann ist gilt mit Theorem 4.10 für das robuste Gegenstück:
%\begin{align*}
%\min_{k,l \in [n]} \min_{x \in \{0,1\}^n} & \Gamma \Delta p_{kl} + \sum_{i \in[n]} \sum_{j\in [n]} \bar{p}_{ij} x_ix_j + \max \{0, \Delta p_{ij}x_i x_j - \Delta p_{ij}x_k x_l\}\\
%\text{s.t} &\sum_{j\in n} \omega_j x_j \le c
%\end{align*}
%\todo[inline][inline]{Du meinst schon immer $p_{i,j}x_kx_l$, oder?}
%Wir nehmen an $x_lx_k = 1$ mit der gleichen Argumentation wie beim QAP. \todo[inline][inline]{Wieso geht das hier? Die Bedingungen für das QAP sind hier ja nicht da, also dass man für alle $j$ ein $i$ braucht -- können nicht auch $k$ und $l$ in der Optimallösung nicht eingepackt werden?}
%Dann wird aus dem maximum   
%\[\max \{0, \Delta p_{ij}x_i x_j - \Delta p_{ij}\}:\]
%Da $x_ix_j = 1 \vee 0$ kann man die $x$ aus dem Maximum ziehen denn:\\
%$x_ix_j = 1$
%\[\max \{0, \Delta p_{ij}\cdot 1 - \Delta p_{ij}\} = \max \{0, \Delta p_{ij} - \Delta p_{ij}\} \cdot 1\]
%$x_ix_j = $
%\[\max \{0, \underbrace{\Delta p_{ij} \cdot0 - \Delta p_{ij}}_{\le 0}\} = 0 =\max \{0, \Delta p_{ij} - \Delta p_{ij}\} \cdot 0\]
%\todo[inline][inline][inline]{Ich würde auhc nicht erwarten, dass es genauso funktioniert wie beim QAP: Unser Theorem 4.12 sagt in Prinzip "sobald wir Assignment-Strukturen haben, können wir alle Korrelatoinen ignorieren" und wir haben hier keine Assignment-Struktur. Wenn ich mich nicht vertue, müsste es irgendwie so sein:}
%{\color{red} Forme $\max \{0, \Delta p_{i,j} x_ix_j - \Delta p_{k,l}x_kx_l\}$ um. Ohne weitere Voraussetzungen führen wir folgende Fallunterscheidung durch: \\
%1. Fall: $x_k = 0 \vee x_l = 0$. Dann ist $\max \{0, \Delta p_{i,j} x_ix_j - \Delta p_{k,l}x_kx_l\} = \\ \max \{0, \Delta p_{i,j}\}x_ix_j $.\\
%2. Fall: $x_k = x_l = 1$. Dann ist $\max \{0, \Delta p_{i,j} x_ix_j - \Delta p_{k,l}x_kx_l\} = max \{0, \Delta p_{i,j} - - \Delta p_{k,l}\}x_ix_j $. \\
%Nun glaube ich schon, dass es so geht, dass man annehmen kann, dass im Optimum irgendwo mal der 2. Fall auftritt -- wäre das nicht so, wäre $x_{k}x_l = 0$ für alle $k,l \in [n]$ und es wäre optimal, gar nichts mit zunehmen. Dann wäre das Budget aber kleiner als alle Gewichte, und sobald du irgendwas einpackst, gibt es ein $x_kx_l = 1$, da $k=l$ gelten kann (richtig?)... Was ich damit sagen will: ich glaube schon, dass es geht, die Argumentationsstruktur läuft nur anders als beim QAP, wo wir wussten, dass die Nullösung nicht funktioniert.}
%Damit müssen $n\times n$ Knapsacks gelöst werden
\begin{align*}
\min_{(k,l) \in \mathcal{M} \cup \{(0,0)\}} \left\{ \Gamma \Delta p_{k,l} + \min_{x \in \mathcal{X}}   \left\{ \sum_{i \in[n]} \sum_{j\in [i]} (\bar{p}_{ij} + \max \{0, \Delta p_{i,j} - \Delta p_{k,l}\}) x_ix_j  \right\} \right\}
\end{align*}
where $\Delta p_{0,0} := 0$ and we can solve the robust counterpart with $m+1$ calls of an optimization oracle of program~\eqref{Prob:QuadUnc}.

%Linearisierung: Standart
%\begin{align*}
% \min_{x \in \{0,1\}^n, y\in \{0,1\}^{n\cdot n}}& \sum_{i \in[n]} \sum_{j\in [n]} p_{ij} y_{ij}\\
%\text{s.t} &\sum_{j\in n} \omega_j x_j \le c\\
%&y_{ij} \ge x_i +x_j -1\\
%&y_{ij} \le x_i \\
%&y_{ij} \le x_j
%\end{align*}
%Reformuliert dann zu
%\begin{align*}
% \min_{x \in \{0,1\}^n, y\in \{0,1\}^{n\cdot n}}& \sum_{i \in[n]} \sum_{j\in [n]} p_{ij} y_{ij} +\max_{S\subseteqeq [n]\times [n]:|S|\le \Gamma}  \sum_{(i,j) \in S}  \Delta p_{ij} y_{ij}\\
%\text{s.t} &\sum_{j\in n} \omega_j x_j \le c\\
%&y_{ij} \ge x_i +x_j -1\\
%&y_{ij} \le x_i \\
%&y_{ij} \le x_j
%\end{align*}
%
%\begin{align*}
% \min_{x \in \{0,1\}^n, y\in \{0,1\}^{n\cdot n}, z}& \sum_{i \in[n]} \sum_{j\in [n]} p_{ij} y_{ij} +\Gamma z_0 + \sum_{i,j \in [n]} z_{ij}\\
%\text{s.t} &\sum_{j\in n} \omega_j x_j \le c\\
%&y_{ij} \ge x_i +x_j -1\\
%&y_{ij} \le x_i \\
%&y_{ij} \le x_j\\
%& z_{ij}+z_0 \ge \Delta p_{ij} y_{ij}\\
%& z_{ij} \ge 0
%\end{align*}
%\todo[inline][inline]{Da vertraue ich dir mal, dass das passt :P Erstmal klären, ob das mit dem Knapsack wirlkich alles passt.}
\end{example}
To conclude the discussion of quadratic programs under uncertainty, we demonstrate the  approach of applying the notion of term--wise parallel vectors and hidden concavity \cite{TermWise} for interval uncertainty. 
\begin{example}
Let $\mathcal{X}$ be a convex set. We consider the following program:
\begin{align}\label{Prob:NomQuad}
\inf_{x \in \mathcal{X}} \sum_{i \in [m]} (x_i - u_i)^2.
\end{align}
For every $i \in [m]$, $u_i$ is subject to uncertainty $\mathcal{U}_i := [\overline{u}_i, \overline{u}_i + \Delta u_i]$. For $\Gamma \in [m]$, the $\Gamma$--counterpart of program~\eqref{Prob:NomQuad} after applying Lemma~\ref{Lem:ReModel} is given by
\begin{align}\label{Prob:FirstQuad}
\begin{split}
\inf_{x, p, \theta} & \ \Gamma \theta + \sum_{i \in [m]} (x_i - \overline{u}_i)^2 + p_i, \\
\mathrm{s.t.} & \ x \in \mathcal{X}, \\
& \max_{u_i \in \mathcal{U}_i} (x_i - u_i)^2 - (x_i - \overline{u}_i)^2 \leq p_i + \theta \ \forall i \in [m].
\end{split}
\end{align}
The inequalities of program~\eqref{Prob:FirstQuad} are equivalent to
\begin{gather}\label{Ineq:ReformedQuad}
-2x_i u_i + u_i^2 \leq p_i + \theta - 2x_i \overline{u}_i + \overline{u}_i^2 \ \forall u_i \in \mathcal{U}_i
\end{gather}
for each $i \in [m]$. The left--hand side of \eqref{Ineq:ReformedQuad} is not concave in $u_i$ and thus, we cannot apply the reformulations of Subsection~\ref{subsec:Concave}. We set $h(y) := y^2$ for all $y \in \R$  
%\eqref{Ineq:ReformedQuad} is of the form \eqref{Ineq:SecondApproach}: We set
and consider the following formulation of the uncertainty set:
\begin{gather*}
[\overline{u}_i, \overline{u}_i + \Delta u_i] = \{u_i \in \R\colon (-2 \overline{u}_i - \Delta u_i)u_i + u_i^2 \leq -\overline{u}_i^2 - \overline{u}_i \cdot \Delta u_i\}.
\end{gather*}
Finally, define
\begin{gather*}
\alpha := -2\overline{u}_i - \Delta u_i, \ \beta := 1, \ \gamma = -\overline{u}_i^2 - \overline{u}_i \Delta u_i. \
\end{gather*}
Since $\alpha$ and $\beta$ are scalars, they are clearly term--wise parallel \cite{TermWise}. Thus, we obtain that \eqref{Ineq:ReformedQuad} is satisfied for $(x, p, \theta)$ if and only if there exist $v_1, \dots, v_m \in \R$, such that
\begin{align*}
&(1 + v)h_i^*\left(\frac{2x + 2 \overline{u}_iv_i + \Delta u_iv_i}{1+v_i}\right) - \overline{u}_i^2v_i - \overline{u}_iv_i \Delta u_iv_i + 2x_i \overline{u}_i\le p_i + \theta  + \overline{u}_i^2,\\
&1 + v_i \ge 0,\\
&v_i\ge 0,
\end{align*}
see \cite{Fenchel}, Subsection 4.3, for details. Clearly, the second inequality is redundant. Furthermore, since
$h_i^*(z) = \frac{z^2}{4}$, the first inequality is convex in $(x,v_i)$ if it is assumed that $x \geq 0$. If $\mathcal{X} \subseteq \R^n_{\geq \overline{u}}$, then the $\Gamma$--counterpart of program~\eqref{Prob:NomQuad} is a convex optimization problem, although the uncertainty is not concave.
\end{example}

\paragraph*{Deadline uncertainties in a piecewise linear setting}
%A piecewise linear function is a function $f$ with domain $\mathcal{D}$ and that there exists a finite number of polyhedra $\mathcal{P}_i$ and $(m_{\mathcal{P}_i}, c_{\mathcal{P}_i})$, such that $\cup_{i=1}^m \mathcal{P}_i = \mathcal{X}$ and $f(x) = m_{\mathcal{P}_i}^Tx + c_{\mathcal{P}_i}$ for $x \in \mathcal{P}_i$. We assume that $f$ is continuous and that the interior of the polyhedra are pairwise disjoint. Furthermore, we assume that $f$ is subject to uncertaintyWe employ our reformulations for a fixed number of reformulations, e.g. for cases of Example~\ref{Ex:UncertainBounds}. 
%We consider continuous piecewise linear functions as considered in XXX:
%\begin{definition}
%Let $\mathcal{X}$ be the domain of a function $f \colon \mathcal{X} \to \R$. $f$ is called \emph{piecewise linear}, if there is a finite number of polyhedra $\mathcal{P}_i$ and $(m_{\mathcal{P}_i}, c_{\mathcal{P}_i})$, such that $\cup_{i=1}^m \mathcal{P}_i = \mathcal{X}$ and $f(x) = m_{\mathcal{P}_i}^Tx + c_{\mathcal{P}_i}$ for $x \in \mathcal{P}_i$. The definition already implies that $f$ is continuous. W.l.o.g. we assume that the relative interior of the polyhedra are pairwise disjoint.
%%\end{definition}
%we consider model~\eqref{Prob:GeneralStrictOpt} 
%where each function $f_i$ is continuous piecewise linear. We start by the assumption that $f_i$ is concave in the uncertainty.
%\paragraph*{Concavity in the uncertainty} 
%As pointed out in Remark~\ref{Rem:Concave}, under Assumption~\ref{Ass:General} one can state a reformulation. In the following, we furthermore assume that $f_i(x,u_i) = \min_{j \in \mathcal{I}_i} \{a_jx_i - b_j + u_i\}$.
%
%\paragraph*{Application: Deadline Uncertainty}
%Since those are in general neither convex nor concave, thus, if the underlying vectors $(m_{\mathcal{P}_i}, c_{\mathcal{P}_i})$ are subject to uncertainty, we can in general not apply reformulations of Subsection~\ref{subsec:Concave}. 
%\todo[inline][inline]{Beispiel, so dass sich auch die Polyeder ändern?}. 
%Furthermore, because of the inherent definition, it is not clear how a robust counterpart can be formulated algebrically. However, applying our recent results, we obtain the following result:
%\begin{theorem}
%For $i \in [m]$, let $f_i \colon \mathcal{X}$ be a continuous piecewise linear function...
%\end{theorem}
%% Therein, a continuous function $f$ is called piecewise linear on its domain $\mathcal{D}\subseteq \R^n$, if there exists a set $\mathcal{P}$ that contains polyhedra and for each $P \in \mathcal{P}$, there is a vector $m_P$ and a scalar $c_P$, such that for all $x \in D$ there exists a polyhedron $P$, such that $f(x) = m_p^Tx + c_p$. Without loss of generality, we can assume that the polyhedra are pairwise disjoint. In practice... \todo[inline][inline]{Drauf eingehen wieso $\Gamma$ hier nicht einfach über MIP anwendbar ist}. In this definition of a function, there are many ways uncertainty can appear:
%\begin{itemize}
%\item The polyhedra are subject to change, i.e., $\mathcal{P}$
%\item The polyhedra 
%\item 
%\end{itemize}

%We show next that with
%Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear},
%Proposition~\ref{Prop:Tractable_Gamma_Comb} can be applied as well: If we consider $u_{i,j} := p_i q_j$ with uncertainty set $\mathcal{U}_{i,j} := [\overline{p}_i q_j, \overline{p}_iq_j + \Delta p_i q_j]$ for each $(i,j) \in \mathcal{I} \times \mathcal{J}$, the $\Gamma$--counterpart of $\min_{x \in \mathcal{X}} u^Tx$ is given by
%\begin{gather*}
%\min_{x \in \mathcal{X}} \left\{ \sum_{(i,j) \in \mathcal{I} \times \mathcal{J}} \overline{p}_iq_j x_{i,j} + \max_{\mathcal{S} \subseteq \mathcal{I} \times \mathcal{J}, |\mathcal{S}| \leq \Gamma} \sum_{(i,j) \in \mathcal{S}} u_{i,j} \Delta p_i q_j x_{i,j} \right\}.
%\end{gather*}
%Technically, we applied that the uncertainty of the coefficients of $x_{i,j}$ are not correlated although they are in the original setting. However, applying Proposition~\ref{Prop:Tractable_Gamma_Comb} results exactly in the problems~\eqref{Prob:SchedulingFamily} and ~\eqref{Prob:Scheduling0}. This is a consequence of the worst-cases of the two settings being equivalent: In the first setting, a coefficient $p_i$ realizes its worst case when $p_i = \overline{p}_i + \Delta p_i$ and in the second setting, a coefficient $u_i = p_i q_j$ realizes its worst case when $u_{i,j} = \overline{p}_iq_j + \Delta p_i q_j = (\overline{p}_i + \Delta p_i)q_j$. Thus, for every $j \in \mathcal{J}$, the worst-case of $u_{i,j}$ realizes if and only if the worst-case of $q_i$ realizes. Since we only consider worst-case scenarios in our $\Gamma$--counterparts, the reformulations of Proposition~\ref{Prop:Tractable_Gamma_Comb} and \cite{RobustScheduling} are identical.
%has been determined, namely in Proposition 1 in \cite{RobustScheduling}. 
%This setting covers e.g. the single-machine scheduling of Example~\ref{Ex:Scheduling}:\\ The authors assumed that, for every $i \in \mathcal{I}$, the parameter $\overline{p}_i$ is uncertain and lies in the uncertainty set $\mathcal{U}_i := [\overline{p}_i, \overline{p}_i + \Delta p_i]$. Although Problem~\eqref{Prob:NomScheduling} is linear in the uncertainty and the decision variables, one can not simply apply Proposition~\ref{Prop:Tractable_Gamma_Comb} since the number of uncertain parameters and decision variables do not match, as the authors of \cite{RobustScheduling} have pointed out. They explicitly stated the $\Gamma$--counterpart
%\begin{gather*}
%\min_{x \in \mathcal{X}} \sum_{i \in \mathcal{I}} \overline{p}_i \sum_{j \in \mathcal{J}} q_j x_{ij} + \max_{\mathcal{S} \subseteq \mathcal{I}: |\mathcal{S}| \leq \Gamma} \sum_{i \in \mathcal{S}} \Delta p_i \sum_{j \in \mathcal{J}} q_i x_{ij} 
%\end{gather*} 
%is equivalent to obtaining the minimum of 
%\begin{align}\label{Prob:SchedulingFamily}
%\min_{(k,l) \in \mathcal{I} \times \mathcal{J}} \Gamma q_k \Delta p_l + \min_{x \in \mathcal{X}} \sum_{i,j \in \mathcal{I}, \mathcal{J}} (\overline{p}_i + \max\{0, \Delta p_i - \frac{\Delta p_k q_l}{q_j}\})q_jx_{i,j}
%\end{align}
%and 
%\begin{align}\label{Prob:Scheduling0}
%\begin{split}
%\min_{x \in \mathcal{X}} \sum_{i,j \in \mathcal{I}, \mathcal{J}} (\overline{p}_i + \Delta p_i)q_jx_{i,j}.
%\end{split}
%\end{align}
%We can prove this with Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear}: We set
%\begin{gather*}
%\overline{u}^i := \overline{p}^i, \ l_i(x) = \sum_{j \in \mathcal{J}} q_j x_{i,j}, \ f_i(x,u^i) = p_i l_i(x), \ \mathcal{U}_i = \{p_i = \overline{p}_i + \alpha \Delta p_i \mid \alpha \in [0,1]\}, \mathcal{Z}_i = [0,1]
%\end{gather*}
%and obtain 
%\begin{gather*}
%\theta^k := \delta^*(\Delta p_k l_k(x) \mid \mathcal{Z}_k) = \Delta p_k \sum_{j \in \mathcal{J}} q_j x_{k,j}.
%\end{gather*}
%Thus, applying Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear} results in 
%\begin{align}\label{Prob:GeneralGammaCounterpartWithoutDualScheduling}
%\begin{split}
%\min_{k \in \{1, \dots, m\}} & \min_{x} \Gamma \Delta p_k \sum_{j \in \mathcal{J}} q_j x_{k,j} + \sum_{i \in [m]} \overline{p}_i\sum_{j \in \mathcal{J}} q_j x_{i,j} + \max \{0, \Delta p_i \sum_{j \in \mathcal{J}} q_j x_{i,j} - \Delta p_k \sum_{j \in \mathcal{J}} q_j x_{k,j} \} \\
%\text{s.t.} & x \in \mathcal{X} \\
%%& \theta^k \geq 0. \\
%%& \theta^k = \overline{u^k}^Tv^k - f_k(x,\overline{u}^k) - f_{k,*}(x,v^k) + \support{k}).
%\end{split}
%\end{align}
%For obtaining a computationally tractable counterpart which a linear objective function, we use that for each $k \in \mathcal{I}$, $\sum_{j \in \mathcal{J}} x_{k,j} = 1$, i.e., for each $k \in \mathcal{I}$, there exists exactly one $l \in \mathcal{J}$, such that $x_{k,l} = 1$. Thus, we minimize over $(k,l) \in \mathcal{I} \times \mathcal{J}$ instead of only $k \in \mathcal{I}$ and obtain as an objective, for fixed $(k,l)$,
%\begin{align*}
%\Gamma \Delta p_k q_l + \sum_{i \in [m]} \overline{p}_i \sum_{j \in \mathcal{J}} q_j x_{i,j} + \max\{0, \Delta p_i \sum_{j \in \mathcal{J}} q_j x_{i,j} - \Delta p_k q_l \}= \\
% \Gamma \Delta p_k q_l + \sum_{i \in [m]} \overline{p}_i \sum_{j \in \mathcal{J}} q_j x_{i,j} + \sum_{j \in \mathcal{J}} \max\{0, \Delta p_i - \frac{\Delta p_k q_l}{q_j}\} q_j x_{i,j}
%\end{align*}
%due to $\sum_{j \in \mathcal{J}} x_{i,j} = 1.$ This results in Problem~\eqref{Prob:SchedulingFamily}. For $\theta^0 := 0$, we easily obtain Problem~\eqref{Prob:Scheduling0}: Applying Theorem~\ref{Theo:CombinatorialGammaCounterPartWithoutDualLinear}, this results in
%\begin{gather*}
%\min_{x \in \mathcal{X}} \sum_{i \in \mathcal{I}} \overline{p}_i \sum_{j \in \mathcal{J}} q_j x_{i,j} + \max\{0, \Delta p_i \sum_{j \in \mathcal{J}} q_j x_{i,j}\}
%\end{gather*}
%which is, due to $\Delta p_i \sum_{j \in \mathcal{J}} q_j x_{i,j} \geq 0$, exactly Problem~\eqref{Prob:Scheduling0}.
%\end{example}
%%Example~\ref{Ex:Scheduling} shows that there exist cases where, although the objective is linear in the uncertainty and the decision variable, one can not apply Proposition~\ref{Prop:Tractable_Gamma_Comb}. This is due to uncertainty and decision vector not having the same dimension.\\
%
%We note that for Example~\ref{Ex:SchedulingGeneral}, one could have applied a similar proof to obtain the computationally tractable counterpart. \\
We conclude our discussion of applications with the deadline uncertainty setting we introduced in Section~\ref{sec:Rev}.
%This concludes our discussion of concavity in the uncertainty. In the next subsection, we propose methods to tackle the general case.

%Looking at \ref{Prob:GeneralReModel}, we try to compute with Fenchel duality a tractable formulation for $p_i+\theta \ge \max_{u^i \in \mathcal{U}_i} f_i(x,u^i) -f_i(x, \bar{u}^i)$. This equals $ p_i+\theta - \max_{u^i \in \mathcal{U}_i} f_i(x,u^i) +f_i(x, \bar{u}^i)\ge 0$. Here it is possible to replace the maximum with a for all condition. We also assume that $f_i(x,u)$ is separable:
%\[-p_i - \theta - f_i(x, \bar{u}^i) + \bar{f}_i(u^i)^Tg_i(x)\le 0\]
%Following approach on we replace $\bar{f}_(u)=b$. With this we obtain:
%\[b_i^T\bar{g}_i(x) \le 0, \qquad \forall (u_i,b_i) \in \bar{U}^i=\{(u,b): u \in \mathcal{U}^i, \bar{f}_i(u^i)=b_i\} \}.\]
%Now we have to obtain $conv(\bar{U}^i)$. However, this depends strongly on the structure of $\mathcal{U}_i$. For a general $conv(\bar{U}_i)$ the resulting robust counterpart can be determined as:
%\begin{align*}
%\min_{x,p,\theta} & \Gamma \theta + \sum_{i \in [m]} f_i(x, \bar{u}^i +p_i\\
%\text{s.t} & x \in \mathcal{X}\\
%& a^{0T}\bar{g}_i(x)+\delta^*(A^T\bar{g}_i(x)|Z_i)\le 0\\
%&p,\theta \ge 0
%\end{align*} 
%%Apart from these approaches, there are cases that enable a formula for $\max_{u^i \in \mathcal{U}_i}
%%f_i(x,\overline{u}^i)$ analytically. We apply this approach to the problem introduced in
%%Example~\ref{Ex:VRP}:
\begin{example}\label{Ex:UncertainBounds}
Consider the $\Gamma$--counterpart of program~\eqref{Prob:BoundNom} as introduced in Section~\ref{sec:Rev}:%Example~\ref{Ex:VRP}:
\begin{align*}
\inf_{x \in \mathcal{X}}  \left\{ \sup_{\mathcal{S} \subseteq [m]: |\mathcal{S}| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} \max\{0,x_i - \overline{b}_i + \Delta b_i\} + \sum_{i \in [m] \setminus \mathcal{S}} \max\{0, x_i - \overline{b}_i\} \right\} \right\}.
\end{align*}
An equivalent reformulation, given in Remark~\ref{Rem:NoFenchel} as program~\eqref{Prob:GammaCombCounterpartWithoutFenchel}, is
\begin{align}\label{Prob:PiecewiseLinearFirstStep}
\begin{split}
\inf_{k \in [m]_0} \left\{ \inf_{x \in \mathcal{X}} \left\{  \Gamma \theta^k(x) + 
\sum_{i \in [m]}  \max \{0, x_i - \overline{b}_i, \max\{0,x_i - \overline{b}_i + \Delta b_i\} - \theta^k(x)\} \right\} \right\}
\end{split}
\end{align}
with $\theta^k(x) := \max \{0, x_k - \overline{b}_k + \Delta b_k\} - \max\{0,x_k - \overline{b}_k\}$ and $\theta^0(x) := 0$. Thus, for $k = 0$, it is necessary to solve
%We apply 
%\begin{gather*}
%\max_{u^i \in \mathcal{U}_i} f_i(x,u^i) := \max_{u^i \in \mathcal{U}_i} \max \{0,x_i-u^i\} = \max \{0,x_i - \min_{u^i \in \mathcal{U}_i} u^i \} = \max \{0,x_i - \overline{b}_i + \Delta b_i\}
%\end{gather*}
%for $\mathcal{U}_i := [\overline{b}_i, \overline{b}_i + \Delta b_i]$.
%%Note that in this problem, technically only additive terms are uncertain. This was, to the best of our knowledge, first studied in \cite{RobCombOpt}.\\
%gztfzu \begin{alignat}{2}
%p_i + \max\{0, x_i - u_i\} &= \max\{0, x_i - u_i, x_i - u_i + \Delta u_i - (x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\})\} \\
%&= \max\{0, x_i - u_i, x_i - u_i + \Delta u_i - (x_l - u_l + \Delta u_l), x_i - u_i + \Delta u_i - \Delta u_l \}\label{Eq:p}
%\end{alignat}
%We set $\theta^k(x) := \max \{0, x_k - \overline{b}_k + \Delta b_k\} - \max\{0,x_k - \overline{b}_k\}$. Since $\Gamma$ is integral and with Remark~\ref{Rem:NoFenchel}, one obtains
%\begin{align}\label{Prob:PiecewiseLinearFirstStep}
%\begin{split}
%\min_{k \in \{0, \dots, m\}} & \min_{x} \Gamma \theta^k + \sum_{i \in [n]} \max \{0,x_i - \overline{b}_i\} + \max \{0, \theta^i(x) - \theta^k(x) \}, \\
%\text{s.t.} & x \in \mathcal{X}
%\end{split}
%\end{align}
%with $\theta^0(x) = 0$ and 
%\begin{align}\label{Eq:Bound_Piecewiselinear}
%\begin{split}
%\theta^k(x) &= \max\{0,x_k - \overline{b}_k + \Delta \overline{b}_k\} - \max \{0, x_k - \overline{b}_k\}. \\
%%&= \max\{0, x_k - \overline{b}_k + \Delta \overline{b}_k, \Delta b_k\}. \\
%%&= \max\{x_k - \overline{b}_k + \Delta b_k, \Delta b_k\} \\
%%&= \Delta b_k + \max\{0, x_k - \overline{b}_k\}.
%\end{split}
%\end{align}
%Thus,
%\begin{align}\label{Eq:ObjBounds}
%\begin{split}
%\max \{0,x_i - \overline{b}_i\} + \max \{0, \theta^i(x) - \theta^k(x) \} %&= \max \{\max \{0,x_i - \overline{b}_i\}, \max \{0,x_i - \overline{b}_i\} + \theta^i(x) - \theta^k(x)\} \\
%&= \max \{0, x_i - \overline{b}_i, \max \{0,x_i - \overline{b}_i + \Delta b_i\} - \theta^k(x)\}\\
%%&= \max \{0, x_i - b_i, \Delta b_i - \max\{0, x_k - b_k + \Delta b_k, \Delta b_k\}\} - \max\{0, x_i - b_i + \Delta b_i, \Delta b_i - \max\{0, x_k - b_k + \Delta b_k, \Delta b_k\}\}
%&=\max \{0, x_i - \overline{b}_i, x_i - \overline{b}_i + \Delta b_i- \theta^k(x)\}
%\end{split}
%\end{align}
$ \min_{x \in \mathcal{X}} \sum_{i \in [m]} \max \{0, x_i - \overline{b}_i + \Delta b_i\}$. For $k > 0$, we distinguish between three cases:
\begin{enumerate}
\item[i)] $x_k \geq \overline{b}_k$, i.e., $\theta^k(x) = \Delta b_k$ and
\begin{gather}\label{Eq:Case1}
\max \{0, x_i - \overline{b}_i, \max \{0,x_i - \overline{b}_i + \Delta b_i\} - \theta^k(x)\} = \max\{0, x_i - \overline{b}_i, x_i - \overline{b}_i + \Delta b_i -\Delta b_k\}.
\end{gather}
\item[ii)] $x_k \in [\overline{b}_k- \Delta b_k, \overline{b}_k]$, i.e., $\theta^k(x)  = x_k - \overline{b}_k + \Delta b_k$ and
%Continuing with \eqref{Eq:ObjBounds} results in 
\begin{align}\label{Eq:Case2}
\begin{split}
&\max \{0, x_i - \overline{b}_i, \max \{0,x_i - \overline{b}_i + \Delta b_i\} - \theta^k(x)\} =\\ & \max\{0, x_i - \overline{b}_i, x_i - \overline{b}_i + \Delta b_i - x_k + \overline{b}_k - \Delta b_k\}.
\end{split}
\end{align}
\item[iii)] $x_k \leq \overline{b}_k - \Delta b_k$, i.e., $\max \{0, x_k - \overline{b}_k\} = \max \{0, x_k - \overline{b}_k + \Delta b_k\}=0$. Thus, $\theta^k(x) = 0$ and we refer to the case of $k = 0$.
\end{enumerate}
For each $k \in [m]$, by applying equations~\eqref{Eq:Case1} and \eqref{Eq:Case2}, we solve 
\begin{align}\label{Prob:SubProbVRPNOTRec}
\begin{split}
\inf_{x \in \mathcal{X}} & \ \sum_{i \in [m]} \max\{0, x_i - \overline{b}_i, x_i - \overline{b}_i + \Delta b_i - \Delta b_k \} + \Gamma \Delta b_k \\
\mathrm{s.t.} & \ x_k \in [\overline{b}_k - \Delta b_k, \overline{b}_k]
\end{split}
\end{align}
and
\begin{align}\label{Prob:SubProbVRPRec}
\begin{split}
\inf_{x \in \mathcal{X}} & \ \sum_{i \in [m]} \max\{0, x_i - \overline{b}_i, x_i - \overline{b}_i + \Delta b_i - x_k + \overline{b}_k -\Delta b_k \} + \Gamma (x_k - \overline{b}_k + \Delta b_k) \\
\mathrm{s.t.} & \ x_k \geq b_k.
\end{split}
\end{align}
%For $k = 0$, we need to solve
%\begin{align*}
%\min_{x \in \mathcal{X}} & \ \sum_{i \in [m]} \max \{0,x_i - \overline{b}_i + \Delta b_i\}.
%\end{align*}
Therefore, in total, we need to solve $2m + 1$ optimization programs with a piecewise linear objective with the addition of one additional hard bound for exactly one variable for $k \in [m]$. In the electric companion, we apply this reformulation to a special case of the vehicle routing problem with general time windows.
%Applying the example of logistics, one can interpret this in the following way: For $k \in [m]$, we solve two optimization problems: we distinct between the nominal bound $\overline{b}_k$ being satisfied and not being satisfied. In both cases, one compares the violations for $x_i$ and $x_k$ and adds $\Gamma$ times the violation of bound $x_k$. For $k = 0$, $\Gamma$ is multiplied and $0$ and vanished but all bounds realize their worst-case scenario. So basically, it is a trade-off between worst-case scenarios and the impact of bound $\overline{b}_k$ being not satisfied.
%We note that (except for $k = 0$), the number of pieces doubles ($2$ instead of $4$). For piecewise linear optimization it is crucial that the number of pieces does not rise exponentially.
\end{example}
%Example~\ref{Ex:UncertainBounds} shows that, even without concavity in the uncertainty, one can directly give a robust counterpart for some examples. \\
%A more detailed discussion of this topic can be found in Appendix A.
%Next, we discuss the case of uncertainty in the constraints.
%In this section, we show that the $\Gamma$-flexible approach can be applied to problems of the form
%\begin{alignat*}{2}
%\min & \ \sum_{i \in [n]} \max\{0,x_i - u_i\}\\
%\text{s.t.} & x \in \mathcal{X}. \\
%\end{alignat*} 
%As already discussed, problems of this form can occur whenever the bounds of the problem are increasing the complexity of the problem from polynomial complexity to being NP-hard and when it is actually beneficial to shift the bonds into the objective function, see e.g. Chapter 4 in \cite{Probust}.
%Now, it is possible that one wants again that these soft bounds can be subject to uncertainty with not every bound allowing to change. This results in the $\Gamma$-robust counterpart
%\begin{alignat*}{2}
%\min_{x \in \mathcal{X}} & \ \max_{S \subseteq [n]: |S| \leq \Gamma} \sum_{i \in S} \max\{0,x_i - u_i + \Delta u_i\} + \sum_{i \in [n] \setminus S} \max\{0, x_i - u_i\}\\
%\text{s.t.} & x \in \mathcal{X}. \\
%\end{alignat*}
%%\textbf{TO DO: Looking up: Buchheim, !!!!}\\
%Note that this is a problem with uncertainty in a \emph{constant} of the objective function and not in a coefficient. To the best of our knowledge, this has first been introduced in \cite{RobCombOpt}. \\
%In the following, we will denote a problem over the set $\mathcal{X}$ as \emph{nominal}, if its objective function is a piecewise-linear function. The following theorem shows that we can, similar to the combinatorial case, reformulate the $\Gamma$-Robust counterpart to such a nominal problem:
%\begin{theorem}\label{Theo:GammaBounds}
%The $\Gamma$-robust counterpart can be solved by solving $2n + 1$ problems in nominal form.
%\end{theorem}
%%\begin{proof}
%%Similar to the combinatorial case, we introduce binary variables $y_i \in \{0,1\}$ to re-model the inner optimization problem:
%%\begin{alignat*}{3}
%%\max_{y} & \sum_{i \in [n]} \max\{0, x_i - u_i\} + (\max\{0, x_i - u_i + \Delta u_i\} - \max\{0, x_i - u_i\})y_i & \\
%%\text{s.t.} & \sum_{i \in [n]} y_i \leq \Gamma & \\
%%& y_i \in \{0,1\} & \forall i \in [n]. 
%%\end{alignat*}
%%Since $\Gamma$ is a positive integer, the knapsack constraint is TDI and we can substitute this binary programm with a linear programm: 
%%\begin{alignat*}{3}
%%\max_{y} & \sum_{i \in [n]} \max\{0, x_i - u_i\} + (\max\{0, x_i - u_i + \Delta u_i\} - \max\{0, x_i - u_i\})y_i & \\
%%\text{s.t.} & \sum_{i \in [n]} y_i \leq \Gamma & \\
%%& y_i \in [0,1] & \forall i \in [n]. 
%%\end{alignat*}
%%By neglecting the first additive term and by strong duality for linear programs, we obtain
%%\begin{alignat*}{3}
%%\min_{p,\theta} & \ \sum_{i \in [n]} p_i + \Gamma \theta & \\
%%\text{s.t.} & p_i + \theta \geq \max\{0, x_i - u_i + \Delta u_i\} - \max\{0, x_i - u_i\} & \\
%%& p, \theta \geq 0 . 
%%\end{alignat*}
%%Inserting this equivalent form of the inner optimization problem in the original problem results in
%%\begin{alignat*}{2}
%%\min_{x,p,\theta} & \ \sum_{i \in [n]} \max\{0, x_i - u_i\} + p_i + \Gamma \theta &\\
%%\text{s.t.} & x \in \mathcal{X}, \\
%%& p_i + \theta \geq \max\{0, x_i - u_i + \Delta u_i\} - \max\{0, x_i - u_i\} & \forall i \in [n], \\
%%& p, \theta \geq 0.
%%\end{alignat*}
%%Since $p_i + \theta \geq 0$, we can re-write the above constraint to 
%%\begin{gather*}
%%p_i + \theta \geq x_i - u_i + \Delta u_i - \max \{0, x_i - u_i\} 
%%\end{gather*} 
%%The next step is eliminating the new variables $p_i$ and $\theta$. First, we will give a formula for the optimal value of $\theta$:\\
%%Assume that $(x^*,p^*,\theta^*)$ is feasible. We assume \begin{gather*}
%%\theta^* \neq x_j^* - u_j + \Delta u_j - \max \{0, x^*_j - u_j\} =: b_j \text{ for $j = 0, \dots, n$.}
%%\end{gather*} 
%%We note that we defined $b_0 := 0$.
%%Then, with $b_{n+1} := \infty$ (after a possible re-ordering), there is $j$, such that $\theta^* \in (b_j, b_{j+1})$. We consider, two cases:
%%\begin{enumerate}
%%\item[i)] $n - j \leq \Gamma$: Set \begin{gather*}
%%\overline{\theta} := b_j - p_j^*, \ \overline{p_i} := \begin{cases} p_i^*, i \leq j - 1, \\ p_i^* + (\theta^* - \overline{\theta}), i \geq j \end{cases}
%%\end{gather*}
%%Then, $(x^*, \overline{p}, \overline{\theta})$ is obviously still feasible. Furthermore, the objective value does not increase: \begin{alignat*}{2}
%%\sum_{i=1}^n \overline{p_i} + \Gamma \overline{\theta} &= \sum_{i=1}^n p_i^* + (n-j)(\theta^* - \overline{\theta}) + \Gamma \overline{\theta} \\
%%&= \sum_{i=1}^n p_i^* + \Gamma \theta^* + (\theta^* - \overline{\theta})(n-j-\Gamma) \\
%%&\leq \sum_{i=1}^n p_i^* + \Gamma \theta^*.
%%\end{alignat*}
%%\item[ii)] $\Gamma \leq n-j + 1$: Set 
%%\begin{gather*}
%%\overline{\theta} := b_{j+1} - p_{j+1}^*, \ \overline{p_i} := \begin{cases} p_i^*, i \leq j , \\ p_i^* + \theta^* - \overline{\theta}, i \geq j + 1 \end{cases}
%%\end{gather*}
%%Then, like in the first case, $(x^*, \overline{p}, \overline{\theta})$ is obviously still feasible and the objective value does not increase: \begin{alignat*}{2}
%%\sum_{i=1}^n \overline{p_i} + \Gamma \overline{\theta} &= \sum_{i=1}^n p_i^* - (n-(j+1))(\overline{\theta} - \theta^*) + \Gamma \overline{\theta} \\
%%&= \sum_{i=1}^n p_i^* + \Gamma \theta^* + (\overline{\theta} - \theta^*)(\Gamma - (n-(j+1)) \\
%%&\leq \sum_{i=1}^n p_i^* + \Gamma \theta^*.
%%\end{alignat*} 
%%\end{enumerate} 
%%Since we have chosen an arbitrary feasible point, an optimal $\theta$ is, for any optimal $x$, an element of $\{0\} \cup \bigcup_{l \in [n]} \{ x_i - u_i + \Delta u_i - \max \{0, x_i - u_i\} \}$. In other words, the optimization problem is 
%%\begin{alignat*}{3} 
%%\min_{l\in [n+1] }\min_{x,p} & \ \sum_{i \in [n]} \max\{0, x_i - u_i\} + p_i + \Gamma (x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\}) &\\
%%\text{s.t.} & x \in \mathcal{X}, \\
%%& p_i + x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\} \geq x_i - u_i + \Delta u_i - \max \{0, x_i - u_i\} & \ \forall i \in [n], \\
%%%& \theta^l = \Delta u_l + \max\{0, u_l - x_l\} , \\
%%& p \geq 0, \\
%%& x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\} \geq 0.
%%\end{alignat*}
%%(note that we defined $\Delta u_{n+1} := u_{n+1} := x_{n+1} := 0$).
%%To finish the proof of part (a), we will eliminate $p$: It is obvious that an optimal $p_i$ is
%%\begin{gather*}
%%p_i = \max\{0, x_i - u_i + \Delta u_i - \max \{0, x_i - u_i\} - (x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\})\}.
%%\end{gather*}
%%and that 
%%\begin{alignat*}{3} 
%%\min_{l\in [n+1] } \min_{x} & \ \sum_{i \in [n]} \max\{0, x_i - u_i, x_i - u_i + \Delta u_i - (x_l - u_l + \Delta u_l), x_i - u_i + \Delta u_i - \Delta u_l \}+ \Gamma (x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\}) &\\
%%\text{s.t.} & x \in \mathcal{X}, \\
%%& x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\} \geq 0.
%%\end{alignat*}
%%However, due to $\theta^l \geq 0$, $\max\{0, u_l - x_l\} = 0$ and thus, 
%%\begin{gather*}
%%p_i = \max\{0, \Delta u_i - \max \{0, u_i - x_i\} - \Delta u_l\}
%%\end{gather*}
%%Inserting $p_i$ into the objective function finally results in
%%\begin{align*}
%%\sum_{i \in [n]} \max\{0, x_i - u_i\} + \max\{0, x_i - u_i + \Delta u_i - \max \{0, x_i - u_i\} - (x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\})\} - \Gamma (x_l - u_l + \Delta u_l - \max \{0, x_l - u_l\}) \= \sum_{i \in [n]} + \max\{\max \{0, x_i - u_i\}, x_i - u_i + \Delta u_i - \Delta u_l\} + \Gamma (\Delta u_l)\\
%%&= \max \{0, x_i - u_i, x_i - u_i + \Delta u_i - \Delta u_l\} + \Gamma (\Delta u_l).
%%\end{align*}
%%which proves part (a).
%%\end{proof}
%%Note that there was no point in this proof in which we required the structure of the optimization problem, i.e., there was no point in which it was important if the underlying problem is a discrete, continuous, convex, linear or non-convex optimization problem. \\
%%\paragraph{Generalization for convex, piecewise linear functions}
%\begin{theorem}
%Let $f(x,u) := \sum_{i=1}^n f_i(x_i, u_i)$ be a separable, piecewise linear, convex function with uncertainty $u$. Then the $\Gamma$-robust counterpart
%\begin{alignat}{2}
%\min_x & \max_{S \subseteq [n]: |S| \leq \Gamma} \{ \sum_{i \in S} \max_{u_i \in \mathcal{U}_i} f_i(x_i, u_i) + \sum_{i \in [n] \setminus S} f_i(x_i, \overline{u}_i) \} \\
%\text{s.t.} & x \in \mathcal{X}
%\end{alignat}
%is equivalent to...
%\end{theorem}
%\begin{proof}
%Since $f_i(x_i)$ is a convex, piecewise linear function in $x_i$, there is a finite index set $\mathcal{I}^i$ and $(a_1^i, b_1^i), \dots, (a_j^i, b_j^i)$, such that
%\begin{gather*}
%f_i(x_i) = \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\}.
%\end{gather*}
%For the sake of technical issues, we avoid the superscript $i$ unless necessary. \\
%The proof is analogous to the one of Theorem~\ref{Theo:GammaBounds}. Firstly, we have to reformulate the inner optimization problem:
%\begin{alignat*}{2}
%\max_y & \sum_{i \in [n]} \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} + (\max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j + \Delta b^i_j\} - \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\})y_i \\
%\text{s.t.} & \sum_{i \in [n]} y_i \leq \Gamma \\
%& y_i \in \{0,1\} \ \forall i \in [n].
%\end{alignat*}
%Once again, the inequality is TDI and the binary problem is equivalent to its LP relaxation:
%\begin{alignat*}{2}
%\max_y & \sum_{i \in [n]} \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} + (\max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j + \Delta b^i_j\} - \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\})y_i \\
%\text{s.t.} & \sum_{i \in [n]} y_i \leq \Gamma \\
%& y_i \in [0,1] \ \forall i \in [n]
%\end{alignat*}
%and we dualize:
%\begin{alignat*}{3}
%\min_{p,\theta} & \ \sum_{i \in [n]} p_i + \Gamma \theta & \\
%\text{s.t.} & p_i + \theta \geq \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j + \Delta b^i_j\} - \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} \ \forall i \in [n] & \\
%& p, \theta \geq 0 . 
%\end{alignat*}
%Inserting this into our optimization problem leads to
%\begin{alignat*}{2}
%\min_{x,p,\theta} & \ \sum_{i \in [n]} \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} + p_i + \Gamma \theta &\\
%\text{s.t.} & x \in \mathcal{X}, \\
%& p_i + \theta \geq \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j + \Delta b^i_j\} - \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} & \forall i \in [n], \\
%& p, \theta \geq 0.
%\end{alignat*}
%To obtain a tractable formula, we reformulate the right-hand-side of the inequalities (and for the sake of simplicity, neglect the script $i$). \\
%Since $f_i$ is piecewise linear, we can re-write $f_i$ as
%\begin{gather*}
%f_i(x) = \begin{cases}
%a_1x - b_1, x \leq k_1, \\
%a_2x - b_2, x \in [k_1,k_2], \\
%\dots, \\
%a_mx - b_m, x \geq k_m
%\end{cases}
%\end{gather*}
%and $\Delta f_i(x) := \max_{j \in \mathcal{I}} \{a_j x - b_j + \Delta b_j\}$ as 
%\begin{gather*}
%\Delta f_i(x) = \begin{cases}
%a_1x - b_1 + \Delta b_1, x \leq k_1 + \tfrac{\Delta b_2 - \Delta b_1}{a_1 - a_2}, \\
%a_2x - b_2 + \Delta b_2, x \in [k_1 + \tfrac{\Delta b_2 - \Delta b_1}{a_1 - a_2},k_2 + \tfrac{\Delta b_3 - \Delta b_2}{a_2 - a_3}], \\
%\dots, \\
%a_mx - b_m + \Delta b_m, x \geq k_m + \tfrac{\Delta b_m - \Delta b_{m-1}}{a_{m-1} - a_m}
%\end{cases}
%\end{gather*}
%Hence
%\begin{gather*}
%\Delta f_i(x_i) - f_i(x_i) = \begin{cases}
%\Delta b_1, & x \leq k_1, \\
%(a_1-a_2)x - b_1 + \Delta b_1 + b_2, & x \in [k_1, k_1 + \tfrac{\Delta b_2 - \Delta b_1}{a_1 - a_2}], \\
%\Delta b_2, & x \in [k_1 + \tfrac{\Delta b_2 - \Delta b_1}{a_1 - a_2}, k_2],\\
%(a_2-a_3)x - b_2 + \Delta b_2 + b_3, & x \in [k_2, k_2 + \tfrac{\Delta b_3 - \Delta b_2}{a_2 - a_3}], \\
%\dots, \\
%\Delta b_m, & x \geq k_m + \tfrac{\Delta b_m - \Delta b_{m-1}}{a_{m-1} - a_m}
%\end{cases} 
%\end{gather*}
%$\Delta f_i(x_i) - f_i(x_i)$ is a continuous, piecewise linear function which is in general not convex or concave, i.e., for a fitting and finite $\Pi \subseteq \R^2$,
%\begin{alignat*}{2}
%\Delta f(x) - f(x) &= \max_{j \in \mathcal{I}} \{a_j x - b_j + 								\Delta b_j\} - \max_{j \in \mathcal{I}} \{a_jx - b_j\} \\
%& = \max_{j \in \mathcal{I}} \{a_j x - b_j + \Delta b_j - \max_{k \in \mathcal{I}} \{a_kx - b_k\}\} \\
%& = - \min_{j \in \mathcal{I}} \{-a_jx + b_j - \Delta b_j + \max_{k \in \mathcal{I}} \{a_kx - b_k\} \} \\
%&= - \min_{j \in \mathcal{I}} \{\max_{k \in \mathcal{I}} \{(a_k - a_j)x + b_j - b_k - \Delta b_j\} \}\\
%&= \max_{j \in \mathcal{I}} \{\min_{k \in \mathcal{I}} \{(a_j - a_k)x - b_j + b_k + \Delta b_j\}\}
%% {\Sigma \in \Pi} \max_{(a,b) \in \Sigma} \{ax_i - b\}
%\end{alignat*}
%In other words, with \begin{gather*}
%\Pi := \bigcup_{j \in \mathcal{I}} \{\{(a_j - a_1)x - b_j + b_1 + \Delta b_j, \dots, (a_j - a_{|\mathcal{I}|} )x - b_j + b_{|\mathcal{I}|} + \Delta b_j\}\},
%\end{gather*}
%one can re-write 
%\begin{gather*}
%\Delta f(x) - f(x) = \max_{\Sigma \in \Pi} \min_{(a,b) \in \Sigma} \{ax + b\} =: \overline{f}(x)
%\end{gather*}
%%\overline{f_i}(x_i):= 
%%\textcolor{red}{Vermutung: In jedem StÃ¼ck $j = 1, \dots, m$ hat $\Delta f_i - f_i$ die Form
%%\begin{gather*}
%%\Delta f_i(x) - f_i(x) = 
%%\begin{cases} 
%%\begin{cases} 
%%\Delta b_j, & \text{ if } x \leq k_j + \frac{\Delta b_{j+1} - \Delta b_j}{a_j - a_{j+1}},\\
%%(a_{j+1} - a_j)x - b_{j+1} + \Delta b_j + b_j, & \text{ if } x \in [k_j + \frac{\Delta b_{j+1} - \Delta b_j}{a_j - a_{j+1}}, \min \{k_{j+1} + \frac{\Delta b_{j+2} - \Delta b_{j+1}}{a_{j+1} - a_{j+2}},k_j]
%%\end{cases}, \\
%%\begin{cases} 
%%\Delta b_j, & \text{ if } x \leq k_j ,\\
%%(a_{j} - a_{j+1})x + b_{j+1} - \Delta b_j - b_j, & \text{ if } x \in [k_j , \min \{k_{j} + \frac{\Delta b_{j+2} - \Delta b_{j+1}}{a_{j+1} - a_{j+2}},k_{j+1} + \frac{\Delta b_{j+2} - \Delta b_{j+1}}{a_{j+1}-a_{j+2}}\}]
%%\end{cases}
%%\end{cases}
%%\end{gather*}
%%abhÃ¤ngig davon, ob $\Delta b_j \leq \Delta b_{j+1}$ gilt.\\
%%}
%with $\overline{f}$ being a continuous, piecewise linear function (which is general and very likely not convex anymore!). Hence, the optimization problem is equivalent to
%\begin{alignat*}{2}
%\min_{x,p,\theta} & \ \sum_{i \in [n]} \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} + p_i + \Gamma \theta &\\
%\text{s.t.} & x \in \mathcal{X}, \\
%&
%p_i + \theta \geq \overline{f_i}(x_i) & \forall i \in [n], \\
%& p, \theta \geq 0.
%\end{alignat*}
%Once again, it is easy to show that an optimal $\theta^*$ is an element of
%\begin{gather*}
%\{0, \overline{f_1}(x_1^*), \dots, \overline{f_n}(x_n^*)\}.
%\end{gather*}
%Therefore, to solve the $\Gamma$-robust counterpart, one has to solve (we define $\overline{f_0}:= 0 =: x_0$)
%\begin{alignat*}{3} 
%\min_{l\in [n+1] }\min_{x,p} & \ \sum_{i \in [n]} \max_{j \in \mathcal{I}^i} \{a_j^i x_i - b^i_j\} + p_i + \Gamma \overline{f_l}(x_l) &\\
%\text{s.t.} & x \in \mathcal{X}, \\
%& p_i + \overline{f_l}(x_l) \geq \overline{f_i}(x_i) & \ \forall i \in [n], \\
%%& \theta^l = \Delta u_l + \max\{0, u_l - x_l\} , \\
%& p \geq 0, \\
%\end{alignat*}
%Again, for fixed $l$, \begin{gather*}
%p^*_i = \max\{0, \overline{f_i}(x^*_i) - \overline{f_l}(x^*_l)\} \ \forall i \in [n] 
%\end{gather*}
%which can be re-written... \textcolor{red}{TO BE CONTINUED!}
%$\rightarrow$ idea: Splitting the $\overline{f_l}$ into minimum and solving even more inner problems. Re-writing as easy as possible!
%\textcolor{red}{Till this point separability is not necessary. It is possible to define $f_i(x)= \max_{j \in \mathcal{I}^i} \{a_j^T x - b^i_j\} $ }\\
%$\rightarrow$ idea: Splitting the $\overline{f_l}$ into minimum and solving even more inner problems. Re-writing as easy as possible!
%\end{proof}


==> Revisiting_OR.tex <==
\section{Our modeling framework} \label{sec:Rev}
\subsection{Revisiting $\Gamma$--uncertainties for binary programs}
Since our focus lies on reformulations of robust counterparts, we revisit a reformulation result of \cite{IntroGamma}. We consider a combinatorial
program with cost vector $\overline{c} \in \R^n$ and feasible set $\mathcal{X} \subseteq \{0,1\}^n$:
\begin{align}\label{Prob:NomComb}
\begin{split}
\min_{x \in \mathcal{X}} & \ \overline{c}^Tx. \\
\end{split}
\end{align} 
%The feasible set $\mathcal{X} \subseteq \{0,1\}^n$ encodes its combinatorial structure. %of
%problem~\eqref{Prob:NomComb}.%, e.g. the spanning trees or the paths
%of a graph.
We assume that the cost coefficients are subject to interval uncertainty, i.e., $c_i \in [\overline{c}_i, \overline{c}_i + \Delta c_i]$ for a given $\Delta c_i \geq 0$ for all $i \in [n]:=\{1, \dots, n\}$. We aim to find solutions that are robust against at most $\Gamma \in [n]$ coefficients deviating from their nominal scenario $\overline{c}_i$: %In this case, we obtain the following robust counterpart
\begin{align}\label{Prob:Gamma_Comb}
\min_{x \in \mathcal{X}} \ \left\{ \overline{c}^Tx + \max_{\mathcal{S} \subseteq [n]: \left| \mathcal{S} \right| \leq \Gamma} \left\{ \sum_{i \in \mathcal{S}} \Delta c_i x_i \right\} \right\}.
\end{align} 
%Assuming that $\mathcal{X}$ is the intersection of a polyhedron with $\{0,1\}^n$, one could apply Proposition~\ref{Prop:Gamma_MIP}. However, one would change the feasible set $\mathcal{X}$ and thus would in general not be able to apply combinatorial algorithms which were applicable for the nominal problem. This can drastically improve the running time (e.g. Shortest-Path-Problem...) of solving the optimization problem.
%\todo[inline]{Dennis: Quelle für Kürzestes-Wege-Probleme mit MIP-Formulierung} 
%Especially in the case of combinatorial optimization problems for
%which the costs are not correlated, this notion makes sense.
In \cite{IntroGamma}, Bertsimas and Sim have shown that the optimal solutions of program~\eqref{Prob:Gamma_Comb} can be found by applying
an optimization oracle of program~\eqref{Prob:NomComb}: % feasible set $\mathcal{X}$ only consists of binary vectors, one can reformulate Problem~\eqref{Prob:RobCounterpartMIP} into a problem where combinatorial algorithms are still applicable:
\begin{prop}(\cite{IntroGamma}, Theorem 3)\label{Prop:Tractable_Gamma_Comb}
  %Consider problem~\eqref{Prob:Gamma_Comb} and
Assume that $\mathcal{X} \subseteq \{0,1\}^n$ and set $\Delta c_{0}:=0$.  Then program~\eqref{Prob:Gamma_Comb} is equivalent to 
\begin{align}\label{Prob:RobustCounterpartComb}
\min_{k \in [n]_0} \left\{ \Gamma \Delta c_k + \min_{x \in \mathcal{X}} \left\{\overline{c}^Tx + \sum_{j \in [n]} \max\{0,\Delta c_j - \Delta c_k\}x_j \right\} \right\}
\end{align}
where $[n]_0 := \{0, 1, \dots, n\}$.
\end{prop}
%\begin{proof}
%We briefly sketch the proof of \cite{IntroGamma} as we will need it in
%later sections. %For more details, see Theorem 3 in \cite{IntroGamma}. \\
%
%Consider problem~\eqref{Prob:Gamma_Comb}, in particular the inner maximization problem. By introducing binary variables $s_i \in \{0,1\}$ for all $i \in [n]$, one can reformulate the maximization problem as 
%\begin{align*}
%\max_{s} &\sum_{i \in [n]} \Delta c_i x_i s_i, \\ 
%\text{s.t.} & \sum_{i \in [n]} s_i \leq \Gamma, \\
%& s_i \in \{0,1\} \ \forall i \in [n].
%\end{align*}
%Optima of its linear programming (LP) relaxation are integral. Therefore,
%integrality restrictions are redundant, and the
%dual of the LP relaxation can be inserted into 
%%Since the inequality constraint of this optimization problem is a
%%knapsack constraint with integral capacity and equal weights, the
%%inequality is TDI and the problem is equivalent to its LP
%%relaxation. Inserting the dual into
%\eqref{Prob:Gamma_Comb}, which yields %results in 
%\begin{align}\label{Prob:DualIntoPrimalLP}
%\begin{split}
%\min_{x,p,\theta} & \ c^Tx + \Gamma \theta + \sum_{i \in [n]} p_i, \\
%\text{s.t.} & x \in \mathcal{X}, \\
%& p_i + \theta \geq \Delta c_i x_i \ \forall i \in [n], \\
%& p, \theta \geq 0.
%\end{split}
%\end{align}
%If $(x,p,\theta)$ is an optimal solution, it is
%\begin{gather*}
%p_i = \max\{0, \Delta c_i x_i - \theta\} = \max\{0, \Delta c_i - \theta\}x_i \ \forall i \in [n]
%\end{gather*}
%since we minimize and $x_i \in \{0,1\}$ for all $i \in [n]$. Thus, problem~\eqref{Prob:DualIntoPrimalLP} is equivalent to \begin{align}\label{Prob:OnlyThetaRevisit}
%\begin{split}
%\min_{x,\theta} & \ c^Tx + \Gamma \theta + \sum_{i \in [n]} \max\{0, \Delta c_i - \theta\}x_i, \\
%\text{s.t.} & x \in \mathcal{X}, \\
%& \theta \geq 0.
%\end{split}
%\end{align}
%Since $\Delta c_1 \geq \Delta c_2 \geq \dots \geq \Delta c_n \geq \Delta c_{n+1} = 0$, there exists an integer $l \in [n+1]$, such that $\theta \in [\Delta c_{l+1}, \Delta c_l]$. Thus, problem \eqref{Prob:OnlyThetaRevisit} is equivalent to
%\begin{gather*}
%\min_{l \in [n+1]} \min_{x \in \mathcal{X}} c^Tx + \min_{\theta \in [\Delta c_{l+1}, \Delta c_l]} \Gamma \theta + \sum_{i \in [l]} (\Delta c_i - \theta)x_i.
%\end{gather*}
%Since the inner minimization problem over $\theta$ is a
%one-dimensional linear program over an interval, an optimal $\theta$
%is either $\Delta c_l$ or $\Delta c_{l+1}$, i.e., $\theta = \Delta
%c_i$ for one $i \in [n]_0$. With further algebraic manipulations, the claim is proven.
%\end{proof}
Proposition~\ref{Prop:Tractable_Gamma_Comb} implies that program~\eqref{Prob:Gamma_Comb} can be solved to optimality in oracle--polynomial time, assuming that an oracle for program~\eqref{Prob:NomComb} is at hand. We note that it is crucial that $\mathcal{X} \subseteq\{0,1\}^n$. If $\mathcal{X} = \{x \in \Z^p \times \R^{n-p}: \ Ax \leq b, \ x \in [r,s] \}$ for $r,s \in \R^n$ and $p \in [n]$, then one can reformulate the robust counterpart as a computationally tractable MIP but has to introduce additional variables while losing the structure of the original program. Thus, the oracle for solving program~\eqref{Prob:Gamma_Comb} is in general not applicable. For details, we refer the reader to the proofs in \cite{IntroGamma}. 



%In particular, one optimizes over the original feasible set with a slightly modified, but still linear objective with deterministic coefficients. This is crucial regarding combinatorial optimization: Assuming we have an optimization oracle for problem~\eqref{Prob:NomComb}, we only need to call that oracle $n+1$ times for solving \eqref{Prob:Gamma_Comb}, i.e., the robust counterpart is solvable in oracle polynomial time. \\
%Now, we consider an MIP
%\begin{align}\label{Prob:NominalMIP}
%\begin{split}
%\min_{x \in \Z^{r} \times \R^{n-r}} & \ \overline{c}^Tx, \\ 
%\text{s.t.} & \ \overline{A}x \leq b, \\ 
%%& l \leq x \leq u & \\
%%& \ x \in \Z^r \times \R^{n-r}
%\end{split}
%\end{align} 
%with $r \in [n]_0$ integral variables. We assume without loss of generality that $b$ is not subject to uncertainty, and that $\overline{A} := (\overline{a}_{i,j})_{i = 1, \dots, m, \newline j = 1, \dots, n}$ and $\overline{c} := (\overline{c}_i)_{i = 1, \dots, n}$ are the nominal scenario with perturbations $\Delta A := (\Delta {a}_{i,j})_{i = 1, \dots, m, \newline j = 1, \dots, n}$ and $\Delta c := (\Delta c_i)_{i = 1, \dots, n}$.
%%with per$(\overline{A}, \overline{c})$, \begin{gather*}
%%%a_{i,j} \in [\overline{a}_{i,j} - \Delta a_{i,j}, \overline{a}_{i,j} + \Delta a_{i,j}] \ \text{and} \ c_j \in [\overline{c}_j - \Delta c_j, \overline{c}_j + \Delta c_j] \ \forall i \in [m], j \in [n].
%%%\end{gather*} 
%With integer parameters $\Gamma_0, \Gamma_1, \dots, \Gamma_m \in [n]_0$, we apply the flexible $\Gamma$-approach:%This results in \emph{interval uncertainty set} and we could formulate this as a problem of the form \eqref{Prob:GeneralStrictRobust} with integer variables. This can be reformulated again with techniques of \cite{RobustBook} and one would obtain a computationally tractable MIP which did not grow exponentially in size. However, since we wish to be not overly conservative, one can introduce non-negative integers $\Gamma_0, \dots, \Gamma_m$ an can consider the following problem:
%\begin{align}\label{Problem:Gamma_MIP}
%\begin{split}
%\min_{x \in \Z^{r} \times \R^{n-r}}  & \ \overline{c}^Tx + \max_{\mathcal{S} \subseteq [n]: \left| \mathcal{S} \right| \leq \Gamma_0} \sum_{i \in \mathcal{S}} \Delta c_i x_i,  \\
%\text{s.t.} & \sum_{j \in [n]} \overline{a}_{i,j} x_j + \max_{\mathcal{S}_i \subseteq [n]: \left| \mathcal{S}_i \right| \leq \Gamma_i} \sum_{j \in \mathcal{S}_i} \Delta a_{i,j} |x_i| \leq b_i  \ \forall i \in [m]. 
%\end{split}
%\end{align}
%In this case, for a constraint $i \in [m]$, we aim to obtain solutions that are robust against at most $\Gamma_i$ coefficients deviating
%from their nominal scenario. The same holds for the objective, for which only $\Gamma_0$ coefficients are allowed to deviate from their
%nominal scenario. In \cite{IntroGamma}, the authors proved that problem~\eqref{Problem:Gamma_MIP} is equivalent to another MIP: %without uncertainty: 
%\begin{prop}(\cite{IntroGamma}, Theorem 1)\label{Prop:Gamma_MIP}
%Let $\Gamma_0, \dots, \Gamma_m \in [n]$. Then  problem~\eqref{Problem:Gamma_MIP} is equivalent to
%\begin{align}\label{Prob:RobCounterpartMIP}
%\begin{split}
%\min_{x,y,z,p} & \ \overline{c}^Tx + z_0 \Gamma_0 + \sum_{j \in [n]} p_{0j},  \\
%\mathrm{s.t.} & \sum_{j \in [n]} \overline{a}_{i,j} x_j + z_i \Gamma_i + \sum_{j \in [n]} p_{i,j}  \leq b_i \  \forall i \in [m], \\
%& z_0 + p_{0j} \geq \Delta c_j y_j \ \forall j \in [n], \\
%& z_i + p_{i,j} \geq \Delta a_{i,j} y_j \ \forall i \in [m], j \in [n], \\
%& p, y, z \geq 0,  \\
%& x_j \in [-y_j, y_j] \ \forall j \in [n], \\
%& x \in \Z^{p} \times \R^{n-p}.
%\end{split}
%\end{align}
%\end{prop}
%%\begin{proof}
%%See Theorem 1 in \cite{IntroGamma}.
%%\end{proof}
%Thus, problem~\eqref{Problem:Gamma_MIP} can be solved by solving
%another MIP which only grows in terms of the number of variables and
%constraints in polynomial size. Thus it is computationally
%tractable.\\





%We note that one could apply Proposition~\ref{Prop:Gamma_MIP} for (combinatorial) problems of the form~\eqref{Prob:Gamma_Comb} to obtain a tractable counterpart even if the variables are not assumed to be binary. However, one would obtain additional variables $p,y,z$ and could lose the combinatorial structure encoded in $\mathcal{X}$. Thus, while the flexible $\Gamma$-approach is applicable for general MIPs, the structure of the problem is very likely to change unless the respective problem is a binary program. \\
%We note that this does not have to be the end of line - Berstimas and Sim show in \cite{IntroGamma} that, for network problems with uncertain costs, one can still, for a given integral $\Gamma$, approximate the optimal solution although the variables are not binary.\\
%This finishes our brief revisiting of the reformulations in the
%linear case.
%In the next section, we focus on general non-linear (combinatorial) optimization problems with uncertainties in the objective function.

%Assuming that $\mathcal{X}$ is the intersection of a polyhedron with $\{0,1\}^n$, one could apply Proposition~\ref{Prop:Gamma_MIP}. However, one would change the feasible set $\mathcal{X}$ and thus would in general not be able to apply combinatorial algorithms which were applicable for the nominal problem. This can drastically improve the running time (e.g. Shortest-Path-Problem...) of solving the optimization problem.
%\todo[inline]{Dennis: Quelle für Kürzestes-Wege-Probleme mit MIP-Formulierung} 
%We note that it is crucial that $\mathcal{X} \subseteq \{0,1\}^n$ holds - one reformulation technique requires all elements to be binary. 
%\todo[inline]{Dennis: Schritt darstellen}
%Other results regarding the Flexible $\Gamma$-approach - like the Price of Robustness and Approximation results (see \cite{PriceRobust} and \cite{IntroGamma}) will not be discussed in this paper since we only intend to reformulate the robust counterparts.

%\todo[inline]{Dennis: Approximationen? Price of Robustness? Follow-Ups?}
%\todo[inline]{Dennis: Genauer auf Modifikationen eingehen}
%\todo[inline]{Dennis: Als Motivation könnte man hier (oder in der Einleitung) auch angeben, dass der bisherige Ansatz nicht mal mit Linearitäten in der Unsicherheit und in der Entscheidung fertig wird, wenn die Dimensionen nicht gleich sind, also statt $u^Tx$ hat man $u^Tl(x)$.}
% for the $\Gamma$-robust counterpart, a combinatorial optimization problem which is solved in polynomial time can be solved in polynomial time as well - or in other words, any combinatorial optimization problem which is solved by an oracle can be solved in oracle-polynomial time. \\
%Indeed, while one does not require additional variables in Proposition~\ref{Prop:Tractable_Gamma_Comb} (apart from $x_{n+1}$ which is set to $0$ anyways), for reformulating the MIP, one requires $O(n^2)$ more variables and changes to the structure of the feasible set. The main reason in this lies the proof of Proposition ~\ref{Prop:Tractable_Gamma_Comb}: It is crucial that the variables are supposed to be binary, such that the additional variables can be eliminated.   \\

% For combinatorial optimization problems of the form
%
%with interval uncertainties in the costs, i.e., the random variable $c_i$ realizes in $[\overline{c}_i, \overline{c}_i + \Delta c_i]$ with $\Delta c_i \geq 0$ for every $i \in [n]$, Berstimas and Sim introduced the \emph{$\Gamma$-}flexible approach in \cite{IntroGamma} to circumvent manipulating the combinatorial structure by an epigraphic re-formulation: Instead of allowing all $c_i$ to change, they modify the uncertainty set $\mathcal{U}$: 
%\begin{gather*}
%\mathcal{U}^\Gamma := \{c \in \times_{i \in [n]} [\overline{c}_i, \overline{c}_i + \Delta c_i] \mid c_i > \overline{c}_i \ \text{ for at most $\Gamma$ coefficients}\}.
%\end{gather*}
%In other words, the robust counterpart they aimed to re-formulate - without changing the feasible set of the optimization problem - is
%
%In \cite{IntroGamma}, Bertsimas and Sim showed that Problem~\eqref{Prob:Gamma_Comb} can be reformulated and is computationally tractable by solving $n+1$ problems of the form \eqref{Prob:NomComb}
%\begin{prop}\label{Prop:Tractable_Gamma_Comb}
%Let $\min_{x \in \mathcal{X}} c^Tx$ be a combinatorial optimization problem with $\mathcal{X} \subseteq \{0,1\}^n$. Let furthermore $x_{n+1} := 0$ and $\Delta c_{n+1}:=0$. Then, the $\Gamma$--counterpart is equivalent to the problem 
%\begin{gather*}
%\min_{l = 1, \dots, n+1} \{ \Gamma \Delta c_l + \min_{x \in \mathcal{X}} \{c^Tx + \sum_{j=1}^l (\Delta c_j - \Delta c_l)x_j \} \},
%\end{gather*}
%assuming that $\Delta c_i \geq \Delta c_{i+1} \geq 0 \ \forall i = 1, \dots, n-1$.
%\end{prop}



==> introduction_OR.tex <==
\section{Introduction} \label{sec:Intro} 
In recent years, optimization under uncertainty has gained importance and popularity. When an optimization program is subject to uncertainty, one can aim to solve it before all data are known -- sometimes, this is even mandatory. % Reasons for this uncertainty may include fluctuating input parameters, inaccuracies in measurement or a pressing need to make decisions before all data have been disclosed. 
Two fields of research how to treat said uncertainties are stochastic and robust optimization. In stochastic optimization, one usually requires a sufficient amount of data to estimate or determine the underlying probability distribution. For further information on this, we refer the reader to the monograph \cite{Stochastic}. For robust optimization, one does not require probability distributions. Instead, for modeling the real--life situation, an uncertainty set is pre--determined and one optimizes over the variables while taking the uncertainty set into account simultaneously. Several approaches in robust optimization have been conducted in the past decades, especially in the field of (mixed--integer) linear programming. However, for combinatorial optimization, those are usually not applicable since the underlying program's structure is changed, rendering solution algorithms for the nominal problem not applicable. To circumvent this, Bertsimas and Sim introduced $\Gamma$--uncertainty sets in \cite{IntroGamma} and \cite{PriceRobust} for combinatorial optimization under interval uncertainty in a linear objective. Since recent research has focused on nonlinear robust optimization programming, we extend their approach for combinatorial and discrete programming with nonlinearities.

% ´

%%%: %This can however result in very conservative solutions since there is no guarantee that solutions which perform optimal in the worst case perform well in other scenarios.  %This can take different forms.  A classical example is the box uncertainty. Every uncertain parameter can fluctuate within a given interval. The robust solution remains valid even if all parameters fluctuate in the uncertainty set.
%Therefore, Bertsimas and Sim introduced the so-called \emph{flexible $\Gamma$-approach} in \cite{IntroGamma} for MIPs and in particular combinatorial optimization problems. 
%They assume that robust protection is sought against an uncertain cost $c$ given by a nominal scenario $\overline{c}$ and some perturbation $\Delta c$ in problem~\eqref{Prob:NominalProbLP}.
%%\begin{gather*}
%%c_i \in [\overline{c}_i, \overline{c}_i + \Delta c_i] \ \forall i \in [n]$.
%%\end{gather*} 
%This results in an interval uncertainty set.
%%$\mathcal{U} := \bigtimes_{i \in [n]} [\overline{c}_i, \overline{c}_i + \Delta
%%  c_i]$.
%In \cite{IntroGamma}, Bertsimas and Sim modify the uncertainty that obtains solutions that are robust against at most $\Gamma$ % \in \N$, 
%% $0\leq \Gamma\leq n$ 
%deviations of the cost coefficients $c_i$ and obtain computationally tractable reformulations, in particular for MIPs. If the decision variables that are subject to uncertainty are also binary and an oracle is available to solve problem~\eqref{Prob:NominalProbLP}, the robust counterpart %problem~\eqref{Prob:IntroGamma},
%can be solved to optimality with $n+1$ oracle calls. This is especially important for combinatorial optimization problems, since
%they can often be modeled as binary problems (BPs) with a linear objective. In general, the applicability of the original reformulation relies on the fact that the original objective function is linear and that the variables are binary.
\paragraph*{Contribution:}
We propose and study a generic framework for mixed--integer nonlinear programs (MINLPs) under uncertainties that generalizes the $\Gamma$--uncertainties for mixed--integer linear programs (MIPs) in \cite{IntroGamma} and \cite{PriceRobust}. We focus on objective uncertainty: On the one hand, we provide reformulations, in particular for the case of nonlinear, concave and linear uncertainty. On the other hand, we show that the programs 
\begin{gather}\label{Form1}
\min_{x \in \mathcal{X}} u^TBg(x)
\end{gather}
underlying an 'assignment structure' and
\begin{gather}\label{Form2}
\min_{x \in \mathcal{X}} u^Tl(x)
\end{gather}
where $l$ is a $0/1$--function\footnote{We call a function $l\colon M \to N$ a $0/1$--function when $l(x) \in \{0,1\}$ for all $x \in M$.} and, in both cases, $u$ is a vector of uncertain parameters in $[\overline{u}, \overline{u} + \Delta u]$ can be solved by a polynomial number of oracle calls (With an oracle, we henceforth mean a black box that can solve the original program without uncertainties). To be more precise, we conduct the following:
\begin{enumerate}
\item Programs with concave uncertainty can be reformulated into programs including support functions and concave conjugations. If the uncertainty is linear, then support functions are sufficient.
%\item If only the objective is subject to (linear) uncertainty and of the form $u^Tl(x)$ with $l$ being a $0/1$--function, then one can solve (and approximate) the problem under uncertainty with a polynomial number of oracle--calls.
%\item Blubb. \todo[inline]{Hier müsste man noch einnähen, ob das andere eine exponential number wird}
\item A black box for solving the program without uncertainty is sufficient for solving programs either~\eqref{Form1} or~\eqref{Form2} under $\Gamma$--uncertainty with intervals. 
\item We propose a new model to handle deadline uncertainty with $\Gamma$--uncertainty sets and show its computational tractability.
\item Our model unifies several applications of $\Gamma$--uncertainty sets in the literature.
\end{enumerate}
In our appendix, we demonstrate the practical applicability of our presented reformulations for the quadratic assignment problem (QAP, \cite{QAPintro}) and a special case of the vehicle routing problem with general time windows (VRPGTW, \cite{VRPSTW}), both under $\Gamma$--uncertainty, in terms of a prototypical numerical study. Uncertainty in the constraints can be handled analogously and is also briefly discussed in the electronic companion. In total, our goal is to present a unifying framework for nonlinear optimization under uncertainty that is of interest for future research, in particular the combination of combinatorial optimization and nonlinear programming under uncertainty.\\
%We foOur proposed model can be reformulated into a MINLP not influenced by uncertainty but where one has to deal with support functions and concave conjugates. Furthermore, if $f_i(x,u^i) = (u^i)^Tl_i(x)$ where $l_i(x)$ is $0/1$--valued and $u^i$ lies in an interval uncertainty, then we show that its robust counterpart can be solved with a polynomial number of oracle calls . 

\paragraph*{Outline:}
The paper is structured as follows. In Section~\ref{sec:Rev}, we briefly revisit the the oracle--polynomial reformulation of the $\Gamma$--counterpart from \cite{IntroGamma} before we introduce the $\Gamma$--counterpart for MINLPs. We motivate our generalization with several applications. In Section~\ref{sec:Non_Linear_Objective_Functions}, we obtain reformulations of our robust counterparts and demonstrate our main results by showing and show that in special cases, oracle--polynomiality holds. In Section~\ref{Sec:Reformulations}, we present various examples and applications of our results with a focus on quadratic problems under uncertainty. Finally, in Section~\ref{Sec:Conclus}, we provide a conclusion and propose some interesting avenues for research. In our electric electronic companion, we demonstrate the case of uncertain constraints and a prototypical numerical study for the QAP and the VRPGTW under $\Gamma$--uncertainty. %In Section~\ref{Sec:App}, we present computational results of the QAP and the VRPGTW under $\Gamma$--uncertainty. 
% We start by extending the original results for cases where the uncertainty is linear, the objective is separable in the uncertainty and the decision vectors with $0/1$--valued functions. For the rest of Section~\ref{sec:Non_Linear_Objective_Functions}, we apply different reformulations and techniques, mainly based on \cite{IntroGamma} and \cite{Fenchel} to obtain a reformulation of the counterpart for the underlying problem under uncertainty (both in the combinatorial and the general case). We also obtain reformulations for objective functions of the form $u^TBx$ where $u$ is subject to interval uncertainty. We close this section by providing some notes about the complexity class of our counterparts. 
% and state examples for computationally tractable combinatorial optimization problems that fall in this category, e.g. the Quadratic Assignment Problem. 
%Furthermore, we analyze a special case for which the reformulations of Bertismas and Sim are applicable even when the uncertainties are correlated among the variables. This case generalizes binary problems with an assignment structure and we demonstrate this for a single-machine scheduling problem. %For the non-concave case, we present two methods from \cite{Fenchel} and demonstrate that we can generate robust counterparts for optimization problems with a quadratic objective. 


\paragraph*{Literature review:}
A first discussion of a program subject to uncertainty has been conducted by Soyster \cite{Soyster} for column--wise uncertainty of a constraint matrix where the uncertainty set is a convex set. To deal with the resulting over--conservatism, several approaches have been introduced in the literature. In \cite{ben-tal1} and \cite{ben-tal3}, the authors have presented and discussed linear programs under uncertainty from a theoretical and a practical point of view, focusing on convex/interval uncertainties, respectively. The case of reformulating convex/concave rather than linear functions under uncertainty has been addressed in \cite{ben-tal2}.  A framework for treating robust programming with reformulation approaches is \cite{RobustBook}. Another approach for treating uncertainties is the adversarial approach presented in \cite{ApplDec2} that, instead of reformulating, tries to iteratively add scenarios of the uncertainty to the nominal program, finds optimal solutions and checks whether the found solutions are already robust. The approaches are compared in \cite{BertsimasCutting}. For broad overviews of robust optimization in a theoretical and applied sense, we refer to the surveys \cite{survey2011}, \cite{survey2014} and \cite{SurveyAdj}. In the context of combinatorial/discrete programs under uncertainty, we reference \cite{Kouvelis_1997} as the first framework and the surveys \cite{RobCombOpt} and \cite{Kasperski2016} that tackle interval, discrete and convex uncertainties in the objective. $\Gamma$--uncertainties were introduced in \cite{PriceRobust} and applied to combinatorial programs in \cite{IntroGamma}.  
% For the sake of completeness, an overview over the concept of adjustable robustness (that also tackles discrete problems), we refer to \cite{SurveyAdj}. 
%Thus, Bertsimas and Sim introduced $\Gamma$--uncertainties in \cite{IntroGamma} and \cite{PriceRobust}.
Throughout the last two decades, they have been generalized and extended. In \cite{BusingBand} and in \cite{Fischetti2009}, new uncertainty concepts, namely multi--band uncertainty and light robustness, based on $\Gamma$--uncertainties, have been introduced. In \cite{Poss12}, \cite{Poss14} and \cite{POSS2018}, uncertainty sets that generalized $\Gamma$--uncertainty sets were introduced. Furthermore, \cite{Buesing2019} discussed $\Gamma$--uncertainty sets in the context of global robust optimization and \cite{Goerigk2021} introduced locally budgeted uncertainty sets. Finally, $\Gamma$--uncertainty sets have also been applied in a dynamic robust sense, e.g. in \cite{ApplicationBudget}. Optimization under uncertainties including nonlinearities are fairly new in the literature. For an overview over theory, solution approaches and applications, we refer to \cite{NonlinearRO}. The reformulation techniques that our framework is based on have been derived in \cite{Fenchel}.

Finally, for our applications, we refer to the following sources. The QAP under uncertainty was discussed in \cite{QAP2015}, \cite{QAP2012} and \cite{QAM}. The VRPTGW under uncertainty is motivated by the patient transport problem described in \cite{Dummies} and based on the VRPGTW described in \cite{VRPSTW}. To the best of our knowledge, the aforementined $\Gamma$--uncertainty set for piecewise linear objective functions is new in the literature, although piecewise linear functions under uncertainty have been discussed e.g. in \cite{ApplPWL2013} and \cite{Gorissen_2013}.
%    To circumvent this problem, approximation techniques \cite{ApproxNRO}
%or piecewise linear relaxations \cite{assmann1} have been proposed 
%\cite{NonlinearRO} and optimality certificates similar to KKT conditions have been established together with a survey of
%non-linear robust optimization.
%Furthermore, in \cite{Fenchel} the authors established reformulation techniques for non--linear robust optimization problems that generalize the reformulations provided in \cite{RobustBook}. While they focus on the case where the uncertainty is concave, they also present methods to address the general case. \\
%Requiring $x$ to be robust optimal might result in overly conservative solutions, since $x$ has to be feasible for all elements of $\mathcal{U}$ and also has to perform better than every feasible solution $x$ for any scenario. Furthermore, for many combinatorial optimization problems, finite uncertainty sets result in NP-hard optimization problems \cite{Kouvelis_1997}.

 
% Also, if $\Gamma$ is not limited to be integral but can also be rational number, the $\Gamma$--approach has been applied successfully for example in \cite{ApplicationBudget}.
%%  In this work, we extend the approach to non--linear combinatorial optimization problems: Under the assumption that the objective function is the sum of $m$ functions under uncorrelated uncertainty, our robust counterparts ensure that the solutions obtained are robust against $\Gamma$ deviations from their nominal scenario. With uncorrelated, we mean that a term $c_ix_i$ is replaced with a function $f_i(x,u^i)$ where $u^i$ is uncertain and not necessarily 'only' a number but a vector of uncertain parameters. This is new in the literature: While there are examples of applying the reformulations of \cite{IntroGamma} to the non--linear case by linearizing the non--linearities, e.g. for the Quadratic Assignment Problem under uncertainty \cite{QAP2015}, we propose reformulations which work for a more general class of optimization problems. To make the counterpart tractable, we apply reformulation techniques from \cite{Fenchel}. While our focus is on linear or concave uncertainty, we also discuss alternative situations. 
%\\


%In general, such a robust optimization is a family of optimization problems:
%%\begin{gather}\label{Mod:RobustGeneral}
%\left\{ \min_x\{f(x,u): x \in \mathcal{X}(u)\} \right\}_{u \in \mathcal{U}} 
%\end{gather}
%where $x$ is the decision variable, $f(x,u)$ the objective that is subject to an uncertain parameter $u$ and $\mathcal{X}(u)$ is the feasible set that depends on the uncertainty. If only the objective is subject to uncertainty, $\mathcal{X}(u) =: \mathcal{X}$ for all $u \in \mathcal{U}}$ which is usually the case of combinatorial optimization problems. In model~\eqref{Mod:RobustGeneral}
%As an example, we consider the linear program (LP) \todo[inline]{LP streichen? Wie machen das andere mit der Beschreibung von statischer Robustheit?}
%\begin{align}\label{Prob:NominalProbLP}
%\begin{split}
%\inf_x & \ c^Tx, \\ 
%\text{s.t.} & \ Ax \leq b
%\end{split}
%\end{align} 
%with input data $A \in \R^{m \times n},b \in \R^m$ and $c\in \R^n$. The uncertainty set is denoted as $\mathcal{U}$ and contains scenarios of the input data $(c,A,b)$. % and $l$ and $u$ being the lower and upper bounds for the variables where we  allow $l_i = -\infty$ and $u_i = \infty$ for $i \in [n]$. \\
%The robust counterpart is 
%\begin{gather}\label{Prob:GeneralStrictRobust}
%\inf_x  \left\{ \sup_{(c,A,b) \in \mathcal{U}} c^T x\colon \ Ax \leq b \ \forall (c,A,b) \in \mathcal{U}  \right\}.
%\end{gather}

%A first analysis of problem~\eqref{Prob:GeneralStrictRobust} has been conducted by Soyster \cite{Soyster} for column-wise uncertainty of the matrix $A$. Solutions that are optimal for
%problem~\eqref{Prob:GeneralStrictRobust} are called robust optimal. In \cite{ben-tal1} and \cite{ben-tal3} \todo[inline]{Passen die Quellen wirklich? Selbes mit [7] zu konvexen Funktionen}, the authors have presented a methodology to reformulate
%~\eqref{Prob:GeneralStrictRobust}
%as a computationally
%tractable optimization problem, without loss of generality assuming
%that $\mathcal{U}$ is convex.
% These 
%reformulations can also be applied to 
%mixed-integer linear problems (MIPs). 
%\paragraph*{Notation:}
%\todo[inline]{In Kapitel 2 schieben}
%The sets $\Z, \Q$ and $\R$ denote the integer numbers, the rational numbers and the real numbers, respectively. The lower-case letters $m, n \in \Z_{\geq 0}$ denote non-negative numbers, while the set $[m]$ denotes the set $\{1, 2 \dots, m\}$, and $[m]_0$ denotes $\{0,1, \dots, m\}$. Caligraphic letters are used for sets. For a matrix $A \in \R^{m \times n}$, $i \in [m]$, and $j \in [n]$, $A_{i,.}$ denotes its $i$-th row and $A_{.,j}$ its $j$-th column. The vector $e^m \in \R^m$ denotes the vector with only ones. % $n%With $\mathrm{relint}(\mathcal{A})$, we denote the relative interior of a set $\mathcal{A} \subset \R^n$. \\
%With $\mathcal{U}$, we denote the uncertainty set, with $\overline{u}$, we denote the respective nominal scenario.


